On fast computation of finite-time coherent sets using radial basis functions

Finite-time coherent sets inhibit mixing over finite times. The most expensive part of the transfer operator approach to detecting coherent sets is the construction of the operator itself. We present a numerical method based on radial basis function collocation and apply it to a recent transfer operator construction that has been designed specifically for purely advective dynamics. The construction is based on a "dynamic" Laplacian operator and minimises the boundary size of the coherent sets relative to their volume. The main advantage of our new approach is a substantial reduction in the number of Lagrangian trajectories that need to be computed, leading to large speedups in the transfer operator analysis when this computation is costly.

==> cyl_cheeger.tex <==
  -9.8428626527176233e-01   2.0727501072055070e+01
  -9.6454340261904470e-01   9.5602604857199282e+01
  -9.4480053996632707e-01   6.0934954128052865e+01
  -9.2505767731360944e-01   4.5320629370722592e+01
  -9.0531481466089181e-01   3.5869102413710529e+01
  -8.8557195200817418e-01   2.9904677519813756e+01
  -8.6582908935545655e-01   2.5790708476594858e+01
  -8.4608622670273892e-01   2.3169552822705587e+01
  -8.2634336405002129e-01   2.0346346798966003e+01
  -8.0660050139730366e-01   1.8254965746583494e+01
  -7.8685763874458603e-01   1.6562864533027998e+01
  -7.6711477609186851e-01   1.5367940136081112e+01
  -7.4737191343915088e-01   1.4221579289693711e+01
  -7.2762905078643325e-01   1.3333638255626477e+01
  -7.0788618813371562e-01   1.2524964721705786e+01
  -6.8814332548099799e-01   1.1725945861924050e+01
  -6.6840046282828036e-01   1.1117623833568151e+01
  -6.4865760017556273e-01   1.0469501078384406e+01
  -6.2891473752284510e-01   9.9570890945278432e+00
  -6.0917187487012747e-01   9.5380834026002486e+00
  -5.8942901221740984e-01   9.1225579273468949e+00
  -5.6968614956469232e-01   8.7272877422808399e+00
  -5.4994328691197469e-01   8.3700147957095297e+00
  -5.3020042425925706e-01   7.9664912916863875e+00
  -5.1045756160653943e-01   7.6825632802298065e+00
  -4.9071469895382175e-01   1.1890452202258771e+01
  -4.7097183630110417e-01   7.1828689042053560e+00
  -4.5122897364838654e-01   6.9691620209265874e+00
  -4.3148611099566891e-01   6.8458725946709018e+00
  -4.1174324834295128e-01   1.0367437778873082e+01
  -3.9200038569023365e-01   6.5979083335518629e+00
  -3.7225752303751602e-01   6.6136384468645621e+00
  -3.5251466038479840e-01   6.5669554290549774e+00
  -3.3277179773208077e-01   1.5932427722599426e+01
  -3.1302893507936314e-01   1.2370526313088767e+01
  -2.9328607242664551e-01   1.2427778689390284e+01
  -2.7354320977392788e-01   9.8312342101114343e+00
  -2.5380034712121025e-01   7.1213248814270003e+00
  -2.3405748446849262e-01   9.4440512509438008e+00
  -2.1431462181577499e-01   6.8950940706820489e+00
  -1.9457175916305736e-01   9.2619963894006982e+00
  -1.7482889651033984e-01   2.3344418762368541e+01
  -1.5508603385762221e-01   3.5608031786398563e+01
  -1.3534317120490458e-01   3.3089091776713758e+01
  -1.1560030855218695e-01   3.9851484463250287e+01
  -9.5857445899469318e-02   6.2685988839886001e+01
  -7.6114583246751688e-02   7.1791520627347197e+01
  -5.6371720594034058e-02   9.2341799911145813e+01
  -3.6628857941316428e-02   9.3688527808503380e+01
  -1.6885995288598799e-02   1.0744814946813524e+02
   2.8568673641188314e-03   2.3372761259766108e+02
   2.2599730016836461e-02   1.0853677423328047e+02
   4.2342592669554091e-02   7.2914706536293906e+01
   6.2085455322271721e-02   5.1177147418183758e+01
   8.1828317974989351e-02   3.5674002356364895e+01
   1.0157118062770698e-01   2.2606375687021110e+01
   1.2131404328042461e-01   1.6335778158211419e+01
   1.4105690593314224e-01   1.2073040976439829e+01
   1.6079976858585987e-01   1.1631730655087420e+01
   1.8054263123857750e-01   7.1488203065855433e+00
   2.0028549389129502e-01   5.2324936470693730e+00
   2.2002835654401265e-01   4.4263491556150232e+00
   2.3977121919673028e-01   4.4049674438793183e+00
   2.5951408184944791e-01   4.4373090477468429e+00
   2.7925694450216554e-01   4.2780264208659649e+00
   2.9899980715488317e-01   3.7810105526210860e+00
   3.1874266980760080e-01   3.5664935963794120e+00
   3.3848553246031843e-01   3.4888224000729897e+00
   3.5822839511303606e-01   3.3713049609085242e+00
   3.7797125776575369e-01   3.2663164284443291e+00
   3.9771412041847132e-01   3.1248818452855245e+00
   4.1745698307118895e-01   3.0589206296237896e+00
   4.3719984572390658e-01   3.0411491997025313e+00
   4.5694270837662421e-01   3.0580920430161225e+00
   4.7668557102934184e-01   3.0609398583957055e+00
   4.9642843368205941e-01   3.1152564791716189e+00
   5.1617129633477710e-01   3.1458838916376526e+00
   5.3591415898749473e-01   3.2084231215005117e+00
   5.5565702164021236e-01   3.2585811391440673e+00
   5.7539988429292999e-01   3.3424512428757334e+00
   5.9514274694564751e-01   3.4265102245758787e+00
   6.1488560959836513e-01   3.5226319729756321e+00
   6.3462847225108276e-01   3.5998003469149475e+00
   6.5437133490380039e-01   3.7227961853699694e+00
   6.7411419755651802e-01   3.8250858885860812e+00
   6.9385706020923565e-01   3.9642013217446395e+00
   7.1359992286195328e-01   4.1062207925102951e+00
   7.3334278551467091e-01   4.2502590157942919e+00
   7.5308564816738854e-01   4.4467205491657262e+00
   7.7282851082010617e-01   4.6128595229393401e+00
   7.9257137347282369e-01   4.8466288040373264e+00
   8.1231423612554132e-01   5.1148882960454838e+00
   8.3205709877825895e-01   5.4224098740677693e+00
   8.5179996143097658e-01   5.8322682250153672e+00
   8.7154282408369421e-01   6.3284449481714313e+00
   8.9128568673641184e-01   6.8702546489889942e+00
   9.1102854938912947e-01   7.4719469533327798e+00
   9.3077141204184710e-01   8.4678177417259644e+00
   9.5051427469456473e-01   1.0237350260540723e+01
   9.7025713734728236e-01   1.3348756237966487e+01
   9.8999999999999999e-01   2.3062536666819259e+01


==> cyl_non_coh_set.tex <==
   2.5367545237289093e+00   1.5549296972313116e+00
   2.5367545237289093e+00   1.5866629563584815e+00
   2.5367545237289093e+00   1.6183962154856510e+00
   2.5367545237289093e+00   1.6501294746128208e+00
   2.5367545237289093e+00   1.6818627337399903e+00
   2.5367545237289093e+00   1.7135959928671598e+00
   2.5367545237289093e+00   1.7453292519943295e+00
   2.5683283192423745e+00   1.4914631789769726e+00
   2.5683283192423745e+00   1.5231964381041421e+00
   2.5683283192423745e+00   1.5549296972313116e+00
   2.5683283192423745e+00   1.5866629563584815e+00
   2.5683283192423745e+00   1.6183962154856510e+00
   2.5683283192423745e+00   1.6501294746128208e+00
   2.5683283192423745e+00   1.6818627337399903e+00
   2.5683283192423745e+00   1.7135959928671598e+00
   2.5683283192423745e+00   1.7453292519943295e+00
   2.5683283192423745e+00   1.7770625111214990e+00
   2.5683283192423745e+00   1.8087957702486686e+00
   2.5683283192423745e+00   1.8405290293758385e+00
   2.5683283192423745e+00   1.8722622885030080e+00
   2.5683283192423745e+00   1.9039955476301775e+00
   2.5683283192423745e+00   1.9357288067573473e+00
   2.5683283192423745e+00   1.9674620658845168e+00
   2.5999021147558397e+00   1.3327968833411243e+00
   2.5999021147558397e+00   1.3645301424682938e+00
   2.5999021147558397e+00   1.3962634015954634e+00
   2.5999021147558397e+00   1.4279966607226333e+00
   2.5999021147558397e+00   1.4597299198498028e+00
   2.5999021147558397e+00   1.4914631789769726e+00
   2.5999021147558397e+00   1.5231964381041421e+00
   2.5999021147558397e+00   1.5549296972313116e+00
   2.5999021147558397e+00   1.5866629563584815e+00
   2.5999021147558397e+00   1.6183962154856510e+00
   2.5999021147558397e+00   1.6501294746128208e+00
   2.5999021147558397e+00   1.6818627337399903e+00
   2.5999021147558397e+00   1.7135959928671598e+00
   2.5999021147558397e+00   1.7453292519943295e+00
   2.5999021147558397e+00   1.7770625111214990e+00
   2.5999021147558397e+00   1.8087957702486686e+00
   2.5999021147558397e+00   1.8405290293758385e+00
   2.5999021147558397e+00   1.8722622885030080e+00
   2.5999021147558397e+00   1.9039955476301775e+00
   2.5999021147558397e+00   1.9357288067573473e+00
   2.5999021147558397e+00   1.9674620658845168e+00
   2.5999021147558397e+00   1.9991953250116867e+00
   2.5999021147558397e+00   2.0309285841388562e+00
   2.6314759102693053e+00   1.2693303650867851e+00
   2.6314759102693053e+00   1.3010636242139546e+00
   2.6314759102693053e+00   1.3327968833411243e+00
   2.6314759102693053e+00   1.3645301424682938e+00
   2.6314759102693053e+00   1.3962634015954634e+00
   2.6314759102693053e+00   1.4279966607226333e+00
   2.6314759102693053e+00   1.4597299198498028e+00
   2.6314759102693053e+00   1.4914631789769726e+00
   2.6314759102693053e+00   1.5231964381041421e+00
   2.6314759102693053e+00   1.5549296972313116e+00
   2.6314759102693053e+00   1.5866629563584815e+00
   2.6314759102693053e+00   1.6183962154856510e+00
   2.6314759102693053e+00   1.6501294746128208e+00
   2.6314759102693053e+00   1.6818627337399903e+00
   2.6314759102693053e+00   1.7135959928671598e+00
   2.6314759102693053e+00   1.7453292519943295e+00
   2.6314759102693053e+00   1.7770625111214990e+00
   2.6314759102693053e+00   1.8087957702486686e+00
   2.6314759102693053e+00   1.8405290293758385e+00
   2.6314759102693053e+00   1.8722622885030080e+00
   2.6314759102693053e+00   1.9039955476301775e+00
   2.6314759102693053e+00   1.9357288067573473e+00
   2.6314759102693053e+00   1.9674620658845168e+00
   2.6314759102693053e+00   1.9991953250116867e+00
   2.6314759102693053e+00   2.0309285841388562e+00
   2.6314759102693053e+00   2.0626618432660258e+00
   2.6314759102693053e+00   2.0943951023931953e+00
   2.6630497057827704e+00   1.2375971059596154e+00
   2.6630497057827704e+00   1.2693303650867851e+00
   2.6630497057827704e+00   1.3010636242139546e+00
   2.6630497057827704e+00   1.3327968833411243e+00
   2.6630497057827704e+00   1.3645301424682938e+00
   2.6630497057827704e+00   1.3962634015954634e+00
   2.6630497057827704e+00   1.4279966607226333e+00
   2.6630497057827704e+00   1.4597299198498028e+00
   2.6630497057827704e+00   1.4914631789769726e+00
   2.6630497057827704e+00   1.5231964381041421e+00
   2.6630497057827704e+00   1.5549296972313116e+00
   2.6630497057827704e+00   1.5866629563584815e+00
   2.6630497057827704e+00   1.6183962154856510e+00
   2.6630497057827704e+00   1.6501294746128208e+00
   2.6630497057827704e+00   1.6818627337399903e+00
   2.6630497057827704e+00   1.7135959928671598e+00
   2.6630497057827704e+00   1.7453292519943295e+00
   2.6630497057827704e+00   1.7770625111214990e+00
   2.6630497057827704e+00   1.8087957702486686e+00
   2.6630497057827704e+00   1.8405290293758385e+00
   2.6630497057827704e+00   1.8722622885030080e+00
   2.6630497057827704e+00   1.9039955476301775e+00
   2.6630497057827704e+00   1.9357288067573473e+00
   2.6630497057827704e+00   1.9674620658845168e+00
   2.6630497057827704e+00   1.9991953250116867e+00
   2.6630497057827704e+00   2.0309285841388562e+00
   2.6630497057827704e+00   2.0626618432660258e+00
   2.6630497057827704e+00   2.0943951023931953e+00
   2.6630497057827704e+00   2.1261283615203652e+00
   2.6946235012962356e+00   1.1741305877052763e+00
   2.6946235012962356e+00   1.2058638468324459e+00
   2.6946235012962356e+00   1.2375971059596154e+00
   2.6946235012962356e+00   1.2693303650867851e+00
   2.6946235012962356e+00   1.3010636242139546e+00
   2.6946235012962356e+00   1.3327968833411243e+00
   2.6946235012962356e+00   1.3645301424682938e+00
   2.6946235012962356e+00   1.3962634015954634e+00
   2.6946235012962356e+00   1.4279966607226333e+00
   2.6946235012962356e+00   1.4597299198498028e+00
   2.6946235012962356e+00   1.4914631789769726e+00
   2.6946235012962356e+00   1.5231964381041421e+00
   2.6946235012962356e+00   1.5549296972313116e+00
   2.6946235012962356e+00   1.5866629563584815e+00
   2.6946235012962356e+00   1.6183962154856510e+00
   2.6946235012962356e+00   1.6501294746128208e+00
   2.6946235012962356e+00   1.6818627337399903e+00
   2.6946235012962356e+00   1.7135959928671598e+00
   2.6946235012962356e+00   1.7453292519943295e+00
   2.6946235012962356e+00   1.7770625111214990e+00
   2.6946235012962356e+00   1.8087957702486686e+00
   2.6946235012962356e+00   1.8405290293758385e+00
   2.6946235012962356e+00   1.8722622885030080e+00
   2.6946235012962356e+00   1.9039955476301775e+00
   2.6946235012962356e+00   1.9357288067573473e+00
   2.6946235012962356e+00   1.9674620658845168e+00
   2.6946235012962356e+00   1.9991953250116867e+00
   2.6946235012962356e+00   2.0309285841388562e+00
   2.6946235012962356e+00   2.0626618432660258e+00
   2.6946235012962356e+00   2.0943951023931953e+00
   2.6946235012962356e+00   2.1261283615203652e+00
   2.6946235012962356e+00   2.1578616206475347e+00
   2.7261972968097008e+00   1.1423973285781066e+00
   2.7261972968097008e+00   1.1741305877052763e+00
   2.7261972968097008e+00   1.2058638468324459e+00
   2.7261972968097008e+00   1.2375971059596154e+00
   2.7261972968097008e+00   1.2693303650867851e+00
   2.7261972968097008e+00   1.3010636242139546e+00
   2.7261972968097008e+00   1.3327968833411243e+00
   2.7261972968097008e+00   1.3645301424682938e+00
   2.7261972968097008e+00   1.3962634015954634e+00
   2.7261972968097008e+00   1.4279966607226333e+00
   2.7261972968097008e+00   1.4597299198498028e+00
   2.7261972968097008e+00   1.4914631789769726e+00
   2.7261972968097008e+00   1.5231964381041421e+00
   2.7261972968097008e+00   1.5549296972313116e+00
   2.7261972968097008e+00   1.5866629563584815e+00
   2.7261972968097008e+00   1.6183962154856510e+00
   2.7261972968097008e+00   1.6501294746128208e+00
   2.7261972968097008e+00   1.6818627337399903e+00
   2.7261972968097008e+00   1.7135959928671598e+00
   2.7261972968097008e+00   1.7453292519943295e+00
   2.7261972968097008e+00   1.7770625111214990e+00
   2.7261972968097008e+00   1.8087957702486686e+00
   2.7261972968097008e+00   1.8405290293758385e+00
   2.7261972968097008e+00   1.8722622885030080e+00
   2.7261972968097008e+00   1.9039955476301775e+00
   2.7261972968097008e+00   1.9357288067573473e+00
   2.7261972968097008e+00   1.9674620658845168e+00
   2.7261972968097008e+00   1.9991953250116867e+00
   2.7261972968097008e+00   2.0309285841388562e+00
   2.7261972968097008e+00   2.0626618432660258e+00
   2.7261972968097008e+00   2.0943951023931953e+00
   2.7261972968097008e+00   2.1261283615203652e+00
   2.7261972968097008e+00   2.1578616206475347e+00
   2.7261972968097008e+00   2.1895948797747042e+00
   2.7577710923231660e+00   1.1106640694509369e+00
   2.7577710923231660e+00   1.1423973285781066e+00
   2.7577710923231660e+00   1.1741305877052763e+00
   2.7577710923231660e+00   1.2058638468324459e+00
   2.7577710923231660e+00   1.2375971059596154e+00
   2.7577710923231660e+00   1.2693303650867851e+00
   2.7577710923231660e+00   1.3010636242139546e+00
   2.7577710923231660e+00   1.3327968833411243e+00
   2.7577710923231660e+00   1.3645301424682938e+00
   2.7577710923231660e+00   1.3962634015954634e+00
   2.7577710923231660e+00   1.4279966607226333e+00
   2.7577710923231660e+00   1.4597299198498028e+00
   2.7577710923231660e+00   1.4914631789769726e+00
   2.7577710923231660e+00   1.5231964381041421e+00
   2.7577710923231660e+00   1.5549296972313116e+00
   2.7577710923231660e+00   1.5866629563584815e+00
   2.7577710923231660e+00   1.6183962154856510e+00
   2.7577710923231660e+00   1.6501294746128208e+00
   2.7577710923231660e+00   1.6818627337399903e+00
   2.7577710923231660e+00   1.7135959928671598e+00
   2.7577710923231660e+00   1.7453292519943295e+00
   2.7577710923231660e+00   1.7770625111214990e+00
   2.7577710923231660e+00   1.8087957702486686e+00
   2.7577710923231660e+00   1.8405290293758385e+00
   2.7577710923231660e+00   1.8722622885030080e+00
   2.7577710923231660e+00   1.9039955476301775e+00
   2.7577710923231660e+00   1.9357288067573473e+00
   2.7577710923231660e+00   1.9674620658845168e+00
   2.7577710923231660e+00   1.9991953250116867e+00
   2.7577710923231660e+00   2.0309285841388562e+00
   2.7577710923231660e+00   2.0626618432660258e+00
   2.7577710923231660e+00   2.0943951023931953e+00
   2.7577710923231660e+00   2.1261283615203652e+00
   2.7577710923231660e+00   2.1578616206475347e+00
   2.7577710923231660e+00   2.1895948797747042e+00
   2.7577710923231660e+00   2.2213281389018737e+00
   2.7893448878366316e+00   1.0789308103237674e+00
   2.7893448878366316e+00   1.1106640694509369e+00
   2.7893448878366316e+00   1.1423973285781066e+00
   2.7893448878366316e+00   1.1741305877052763e+00
   2.7893448878366316e+00   1.2058638468324459e+00
   2.7893448878366316e+00   1.2375971059596154e+00
   2.7893448878366316e+00   1.2693303650867851e+00
   2.7893448878366316e+00   1.3010636242139546e+00
   2.7893448878366316e+00   1.3327968833411243e+00
   2.7893448878366316e+00   1.3645301424682938e+00
   2.7893448878366316e+00   1.3962634015954634e+00
   2.7893448878366316e+00   1.4279966607226333e+00
   2.7893448878366316e+00   1.4597299198498028e+00
   2.7893448878366316e+00   1.4914631789769726e+00
   2.7893448878366316e+00   1.5231964381041421e+00
   2.7893448878366316e+00   1.5549296972313116e+00
   2.7893448878366316e+00   1.5866629563584815e+00
   2.7893448878366316e+00   1.6183962154856510e+00
   2.7893448878366316e+00   1.6501294746128208e+00
   2.7893448878366316e+00   1.6818627337399903e+00
   2.7893448878366316e+00   1.7135959928671598e+00
   2.7893448878366316e+00   1.7453292519943295e+00
   2.7893448878366316e+00   1.7770625111214990e+00
   2.7893448878366316e+00   1.8087957702486686e+00
   2.7893448878366316e+00   1.8405290293758385e+00
   2.7893448878366316e+00   1.8722622885030080e+00
   2.7893448878366316e+00   1.9039955476301775e+00
   2.7893448878366316e+00   1.9357288067573473e+00
   2.7893448878366316e+00   1.9674620658845168e+00
   2.7893448878366316e+00   1.9991953250116867e+00
   2.7893448878366316e+00   2.0309285841388562e+00
   2.7893448878366316e+00   2.0626618432660258e+00
   2.7893448878366316e+00   2.0943951023931953e+00
   2.7893448878366316e+00   2.1261283615203652e+00
   2.7893448878366316e+00   2.1578616206475347e+00
   2.7893448878366316e+00   2.1895948797747042e+00
   2.7893448878366316e+00   2.2213281389018737e+00
   2.7893448878366316e+00   2.2530613980290437e+00
   2.8209186833500968e+00   1.0471975511965976e+00
   2.8209186833500968e+00   1.0789308103237674e+00
   2.8209186833500968e+00   1.1106640694509369e+00
   2.8209186833500968e+00   1.1423973285781066e+00
   2.8209186833500968e+00   1.1741305877052763e+00
   2.8209186833500968e+00   1.2058638468324459e+00
   2.8209186833500968e+00   1.2375971059596154e+00
   2.8209186833500968e+00   1.2693303650867851e+00
   2.8209186833500968e+00   1.3010636242139546e+00
   2.8209186833500968e+00   1.3327968833411243e+00
   2.8209186833500968e+00   1.3645301424682938e+00
   2.8209186833500968e+00   1.3962634015954634e+00
   2.8209186833500968e+00   1.4279966607226333e+00
   2.8209186833500968e+00   1.4597299198498028e+00
   2.8209186833500968e+00   1.4914631789769726e+00
   2.8209186833500968e+00   1.5231964381041421e+00
   2.8209186833500968e+00   1.5549296972313116e+00
   2.8209186833500968e+00   1.5866629563584815e+00
   2.8209186833500968e+00   1.6183962154856510e+00
   2.8209186833500968e+00   1.6501294746128208e+00
   2.8209186833500968e+00   1.6818627337399903e+00
   2.8209186833500968e+00   1.7135959928671598e+00
   2.8209186833500968e+00   1.7453292519943295e+00
   2.8209186833500968e+00   1.7770625111214990e+00
   2.8209186833500968e+00   1.8087957702486686e+00
   2.8209186833500968e+00   1.8405290293758385e+00
   2.8209186833500968e+00   1.8722622885030080e+00
   2.8209186833500968e+00   1.9039955476301775e+00
   2.8209186833500968e+00   1.9357288067573473e+00
   2.8209186833500968e+00   1.9674620658845168e+00
   2.8209186833500968e+00   1.9991953250116867e+00
   2.8209186833500968e+00   2.0309285841388562e+00
   2.8209186833500968e+00   2.0626618432660258e+00
   2.8209186833500968e+00   2.0943951023931953e+00
   2.8209186833500968e+00   2.1261283615203652e+00
   2.8209186833500968e+00   2.1578616206475347e+00
   2.8209186833500968e+00   2.1895948797747042e+00
   2.8209186833500968e+00   2.2213281389018737e+00
   2.8209186833500968e+00   2.2530613980290437e+00
   2.8524924788635619e+00   1.0154642920694281e+00
   2.8524924788635619e+00   1.0471975511965976e+00
   2.8524924788635619e+00   1.0789308103237674e+00
   2.8524924788635619e+00   1.1106640694509369e+00
   2.8524924788635619e+00   1.1423973285781066e+00
   2.8524924788635619e+00   1.1741305877052763e+00
   2.8524924788635619e+00   1.2058638468324459e+00
   2.8524924788635619e+00   1.2375971059596154e+00
   2.8524924788635619e+00   1.2693303650867851e+00
   2.8524924788635619e+00   1.3010636242139546e+00
   2.8524924788635619e+00   1.3327968833411243e+00
   2.8524924788635619e+00   1.3645301424682938e+00
   2.8524924788635619e+00   1.3962634015954634e+00
   2.8524924788635619e+00   1.4279966607226333e+00
   2.8524924788635619e+00   1.4597299198498028e+00
   2.8524924788635619e+00   1.4914631789769726e+00
   2.8524924788635619e+00   1.5231964381041421e+00
   2.8524924788635619e+00   1.5549296972313116e+00
   2.8524924788635619e+00   1.5866629563584815e+00
   2.8524924788635619e+00   1.6183962154856510e+00
   2.8524924788635619e+00   1.6501294746128208e+00
   2.8524924788635619e+00   1.6818627337399903e+00
   2.8524924788635619e+00   1.7135959928671598e+00
   2.8524924788635619e+00   1.7453292519943295e+00
   2.8524924788635619e+00   1.7770625111214990e+00
   2.8524924788635619e+00   1.8087957702486686e+00
   2.8524924788635619e+00   1.8405290293758385e+00
   2.8524924788635619e+00   1.8722622885030080e+00
   2.8524924788635619e+00   1.9039955476301775e+00
   2.8524924788635619e+00   1.9357288067573473e+00
   2.8524924788635619e+00   1.9674620658845168e+00
   2.8524924788635619e+00   1.9991953250116867e+00
   2.8524924788635619e+00   2.0309285841388562e+00
   2.8524924788635619e+00   2.0626618432660258e+00
   2.8524924788635619e+00   2.0943951023931953e+00
   2.8524924788635619e+00   2.1261283615203652e+00
   2.8524924788635619e+00   2.1578616206475347e+00
   2.8524924788635619e+00   2.1895948797747042e+00
   2.8524924788635619e+00   2.2213281389018737e+00
   2.8524924788635619e+00   2.2530613980290437e+00
   2.8840662743770271e+00   1.0154642920694281e+00
   2.8840662743770271e+00   1.0471975511965976e+00
   2.8840662743770271e+00   1.0789308103237674e+00
   2.8840662743770271e+00   1.1106640694509369e+00
   2.8840662743770271e+00   1.1423973285781066e+00
   2.8840662743770271e+00   1.1741305877052763e+00
   2.8840662743770271e+00   1.2058638468324459e+00
   2.8840662743770271e+00   1.2375971059596154e+00
   2.8840662743770271e+00   1.2693303650867851e+00
   2.8840662743770271e+00   1.3010636242139546e+00
   2.8840662743770271e+00   1.3327968833411243e+00
   2.8840662743770271e+00   1.3645301424682938e+00
   2.8840662743770271e+00   1.3962634015954634e+00
   2.8840662743770271e+00   1.4279966607226333e+00
   2.8840662743770271e+00   1.4597299198498028e+00
   2.8840662743770271e+00   1.4914631789769726e+00
   2.8840662743770271e+00   1.5231964381041421e+00
   2.8840662743770271e+00   1.5549296972313116e+00
   2.8840662743770271e+00   1.5866629563584815e+00
   2.8840662743770271e+00   1.6183962154856510e+00
   2.8840662743770271e+00   1.6501294746128208e+00
   2.8840662743770271e+00   1.6818627337399903e+00
   2.8840662743770271e+00   1.7135959928671598e+00
   2.8840662743770271e+00   1.7453292519943295e+00
   2.8840662743770271e+00   1.7770625111214990e+00
   2.8840662743770271e+00   1.8087957702486686e+00
   2.8840662743770271e+00   1.8405290293758385e+00
   2.8840662743770271e+00   1.8722622885030080e+00
   2.8840662743770271e+00   1.9039955476301775e+00
   2.8840662743770271e+00   1.9357288067573473e+00
   2.8840662743770271e+00   1.9674620658845168e+00
   2.8840662743770271e+00   1.9991953250116867e+00
   2.8840662743770271e+00   2.0309285841388562e+00
   2.8840662743770271e+00   2.0626618432660258e+00
   2.8840662743770271e+00   2.0943951023931953e+00
   2.8840662743770271e+00   2.1261283615203652e+00
   2.8840662743770271e+00   2.1578616206475347e+00
   2.8840662743770271e+00   2.1895948797747042e+00
   2.8840662743770271e+00   2.2213281389018737e+00
   2.8840662743770271e+00   2.2530613980290437e+00
   2.9156400698904923e+00   9.8373103294225839e-01
   2.9156400698904923e+00   1.0154642920694281e+00
   2.9156400698904923e+00   1.0471975511965976e+00
   2.9156400698904923e+00   1.0789308103237674e+00
   2.9156400698904923e+00   1.1106640694509369e+00
   2.9156400698904923e+00   1.1423973285781066e+00
   2.9156400698904923e+00   1.1741305877052763e+00
   2.9156400698904923e+00   1.2058638468324459e+00
   2.9156400698904923e+00   1.2375971059596154e+00
   2.9156400698904923e+00   1.2693303650867851e+00
   2.9156400698904923e+00   1.3010636242139546e+00
   2.9156400698904923e+00   1.3327968833411243e+00
   2.9156400698904923e+00   1.3645301424682938e+00
   2.9156400698904923e+00   1.3962634015954634e+00
   2.9156400698904923e+00   1.4279966607226333e+00
   2.9156400698904923e+00   1.4597299198498028e+00
   2.9156400698904923e+00   1.4914631789769726e+00
   2.9156400698904923e+00   1.5231964381041421e+00
   2.9156400698904923e+00   1.5549296972313116e+00
   2.9156400698904923e+00   1.5866629563584815e+00
   2.9156400698904923e+00   1.6183962154856510e+00
   2.9156400698904923e+00   1.6501294746128208e+00
   2.9156400698904923e+00   1.6818627337399903e+00
   2.9156400698904923e+00   1.7135959928671598e+00
   2.9156400698904923e+00   1.7453292519943295e+00
   2.9156400698904923e+00   1.7770625111214990e+00
   2.9156400698904923e+00   1.8087957702486686e+00
   2.9156400698904923e+00   1.8405290293758385e+00
   2.9156400698904923e+00   1.8722622885030080e+00
   2.9156400698904923e+00   1.9039955476301775e+00
   2.9156400698904923e+00   1.9357288067573473e+00
   2.9156400698904923e+00   1.9674620658845168e+00
   2.9156400698904923e+00   1.9991953250116867e+00
   2.9156400698904923e+00   2.0309285841388562e+00
   2.9156400698904923e+00   2.0626618432660258e+00
   2.9156400698904923e+00   2.0943951023931953e+00
   2.9156400698904923e+00   2.1261283615203652e+00
   2.9156400698904923e+00   2.1578616206475347e+00
   2.9156400698904923e+00   2.1895948797747042e+00
   2.9156400698904923e+00   2.2213281389018737e+00
   2.9156400698904923e+00   2.2530613980290437e+00
   2.9472138654039579e+00   9.8373103294225839e-01
   2.9472138654039579e+00   1.0154642920694281e+00
   2.9472138654039579e+00   1.0471975511965976e+00
   2.9472138654039579e+00   1.0789308103237674e+00
   2.9472138654039579e+00   1.1106640694509369e+00
   2.9472138654039579e+00   1.1423973285781066e+00
   2.9472138654039579e+00   1.1741305877052763e+00
   2.9472138654039579e+00   1.2058638468324459e+00
   2.9472138654039579e+00   1.2375971059596154e+00
   2.9472138654039579e+00   1.2693303650867851e+00
   2.9472138654039579e+00   1.3010636242139546e+00
   2.9472138654039579e+00   1.3327968833411243e+00
   2.9472138654039579e+00   1.3645301424682938e+00
   2.9472138654039579e+00   1.3962634015954634e+00
   2.9472138654039579e+00   1.4279966607226333e+00
   2.9472138654039579e+00   1.4597299198498028e+00
   2.9472138654039579e+00   1.4914631789769726e+00
   2.9472138654039579e+00   1.5231964381041421e+00
   2.9472138654039579e+00   1.5549296972313116e+00
   2.9472138654039579e+00   1.5866629563584815e+00
   2.9472138654039579e+00   1.6183962154856510e+00
   2.9472138654039579e+00   1.6501294746128208e+00
   2.9472138654039579e+00   1.6818627337399903e+00
   2.9472138654039579e+00   1.7135959928671598e+00
   2.9472138654039579e+00   1.7453292519943295e+00
   2.9472138654039579e+00   1.7770625111214990e+00
   2.9472138654039579e+00   1.8087957702486686e+00
   2.9472138654039579e+00   1.8405290293758385e+00
   2.9472138654039579e+00   1.8722622885030080e+00
   2.9472138654039579e+00   1.9039955476301775e+00
   2.9472138654039579e+00   1.9357288067573473e+00
   2.9472138654039579e+00   1.9674620658845168e+00
   2.9472138654039579e+00   1.9991953250116867e+00
   2.9472138654039579e+00   2.0309285841388562e+00
   2.9472138654039579e+00   2.0626618432660258e+00
   2.9472138654039579e+00   2.0943951023931953e+00
   2.9472138654039579e+00   2.1261283615203652e+00
   2.9472138654039579e+00   2.1578616206475347e+00
   2.9472138654039579e+00   2.1895948797747042e+00
   2.9472138654039579e+00   2.2213281389018737e+00
   2.9472138654039579e+00   2.2530613980290437e+00
   2.9787876609174231e+00   9.8373103294225839e-01
   2.9787876609174231e+00   1.0154642920694281e+00
   2.9787876609174231e+00   1.0471975511965976e+00
   2.9787876609174231e+00   1.0789308103237674e+00
   2.9787876609174231e+00   1.1106640694509369e+00
   2.9787876609174231e+00   1.1423973285781066e+00
   2.9787876609174231e+00   1.1741305877052763e+00
   2.9787876609174231e+00   1.2058638468324459e+00
   2.9787876609174231e+00   1.2375971059596154e+00
   2.9787876609174231e+00   1.2693303650867851e+00
   2.9787876609174231e+00   1.3010636242139546e+00
   2.9787876609174231e+00   1.3327968833411243e+00
   2.9787876609174231e+00   1.3645301424682938e+00
   2.9787876609174231e+00   1.3962634015954634e+00
   2.9787876609174231e+00   1.4279966607226333e+00
   2.9787876609174231e+00   1.4597299198498028e+00
   2.9787876609174231e+00   1.4914631789769726e+00
   2.9787876609174231e+00   1.5231964381041421e+00
   2.9787876609174231e+00   1.5549296972313116e+00
   2.9787876609174231e+00   1.5866629563584815e+00
   2.9787876609174231e+00   1.6183962154856510e+00
   2.9787876609174231e+00   1.6501294746128208e+00
   2.9787876609174231e+00   1.6818627337399903e+00
   2.9787876609174231e+00   1.7135959928671598e+00
   2.9787876609174231e+00   1.7453292519943295e+00
   2.9787876609174231e+00   1.7770625111214990e+00
   2.9787876609174231e+00   1.8087957702486686e+00
   2.9787876609174231e+00   1.8405290293758385e+00
   2.9787876609174231e+00   1.8722622885030080e+00
   2.9787876609174231e+00   1.9039955476301775e+00
   2.9787876609174231e+00   1.9357288067573473e+00
   2.9787876609174231e+00   1.9674620658845168e+00
   2.9787876609174231e+00   1.9991953250116867e+00
   2.9787876609174231e+00   2.0309285841388562e+00
   2.9787876609174231e+00   2.0626618432660258e+00
   2.9787876609174231e+00   2.0943951023931953e+00
   2.9787876609174231e+00   2.1261283615203652e+00
   2.9787876609174231e+00   2.1578616206475347e+00
   2.9787876609174231e+00   2.1895948797747042e+00
   2.9787876609174231e+00   2.2213281389018737e+00
   2.9787876609174231e+00   2.2530613980290437e+00
   3.0103614564308883e+00   9.5199777381508877e-01
   3.0103614564308883e+00   9.8373103294225839e-01
   3.0103614564308883e+00   1.0154642920694281e+00
   3.0103614564308883e+00   1.0471975511965976e+00
   3.0103614564308883e+00   1.0789308103237674e+00
   3.0103614564308883e+00   1.1106640694509369e+00
   3.0103614564308883e+00   1.1423973285781066e+00
   3.0103614564308883e+00   1.1741305877052763e+00
   3.0103614564308883e+00   1.2058638468324459e+00
   3.0103614564308883e+00   1.2375971059596154e+00
   3.0103614564308883e+00   1.2693303650867851e+00
   3.0103614564308883e+00   1.3010636242139546e+00
   3.0103614564308883e+00   1.3327968833411243e+00
   3.0103614564308883e+00   1.3645301424682938e+00
   3.0103614564308883e+00   1.3962634015954634e+00
   3.0103614564308883e+00   1.4279966607226333e+00
   3.0103614564308883e+00   1.4597299198498028e+00
   3.0103614564308883e+00   1.4914631789769726e+00
   3.0103614564308883e+00   1.5231964381041421e+00
   3.0103614564308883e+00   1.5549296972313116e+00
   3.0103614564308883e+00   1.5866629563584815e+00
   3.0103614564308883e+00   1.6183962154856510e+00
   3.0103614564308883e+00   1.6501294746128208e+00
   3.0103614564308883e+00   1.6818627337399903e+00
   3.0103614564308883e+00   1.7135959928671598e+00
   3.0103614564308883e+00   1.7453292519943295e+00
   3.0103614564308883e+00   1.7770625111214990e+00
   3.0103614564308883e+00   1.8087957702486686e+00
   3.0103614564308883e+00   1.8405290293758385e+00
   3.0103614564308883e+00   1.8722622885030080e+00
   3.0103614564308883e+00   1.9039955476301775e+00
   3.0103614564308883e+00   1.9357288067573473e+00
   3.0103614564308883e+00   1.9674620658845168e+00
   3.0103614564308883e+00   1.9991953250116867e+00
   3.0103614564308883e+00   2.0309285841388562e+00
   3.0103614564308883e+00   2.0626618432660258e+00
   3.0103614564308883e+00   2.0943951023931953e+00
   3.0103614564308883e+00   2.1261283615203652e+00
   3.0103614564308883e+00   2.1578616206475347e+00
   3.0103614564308883e+00   2.1895948797747042e+00
   3.0103614564308883e+00   2.2213281389018737e+00
   3.0103614564308883e+00   2.2530613980290437e+00
   3.0419352519443534e+00   9.5199777381508877e-01
   3.0419352519443534e+00   9.8373103294225839e-01
   3.0419352519443534e+00   1.0154642920694281e+00
   3.0419352519443534e+00   1.0471975511965976e+00
   3.0419352519443534e+00   1.0789308103237674e+00
   3.0419352519443534e+00   1.1106640694509369e+00
   3.0419352519443534e+00   1.1423973285781066e+00
   3.0419352519443534e+00   1.1741305877052763e+00
   3.0419352519443534e+00   1.2058638468324459e+00
   3.0419352519443534e+00   1.2375971059596154e+00
   3.0419352519443534e+00   1.2693303650867851e+00
   3.0419352519443534e+00   1.3010636242139546e+00
   3.0419352519443534e+00   1.3327968833411243e+00
   3.0419352519443534e+00   1.3645301424682938e+00
   3.0419352519443534e+00   1.3962634015954634e+00
   3.0419352519443534e+00   1.4279966607226333e+00
   3.0419352519443534e+00   1.4597299198498028e+00
   3.0419352519443534e+00   1.4914631789769726e+00
   3.0419352519443534e+00   1.5231964381041421e+00
   3.0419352519443534e+00   1.5549296972313116e+00
   3.0419352519443534e+00   1.5866629563584815e+00
   3.0419352519443534e+00   1.6183962154856510e+00
   3.0419352519443534e+00   1.6501294746128208e+00
   3.0419352519443534e+00   1.6818627337399903e+00
   3.0419352519443534e+00   1.7135959928671598e+00
   3.0419352519443534e+00   1.7453292519943295e+00
   3.0419352519443534e+00   1.7770625111214990e+00
   3.0419352519443534e+00   1.8087957702486686e+00
   3.0419352519443534e+00   1.8405290293758385e+00
   3.0419352519443534e+00   1.8722622885030080e+00
   3.0419352519443534e+00   1.9039955476301775e+00
   3.0419352519443534e+00   1.9357288067573473e+00
   3.0419352519443534e+00   1.9674620658845168e+00
   3.0419352519443534e+00   1.9991953250116867e+00
   3.0419352519443534e+00   2.0309285841388562e+00
   3.0419352519443534e+00   2.0626618432660258e+00
   3.0419352519443534e+00   2.0943951023931953e+00
   3.0419352519443534e+00   2.1261283615203652e+00
   3.0419352519443534e+00   2.1578616206475347e+00
   3.0419352519443534e+00   2.1895948797747042e+00
   3.0419352519443534e+00   2.2213281389018737e+00
   3.0419352519443534e+00   2.2530613980290437e+00
   3.0419352519443534e+00   2.2847946571562132e+00
   3.0735090474578186e+00   9.5199777381508877e-01
   3.0735090474578186e+00   9.8373103294225839e-01
   3.0735090474578186e+00   1.0154642920694281e+00
   3.0735090474578186e+00   1.0471975511965976e+00
   3.0735090474578186e+00   1.0789308103237674e+00
   3.0735090474578186e+00   1.1106640694509369e+00
   3.0735090474578186e+00   1.1423973285781066e+00
   3.0735090474578186e+00   1.1741305877052763e+00
   3.0735090474578186e+00   1.2058638468324459e+00
   3.0735090474578186e+00   1.2375971059596154e+00
   3.0735090474578186e+00   1.2693303650867851e+00
   3.0735090474578186e+00   1.3010636242139546e+00
   3.0735090474578186e+00   1.3327968833411243e+00
   3.0735090474578186e+00   1.3645301424682938e+00
   3.0735090474578186e+00   1.3962634015954634e+00
   3.0735090474578186e+00   1.4279966607226333e+00
   3.0735090474578186e+00   1.4597299198498028e+00
   3.0735090474578186e+00   1.4914631789769726e+00
   3.0735090474578186e+00   1.5231964381041421e+00
   3.0735090474578186e+00   1.5549296972313116e+00
   3.0735090474578186e+00   1.5866629563584815e+00
   3.0735090474578186e+00   1.6183962154856510e+00
   3.0735090474578186e+00   1.6501294746128208e+00
   3.0735090474578186e+00   1.6818627337399903e+00
   3.0735090474578186e+00   1.7135959928671598e+00
   3.0735090474578186e+00   1.7453292519943295e+00
   3.0735090474578186e+00   1.7770625111214990e+00
   3.0735090474578186e+00   1.8087957702486686e+00
   3.0735090474578186e+00   1.8405290293758385e+00
   3.0735090474578186e+00   1.8722622885030080e+00
   3.0735090474578186e+00   1.9039955476301775e+00
   3.0735090474578186e+00   1.9357288067573473e+00
   3.0735090474578186e+00   1.9674620658845168e+00
   3.0735090474578186e+00   1.9991953250116867e+00
   3.0735090474578186e+00   2.0309285841388562e+00
   3.0735090474578186e+00   2.0626618432660258e+00
   3.0735090474578186e+00   2.0943951023931953e+00
   3.0735090474578186e+00   2.1261283615203652e+00
   3.0735090474578186e+00   2.1578616206475347e+00
   3.0735090474578186e+00   2.1895948797747042e+00
   3.0735090474578186e+00   2.2213281389018737e+00
   3.0735090474578186e+00   2.2530613980290437e+00
   3.0735090474578186e+00   2.2847946571562132e+00
   3.1050828429712842e+00   9.5199777381508877e-01
   3.1050828429712842e+00   9.8373103294225839e-01
   3.1050828429712842e+00   1.0154642920694281e+00
   3.1050828429712842e+00   1.0471975511965976e+00
   3.1050828429712842e+00   1.0789308103237674e+00
   3.1050828429712842e+00   1.1106640694509369e+00
   3.1050828429712842e+00   1.1423973285781066e+00
   3.1050828429712842e+00   1.1741305877052763e+00
   3.1050828429712842e+00   1.2058638468324459e+00
   3.1050828429712842e+00   1.2375971059596154e+00
   3.1050828429712842e+00   1.2693303650867851e+00
   3.1050828429712842e+00   1.3010636242139546e+00
   3.1050828429712842e+00   1.3327968833411243e+00
   3.1050828429712842e+00   1.3645301424682938e+00
   3.1050828429712842e+00   1.3962634015954634e+00
   3.1050828429712842e+00   1.4279966607226333e+00
   3.1050828429712842e+00   1.4597299198498028e+00
   3.1050828429712842e+00   1.4914631789769726e+00
   3.1050828429712842e+00   1.5231964381041421e+00
   3.1050828429712842e+00   1.5549296972313116e+00
   3.1050828429712842e+00   1.5866629563584815e+00
   3.1050828429712842e+00   1.6183962154856510e+00
   3.1050828429712842e+00   1.6501294746128208e+00
   3.1050828429712842e+00   1.6818627337399903e+00
   3.1050828429712842e+00   1.7135959928671598e+00
   3.1050828429712842e+00   1.7453292519943295e+00
   3.1050828429712842e+00   1.7770625111214990e+00
   3.1050828429712842e+00   1.8087957702486686e+00
   3.1050828429712842e+00   1.8405290293758385e+00
   3.1050828429712842e+00   1.8722622885030080e+00
   3.1050828429712842e+00   1.9039955476301775e+00
   3.1050828429712842e+00   1.9357288067573473e+00
   3.1050828429712842e+00   1.9674620658845168e+00
   3.1050828429712842e+00   1.9991953250116867e+00
   3.1050828429712842e+00   2.0309285841388562e+00
   3.1050828429712842e+00   2.0626618432660258e+00
   3.1050828429712842e+00   2.0943951023931953e+00
   3.1050828429712842e+00   2.1261283615203652e+00
   3.1050828429712842e+00   2.1578616206475347e+00
   3.1050828429712842e+00   2.1895948797747042e+00
   3.1050828429712842e+00   2.2213281389018737e+00
   3.1050828429712842e+00   2.2530613980290437e+00
   3.1050828429712842e+00   2.2847946571562132e+00
   3.1366566384847490e+00   9.5199777381508877e-01
   3.1366566384847490e+00   9.8373103294225839e-01
   3.1366566384847490e+00   1.0154642920694281e+00
   3.1366566384847490e+00   1.0471975511965976e+00
   3.1366566384847490e+00   1.0789308103237674e+00
   3.1366566384847490e+00   1.1106640694509369e+00
   3.1366566384847490e+00   1.1423973285781066e+00
   3.1366566384847490e+00   1.1741305877052763e+00
   3.1366566384847490e+00   1.2058638468324459e+00
   3.1366566384847490e+00   1.2375971059596154e+00
   3.1366566384847490e+00   1.2693303650867851e+00
   3.1366566384847490e+00   1.3010636242139546e+00
   3.1366566384847490e+00   1.3327968833411243e+00
   3.1366566384847490e+00   1.3645301424682938e+00
   3.1366566384847490e+00   1.3962634015954634e+00
   3.1366566384847490e+00   1.4279966607226333e+00
   3.1366566384847490e+00   1.4597299198498028e+00
   3.1366566384847490e+00   1.4914631789769726e+00
   3.1366566384847490e+00   1.5231964381041421e+00
   3.1366566384847490e+00   1.5549296972313116e+00
   3.1366566384847490e+00   1.5866629563584815e+00
   3.1366566384847490e+00   1.6183962154856510e+00
   3.1366566384847490e+00   1.6501294746128208e+00
   3.1366566384847490e+00   1.6818627337399903e+00
   3.1366566384847490e+00   1.7135959928671598e+00
   3.1366566384847490e+00   1.7453292519943295e+00
   3.1366566384847490e+00   1.7770625111214990e+00
   3.1366566384847490e+00   1.8087957702486686e+00
   3.1366566384847490e+00   1.8405290293758385e+00
   3.1366566384847490e+00   1.8722622885030080e+00
   3.1366566384847490e+00   1.9039955476301775e+00
   3.1366566384847490e+00   1.9357288067573473e+00
   3.1366566384847490e+00   1.9674620658845168e+00
   3.1366566384847490e+00   1.9991953250116867e+00
   3.1366566384847490e+00   2.0309285841388562e+00
   3.1366566384847490e+00   2.0626618432660258e+00
   3.1366566384847490e+00   2.0943951023931953e+00
   3.1366566384847490e+00   2.1261283615203652e+00
   3.1366566384847490e+00   2.1578616206475347e+00
   3.1366566384847490e+00   2.1895948797747042e+00
   3.1366566384847490e+00   2.2213281389018737e+00
   3.1366566384847490e+00   2.2530613980290437e+00
   3.1366566384847490e+00   2.2847946571562132e+00
   3.1682304339982146e+00   9.5199777381508877e-01
   3.1682304339982146e+00   9.8373103294225839e-01
   3.1682304339982146e+00   1.0154642920694281e+00
   3.1682304339982146e+00   1.0471975511965976e+00
   3.1682304339982146e+00   1.0789308103237674e+00
   3.1682304339982146e+00   1.1106640694509369e+00
   3.1682304339982146e+00   1.1423973285781066e+00
   3.1682304339982146e+00   1.1741305877052763e+00
   3.1682304339982146e+00   1.2058638468324459e+00
   3.1682304339982146e+00   1.2375971059596154e+00
   3.1682304339982146e+00   1.2693303650867851e+00
   3.1682304339982146e+00   1.3010636242139546e+00
   3.1682304339982146e+00   1.3327968833411243e+00
   3.1682304339982146e+00   1.3645301424682938e+00
   3.1682304339982146e+00   1.3962634015954634e+00
   3.1682304339982146e+00   1.4279966607226333e+00
   3.1682304339982146e+00   1.4597299198498028e+00
   3.1682304339982146e+00   1.4914631789769726e+00
   3.1682304339982146e+00   1.5231964381041421e+00
   3.1682304339982146e+00   1.5549296972313116e+00
   3.1682304339982146e+00   1.5866629563584815e+00
   3.1682304339982146e+00   1.6183962154856510e+00
   3.1682304339982146e+00   1.6501294746128208e+00
   3.1682304339982146e+00   1.6818627337399903e+00
   3.1682304339982146e+00   1.7135959928671598e+00
   3.1682304339982146e+00   1.7453292519943295e+00
   3.1682304339982146e+00   1.7770625111214990e+00
   3.1682304339982146e+00   1.8087957702486686e+00
   3.1682304339982146e+00   1.8405290293758385e+00
   3.1682304339982146e+00   1.8722622885030080e+00
   3.1682304339982146e+00   1.9039955476301775e+00
   3.1682304339982146e+00   1.9357288067573473e+00
   3.1682304339982146e+00   1.9674620658845168e+00
   3.1682304339982146e+00   1.9991953250116867e+00
   3.1682304339982146e+00   2.0309285841388562e+00
   3.1682304339982146e+00   2.0626618432660258e+00
   3.1682304339982146e+00   2.0943951023931953e+00
   3.1682304339982146e+00   2.1261283615203652e+00
   3.1682304339982146e+00   2.1578616206475347e+00
   3.1682304339982146e+00   2.1895948797747042e+00
   3.1682304339982146e+00   2.2213281389018737e+00
   3.1682304339982146e+00   2.2530613980290437e+00
   3.1682304339982146e+00   2.2847946571562132e+00
   3.1998042295116798e+00   9.5199777381508877e-01
   3.1998042295116798e+00   9.8373103294225839e-01
   3.1998042295116798e+00   1.0154642920694281e+00
   3.1998042295116798e+00   1.0471975511965976e+00
   3.1998042295116798e+00   1.0789308103237674e+00
   3.1998042295116798e+00   1.1106640694509369e+00
   3.1998042295116798e+00   1.1423973285781066e+00
   3.1998042295116798e+00   1.1741305877052763e+00
   3.1998042295116798e+00   1.2058638468324459e+00
   3.1998042295116798e+00   1.2375971059596154e+00
   3.1998042295116798e+00   1.2693303650867851e+00
   3.1998042295116798e+00   1.3010636242139546e+00
   3.1998042295116798e+00   1.3327968833411243e+00
   3.1998042295116798e+00   1.3645301424682938e+00
   3.1998042295116798e+00   1.3962634015954634e+00
   3.1998042295116798e+00   1.4279966607226333e+00
   3.1998042295116798e+00   1.4597299198498028e+00
   3.1998042295116798e+00   1.4914631789769726e+00
   3.1998042295116798e+00   1.5231964381041421e+00
   3.1998042295116798e+00   1.5549296972313116e+00
   3.1998042295116798e+00   1.5866629563584815e+00
   3.1998042295116798e+00   1.6183962154856510e+00
   3.1998042295116798e+00   1.6501294746128208e+00
   3.1998042295116798e+00   1.6818627337399903e+00
   3.1998042295116798e+00   1.7135959928671598e+00
   3.1998042295116798e+00   1.7453292519943295e+00
   3.1998042295116798e+00   1.7770625111214990e+00
   3.1998042295116798e+00   1.8087957702486686e+00
   3.1998042295116798e+00   1.8405290293758385e+00
   3.1998042295116798e+00   1.8722622885030080e+00
   3.1998042295116798e+00   1.9039955476301775e+00
   3.1998042295116798e+00   1.9357288067573473e+00
   3.1998042295116798e+00   1.9674620658845168e+00
   3.1998042295116798e+00   1.9991953250116867e+00
   3.1998042295116798e+00   2.0309285841388562e+00
   3.1998042295116798e+00   2.0626618432660258e+00
   3.1998042295116798e+00   2.0943951023931953e+00
   3.1998042295116798e+00   2.1261283615203652e+00
   3.1998042295116798e+00   2.1578616206475347e+00
   3.1998042295116798e+00   2.1895948797747042e+00
   3.1998042295116798e+00   2.2213281389018737e+00
   3.1998042295116798e+00   2.2530613980290437e+00
   3.1998042295116798e+00   2.2847946571562132e+00
   3.2313780250251449e+00   9.5199777381508877e-01
   3.2313780250251449e+00   9.8373103294225839e-01
   3.2313780250251449e+00   1.0154642920694281e+00
   3.2313780250251449e+00   1.0471975511965976e+00
   3.2313780250251449e+00   1.0789308103237674e+00
   3.2313780250251449e+00   1.1106640694509369e+00
   3.2313780250251449e+00   1.1423973285781066e+00
   3.2313780250251449e+00   1.1741305877052763e+00
   3.2313780250251449e+00   1.2058638468324459e+00
   3.2313780250251449e+00   1.2375971059596154e+00
   3.2313780250251449e+00   1.2693303650867851e+00
   3.2313780250251449e+00   1.3010636242139546e+00
   3.2313780250251449e+00   1.3327968833411243e+00
   3.2313780250251449e+00   1.3645301424682938e+00
   3.2313780250251449e+00   1.3962634015954634e+00
   3.2313780250251449e+00   1.4279966607226333e+00
   3.2313780250251449e+00   1.4597299198498028e+00
   3.2313780250251449e+00   1.4914631789769726e+00
   3.2313780250251449e+00   1.5231964381041421e+00
   3.2313780250251449e+00   1.5549296972313116e+00
   3.2313780250251449e+00   1.5866629563584815e+00
   3.2313780250251449e+00   1.6183962154856510e+00
   3.2313780250251449e+00   1.6501294746128208e+00
   3.2313780250251449e+00   1.6818627337399903e+00
   3.2313780250251449e+00   1.7135959928671598e+00
   3.2313780250251449e+00   1.7453292519943295e+00
   3.2313780250251449e+00   1.7770625111214990e+00
   3.2313780250251449e+00   1.8087957702486686e+00
   3.2313780250251449e+00   1.8405290293758385e+00
   3.2313780250251449e+00   1.8722622885030080e+00
   3.2313780250251449e+00   1.9039955476301775e+00
   3.2313780250251449e+00   1.9357288067573473e+00
   3.2313780250251449e+00   1.9674620658845168e+00
   3.2313780250251449e+00   1.9991953250116867e+00
   3.2313780250251449e+00   2.0309285841388562e+00
   3.2313780250251449e+00   2.0626618432660258e+00
   3.2313780250251449e+00   2.0943951023931953e+00
   3.2313780250251449e+00   2.1261283615203652e+00
   3.2313780250251449e+00   2.1578616206475347e+00
   3.2313780250251449e+00   2.1895948797747042e+00
   3.2313780250251449e+00   2.2213281389018737e+00
   3.2313780250251449e+00   2.2530613980290437e+00
   3.2629518205386105e+00   9.8373103294225839e-01
   3.2629518205386105e+00   1.0154642920694281e+00
   3.2629518205386105e+00   1.0471975511965976e+00
   3.2629518205386105e+00   1.0789308103237674e+00
   3.2629518205386105e+00   1.1106640694509369e+00
   3.2629518205386105e+00   1.1423973285781066e+00
   3.2629518205386105e+00   1.1741305877052763e+00
   3.2629518205386105e+00   1.2058638468324459e+00
   3.2629518205386105e+00   1.2375971059596154e+00
   3.2629518205386105e+00   1.2693303650867851e+00
   3.2629518205386105e+00   1.3010636242139546e+00
   3.2629518205386105e+00   1.3327968833411243e+00
   3.2629518205386105e+00   1.3645301424682938e+00
   3.2629518205386105e+00   1.3962634015954634e+00
   3.2629518205386105e+00   1.4279966607226333e+00
   3.2629518205386105e+00   1.4597299198498028e+00
   3.2629518205386105e+00   1.4914631789769726e+00
   3.2629518205386105e+00   1.5231964381041421e+00
   3.2629518205386105e+00   1.5549296972313116e+00
   3.2629518205386105e+00   1.5866629563584815e+00
   3.2629518205386105e+00   1.6183962154856510e+00
   3.2629518205386105e+00   1.6501294746128208e+00
   3.2629518205386105e+00   1.6818627337399903e+00
   3.2629518205386105e+00   1.7135959928671598e+00
   3.2629518205386105e+00   1.7453292519943295e+00
   3.2629518205386105e+00   1.7770625111214990e+00
   3.2629518205386105e+00   1.8087957702486686e+00
   3.2629518205386105e+00   1.8405290293758385e+00
   3.2629518205386105e+00   1.8722622885030080e+00
   3.2629518205386105e+00   1.9039955476301775e+00
   3.2629518205386105e+00   1.9357288067573473e+00
   3.2629518205386105e+00   1.9674620658845168e+00
   3.2629518205386105e+00   1.9991953250116867e+00
   3.2629518205386105e+00   2.0309285841388562e+00
   3.2629518205386105e+00   2.0626618432660258e+00
   3.2629518205386105e+00   2.0943951023931953e+00
   3.2629518205386105e+00   2.1261283615203652e+00
   3.2629518205386105e+00   2.1578616206475347e+00
   3.2629518205386105e+00   2.1895948797747042e+00
   3.2629518205386105e+00   2.2213281389018737e+00
   3.2629518205386105e+00   2.2530613980290437e+00
   3.2945256160520753e+00   9.8373103294225839e-01
   3.2945256160520753e+00   1.0154642920694281e+00
   3.2945256160520753e+00   1.0471975511965976e+00
   3.2945256160520753e+00   1.0789308103237674e+00
   3.2945256160520753e+00   1.1106640694509369e+00
   3.2945256160520753e+00   1.1423973285781066e+00
   3.2945256160520753e+00   1.1741305877052763e+00
   3.2945256160520753e+00   1.2058638468324459e+00
   3.2945256160520753e+00   1.2375971059596154e+00
   3.2945256160520753e+00   1.2693303650867851e+00
   3.2945256160520753e+00   1.3010636242139546e+00
   3.2945256160520753e+00   1.3327968833411243e+00
   3.2945256160520753e+00   1.3645301424682938e+00
   3.2945256160520753e+00   1.3962634015954634e+00
   3.2945256160520753e+00   1.4279966607226333e+00
   3.2945256160520753e+00   1.4597299198498028e+00
   3.2945256160520753e+00   1.4914631789769726e+00
   3.2945256160520753e+00   1.5231964381041421e+00
   3.2945256160520753e+00   1.5549296972313116e+00
   3.2945256160520753e+00   1.5866629563584815e+00
   3.2945256160520753e+00   1.6183962154856510e+00
   3.2945256160520753e+00   1.6501294746128208e+00
   3.2945256160520753e+00   1.6818627337399903e+00
   3.2945256160520753e+00   1.7135959928671598e+00
   3.2945256160520753e+00   1.7453292519943295e+00
   3.2945256160520753e+00   1.7770625111214990e+00
   3.2945256160520753e+00   1.8087957702486686e+00
   3.2945256160520753e+00   1.8405290293758385e+00
   3.2945256160520753e+00   1.8722622885030080e+00
   3.2945256160520753e+00   1.9039955476301775e+00
   3.2945256160520753e+00   1.9357288067573473e+00
   3.2945256160520753e+00   1.9674620658845168e+00
   3.2945256160520753e+00   1.9991953250116867e+00
   3.2945256160520753e+00   2.0309285841388562e+00
   3.2945256160520753e+00   2.0626618432660258e+00
   3.2945256160520753e+00   2.0943951023931953e+00
   3.2945256160520753e+00   2.1261283615203652e+00
   3.2945256160520753e+00   2.1578616206475347e+00
   3.2945256160520753e+00   2.1895948797747042e+00
   3.2945256160520753e+00   2.2213281389018737e+00
   3.2945256160520753e+00   2.2530613980290437e+00
   3.3260994115655409e+00   9.8373103294225839e-01
   3.3260994115655409e+00   1.0154642920694281e+00
   3.3260994115655409e+00   1.0471975511965976e+00
   3.3260994115655409e+00   1.0789308103237674e+00
   3.3260994115655409e+00   1.1106640694509369e+00
   3.3260994115655409e+00   1.1423973285781066e+00
   3.3260994115655409e+00   1.1741305877052763e+00
   3.3260994115655409e+00   1.2058638468324459e+00
   3.3260994115655409e+00   1.2375971059596154e+00
   3.3260994115655409e+00   1.2693303650867851e+00
   3.3260994115655409e+00   1.3010636242139546e+00
   3.3260994115655409e+00   1.3327968833411243e+00
   3.3260994115655409e+00   1.3645301424682938e+00
   3.3260994115655409e+00   1.3962634015954634e+00
   3.3260994115655409e+00   1.4279966607226333e+00
   3.3260994115655409e+00   1.4597299198498028e+00
   3.3260994115655409e+00   1.4914631789769726e+00
   3.3260994115655409e+00   1.5231964381041421e+00
   3.3260994115655409e+00   1.5549296972313116e+00
   3.3260994115655409e+00   1.5866629563584815e+00
   3.3260994115655409e+00   1.6183962154856510e+00
   3.3260994115655409e+00   1.6501294746128208e+00
   3.3260994115655409e+00   1.6818627337399903e+00
   3.3260994115655409e+00   1.7135959928671598e+00
   3.3260994115655409e+00   1.7453292519943295e+00
   3.3260994115655409e+00   1.7770625111214990e+00
   3.3260994115655409e+00   1.8087957702486686e+00
   3.3260994115655409e+00   1.8405290293758385e+00
   3.3260994115655409e+00   1.8722622885030080e+00
   3.3260994115655409e+00   1.9039955476301775e+00
   3.3260994115655409e+00   1.9357288067573473e+00
   3.3260994115655409e+00   1.9674620658845168e+00
   3.3260994115655409e+00   1.9991953250116867e+00
   3.3260994115655409e+00   2.0309285841388562e+00
   3.3260994115655409e+00   2.0626618432660258e+00
   3.3260994115655409e+00   2.0943951023931953e+00
   3.3260994115655409e+00   2.1261283615203652e+00
   3.3260994115655409e+00   2.1578616206475347e+00
   3.3260994115655409e+00   2.1895948797747042e+00
   3.3260994115655409e+00   2.2213281389018737e+00
   3.3576732070790061e+00   9.8373103294225839e-01
   3.3576732070790061e+00   1.0154642920694281e+00
   3.3576732070790061e+00   1.0471975511965976e+00
   3.3576732070790061e+00   1.0789308103237674e+00
   3.3576732070790061e+00   1.1106640694509369e+00
   3.3576732070790061e+00   1.1423973285781066e+00
   3.3576732070790061e+00   1.1741305877052763e+00
   3.3576732070790061e+00   1.2058638468324459e+00
   3.3576732070790061e+00   1.2375971059596154e+00
   3.3576732070790061e+00   1.2693303650867851e+00
   3.3576732070790061e+00   1.3010636242139546e+00
   3.3576732070790061e+00   1.3327968833411243e+00
   3.3576732070790061e+00   1.3645301424682938e+00
   3.3576732070790061e+00   1.3962634015954634e+00
   3.3576732070790061e+00   1.4279966607226333e+00
   3.3576732070790061e+00   1.4597299198498028e+00
   3.3576732070790061e+00   1.4914631789769726e+00
   3.3576732070790061e+00   1.5231964381041421e+00
   3.3576732070790061e+00   1.5549296972313116e+00
   3.3576732070790061e+00   1.5866629563584815e+00
   3.3576732070790061e+00   1.6183962154856510e+00
   3.3576732070790061e+00   1.6501294746128208e+00
   3.3576732070790061e+00   1.6818627337399903e+00
   3.3576732070790061e+00   1.7135959928671598e+00
   3.3576732070790061e+00   1.7453292519943295e+00
   3.3576732070790061e+00   1.7770625111214990e+00
   3.3576732070790061e+00   1.8087957702486686e+00
   3.3576732070790061e+00   1.8405290293758385e+00
   3.3576732070790061e+00   1.8722622885030080e+00
   3.3576732070790061e+00   1.9039955476301775e+00
   3.3576732070790061e+00   1.9357288067573473e+00
   3.3576732070790061e+00   1.9674620658845168e+00
   3.3576732070790061e+00   1.9991953250116867e+00
   3.3576732070790061e+00   2.0309285841388562e+00
   3.3576732070790061e+00   2.0626618432660258e+00
   3.3576732070790061e+00   2.0943951023931953e+00
   3.3576732070790061e+00   2.1261283615203652e+00
   3.3576732070790061e+00   2.1578616206475347e+00
   3.3576732070790061e+00   2.1895948797747042e+00
   3.3576732070790061e+00   2.2213281389018737e+00
   3.3892470025924712e+00   9.8373103294225839e-01
   3.3892470025924712e+00   1.0154642920694281e+00
   3.3892470025924712e+00   1.0471975511965976e+00
   3.3892470025924712e+00   1.0789308103237674e+00
   3.3892470025924712e+00   1.1106640694509369e+00
   3.3892470025924712e+00   1.1423973285781066e+00
   3.3892470025924712e+00   1.1741305877052763e+00
   3.3892470025924712e+00   1.2058638468324459e+00
   3.3892470025924712e+00   1.2375971059596154e+00
   3.3892470025924712e+00   1.2693303650867851e+00
   3.3892470025924712e+00   1.3010636242139546e+00
   3.3892470025924712e+00   1.3327968833411243e+00
   3.3892470025924712e+00   1.3645301424682938e+00
   3.3892470025924712e+00   1.3962634015954634e+00
   3.3892470025924712e+00   1.4279966607226333e+00
   3.3892470025924712e+00   1.4597299198498028e+00
   3.3892470025924712e+00   1.4914631789769726e+00
   3.3892470025924712e+00   1.5231964381041421e+00
   3.3892470025924712e+00   1.5549296972313116e+00
   3.3892470025924712e+00   1.5866629563584815e+00
   3.3892470025924712e+00   1.6183962154856510e+00
   3.3892470025924712e+00   1.6501294746128208e+00
   3.3892470025924712e+00   1.6818627337399903e+00
   3.3892470025924712e+00   1.7135959928671598e+00
   3.3892470025924712e+00   1.7453292519943295e+00
   3.3892470025924712e+00   1.7770625111214990e+00
   3.3892470025924712e+00   1.8087957702486686e+00
   3.3892470025924712e+00   1.8405290293758385e+00
   3.3892470025924712e+00   1.8722622885030080e+00
   3.3892470025924712e+00   1.9039955476301775e+00
   3.3892470025924712e+00   1.9357288067573473e+00
   3.3892470025924712e+00   1.9674620658845168e+00
   3.3892470025924712e+00   1.9991953250116867e+00
   3.3892470025924712e+00   2.0309285841388562e+00
   3.3892470025924712e+00   2.0626618432660258e+00
   3.3892470025924712e+00   2.0943951023931953e+00
   3.3892470025924712e+00   2.1261283615203652e+00
   3.3892470025924712e+00   2.1578616206475347e+00
   3.3892470025924712e+00   2.1895948797747042e+00
   3.3892470025924712e+00   2.2213281389018737e+00
   3.4208207981059369e+00   1.0154642920694281e+00
   3.4208207981059369e+00   1.0471975511965976e+00
   3.4208207981059369e+00   1.0789308103237674e+00
   3.4208207981059369e+00   1.1106640694509369e+00
   3.4208207981059369e+00   1.1423973285781066e+00
   3.4208207981059369e+00   1.1741305877052763e+00
   3.4208207981059369e+00   1.2058638468324459e+00
   3.4208207981059369e+00   1.2375971059596154e+00
   3.4208207981059369e+00   1.2693303650867851e+00
   3.4208207981059369e+00   1.3010636242139546e+00
   3.4208207981059369e+00   1.3327968833411243e+00
   3.4208207981059369e+00   1.3645301424682938e+00
   3.4208207981059369e+00   1.3962634015954634e+00
   3.4208207981059369e+00   1.4279966607226333e+00
   3.4208207981059369e+00   1.4597299198498028e+00
   3.4208207981059369e+00   1.4914631789769726e+00
   3.4208207981059369e+00   1.5231964381041421e+00
   3.4208207981059369e+00   1.5549296972313116e+00
   3.4208207981059369e+00   1.5866629563584815e+00
   3.4208207981059369e+00   1.6183962154856510e+00
   3.4208207981059369e+00   1.6501294746128208e+00
   3.4208207981059369e+00   1.6818627337399903e+00
   3.4208207981059369e+00   1.7135959928671598e+00
   3.4208207981059369e+00   1.7453292519943295e+00
   3.4208207981059369e+00   1.7770625111214990e+00
   3.4208207981059369e+00   1.8087957702486686e+00
   3.4208207981059369e+00   1.8405290293758385e+00
   3.4208207981059369e+00   1.8722622885030080e+00
   3.4208207981059369e+00   1.9039955476301775e+00
   3.4208207981059369e+00   1.9357288067573473e+00
   3.4208207981059369e+00   1.9674620658845168e+00
   3.4208207981059369e+00   1.9991953250116867e+00
   3.4208207981059369e+00   2.0309285841388562e+00
   3.4208207981059369e+00   2.0626618432660258e+00
   3.4208207981059369e+00   2.0943951023931953e+00
   3.4208207981059369e+00   2.1261283615203652e+00
   3.4208207981059369e+00   2.1578616206475347e+00
   3.4208207981059369e+00   2.1895948797747042e+00
   3.4523945936194016e+00   1.0471975511965976e+00
   3.4523945936194016e+00   1.0789308103237674e+00
   3.4523945936194016e+00   1.1106640694509369e+00
   3.4523945936194016e+00   1.1423973285781066e+00
   3.4523945936194016e+00   1.1741305877052763e+00
   3.4523945936194016e+00   1.2058638468324459e+00
   3.4523945936194016e+00   1.2375971059596154e+00
   3.4523945936194016e+00   1.2693303650867851e+00
   3.4523945936194016e+00   1.3010636242139546e+00
   3.4523945936194016e+00   1.3327968833411243e+00
   3.4523945936194016e+00   1.3645301424682938e+00
   3.4523945936194016e+00   1.3962634015954634e+00
   3.4523945936194016e+00   1.4279966607226333e+00
   3.4523945936194016e+00   1.4597299198498028e+00
   3.4523945936194016e+00   1.4914631789769726e+00
   3.4523945936194016e+00   1.5231964381041421e+00
   3.4523945936194016e+00   1.5549296972313116e+00
   3.4523945936194016e+00   1.5866629563584815e+00
   3.4523945936194016e+00   1.6183962154856510e+00
   3.4523945936194016e+00   1.6501294746128208e+00
   3.4523945936194016e+00   1.6818627337399903e+00
   3.4523945936194016e+00   1.7135959928671598e+00
   3.4523945936194016e+00   1.7453292519943295e+00
   3.4523945936194016e+00   1.7770625111214990e+00
   3.4523945936194016e+00   1.8087957702486686e+00
   3.4523945936194016e+00   1.8405290293758385e+00
   3.4523945936194016e+00   1.8722622885030080e+00
   3.4523945936194016e+00   1.9039955476301775e+00
   3.4523945936194016e+00   1.9357288067573473e+00
   3.4523945936194016e+00   1.9674620658845168e+00
   3.4523945936194016e+00   1.9991953250116867e+00
   3.4523945936194016e+00   2.0309285841388562e+00
   3.4523945936194016e+00   2.0626618432660258e+00
   3.4523945936194016e+00   2.0943951023931953e+00
   3.4523945936194016e+00   2.1261283615203652e+00
   3.4523945936194016e+00   2.1578616206475347e+00
   3.4523945936194016e+00   2.1895948797747042e+00
   3.4839683891328672e+00   1.0789308103237674e+00
   3.4839683891328672e+00   1.1106640694509369e+00
   3.4839683891328672e+00   1.1423973285781066e+00
   3.4839683891328672e+00   1.1741305877052763e+00
   3.4839683891328672e+00   1.2058638468324459e+00
   3.4839683891328672e+00   1.2375971059596154e+00
   3.4839683891328672e+00   1.2693303650867851e+00
   3.4839683891328672e+00   1.3010636242139546e+00
   3.4839683891328672e+00   1.3327968833411243e+00
   3.4839683891328672e+00   1.3645301424682938e+00
   3.4839683891328672e+00   1.3962634015954634e+00
   3.4839683891328672e+00   1.4279966607226333e+00
   3.4839683891328672e+00   1.4597299198498028e+00
   3.4839683891328672e+00   1.4914631789769726e+00
   3.4839683891328672e+00   1.5231964381041421e+00
   3.4839683891328672e+00   1.5549296972313116e+00
   3.4839683891328672e+00   1.5866629563584815e+00
   3.4839683891328672e+00   1.6183962154856510e+00
   3.4839683891328672e+00   1.6501294746128208e+00
   3.4839683891328672e+00   1.6818627337399903e+00
   3.4839683891328672e+00   1.7135959928671598e+00
   3.4839683891328672e+00   1.7453292519943295e+00
   3.4839683891328672e+00   1.7770625111214990e+00
   3.4839683891328672e+00   1.8087957702486686e+00
   3.4839683891328672e+00   1.8405290293758385e+00
   3.4839683891328672e+00   1.8722622885030080e+00
   3.4839683891328672e+00   1.9039955476301775e+00
   3.4839683891328672e+00   1.9357288067573473e+00
   3.4839683891328672e+00   1.9674620658845168e+00
   3.4839683891328672e+00   1.9991953250116867e+00
   3.4839683891328672e+00   2.0309285841388562e+00
   3.4839683891328672e+00   2.0626618432660258e+00
   3.4839683891328672e+00   2.0943951023931953e+00
   3.4839683891328672e+00   2.1261283615203652e+00
   3.4839683891328672e+00   2.1578616206475347e+00
   3.5155421846463324e+00   1.1423973285781066e+00
   3.5155421846463324e+00   1.1741305877052763e+00
   3.5155421846463324e+00   1.2058638468324459e+00
   3.5155421846463324e+00   1.2375971059596154e+00
   3.5155421846463324e+00   1.2693303650867851e+00
   3.5155421846463324e+00   1.3010636242139546e+00
   3.5155421846463324e+00   1.3327968833411243e+00
   3.5155421846463324e+00   1.3645301424682938e+00
   3.5155421846463324e+00   1.3962634015954634e+00
   3.5155421846463324e+00   1.4279966607226333e+00
   3.5155421846463324e+00   1.4597299198498028e+00
   3.5155421846463324e+00   1.4914631789769726e+00
   3.5155421846463324e+00   1.5231964381041421e+00
   3.5155421846463324e+00   1.5549296972313116e+00
   3.5155421846463324e+00   1.5866629563584815e+00
   3.5155421846463324e+00   1.6183962154856510e+00
   3.5155421846463324e+00   1.6501294746128208e+00
   3.5155421846463324e+00   1.6818627337399903e+00
   3.5155421846463324e+00   1.7135959928671598e+00
   3.5155421846463324e+00   1.7453292519943295e+00
   3.5155421846463324e+00   1.7770625111214990e+00
   3.5155421846463324e+00   1.8087957702486686e+00
   3.5155421846463324e+00   1.8405290293758385e+00
   3.5155421846463324e+00   1.8722622885030080e+00
   3.5155421846463324e+00   1.9039955476301775e+00
   3.5155421846463324e+00   1.9357288067573473e+00
   3.5155421846463324e+00   1.9674620658845168e+00
   3.5155421846463324e+00   1.9991953250116867e+00
   3.5155421846463324e+00   2.0309285841388562e+00
   3.5155421846463324e+00   2.0626618432660258e+00
   3.5155421846463324e+00   2.0943951023931953e+00
   3.5155421846463324e+00   2.1261283615203652e+00
   3.5471159801597976e+00   1.1741305877052763e+00
   3.5471159801597976e+00   1.2058638468324459e+00
   3.5471159801597976e+00   1.2375971059596154e+00
   3.5471159801597976e+00   1.2693303650867851e+00
   3.5471159801597976e+00   1.3010636242139546e+00
   3.5471159801597976e+00   1.3327968833411243e+00
   3.5471159801597976e+00   1.3645301424682938e+00
   3.5471159801597976e+00   1.3962634015954634e+00
   3.5471159801597976e+00   1.4279966607226333e+00
   3.5471159801597976e+00   1.4597299198498028e+00
   3.5471159801597976e+00   1.4914631789769726e+00
   3.5471159801597976e+00   1.5231964381041421e+00
   3.5471159801597976e+00   1.5549296972313116e+00
   3.5471159801597976e+00   1.5866629563584815e+00
   3.5471159801597976e+00   1.6183962154856510e+00
   3.5471159801597976e+00   1.6501294746128208e+00
   3.5471159801597976e+00   1.6818627337399903e+00
   3.5471159801597976e+00   1.7135959928671598e+00
   3.5471159801597976e+00   1.7453292519943295e+00
   3.5471159801597976e+00   1.7770625111214990e+00
   3.5471159801597976e+00   1.8087957702486686e+00
   3.5471159801597976e+00   1.8405290293758385e+00
   3.5471159801597976e+00   1.8722622885030080e+00
   3.5471159801597976e+00   1.9039955476301775e+00
   3.5471159801597976e+00   1.9357288067573473e+00
   3.5471159801597976e+00   1.9674620658845168e+00
   3.5471159801597976e+00   1.9991953250116867e+00
   3.5471159801597976e+00   2.0309285841388562e+00
   3.5471159801597976e+00   2.0626618432660258e+00
   3.5471159801597976e+00   2.0943951023931953e+00
   3.5471159801597976e+00   2.1261283615203652e+00
   3.5786897756732632e+00   1.2693303650867851e+00
   3.5786897756732632e+00   1.3010636242139546e+00
   3.5786897756732632e+00   1.3327968833411243e+00
   3.5786897756732632e+00   1.3645301424682938e+00
   3.5786897756732632e+00   1.3962634015954634e+00
   3.5786897756732632e+00   1.4279966607226333e+00
   3.5786897756732632e+00   1.4597299198498028e+00
   3.5786897756732632e+00   1.4914631789769726e+00
   3.5786897756732632e+00   1.5231964381041421e+00
   3.5786897756732632e+00   1.5549296972313116e+00
   3.5786897756732632e+00   1.5866629563584815e+00
   3.5786897756732632e+00   1.6183962154856510e+00
   3.5786897756732632e+00   1.6501294746128208e+00
   3.5786897756732632e+00   1.6818627337399903e+00
   3.5786897756732632e+00   1.7135959928671598e+00
   3.5786897756732632e+00   1.7453292519943295e+00
   3.5786897756732632e+00   1.7770625111214990e+00
   3.5786897756732632e+00   1.8087957702486686e+00
   3.5786897756732632e+00   1.8405290293758385e+00
   3.5786897756732632e+00   1.8722622885030080e+00
   3.5786897756732632e+00   1.9039955476301775e+00
   3.5786897756732632e+00   1.9357288067573473e+00
   3.5786897756732632e+00   1.9674620658845168e+00
   3.5786897756732632e+00   1.9991953250116867e+00
   3.5786897756732632e+00   2.0309285841388562e+00
   3.5786897756732632e+00   2.0626618432660258e+00
   3.6102635711867279e+00   1.4279966607226333e+00
   3.6102635711867279e+00   1.4597299198498028e+00
   3.6102635711867279e+00   1.4914631789769726e+00
   3.6102635711867279e+00   1.5231964381041421e+00
   3.6102635711867279e+00   1.5549296972313116e+00
   3.6102635711867279e+00   1.5866629563584815e+00
   3.6102635711867279e+00   1.6183962154856510e+00
   3.6102635711867279e+00   1.6501294746128208e+00
   3.6102635711867279e+00   1.6818627337399903e+00
   3.6102635711867279e+00   1.7135959928671598e+00
   3.6102635711867279e+00   1.7453292519943295e+00
   3.6102635711867279e+00   1.7770625111214990e+00
   3.6102635711867279e+00   1.8087957702486686e+00
   3.6102635711867279e+00   1.8405290293758385e+00
   3.6102635711867279e+00   1.8722622885030080e+00
   3.6102635711867279e+00   1.9039955476301775e+00
   3.6102635711867279e+00   1.9357288067573473e+00
   3.6102635711867279e+00   1.9674620658845168e+00
   3.6102635711867279e+00   1.9991953250116867e+00
   3.6102635711867279e+00   2.0309285841388562e+00
   3.6418373667001935e+00   1.4914631789769726e+00
   3.6418373667001935e+00   1.5231964381041421e+00
   3.6418373667001935e+00   1.5549296972313116e+00
   3.6418373667001935e+00   1.5866629563584815e+00
   3.6418373667001935e+00   1.6183962154856510e+00
   3.6418373667001935e+00   1.6501294746128208e+00
   3.6418373667001935e+00   1.6818627337399903e+00
   3.6418373667001935e+00   1.7135959928671598e+00
   3.6418373667001935e+00   1.7453292519943295e+00
   3.6418373667001935e+00   1.7770625111214990e+00
   3.6418373667001935e+00   1.8087957702486686e+00
   3.6418373667001935e+00   1.8405290293758385e+00
   3.6418373667001935e+00   1.8722622885030080e+00
   3.6418373667001935e+00   1.9039955476301775e+00
   3.6418373667001935e+00   1.9357288067573473e+00
   3.6734111622136587e+00   1.5231964381041421e+00
   3.6734111622136587e+00   1.5549296972313116e+00
   3.6734111622136587e+00   1.5866629563584815e+00
   3.6734111622136587e+00   1.6183962154856510e+00
   3.6734111622136587e+00   1.6501294746128208e+00
   3.6734111622136587e+00   1.6818627337399903e+00
   3.6734111622136587e+00   1.7135959928671598e+00
   3.6734111622136587e+00   1.7453292519943295e+00
   3.6734111622136587e+00   1.7770625111214990e+00
   3.6734111622136587e+00   1.8087957702486686e+00
   3.6734111622136587e+00   1.8405290293758385e+00
   3.7049849577271239e+00   1.5549296972313116e+00
   3.7049849577271239e+00   1.5866629563584815e+00
   3.7049849577271239e+00   1.6183962154856510e+00


==> cyl_non_coh_set_img.tex <==
   1.7338484351864736e+00   1.9124139329779238e-01
   5.3924379410853618e+00   2.7649967660898831e+00
   4.0323075684016985e+00   2.9448456498973994e+00
   4.2621171217847262e+00   2.2988136094472789e+00
   4.9792728855537227e+00   2.7824959131891154e+00
   4.0064755338191134e+00   2.4264730274801383e+00
   5.9154812227031428e-01   3.0415658317511576e+00
   4.6852791978464055e+00   2.4373973538651312e+00
   4.0794198494938101e+00   1.1922071498615212e+00
   1.0634340925299242e+00   2.8058730643896848e+00
   1.6383875814637143e+00   2.3569931887714688e+00
   4.0151123130732422e+00   8.9363656372213585e-01
   3.9105169888197793e+00   6.3037350848593543e-01
   4.0214654502664935e+00   7.1855621484347498e-01
   4.0537780336701950e+00   7.6319987201694306e-01
   4.0084899464062076e+00   7.0978763614705387e-01
   3.8602922333226388e+00   6.3389566875490300e-01
   4.0569299222575914e+00   1.0436758103120491e+00
   3.9952051405619677e+00   7.1499545595344105e-01
   4.7254528579482731e+00   2.1927283643278686e+00
   4.2930114146244236e+00   1.9431552214555330e+00
   1.2200086572324054e+00   3.0227655036330825e-01
   1.8044635108933917e+00   1.1848508008515456e-01
   9.9113495060669976e-01   2.8055647180147294e+00
   4.0782036420726051e+00   1.8811029584504562e+00
   3.8819271195630733e+00   6.0877138698552369e-01
   3.8782612640808196e+00   2.7449157193749700e+00
   5.3320672358611674e+00   2.7308307489304791e+00
   5.2576701685579827e+00   3.7853199716309632e-01
   4.6493718782329161e+00   3.1407222607500640e-01
   1.8970127114606399e+00   6.5819393197601972e-01
   3.4261208161594325e-01   2.8641120524372363e+00
   1.3467450660309623e+00   6.5048029626123682e-01
   1.6191714070333774e+00   2.4355277706726346e+00
   4.5520591132997552e+00   2.6125434726503971e+00
   4.0850172537534597e+00   1.6258804958372646e+00
   4.1412403523088912e+00   1.0099566682214833e+00
   3.8867484836095123e+00   6.6316024732724044e-01
   4.1097911148264004e+00   9.1575486599262856e-01
   5.2819069849200346e+00   3.1140055580736621e+00
   4.2313659240542236e+00   2.3533052101247902e+00
   4.0288125425765067e+00   1.0096158638742918e+00
   1.2827874959066321e+00   2.4615250498665762e+00
   3.6669700685122883e+00   3.4417635973654376e-01
   4.6057539724503300e+00   5.7071392930191922e-01
   4.4364862360156394e+00   8.9789123347710997e-01
   1.0301883015591748e+00   8.7394162016151422e-01
   2.0178055195438809e+00   5.1462334245067398e-01
   1.5875650423114394e+00   1.8160549411968463e+00
   4.8162366493304543e+00   2.7330749599520265e+00
   1.5881757829621641e+00   1.8481828777262246e+00
   4.7147786635812459e+00   2.1871766192220440e-01
   1.5855718632578402e+00   1.8030472932717092e+00
   1.0391566906038072e+00   9.5432332272362974e-01
   9.2806549888937084e-01   2.0675614072198409e+00
   1.0494487508478834e+00   2.8470625675553247e+00
   3.0080691588580706e+00   3.6232840163642199e-01
   1.0010316860975621e-01   3.0899044793762105e+00
   1.6733182004241876e+00   2.9022119823051296e+00
   1.0205840115634501e+00   2.7893095320358476e+00
   4.1646929445899588e+00   1.2268822221174229e+00
   3.8842544182413121e+00   6.4346495331529074e-01
   6.1111916277928842e+00   2.9819495941682614e+00
   4.2785475059286284e+00   2.1441044224503929e+00
   4.7628095505500418e+00   2.9111250575327206e+00
   5.0244934069277498e+00   6.0312006646683958e-01
   1.3949806793345587e+00   1.3834759144704782e+00
   4.5978206491668772e+00   4.8821811814193938e-01
   3.2321413929133840e+00   2.8317316197160536e-01
   4.2939119964563162e+00   2.5395791262320659e+00
   9.2946537775495131e-01   2.7951599990201941e+00
   6.1030504528489331e+00   3.1354571012184489e+00
   3.9736539744304942e+00   3.0761444886274858e+00
   1.6421109729388661e+00   2.9588182016525963e+00
   1.1430675011690674e+00   2.4979596445220422e+00
   4.7457818506978953e+00   1.7960728916588804e+00
   5.3785530105287584e+00   1.8034144567172206e-01
   1.6546702213877520e+00   2.2981190051549829e+00
   1.0999756482518457e+00   2.7620933830592076e+00
   3.9558143523926184e+00   4.7885613399686872e-01
   1.3504864846801290e+00   6.0601195157234611e-02
   1.0931477299238210e+00   2.4384028489865304e+00
   1.2696046803702430e+00   1.7482325658367912e+00
   3.6323419716409440e+00   3.9845233645831535e-01
   1.8916136971659228e+00   6.4432826713362412e-01
   5.2791180192557228e+00   1.0417651114894837e-01
   3.8348366143917332e+00   5.7459054027845624e-01
   4.0173510046355005e+00   7.2837940807061907e-01
   4.1259000664939123e+00   2.1113410794969836e+00
   3.9937239131701716e+00   3.0153141819500187e+00
   4.1418530178815871e+00   2.7582295238453356e+00
   1.0632962301879658e+00   2.6509179585792810e+00
   1.2876093925156571e+00   3.4001709940961800e-01
   3.3655216776210963e+00   3.1663635679572610e-01
   4.5790423396367359e+00   8.6399043779768936e-01
   4.0747817478753774e+00   2.8480804742917760e+00
   4.9184688359825763e+00   1.8591558550122964e+00
   4.1152418455578363e+00   1.2970332431468623e+00
   4.6471115279885709e+00   2.7385263806328122e+00
   4.8296510847093899e+00   1.7378485504690899e+00
   4.0957230549725665e+00   2.2397066005636974e+00
   1.1700207352110787e+00   4.0214643972752501e-01
   4.2940483775000793e+00   9.4504443560950196e-02
   4.2329829902111804e+00   8.0861984880680179e-02
   4.9072654248075409e+00   6.6051718352428179e-01
   3.9058897365968228e+00   2.8276918441087764e+00
   9.6066964911467778e-01   2.2522921302583987e-02
   3.1005294586771885e+00   3.0767385030539369e+00
   1.3323737238607585e+00   4.8695429413701857e-01
   4.1713251172465817e+00   7.8990571817656441e-01
   1.3354685977126257e+00   7.8081286128374089e-02
   3.4447980152403233e+00   2.6051130443196913e-01
   1.1900685433488931e+00   5.0950676043089516e-01
   4.1994883477921547e+00   1.7535709464175180e+00
   4.8073452108628203e+00   1.1196471162492525e+00
   3.6779734447586350e+00   5.4969920839274111e-01
   4.1247265090183518e+00   9.5153450081864788e-01
   4.0649522090597898e+00   2.5034193497153168e+00
   3.7872924730357269e+00   3.0856276741116218e+00
   4.1817834438876176e+00   2.6198366460255991e+00
   1.2098985146469481e+00   3.0208301417464933e+00
   1.3563611461317677e+00   9.3150512220776638e-01
   4.9012733935445851e+00   2.4700944906363764e+00
   4.4330910488687643e+00   1.8114496603753460e+00
   6.9411600925802830e-01   3.1300923448354472e+00
   4.2800635891854348e+00   2.6006762006984698e+00
   1.4137579337591717e+00   2.3839875625727887e+00
   5.0727187590662712e+00   2.9201917947037952e+00
   1.4161358913251050e+00   1.8946625922168281e+00
   4.1387287022968664e+00   1.4657358703204133e+00
   1.0672628593564468e+00   2.8097167354907002e+00
   4.2673407877231568e+00   2.5485842466595421e+00
   4.8630152043548094e+00   2.8698714028938062e+00
   4.4548604001986547e+00   2.2542288513313404e+00
   4.9640963941883527e+00   2.1238770173891675e-01
   4.1238996630304747e+00   8.3448632363084432e-02
   5.1124890715112663e+00   3.0066027607771950e-01
   3.9395264297298596e+00   2.6738565260572709e+00
   1.1906831218220439e+00   6.0006910608285513e-01
   4.8375139489935925e+00   1.2508382533841427e+00
   3.8413783204922289e+00   4.8274713441540990e-01
   8.8105002242859420e-01   2.8782609718840706e+00
   9.9256256945922061e-01   2.3018219003763263e+00
   2.6511631464439986e+00   5.4509657062243755e-01
   1.3225228737528862e+00   8.3628693487863992e-01
   4.7250115577748097e+00   1.2002820366049662e+00
   4.1705980077723481e+00   1.3183466134840829e+00
   4.1127274953962996e+00   9.1469532394515007e-01
   1.4661661597939322e+00   2.9208316879862948e+00
   4.2536174102598423e+00   2.3279261174833881e+00
   2.5544881855227928e+00   3.1318861954153956e+00
   5.9314683934001806e+00   3.0950251905144488e+00
   1.6746196260068729e+00   2.9084424163381075e+00
   4.2562033123453773e+00   8.7499808014919145e-01
   4.4271973094881822e+00   1.8560462246484593e+00
   4.2774611570923931e+00   1.0849358960376894e+00
   4.3125725662572876e+00   2.3919774846293458e+00
   4.0619666758741602e+00   8.5990387346841335e-01
   5.8184978750520902e+00   3.0477456593513903e+00
   4.1360622894752233e+00   1.4027966208600433e+00
   6.1784168194646671e+00   3.0877197976320900e+00
   1.0760508590328364e+00   3.1122384121759601e+00
   4.2709324256417460e+00   2.6061241822405310e+00
   5.8199095738190962e+00   2.9361856302392244e+00
   4.4945241086061785e+00   1.9441476419305073e+00
   9.2733715184849075e-02   2.9878714594820890e+00
   1.4960003603246683e+00   5.6091893222282120e-02
   3.1266803022784515e+00   5.2003151992815766e-01
   4.3544646901315751e+00   8.5701634800944324e-02
   5.3453543020641447e+00   2.7467735396911404e+00
   1.7179013747391387e+00   2.5341914766016083e+00
   5.4752146392068042e+00   9.3883061193333936e-02
   6.0692883162558289e+00   3.0494353205004017e+00
   1.0627922124442168e+00   2.8443231311260671e+00
   4.1315785090834538e+00   1.1840951096544543e+00
   1.1130950847650674e+00   2.7260283322042271e+00
   2.9621931807045456e+00   4.7219236781264556e-01
   5.3722863821662123e+00   1.1005839082485180e-01
   3.8057205007693007e+00   5.6221655954267535e-01
   4.1644675609536819e+00   1.5547759182740559e+00
   5.0189217062822067e+00   2.8981381986061558e+00
   3.6257630173389472e+00   3.1059565382547398e+00
   4.2295878341850184e+00   2.3737919004788441e+00
   3.2787677017971184e+00   3.0891158812550485e+00
   1.4009829335224495e+00   1.4669988159525473e+00
   6.7534330621062821e-01   1.0888377085651367e-01
   3.8374454801576761e+00   2.2870721045955186e-01
   4.5959824188808120e+00   7.5104735637758890e-01
   1.4370750931133038e+00   1.8995802206255421e+00
   4.2909280769496654e+00   2.5651516726450838e+00
   3.7740905738242745e+00   2.9644576241184497e+00
   2.4594488501808645e+00   2.5441992384154677e-01
   1.1976029842986300e+00   6.4669687593191916e-01
   9.5474667012564751e-01   2.8045924567055609e+00
   1.4647297067738343e+00   2.9234761225046748e+00
   4.3197324156070458e+00   2.3451704161828033e+00
   3.7400920534157045e+00   3.3669122059797058e-01
   4.4637315054611086e+00   2.1784347718133152e+00
   1.5922326563725733e+00   2.4766994963386582e+00
   1.3714925551407546e+00   9.6640572350066278e-01
   5.5197225340394560e+00   2.9275135464546080e+00
   1.2743162996590627e+00   2.0830158968141679e+00
   1.6991889310270079e+00   2.8830258270335980e+00
   7.1238049535424253e-01   6.3648073445160280e-01
   5.1583501762182813e+00   1.1381346382385446e-01
   5.6099630899685300e+00   2.9917878463103023e+00
   2.5268716396324731e+00   6.6952630417915104e-01
   1.1206451328426148e+00   2.2880560419601776e+00
   1.7882049826931912e+00   2.9684848525721459e+00
   2.9147852537531271e+00   3.6639705044096965e-01
   1.5185525374244087e+00   2.7172325300722486e-02
   5.6950454323426776e+00   3.0385681303838954e+00
   4.0587895333367783e+00   2.5446759974197311e+00
   4.1496509508724380e+00   1.8447904439292269e+00
   1.5083264948962842e+00   2.1579436779432033e+00
   4.1853740979237202e+00   2.6968142356587843e+00
   4.1814064459242388e+00   2.6249916972278742e+00
   4.1605115379443731e+00   1.8820493311294901e+00
   1.2784920138613423e+00   6.3826966493390175e-02
   1.3361438976665436e+00   1.1968267101460603e+00
   3.0181623378958697e+00   3.1211123136026048e-01
   4.4040502177445937e+00   2.0423150462414363e+00
   3.2510466316970223e+00   2.8550605596702500e-01
   4.4128976758898126e+00   9.1189098101968991e-01
   4.2765330141036415e+00   2.5109203973480305e+00
   3.9707496254094821e+00   2.7571147736533632e+00
   6.1875744184964319e+00   3.0369376255953888e+00
   7.0124769667422981e-01   3.1092138927488508e+00
   5.3279858325338907e+00   2.8430649269479433e+00
   4.2683364501661885e+00   2.6801325663879574e+00
   3.8436116931390529e+00   3.0405369604012642e+00
   4.5295894514464941e+00   1.1474564256807558e+00
   4.3323608180564719e+00   2.7523331746584825e+00
   1.1444427748339407e+00   1.6497831831548384e+00
   8.8520689552250786e-01   7.8402050948494195e-01
   3.6415218376213652e+00   4.5318409017300371e-01
   1.8744953756360978e+00   7.6684426598291555e-01
   4.8416672999086572e+00   1.0314316158938333e+00
   3.2132252110431736e-01   2.2095969698429221e-01
   1.2698150994544761e+00   2.8202908329678906e+00
   1.4943805461133763e+00   8.9218035996662792e-01
   1.5712512853060971e+00   2.5224768580287210e-01
   2.4239942201771001e+00   2.2578823082779856e-01
   3.1539898367881030e+00   3.5722287710291634e-01
   8.9263212749844456e-01   2.8578960996708767e+00
   5.3542925520243116e+00   2.5659948303315588e-01
   7.4659481516326309e-01   3.1083764236382345e+00
   3.3166410823032422e+00   3.0823163136816003e+00
   3.9740601445253034e+00   2.7662539883694230e+00
   1.2438527417931127e+00   1.0460726970686271e-01
   4.0559538462159992e+00   2.9639090832963255e+00
   4.2529822720021926e+00   2.2299054116762238e+00
   4.8754446971012584e+00   1.9422406665687311e+00
   5.0032672002467251e+00   2.1465806184540752e+00
   1.5015324578135001e+00   1.7990872597231289e+00
   4.1413257285182787e+00   8.3939320695731190e-01
   3.6542410581689033e+00   2.2552524130723589e-01
   4.4181943776085824e+00   1.9248562322576011e+00
   3.2248528358868604e+00   2.8066250590995390e-01
   4.2641245643978536e+00   1.9433246397796202e+00
   4.2933730909462362e+00   2.5516402653659460e+00
   5.4685370342389703e+00   3.1247192802459920e+00
   5.4785058678240155e+00   2.8903431481935660e+00
   5.3089699164976736e+00   2.8358548298884361e+00
   4.8302186689794517e+00   3.0390734106764641e+00
   4.2789209376411499e+00   2.6683065560706694e+00
   3.9511777944388093e+00   2.9868335180072711e+00
   4.4029014425092470e+00   3.2202777485895884e-01
   4.4219346473346448e+00   2.6794378748299601e+00
   6.2368544897625604e+00   2.9808416152158208e+00
   4.7687101034465051e+00   4.8962673328900252e-01
   1.4840705546800983e+00   1.7014229817606643e+00
   3.3317302392953998e+00   1.9212767684983142e-01
   1.5753748167603909e+00   2.1213265447031087e+00
   5.0827061166244007e+00   4.5438624154325363e-01
   4.8199090273901390e+00   1.1435047024917160e+00
   4.7129332440117420e+00   9.1964062613392761e-01
   4.5886571817029065e-01   2.7683809631412641e+00
   1.1436040520444593e+00   1.2223355036012253e+00
   1.4414310709405740e+00   1.4421289415231966e+00
   1.3562101981666430e-01   1.3158687579047107e-01
   3.8971490040868666e+00   2.8809875878111475e+00
   5.7782764910994899e-01   3.1233983119303570e+00
   4.9796525628082797e+00   2.8169532485744990e+00
   5.5575476882666628e+00   2.8510397931315357e+00
   4.0306283281076247e+00   2.9870910563126962e+00
   4.2724417994572050e+00   2.1152578400788276e+00
   5.5730906190975738e+00   3.1215405435993380e+00
   3.3656808604580810e+00   4.8245181130526155e-01
   4.9013950984066632e+00   8.2425345358760616e-01
   1.4320421789945001e+00   2.3007374960776574e+00
   5.9034241570221155e+00   3.1100886985976470e+00
   3.1597709428228598e+00   2.5460581592949916e-01
   4.3878133908113419e+00   2.1856600955537884e+00
   4.3209725586324623e+00   2.9431158150791031e-01
   1.6393457559748335e+00   3.1306365291506770e+00
   4.4192608545322898e+00   8.9655361127975264e-01
   4.2992333743888658e+00   2.5092372266832470e+00
   4.2707845411634366e+00   2.5140682828155989e+00
   4.1547232710868265e+00   2.8670889474602723e+00
   4.2552330262790221e+00   2.5585815428103627e+00
   4.2745178783948106e+00   2.6870489005444744e+00
   4.4449378412447729e+00   8.9632386250311735e-01
   4.2664095219569447e+00   1.3366444567949209e+00
   4.3053888198567591e+00   2.9219872534996303e+00
   3.8688473735693414e+00   3.1389457769063025e+00
   1.3198226843672565e+00   1.1602447140578511e+00
   1.7304473318080476e+00   7.4475243964253002e-01
   3.0701027644738943e-01   2.9881972224953910e+00
   3.5447203921350798e+00   2.1528880121092686e-01
   1.5981557339449299e+00   1.4402413009766599e+00
   1.6879261814979554e+00   2.6140151063563808e+00
   5.1824815370619604e+00   2.6670267527139363e-01
   1.7598491419938469e+00   2.5455927372172895e+00
   1.8241529722135859e+00   1.1028643823956135e+00
   4.0685400755393530e+00   3.0037645916632189e-01
   6.2516583783714026e+00   2.8774591133632961e+00
   8.1216651655161698e-01   1.4437012873734709e+00
   6.2625950888050035e+00   1.0384500763733019e-01
   4.6114703358573017e+00   2.8568679717585788e+00
   1.9163021832834417e+00   9.9922439957672304e-02
   4.7607172011064733e+00   2.1732807284415854e+00
   3.4258766028845997e+00   5.0979759039018979e-01
   4.7239968181746725e+00   1.2545605311962842e+00
   1.3420068765200703e+00   6.4247594602849822e-01
   4.6697083584776742e+00   1.7496797699108579e+00
   1.4091820288981154e+00   1.7269586744952758e+00
   2.9781061458537366e+00   2.9084960811129135e-01
   4.4864418008230338e+00   1.4393061760379362e+00
   4.4840428542945681e+00   1.4432024279352129e+00
   3.4340951011073884e+00   2.4160355627661623e-01
   4.8349993038538770e+00   2.5125362603377064e+00
   4.3431763149393525e+00   1.3157288115621331e+00
   4.4230273288894004e+00   1.3950432712493062e+00
   4.3048733112052062e+00   2.4663356509563141e+00
   4.2824028209148537e+00   2.6352152287908055e+00
   4.3032767674309618e+00   2.4843143780582282e+00
   4.4338150755029808e+00   1.2954924294317038e+00
   4.1126071559235768e+00   2.7652111000978534e+00
   3.6308232237073561e+00   3.1922200068135120e-01
   4.3332764924669007e+00   2.7047956766145522e+00
   4.4189254071303310e+00   2.8585303944345166e+00
   3.5020001288575884e+00   3.2765504263608974e-01
   4.8055431271006555e+00   1.4966116608904891e+00
   3.6058827735433674e+00   1.6499557451248484e-01
   1.0685064412357583e+00   2.8603342671522221e+00
   3.5527298937861076e+00   1.8814013480930189e-01
   1.2952299334859347e+00   2.0540491890998775e+00
   4.5575182252680690e-01   3.3521835065629330e-01
   5.1791669537226319e+00   2.8217671018141105e-01
   1.2279031349865335e+00   2.2743287348200121e+00
   1.8283708478363359e+00   1.0002962299047882e+00
   5.8943296269255221e+00   2.6411344315127199e+00
   3.8428830079988430e-01   2.6674758322063963e+00
   8.0060526989495173e-01   3.6606003867787777e-02
   5.8597112915090328e+00   7.4587924065402642e-02
   5.0363677177664492e+00   4.7866102063030419e-01
   1.9722627220931876e+00   5.0541429790733505e-01
   5.2536691280724312e-01   2.8094360054330565e+00
   3.2505658638643453e+00   3.7113568508457179e-01
   3.4803055940473833e+00   3.0791434030714213e+00
   3.0691737648507065e+00   3.1313080555629674e-01
   4.5231227185605576e+00   3.7742038384437748e-01
   4.3851457098779463e+00   2.2121932296477986e+00
   4.4186851681518249e+00   1.9189662139960282e+00
   4.4242293252889446e+00   3.2960426458894637e-01
   3.2378249144588089e+00   2.8285215522948026e-01
   4.9515786297279263e+00   2.9736039811825830e+00
   4.7568960445146722e+00   2.4479791323322209e+00
   4.3785397411482236e+00   1.0661238860305393e+00
   4.4422146241165734e+00   8.9756362167571613e-01
   4.4501664295281493e+00   9.4023115626192044e-01
   4.4282071402731376e+00   8.7934125021797527e-01
   4.2259869438777926e+00   2.2349094022612368e+00
   5.6626392433891191e+00   2.9079048157693022e+00
   3.2373744830179092e+00   2.7010767814601433e-01
   4.3647686809463409e+00   2.3887988770409390e+00
   4.4387215216622060e+00   2.4325521307109801e+00
   4.5021896832126664e+00   3.5842664027949189e-01
   5.9166510689908165e+00   2.9579308110063249e+00
   9.7513729220601064e-01   3.0117192301247617e+00
   1.3580938668591180e+00   8.7573703064040609e-01
   1.4007112980425198e+00   2.7050601317154146e+00
   4.1217055220771392e+00   2.1216156463108976e-01
   1.6068111753398213e+00   1.6672157263272709e+00
   1.7550777961455264e+00   9.3721665661636444e-01
   4.6010213641772140e+00   1.7216789139156119e+00
   4.9859862225866358e+00   1.6925051988315865e+00
   1.3695775515324016e+00   2.7671615290642793e+00
   2.6608009948205797e+00   4.1138709759787088e-03
   8.6397302464639836e-01   2.2559201250431853e+00
   7.8540659904703247e-01   2.3507511470663456e+00
   1.1394546656253581e+00   2.2246926184227043e+00
   6.0100054576231940e+00   8.3804937436201654e-02
   4.8569100377674062e+00   7.7522135902137457e-01
   1.2469937714252843e+00   1.2948814077556707e+00
   4.3345437481739459e+00   7.3928324005063479e-03
   2.8111565969558860e+00   5.9021588333839947e-01
   3.2258047119405155e+00   3.3610106523329025e-01
   1.4561886987367885e+00   1.6040369088267854e+00
   5.3287837086823160e+00   2.6581984034544942e-01
   4.9613425290791788e+00   1.8653320425341682e+00
   4.2405536907642123e+00   1.6601547323959971e+00
   4.9341219176277669e+00   2.4264719202727520e+00
   1.6328126324325645e+00   2.6890751553725178e+00
   1.2429487513241853e+00   4.2716715090525648e-01
   3.8597795613370423e-01   2.9926062423569850e+00
   2.0424142582907301e+00   3.1292514052330387e+00
   3.7291336719173849e+00   3.3498646544890509e-01
   3.4663928281248495e+00   2.4033929709585494e-01
   4.5709616671731474e+00   9.0494307312890510e-01
   4.4230851985124779e+00   2.7421147914592061e+00
   4.4191831081910706e+00   2.8117330622365517e+00
   4.5891035843916406e+00   4.5567969338828040e-01
   5.0879343891590949e+00   2.6359182244544002e+00
   1.1323663353822084e+00   2.9874885641671818e+00
   1.4421325044086295e+00   1.5208616609273253e+00
   1.6442007326088479e+00   1.4741501981830340e-02
   3.7373446859395898e-01   2.8554266705793814e+00
   4.3777796996922973e+00   2.8343140317989396e-01
   9.1328981418071464e-01   2.3188751752706800e+00
   1.1742659693973501e+00   3.7871222691404366e-01
   5.6831246447472736e+00   8.7039938143383053e-02
   4.9858640351554122e+00   5.7188515067097545e-01
   4.7096721749766779e+00   1.3719645889757387e-03
   4.4656277336563477e+00   1.8648942044723147e+00
   1.7741255080772085e+00   4.9175363532253803e-02
   2.7409597260900505e+00   1.7118002311214503e-01
   3.7926678607085584e+00   1.3263122738321662e-01
   1.2113581407065581e+00   2.0791531661940739e+00
   4.9000730919160738e+00   1.2261047072612155e-01
   5.0991524233029430e+00   5.1857123271563790e-02
   5.2095128173408263e+00   2.6101505784243739e-01
   4.3855889254028675e+00   2.6657217324240392e+00
   4.4111117998913301e+00   2.0861551428325481e-01
   4.0734064604497249e+00   2.2340524124614725e-01
   4.0734365408345852e+00   1.6856119442574371e+00
   1.1246104822841474e+00   2.9211669298703002e-01
   5.2902553807767312e+00   2.4255566827150279e-01
   5.5729183306653738e+00   2.9280284067214488e+00
   1.1487446165147119e+00   2.4621942243671966e+00
   3.3696404161842963e+00   3.0308807575344474e+00
   3.5980388395932010e+00   4.9290085680065704e-01
   4.4249592100649160e+00   2.6429802114632843e+00
   4.5515519046590711e+00   3.1250383758737867e+00
   4.5522324166467563e+00   1.0459463558251301e+00
   2.9951612725249923e+00   2.8046319194417652e-01
   8.9531193420004840e-01   2.9854598622925503e+00
   1.1505727425685990e+00   2.5738545931503305e+00
   2.3312895565043945e-01   2.9641905895009244e+00
   5.8977519928128039e+00   3.1761702746013927e-02
   1.3321280257971537e+00   2.0904947093616673e+00
   4.0898717461787832e+00   3.2754512532718100e-01
   1.7997760240812131e+00   2.8036702351773930e+00
   3.8080974846758728e+00   1.9119289308400028e-01
   1.2653421557356239e+00   1.7372457511895454e+00
   1.1953140100772597e+00   5.4431053438068289e-01
   1.7163090216042729e+00   2.8178877157662341e+00
   4.5395620314550769e+00   2.1745201119831621e+00
   5.5278985829324583e+00   7.6822485424906439e-02
   2.6201585018815567e+00   2.1634076829124962e-01
   4.4321720016369710e+00   1.7749195939266311e+00
   5.6187342332313328e+00   3.3238126642719172e-03
   4.4984198253487655e+00   2.0688502598536211e+00
   1.2034376893660976e+00   1.4518162038531015e+00
   4.3057395051981189e+00   3.4702184400279007e-01
   7.9711985563341869e-01   1.6230701787644075e+00
   5.7891280041164173e+00   7.0500915720246402e-02
   5.0943492178414154e+00   3.9379399716496855e-01
   4.9394532331118199e+00   1.1707463448358424e+00
   1.2909366851757653e+00   3.5155479861962535e-01
   1.6699292433575152e+00   9.4195484715594957e-01
   4.3168129096785783e+00   2.5581567722143722e-01
   3.9225342982369789e+00   7.9935741737434962e-01
   1.3354657965598449e+00   4.5827455382162469e-01
   5.3141064465205048e+00   2.0919269762733639e-01
   5.0278044296630959e+00   2.2588606592009164e+00
   1.7700388997857495e+00   2.6662917460707254e+00
   1.3318671275765155e+00   2.6841697163079195e+00
   3.8673814806408160e+00   7.0219777869857958e-01
   4.0252747815001442e+00   6.7851691263821556e-01
   5.1734708785606465e+00   2.7549171042242144e+00
   1.5869491883331790e+00   2.6168314601582328e+00
   5.3929272056375481e+00   2.7876158816464933e+00
   8.7415681898907494e-01   7.3206097160124861e-01
   1.0128266853412633e+00   3.0056515776616886e+00
   5.1658820745625320e+00   3.0377562814684174e+00
   4.0705337301218059e+00   2.0737303858141970e-01
   6.4503276500828832e-01   2.8525322742627974e+00
   3.1336269153491489e+00   4.0514439363199629e-02
   1.6114860132285767e+00   2.3165431863539734e+00
   2.6585641370328617e-01   7.4170902399147351e-02
   4.6149061836632086e+00   1.6597934394932148e+00
   4.8217950916412100e+00   8.6420342971302855e-01
   7.8441796428842281e-01   9.3362428455130220e-01
   3.4477296331682510e+00   1.5588814955278846e-01
   1.2678115146169340e+00   2.8240732157391899e+00
   9.8238081637590113e-01   2.1584607427373896e+00
   4.2239866904029277e+00   2.8088562516027027e-01
   9.3092492104666746e-01   1.9429547900642254e+00
   1.1385302390997012e+00   1.1866478835832075e+00
   1.1424054415452218e+00   7.0911300784291831e-01
   1.6600371526325866e+00   2.8991490045068549e+00
   4.6787466401464002e+00   9.1426835947820875e-02
   4.9994532276044019e+00   5.1572526902822845e-02
   4.6271812992339001e+00   2.4490361784438508e+00
   1.0539295437273104e+00   2.8612723490842571e+00
   1.8932380657644536e+00   2.7097380908567437e+00
   1.5454981074345753e+00   7.7514338093959101e-01
   4.3519095229974347e+00   2.6259166034990622e-01
   3.3937358325175779e+00   4.3245403214074407e-01
   9.5932516283126290e-01   2.0652348937957616e+00
   5.2459116094736942e+00   3.7684630120312124e-01
   4.5614370293261146e+00   2.3021755713483203e+00
   1.3927504140652616e+00   3.1205939288619629e+00
   1.4095129837023634e+00   2.2674931832811498e+00
   1.1076832311051845e+00   2.7853408708984464e+00
   4.0807533223410957e+00   1.4371750910037258e+00
   3.6968816114169414e+00   5.0603702879325663e-01
   4.9491474585044770e+00   2.7088148930811209e+00
   1.5892112558480207e+00   2.6347719841664650e+00
   4.9816192065175713e+00   2.2316726432362186e+00
   4.9091952439027580e+00   1.9505351913184614e+00
   5.0175672702967589e+00   2.3377497397212319e+00
   1.2468126256551102e+00   6.4691115160007129e-01
   3.9550819393641277e+00   2.8130167098197187e+00
   1.3807663983138312e+00   2.7372029662536081e+00
   4.7536038993472367e+00   4.1183674807792930e-01
   1.0354016362409908e+00   2.5826660525926881e+00
   2.1327143761152101e-01   2.6651013656423750e+00
   1.6528599225438256e-03   7.2859370805247632e-03
   1.6934287810560420e+00   1.8856967350029217e+00
   3.9540690639947762e+00   2.8073020913856378e-01
   5.4722677908975719e+00   3.7075823901682363e-03
   4.6391436019283994e+00   1.0583257561048465e+00
   4.5840711894783830e+00   1.1236700189592970e+00
   3.0166062678930849e+00   5.6596496744809786e-02
   5.1158484212911972e+00   1.7834276320191228e-01
   5.1465455522979902e+00   5.3834859847614144e-02
   4.7713165156016544e+00   1.0861792582440039e-01
   4.6021905383411088e+00   2.9442627890481456e+00
   9.0963198335335704e-01   3.5234334311570781e-01
   9.4250093891443143e-01   2.8728786139232794e+00
   4.5366378812408215e+00   8.8562717576416095e-01
   3.1664199044417067e+00   3.9531231465057931e-01
   4.0078377598480373e+00   2.2508996053065672e-01
   5.3018697247712154e+00   2.8899918181373723e+00
   1.3454649217523240e+00   7.4152968479450543e-01
   5.2918091016143798e+00   3.2146432178874257e-01
   4.6585053281459849e+00   1.5219075439184269e+00
   1.2516779657523642e+00   1.6153122779523721e-01
   2.6054768003926121e+00   3.1036401019212891e+00
   1.4311114883005764e+00   1.5947694755856889e+00
   2.0147564084798084e+00   4.7676677264794204e-01
   1.8063390573756237e+00   2.8728479315237907e+00
   3.5255327803013969e+00   5.2752733665728446e-01
   4.1802875050919610e+00   1.4785697391475876e+00
   1.6561153613486752e+00   2.7527612331275195e+00
   5.0889606461987569e+00   2.5021290342413880e+00
   4.8440014863456540e+00   1.9108023013820687e+00
   4.7963800007557964e+00   1.9955670929347975e+00
   4.8824073872699358e+00   1.8857017849756492e+00
   6.0487090420033098e+00   2.9464643175185086e+00
   5.1114982944221197e+00   2.7243572593421570e+00
   3.6013659761725449e+00   5.3070315651605271e-01
   1.5850486171190319e+00   2.9647543503778970e+00
   5.2581640515946653e+00   1.1874765751650947e-01
   4.4440107258122907e-01   3.1411946808277063e+00
   1.1573336024496115e+00   1.7697816169979554e+00
   5.1591034198409211e+00   2.3186222957772407e-01
   4.5222929782963064e+00   6.0027250698920488e-02
   4.4634520100693820e+00   5.9540431560595672e-02
   4.5737711365340665e+00   1.8685836242069953e+00
   4.8515794357659843e+00   8.2222661964829258e-01
   9.2777753907446225e-01   8.0147095831184539e-02
   4.5645993853641826e+00   1.2885093668451033e+00
   1.2778609702867314e+00   2.1589055245108058e+00
   4.3793223315975993e+00   2.0133856723384028e-01
   3.2843339858151523e+00   3.7727164950585546e-01
   4.5533662220130715e+00   3.5221362856457744e-01
   3.6306326869206487e+00   4.4932418632510585e-01
   1.0187405939414980e+00   2.6303502754155499e+00
   8.2225902255772354e-01   2.8918099526890280e+00
   5.3230916004616127e+00   2.6275433528158676e-01
   4.8679035712210528e+00   8.3227804828832652e-01
   4.7213606390327421e+00   1.8265648917129564e+00
   1.4103358271709681e+00   1.8865411466708708e+00
   5.2460607706465723e+00   2.8519317032787743e+00
   1.6350372273332319e+00   3.1197216024231107e+00
   6.0525759331285194e+00   3.0879433710567454e+00
   1.1990105416985912e+00   6.3660768462041739e-01
   1.1850666570143318e+00   2.2777813282385000e+00
   4.0417588981876946e+00   2.1862818906973689e+00
   3.7027085911363713e+00   5.0544951896445001e-01
   5.0697169364614147e+00   2.6908388612640985e+00
   6.1848341309808958e+00   2.9596784926486670e+00
   4.8525865659242697e+00   1.9111054509203034e+00
   4.7154549270349548e+00   2.3475863741473533e+00
   4.7006501516907022e+00   2.4380503122823844e+00
   4.7923551639233324e+00   1.9943279088947088e+00
   5.0072112488538210e+00   2.3040087605528590e+00
   1.6228120315255481e+00   2.5397071606935016e+00
   4.0890777048678686e+00   7.9626851173458379e-01
   1.1014604139761275e+00   2.7898189913486062e+00
   4.5791633608505151e+00   2.0066795074345554e+00
   1.4091659834390100e+00   2.1501354892015216e+00
   1.5200833435142904e+00   2.4099295433482282e+00
   4.1596440183524912e+00   6.4527521821499290e-01
   2.9205323616421381e+00   3.7526537753688388e-01
   7.4001743766724104e-01   2.7957369859974373e+00
   1.8752184431414278e+00   1.3539856667657701e-01
   1.0867086548928313e+00   2.4674806142386929e+00
   1.4185676190912311e+00   1.3880859038058437e+00
   5.9458215662052538e-01   2.8161947747101173e+00
   4.9488085905200982e+00   7.5339443345582158e-01
   5.2955848950932527e+00   2.5994999623390180e-01
   4.9204293655578226e+00   7.3548533218043954e-01
   4.5867211141574344e+00   2.0178583009564406e+00
   4.5708317644098670e+00   2.3776342246197113e+00
   4.5786403914899942e+00   2.3745007684327577e+00
   4.5770817168866955e+00   2.3629398869632960e+00
   4.5787000303392773e+00   2.3547103072646065e+00
   4.6005726620385765e+00   2.2964298775681455e+00
   4.7548329629250752e+00   1.7084630492119104e+00
   6.2102258798311389e+00   2.9527638119806396e+00
   5.6913844645694063e+00   3.0790998213157006e+00
   1.8022411949695289e+00   2.7649831628917436e+00
   1.0466288449204981e+00   2.7430525764694478e+00
   3.8767619983838273e+00   7.1442859707547712e-01
   4.1553689922051191e+00   9.6816556938287068e-01
   1.6462347794826684e+00   2.7883670248872261e+00
   4.9943169709407087e+00   2.2802841410301045e+00
   4.7538339291777518e+00   2.1656849165735821e+00
   4.7082495816476850e+00   2.7964151507337052e+00
   4.7472287524508161e+00   2.9159563822881358e+00
   4.6873054117055020e+00   2.6085926121894771e+00
   4.8177110347259742e+00   1.9233810095711052e+00
   5.1981521086119002e+00   2.6440645239811569e+00
   1.0337293162386985e+00   2.9840430455397473e+00
   3.9452778991724458e+00   6.2386849066832151e-01
   1.0991116021589633e+00   2.6620207349300626e+00
   4.5755633251188250e+00   2.0362595181175203e+00
   1.7553920556611224e+00   2.8222713272659217e+00
   1.3945163066893329e+00   2.9632737835448659e+00
   4.1773320832438969e+00   2.0338253350264699e+00
   2.6457628971596279e+00   4.1447459507767198e-01
   1.2222307287623089e+00   8.2366957663681939e-01
   3.5153254815752071e+00   1.4869921442536102e-01
   2.7966884828069318e+00   1.8767648120810088e-01
   1.2178797137289976e+00   2.1953564738364277e+00
   3.4944951351549314e+00   4.0390193394284107e-01
   6.1713993992269778e+00   3.0463491633227013e+00
   2.8149045892012943e+00   1.7058269928928427e-01
   4.7611124070592794e+00   1.0703618838724540e+00
   6.3461797974348855e-01   9.6824082854331556e-02
   5.1422445961289256e+00   4.6764438549024501e-01
   5.0702325701988826e+00   5.3590439883823249e-01
   4.6619557654529302e+00   1.5294162341348745e+00
   4.8990751784935256e+00   1.4673605344011851e+00
   2.6629084735462634e+00   3.1044337424096278e+00
   1.1686170077265672e+00   2.2355924907589464e+00
   4.0184500741375473e+00   2.3321895904240515e+00
   3.9752652126098056e+00   6.2499987553795344e-01
   1.0143556073740285e+00   2.9842197333209697e+00
   5.0207500978847648e+00   2.3578427163110414e+00
   4.7447258293351879e+00   2.2125231539607846e+00
   4.7767791797474075e+00   2.9515943702268945e+00
   5.3815508165294759e+00   3.1160829419906317e+00
   5.2257607837834854e+00   3.1070035592096499e+00
   4.7258622491314810e+00   2.8809138620685624e+00
   4.7489648827626638e+00   2.1350685949619783e+00
   4.9404717637867179e+00   2.0452010318523768e+00
   1.5467643481692050e+00   2.4368668066184540e+00
   4.9811975277470175e+00   2.8609027908672875e+00
   3.6481001465933716e+00   5.4980109225785223e-01
   1.3884270431151506e+00   2.1248391224974896e+00
   5.2354624616289875e+00   3.0036798661920994e-01
   6.7766031525439985e-01   2.7976683642624387e+00
   1.6938891492067292e+00   2.6656152765818457e+00
   4.1578012142279519e+00   2.1692682845684681e+00
   2.5892861956653697e+00   4.2038898889010717e-01
   1.3255842753522806e+00   7.8336650365698512e-01
   1.6706470884581037e+00   1.1812814684630177e-01
   4.5680001069193423e+00   1.7219300365339931e+00
   3.0384488378346788e+00   1.5416697786812331e-01
   1.2561852468371022e+00   1.2330996117877275e+00
   4.1373503662252915e+00   6.9046328233914589e-01
   6.4079667630169723e-01   3.0174345790541022e+00
   5.3827092731870074e+00   1.7949359562522954e-01
   1.5939327215583177e+00   2.9635050232775506e+00
   4.3476593918920514e+00   1.9121912039451314e-01
   1.4745232614951966e+00   2.1756434503491335e+00
   4.9561403936382931e+00   1.5684674299283180e-01
   4.0252937582717117e+00   8.1072512611373410e-02
   4.8474100142731054e+00   6.8267438609221365e-01
   4.4858046398741429e+00   1.1145946062989738e+00
   4.3714096986843494e+00   5.5358692405487053e-01
   4.2692227250063262e+00   1.7675622030906835e+00
   3.4735172114373398e+00   3.1131241517916082e+00
   3.3154638992131353e+00   3.1208703334692105e+00
   5.0731114903878378e+00   3.0913034226419689e+00
   4.6888205903570395e+00   2.4991393920157585e+00
   4.8712567840046859e+00   1.8555073594294771e+00
   5.6430147324086022e+00   2.8772034744408495e+00
   1.4304139980609563e+00   2.9287694832258704e+00
   4.1738983357019706e+00   1.2805173363770488e+00
   6.2565153509927605e+00   3.0869726260652190e+00
   3.4258003824920635e-01   3.1160228557902228e+00
   5.3195668790173656e+00   1.1408479117575679e-01
   1.0541319353021734e+00   2.4060244464178379e-01
   1.2768339334792493e+00   6.5411179770246175e-01
   4.2230506909333947e+00   1.5197679470013683e+00
   2.6202770390919241e+00   4.1648806349075207e-01
   8.7852624143170743e-02   3.0874839390064142e+00
   4.3435193124384348e+00   2.4544507070510200e+00
   3.0962245983914549e+00   4.2310506083842001e-02
   4.5712170131231069e+00   2.4636970723167215e-01
   1.4345228945604731e+00   2.6055095848474252e+00
   3.7488392705510876e+00   4.3355546609560980e-01
   3.7166325735722445e+00   6.2880018918649583e-01
   1.3436750070421368e+00   5.6394050179831190e-01
   5.1475668889300117e+00   1.1696604627841435e-01
   1.7254236919754682e+00   2.1487700025295764e-01
   1.0484790236460206e+00   2.6840736185516794e+00
   4.8498810706021303e+00   1.6626561407836622e+00
   4.7525900723451429e+00   1.1811983575314439e-01
   4.1242224581424409e+00   8.6552246354854395e-02
   4.7252729741510855e+00   9.8307654460772398e-01
   4.5068521559233439e+00   9.0780592600990384e-01
   4.3669703619884963e+00   5.8089333148082944e-01
   4.2622946314779746e+00   1.8297392227456397e+00
   5.9929840277108859e+00   3.1253432420567360e+00
   4.9838254846337371e+00   3.0333674838491405e+00
   4.0412654293754962e+00   2.8753940919997012e+00
   4.3464310837934903e+00   1.0447882342534902e+00
   4.3848675166530882e+00   5.5720022807382719e-01
   4.5061554987109140e+00   7.3395309456712543e-01
   4.3113341957207680e+00   2.6048523356247433e+00
   4.5850934211352836e+00   1.5698031312161609e+00
   5.0150724033863305e+00   3.6805807908500349e-01
   4.8949509585268274e+00   1.7598557234264139e-01
   3.6087458975209401e+00   3.6423027379323408e-01
   3.3644818850898091e+00   3.6191308400045913e-01
   1.7948479426382171e+00   7.4304204255687190e-01
   9.1722352523864004e-01   3.9478530244191135e-01
   1.0423615082453210e+00   2.5538085349978927e+00
   1.7042866115064665e+00   7.2392795400264243e-01
   3.5953206896531569e+00   4.1048398691973370e-01
   3.4654966971233669e+00   5.4931009090963323e-01
   1.8362413917434850e+00   1.0117226082333273e+00
   5.2383937926402027e+00   2.5675961112075701e-01
   5.6260076030423321e+00   1.3447780058669723e-02
   1.2300123224428212e+00   2.7757052902858437e+00
   4.6919647603570809e+00   2.9675595154878107e+00
   4.5288190081492310e+00   9.5506607264760554e-02
   4.2648029499796891e+00   9.4559575174336080e-02
   4.6445757095024121e+00   1.2737840077291738e+00
   4.5052839008019845e+00   9.2592441834325290e-01
   4.3760567105685126e+00   5.4879038138272995e-01
   4.3496501579972495e+00   9.9386530987086741e-01
   4.2843618397042391e+00   1.6369767024389918e+00
   4.3312983045211482e+00   1.2012254420240158e+00
   4.3688696702925540e+00   6.3266720358353279e-01
   4.4669745823972349e+00   5.9179324542504697e-01
   4.3622809533472768e+00   2.1254103228957737e+00
   4.7203492645582301e+00   1.0025094375911821e+00
   4.8892625080162411e+00   1.7428513802451445e-01
   4.5800548890964699e+00   1.0975248248618499e-01
   5.0961952830078339e+00   3.2188857900694756e-01
   3.5313479797815397e+00   3.1283162890086182e+00
   4.1011126446286497e+00   2.1559924967402826e+00
   4.5007415698881381e+00   1.6655967790708155e+00
   3.9576411289537958e+00   7.3206320191622376e-01
   1.4481218051972391e+00   2.8669957829589916e+00
   3.9430312257612457e+00   3.0480468526964231e+00
   4.3173261590426435e+00   1.9878676099467345e+00
   4.3733541892020042e+00   1.5558609903075222e+00
   4.3919143536284579e+00   1.3136353219677490e+00
   4.3769386497480909e+00   1.2904483074680064e+00
   4.3385617710333761e+00   1.4899053601885641e+00
   4.2850777855945736e+00   1.8691471516189417e+00
   4.2300333777195220e+00   2.2761600146390486e+00
   4.1856057630422470e+00   2.5383248534543705e+00
   4.1713814672795024e+00   2.6032595341023175e+00
   4.6995901598478156e+00   1.0652047791008477e+00
   4.5000133037609800e+00   6.6510071217425903e-01
   4.3665154491671387e+00   6.1690078767479661e-01
   4.3657957670028757e+00   7.0775760954585498e-01
   4.4057020171677728e+00   5.4312481999943074e-01
   4.4261474070321327e+00   1.5824693601587809e+00
   4.8866869800426791e+00   6.1090140480139421e-01
   4.5668184310617193e+00   1.1263499812267742e-01
   5.0865356985583361e+00   3.5123979423206148e-01
   5.2830926559910587e+00   2.7043900471324722e+00
   1.6458864113755496e+00   4.0296908580300000e-01
   5.1815280191270787e+00   2.7760794494446888e+00
   4.2340244748029079e+00   2.5267919955623666e+00
   4.3822438732699993e+00   1.4578004106086997e+00
   4.3468090447448446e+00   1.4435539500955579e+00
   3.9530120778946127e+00   2.9969283811007754e+00
   4.7303219063050150e+00   2.6706238976314167e+00
   4.7384299535101739e+00   2.4320632465175915e+00
   4.7710542192123206e+00   2.1966510805222694e+00
   1.4611313217504929e+00   2.0829752338909784e+00
   3.3260235247245653e+00   4.9774885963811866e-01
   1.2968155055764399e+00   4.1624906580870757e-01
   4.7002008008919063e+00   1.8571970435249199e+00
   4.8810565856805539e+00   8.5280597376676315e-01
   1.5482305403164780e+00   2.6925983195715468e+00
   5.0282288446354073e-02   3.1870231404062199e-02
   1.3518621202109102e+00   2.6642387072013690e-01
   4.3266096882101692e+00   3.0797693498795806e+00
   1.2029218907327675e+00   9.1609639067659843e-01
   5.3763801447452053e-01   2.8286268885389005e+00
   1.5788156396311734e+00   2.9431361251738468e+00
   1.4099876869323751e+00   1.9187508795912731e+00
   4.9718670543616881e+00   1.2965414266058273e+00
   4.7914397753373450e+00   1.4085544168407742e+00
   4.7291555327611192e+00   1.5305625893989021e+00
   4.7204296931083967e+00   1.5469120525034887e+00
   4.7457637487175326e+00   1.4973668053909213e+00
   4.8655758609953175e+00   1.2960920747505578e+00
   5.0529800574155779e+00   2.2823326973496463e+00
   1.3378224399573284e+00   2.9767960523189787e+00
   1.2812098214250760e+00   2.7989093699665650e+00
   1.3146924105406406e+00   2.4436951724577951e+00
   1.0666194359083363e+00   3.1194017923361068e+00
   1.3382880305888172e+00   2.9841812566447010e+00
   1.3146662712922641e+00   2.4440819061123502e+00
   4.6426497255306778e+00   1.9529092373132091e+00
   3.4451886322436778e+00   5.2749054466453127e-01
   1.1335432571320538e+00   2.9509873212174171e+00
   5.0419668939265350e-01   3.1286173640937109e+00
   3.4131404524293352e+00   3.1554599567967245e-01
   3.0253868303422067e+00   2.9354693333691656e-01
   3.1612998384517788e+00   2.6019477932685825e-01
   3.3106174701428017e+00   2.4363697108636542e-01
   3.3783212493217931e+00   2.3894359849647509e-01
   3.3867935563830933e+00   2.3884060250685310e-01
   3.3697107318790351e+00   2.4037789920570915e-01
   3.3468855110247731e+00   2.4231966245112238e-01
   3.3254565578816475e+00   2.4416209392814325e-01
   3.3052310768055584e+00   2.4590754786061789e-01
   3.2827300151984105e+00   2.4790752733422786e-01
   3.2538199312894953e+00   2.5071191741140092e-01
   3.2157689209280456e+00   2.5494148177362302e-01
   3.1690387446162518e+00   2.6113760032671185e-01
   3.1184930444865593e+00   2.6951271264660759e-01
   3.0735140539012562e+00   2.7960059277240196e-01
   3.0469487037901644e+00   2.9000292469194472e-01
   3.0535621321044388e+00   2.9864566734760661e-01
   3.1088666471461046e+00   3.0397593773034837e-01
   3.2280049932032426e+00   3.0717036787178364e-01
   3.4218340206692588e+00   3.1493992445093505e-01
   3.6848073310921770e+00   3.4295546256044551e-01
   3.9733584816281216e+00   4.2294235707712280e-01
   4.1970806522671040e+00   6.2620333173367726e-01
   4.2655644221828162e+00   1.1494733652574960e+00
   4.1608352042930576e+00   2.3152749974121822e+00
   2.6497105103296477e+00   3.1227812986832739e+00
   4.8480099250287765e+00   2.7872713938406060e+00
   4.9092347145958009e+00   2.4578748869072391e+00
   5.1948905394628824e+00   2.7235733250674867e+00
   5.5523460680129588e-01   2.9944325821989413e+00
   1.5274373096273379e+00   2.2659360909726689e+00
   1.3663557547828340e+00   1.5567924893485665e+00
   1.2669525067024665e+00   2.9317236379332221e+00
   3.1442929305393825e+00   2.7832751080171814e-01
   3.1512867393959780e+00   2.6657969055680225e-01
   3.1642677139378677e+00   3.0469291653093011e-01
   1.7482245629075877e-01   2.9899705992759982e+00
   3.5757937076123625e+00   5.5617501051133544e-01
   4.9861123064897122e+00   1.8771960663203877e+00
   1.1318730254368710e+00   1.8368909360886552e+00
   5.6444242696434053e+00   3.0393362556735233e+00
   4.9114829110042670e+00   2.0695360765661515e+00
   1.2609816428586988e+00   6.5052047676752633e-01
   5.0695066131333277e+00   2.5196728346608275e+00
   4.3921239801863692e+00   1.1297993593014373e+00
   4.3141900833680538e+00   2.0938640021318751e+00
   4.1077321170300607e+00   9.4365529397853010e-01
   4.1243888694635764e+00   1.4347510215325809e+00
   4.7151441275535575e+00   1.1123834794220184e+00
   4.8361744901511052e+00   1.5037960339237288e-01
   4.8050447864519796e+00   7.8216521111072568e-01
   4.4360086745157972e+00   1.4909262827440335e+00
   4.4012767291627881e+00   5.7229687551009956e-01
   4.3228047383593022e+00   1.3079801035529208e+00
   3.9914224327449581e+00   2.9389320223435984e+00
   4.0936924048038179e+00   2.7799402776606343e+00
   4.3495196487917553e+00   1.0431163335258546e+00
   4.4191058016470244e+00   5.6871418034551935e-01
   4.4164306907753321e+00   1.6499539168974007e+00
   4.7379415192227654e+00   9.5388619931425567e-01
   4.8883901459623047e+00   1.6742877049691934e-01
   5.0927902807208767e+00   2.9080665212055640e-01
   4.7184892312059112e+00   2.9843497805417107e+00
   1.4154902862564214e+00   2.5370885070625091e+00
   2.8607817659337798e+00   3.1078704222251430e+00
   4.2808534111768708e+00   2.2943673807767491e+00
   4.4150732115132456e+00   1.2506041621974464e+00
   4.2099037670863524e+00   2.3819896397689440e+00
   5.4704403170482792e+00   2.8370738090159162e+00
   1.2287189593545662e+00   7.8321445561145370e-02
   5.1145586558841636e+00   2.5774780706738589e+00
   3.4752101163736526e-01   2.9803986112245409e+00
   2.1224362792596665e+00   3.9666650321679975e-01
   4.8031130968532736e+00   1.0263849963994620e+00
   5.4168343911513261e-01   2.9475670647243994e+00
   5.2310242073691064e+00   8.2415639567906940e-01
   5.4570507227229257e+00   4.4504473480946644e-01
   5.6345546279108163e+00   3.1854300299609584e-01
   5.6590610685732337e+00   2.9492223244189919e-01
   5.5994243048189141e+00   3.1672497217575840e-01
   5.5020261923726501e+00   3.6940615386483133e-01
   5.3924931660511390e+00   4.4358248462436345e-01
   5.2936221336749263e+00   5.2723902588346805e-01
   5.2210202702072088e+00   6.0687697031189236e-01
   5.1762545665832604e+00   6.7282686530836167e-01
   5.1521563688035776e+00   7.2243725470553988e-01
   5.1403522647366451e+00   7.5760484545016127e-01
   5.1348129850835420e+00   7.8105529247733141e-01
   5.1321860742571559e+00   7.9471710606529478e-01
   5.1309540176137105e+00   7.9974372730109999e-01
   5.1306277002298053e+00   7.9690540335450666e-01
   5.1313513671380377e+00   7.8675380163402930e-01
   5.1338760080030710e+00   7.6952107743821430e-01
   5.1397338166072046e+00   7.4492364527101007e-01
   5.1514233815524335e+00   7.1210217314065938e-01
   5.1723957255105191e+00   6.6994418876342277e-01
   5.2066009498558792e+00   6.1792591056639345e-01
   5.2573575269862367e+00   5.5722947443972493e-01
   5.3255256485854225e+00   4.9135712924977731e-01
   5.4077432669585868e+00   4.2547334652603380e-01
   5.4966419289136468e+00   3.6482914726260796e-01
   5.5845436967260262e+00   3.1366457964538608e-01
   5.6678491403364610e+00   2.7508397112374255e-01
   5.7447555732947784e+00   2.5086283306454804e-01
   5.8042672433615330e+00   2.4077133875696907e-01
   5.8206086986150645e+00   2.4358643029804478e-01
   5.7686126101810906e+00   2.6432507754462176e-01
   5.6378139208273943e+00   3.2807744365634012e-01
   5.4142890835250377e+00   4.8980240564752647e-01
   5.2360694066521489e+00   8.1911568764354614e-01
   5.4414398623295739e+00   2.7436609646144157e+00
   6.0627917737714512e+00   2.8877852199454956e+00
   5.9484273356523545e+00   2.7301627523122645e+00
   3.8286226040111515e-01   2.5673178413433280e+00
   5.3366568834938981e+00   2.6938094741897953e+00
   5.0658611438240762e+00   2.2463409601538600e+00
   5.0077581217177283e+00   1.6784549390377141e+00
   5.0447882679584666e+00   1.2975503452152426e+00
   5.0740773310287217e+00   1.1056060557891025e+00
   5.0768702591048793e+00   1.0155509075925788e+00
   5.0667722208378585e+00   9.7405434983930217e-01
   5.0544622694690773e+00   9.5526224607153110e-01
   5.0439158510649378e+00   9.4737289157857396e-01
   5.0358375354895095e+00   9.4486252466208898e-01
   5.0298937937956154e+00   9.4483331007413407e-01
   5.0255462586161279e+00   9.4555631352347413e-01
   5.0223021517633413e+00   9.4593423111424479e-01
   5.0197937457836197e+00   9.4528651861617152e-01
   5.0178115087319739e+00   9.4323923669966969e-01
   5.0163122613275135e+00   9.3965371963057198e-01
   5.0154001275133346e+00   9.3457958101472671e-01
   5.0152786123265720e+00   9.2823404592048875e-01
   5.0161811415102981e+00   9.2100688235109796e-01
   5.0183003373833266e+00   9.1347307168798775e-01
   5.0217450818927922e+00   9.0637914167091371e-01
   5.0265483455047999e+00   9.0057412159371231e-01
   5.0327221976138858e+00   8.9688955508036194e-01
   5.0403144288552006e+00   8.9601992266962538e-01
   5.0493829923478089e+00   8.9848244731795557e-01
   5.0598092358728870e+00   9.0469538680489692e-01
   5.0709802329870932e+00   9.1504897352150583e-01
   5.0816175470969114e+00   9.2956757085638653e-01
   5.0902291196777192e+00   9.4666581045202303e-01
   5.0962600112406733e+00   9.6120837837504991e-01
   5.1008141506639646e+00   9.6385331503467120e-01
   5.1052804628216961e+00   9.4482408104498194e-01
   5.1085153768421705e+00   9.0143212122702943e-01
   5.1094605121257715e+00   8.3840140436055344e-01
   5.1246237539080539e+00   7.4991107379210797e-01
   5.2005324074537214e+00   6.1434162837467921e-01
   5.3688583063663735e+00   4.4899048761203098e-01
   5.5738748403423415e+00   3.1334215612754152e-01
   5.7634537627477123e+00   2.3967989767093023e-01
   5.9126837509357308e+00   2.2557709284411556e-01
   1.4793844221799475e+00   2.2752186199766533e+00
   1.3764339996013639e+00   1.4046823854646640e+00
   1.6699902891066678e+00   2.5323054724129954e+00
   1.6592197751867523e+00   2.4869747693551441e+00
   1.5055282774422984e+00   2.0096561972158131e+00
   1.3280856644053891e+00   9.6868771868575243e-01
   1.2912322687604636e+00   1.8283228875300964e-01
   1.6437424004900194e+00   4.4575559409607435e-03
   8.7042659241355480e-01   6.9431539247754937e-03
   8.0096595782171676e-01   4.8342996905698281e-03
   1.7824439080235415e+00   2.5890068624005230e-03
   1.3475258146690727e+00   4.7816144921764558e-02
   1.2943075289198802e+00   1.6300294166321291e-01
   1.2843911731071671e+00   3.4073331315064598e-01
   1.2920994169054971e+00   5.6558051188854908e-01
   1.3138226904857966e+00   8.3435974802882429e-01
   1.3521301198097291e+00   1.1571463030155595e+00
   1.4091629939540233e+00   1.5328466561835310e+00
   1.4843086806569694e+00   1.9189246603233687e+00
   1.5736539028730938e+00   2.2468331704759157e+00
   1.6560848862957833e+00   2.4751420237744548e+00
   1.7022628383611895e+00   2.5979758653506329e+00
   1.6968857670908157e+00   2.5992537429430254e+00
   1.5823184398512460e+00   2.3115951467549789e+00
   1.2673244461600781e+00   3.8092885670807303e-01
   1.4942808423044269e+00   2.3389188523582929e+00
   5.9556627415923487e+00   2.9158740566015391e+00
   5.0013668844091654e+00   1.8967381530148673e+00
   5.0343402897628913e+00   1.2099625612310723e+00
   5.0220777211110033e+00   1.0270188240117202e+00
   4.9914144203614477e+00   9.6591844250203385e-01
   4.9895851659767239e+00   9.1023955519466349e-01
   5.0060498819591288e+00   8.6056534783189009e-01
   5.0240733525143462e+00   8.3347648670083063e-01
   5.0382401997902662e+00   8.3035497820469306e-01
   5.0521445495561217e+00   8.4124964765073484e-01
   5.0683396240078480e+00   8.5412137169193558e-01
   5.0831530863023140e+00   8.5666349527913177e-01
   5.0937314129946571e+00   8.3113140905103744e-01
   5.1135383293103231e+00   7.5567586684832821e-01
   4.8765469779113424e+00   9.9667359370733788e-01
   5.4451931287086630e+00   2.2949613845338551e-01
   2.1555245692351122e-01   2.3699794045889258e-01
   7.6863693354361828e-01   1.4686555675036430e+00
   5.3923934107555027e-01   2.1880237620299634e+00
   2.3567176425555658e-01   2.3586946292636441e+00
   1.5225193878141141e-02   2.3852199814781656e+00
   6.1614550052267667e+00   2.3770150790739581e+00
   6.0801662498420725e+00   2.3640182676377393e+00
   6.0338082288248351e+00   2.3538804621693887e+00
   6.0105532588116759e+00   2.3479503973949640e+00
   6.0047964711096995e+00   2.3461796701805282e+00
   6.0153619265677385e+00   2.3485741276971415e+00
   6.0449256011774182e+00   2.3553846288194977e+00
   6.1004778429907667e+00   2.3664564803054162e+00
   6.1946254820642821e+00   2.3791214774209943e+00
   6.3193838220467313e-02   2.3824147820087749e+00
   2.9088643859744678e-01   2.3409956423308986e+00
   5.7391703230059576e-01   2.1457471966935708e+00
   7.6778287137384993e-01   1.4695529586011171e+00
   4.2023227833480448e-01   3.3855294458149227e-01
   5.5412440380262140e+00   1.5388705706934902e-01
   5.1991848235107518e+00   4.7659552718041209e-01
   4.8732391478933685e+00   1.1059548575951252e+00
   4.9949200036968939e+00   1.8722234732950584e+00
   1.1892098635293422e+00   2.0699895812683095e-01
   1.7169002474730242e+00   2.6723791699147155e+00
   1.7399462678033153e+00   2.7135634887517490e+00
   1.7217869719837644e+00   2.6448673398598870e+00
   1.7227986389497723e+00   2.6578522037440022e+00
   1.6665756763821875e+00   2.5320897632713768e+00
   1.2700924662393689e+00   1.3537061195245603e-01
   6.6799453161033640e-01   2.9610626479513384e+00
   4.9975841595704580e+00   1.6127332899004176e+00
   5.0234095629850692e+00   1.0433380641484815e+00
   4.9781599275699655e+00   9.4774136278159971e-01
   5.0001724139640800e+00   8.4828550921051826e-01
   5.0356745771218989e+00   7.8559181512929577e-01
   6.2268653026931453e+00   2.4815005144032884e+00
   1.6139271227146423e-02   2.4951066663822186e+00
   8.2406710324242738e-02   2.5034405225593215e+00
   1.4258114177959058e-01   2.5076081757746671e+00
   1.9518827489311619e-01   2.5086168194629228e+00
   2.3838595388436801e-01   2.5076342038901278e+00
   2.7085090535974388e-01   2.5058793328412108e+00
   2.9205150375004152e-01   2.5043862600329474e+00
   3.0207457126029880e-01   2.5038335807648906e+00
   3.0128900839025619e-01   2.5045016310377610e+00
   2.9005896013163834e-01   2.5063161417382966e+00
   2.6861232995045725e-01   2.5089092053080488e+00
   2.3708974022183682e-01   2.5116598814658695e+00
   1.9574121560123814e-01   2.5137245578937759e+00
   1.4518323548979239e-01   2.5140942434940916e+00
   8.6576362224608516e-02   2.5117029834721749e+00
   2.1567890217287555e-02   2.5055613369559024e+00
   6.2351097069848720e+00   2.4948310307876493e+00
   6.1621752908294987e+00   2.4787432636727131e+00
   6.0865872255739504e+00   2.4563506312041783e+00
   6.0089289625150926e+00   2.4263499966268300e+00
   5.9319373789757179e+00   2.3876935371121011e+00
   5.8640308290026546e+00   2.3423124574184397e+00
   5.8225172337144961e+00   2.3008527563005621e+00
   5.8373177801558924e+00   2.2879794302544085e+00
   5.9720557846314684e+00   2.3321076616094971e+00
   1.0498353683889405e-01   2.3777142499116266e+00
   7.4080634617191521e-01   1.7195727433398746e+00
   5.7293892352447315e+00   1.3559193931191318e-01
   4.9580959955756363e+00   7.9975695914828759e-01
   4.9922150856519139e+00   1.8156271308470266e+00
   1.3630277794226764e+00   1.3277154029727647e+00
   1.7275868387273796e+00   2.6960149717668784e+00
   1.7144144078609997e+00   2.6519382639274300e+00
   1.4430092673015906e+00   1.7853684516410893e+00
   1.4268476782179036e+00   2.8382774466030449e+00
   5.0010368128462943e+00   1.5401515549125253e+00
   4.9283074818063710e-02   2.5562827743104815e+00
   6.0112297821689467e+00   2.5122421129907164e+00
   5.7561141987248519e+00   2.4112428736111600e+00
   5.5876403880385048e+00   2.2877751401076121e+00
   5.4867907121243320e+00   2.1715286687014630e+00
   5.4292192211295571e+00   2.0779837797554785e+00
   5.3973612115094056e+00   2.0112908725919878e+00
   5.3809210264991094e+00   1.9703099083861351e+00
   5.3746615728207878e+00   1.9528058372163033e+00
   5.3765757863124080e+00   1.9574074606132243e+00
   5.3870297558442495e+00   1.9841734464291947e+00
   5.4088227545733787e+00   2.0342822230769020e+00
   5.4480056602940010e+00   2.1088053356626713e+00
   5.5150344937861711e+00   2.2061780707230705e+00
   5.6248437934112978e+00   2.3183998795392595e+00
   5.7923524780964613e+00   2.4281044412158082e+00
   6.0186109667283141e+00   2.5115330663962490e+00
   6.2716021749857482e+00   2.5503963194454333e+00
   2.0703915797870209e-01   2.5459231598241034e+00
   3.4232149039577209e-01   2.5215864617264363e+00
   3.8250465389447896e-01   2.5062363567839627e+00
   3.3857996669138757e-01   2.5096916882489273e+00
   2.3113615109269148e-01   2.5191031664781374e+00
   8.9344379979483080e-02   2.5177237561513861e+00
   6.2256161222232258e+00   2.4987636372750548e+00
   6.0885488384645399e+00   2.4629186979956663e+00
   5.9621702295381702e+00   2.4102989638358587e+00
   5.8532788118868559e+00   2.3417805041834674e+00
   5.7978908720171418e+00   2.2811241475939958e+00
   5.8785039400522372e+00   2.2971111878691417e+00
   6.7657645314390891e-02   2.3795068842323328e+00
   7.5578390616550806e-01   1.0669606705785477e+00
   5.3466103655252972e+00   3.3927829184685498e-01
   5.0131318366500359e+00   1.2395201403116944e+00
   1.2704220361459271e+00   4.7270278441278824e-01
   5.1599077368151285e+00   1.6651250200187022e+00
   5.1473263205465578e+00   1.6773916844771017e+00
   5.1380231682446365e+00   1.6836173726464927e+00
   5.1314762224839221e+00   1.6843502689262340e+00
   5.1272300765475158e+00   1.6812299090091314e+00
   5.1249018404037052e+00   1.6763585444086935e+00
   5.1242032620535092e+00   1.6715672909421115e+00
   5.1249812003109838e+00   1.6678479341740793e+00
   5.1272528439699556e+00   1.6650923991732935e+00
   5.1312114341845572e+00   1.6621735620829967e+00
   5.1372013073511518e+00   1.6573415017518531e+00
   5.1456803124826465e+00   1.6488480929302258e+00
   5.1571836702759555e+00   1.6356204082022330e+00
   5.1722863276250273e+00   1.6177536866126674e+00
   5.1915484951094903e+00   1.5967751369686449e+00
   5.2153669237260978e+00   1.5762047026394299e+00
   5.2434197133381382e+00   1.5636547524111191e+00
   5.2733672169300263e+00   1.5753546702976691e+00
   5.3012186579991791e+00   1.6409678176813980e+00
   5.3347618808824500e+00   1.8007362309634689e+00
   5.4306960539809559e+00   2.0732014229210445e+00
   5.7007712029630859e+00   2.3730352502265220e+00
   6.1423038517885402e+00   2.5348801357017607e+00
   2.0615484695530739e-01   2.5429629543088312e+00
   3.0001425703705920e-01   2.5224313537148673e+00
   2.0373710129196709e-01   2.5242809864616751e+00
   2.1173834799181890e-02   2.5147955847883385e+00
   6.1185561600796099e+00   2.4763816160881178e+00
   5.9560047020494302e+00   2.4115785212589365e+00
   5.8249610611010070e+00   2.3240281352378713e+00
   5.7880820453524322e+00   2.2634139405342486e+00
   6.0411135304736554e+00   2.3482207158682433e+00
   5.4507544144254680e+00   8.1128646289678197e-01
   5.5206413868148587e+00   7.4395656613488648e-01
   5.5756167965791157e+00   6.9666330237119301e-01
   5.6164881169525742e+00   6.6444110094331998e-01
   5.6441142363749783e+00   6.4421043867012162e-01
   5.6589791791526345e+00   6.3416635297554091e-01
   5.6612482075923083e+00   6.3342805877112673e-01
   5.6508746528776683e+00   6.4188887090689706e-01
   5.6276173539945447e+00   6.6020027820760008e-01
   5.5909682026335297e+00   6.8987705654452325e-01
   5.5401158005414928e+00   7.3356075636017271e-01
   5.4743191215370786e+00   7.9547379144867136e-01
   5.3943924397708045e+00   8.8184023362482533e-01
   5.3057403864032402e+00   1.0000327163314975e+00
   5.2211296285174065e+00   1.1531903580061400e+00
   5.1577515415860020e+00   1.3279823188026831e+00
   5.1260297066931493e+00   1.4871211831736435e+00
   5.1221688831882837e+00   1.5894627181884160e+00
   5.1363399766799631e+00   1.6228029527311816e+00
   5.1629447252540892e+00   1.6071526087045636e+00
   5.2003263298956135e+00   1.5726490373121405e+00
   5.2463849749995681e+00   1.5500001557936798e+00
   5.2916275689323413e+00   1.5938700966742450e+00
   5.3360421535373099e+00   1.7982285354492851e+00
   5.5070292323562917e+00   2.1910700891128281e+00
   5.9899495527083886e+00   2.5011229300288234e+00
   1.5641623182407116e-01   2.5453407896855249e+00
   2.2608129678274125e-01   2.5290102091156457e+00
   5.5567049220893949e-02   2.5215057382552368e+00
   6.1181595558207817e+00   2.4794167473315674e+00
   5.9286047673845488e+00   2.4005495760217346e+00
   2.7913035325693158e-01   5.5355909739615017e-01
   3.1679297559990260e-01   5.8373513987400549e-01
   3.3819792204517540e-01   6.0391346328711948e-01
   3.4473956341336276e-01   6.1127423206753928e-01
   3.3693937621186976e-01   6.0490031258114152e-01
   3.1428210073005403e-01   5.8579474144938137e-01
   2.7538775520581282e-01   5.5686329041229510e-01
   2.1856488433229160e-01   5.2277759875989349e-01
   1.4278978269555864e-01   4.8952924557071104e-01
   4.8881506775440897e-02   4.6357591196689268e-01
   6.2232658224232793e+00   4.5079019869648401e-01
   6.1042686044572747e+00   4.5571700356543965e-01
   5.9790194086768267e+00   4.8160207486756562e-01
   5.8488695662232857e+00   5.3135874032595998e-01
   5.7107661952805095e+00   6.0966784851670297e-01
   5.5549646157782924e+00   7.2726729744719476e-01
   5.3778281019653278e+00   9.0676437575381996e-01
   5.2183914188867639e+00   1.1649895799986296e+00
   5.1366754132568744e+00   1.4340570565112702e+00
   5.1285635829893650e+00   1.5830139729780968e+00
   5.1562034799756624e+00   1.5982876428785409e+00
   5.2038460540581148e+00   1.5593133488835078e+00
   5.2633542367588468e+00   1.5438932303347666e+00
   5.3140265107874356e+00   1.6749245334438203e+00
   5.4399947233152126e+00   2.0860593568135100e+00
   5.9475561638739656e+00   2.4874830230771705e+00
   4.7064323024416765e-01   1.7320070346420384e+00
   4.8424390152473862e-01   1.6997797546696221e+00
   5.0273862391074431e-01   1.6496690147346509e+00
   5.2403687896717699e-01   1.5772347215340439e+00
   5.4460619072287031e-01   1.4768335937959685e+00
   5.5871550741965237e-01   1.3428646525923731e+00
   5.5746546169710243e-01   1.1731636279154682e+00
   5.2794603552126063e-01   9.7536680930015995e-01
   4.5401463709735879e-01   7.7318814278774084e-01
   3.2254083972639336e-01   6.0275439320181912e-01
   1.3756571552857366e-01   4.9413693043784573e-01
   6.2100422003491502e+00   4.5591151113493539e-01
   6.0016138397838610e+00   4.8067233846217572e-01
   5.8007031118724797e+00   5.6076541392195267e-01
   5.5899075576787567e+00   7.0222403744792050e-01
   5.3538505729947161e+00   9.4033103557147646e-01
   5.1749886888986225e+00   1.2841507889833454e+00
   5.1295668941834407e+00   1.5402445137400129e+00
   5.1568544836462671e+00   1.5856654114063484e+00
   5.2147551790534088e+00   1.5436039520689993e+00
   1.3779626224716424e-01   2.0001069919244565e+00
   1.6471358039769157e-01   1.9933313907677388e+00
   1.9956358310257372e-01   1.9820484480231713e+00
   2.4311851678001517e-01   1.9631099216941168e+00
   2.9579251728012323e-01   1.9316094077686758e+00
   3.5697171020364138e-01   1.8799709358218331e+00
   4.2385676973390574e-01   1.7967587269624967e+00
   4.8965332375386339e-01   1.6658013511596901e+00
   5.4103841762876570e-01   1.4683910022996804e+00
   5.5509615991649852e-01   1.1965232169161499e+00
   4.9784924367511962e-01   8.8422590613187024e-01
   3.3641924087307729e-01   6.2071752734580421e-01
   8.3247400131231331e-02   4.8129714405842727e-01
   6.0922424243061855e+00   4.6646696936973769e-01
   5.8371979961135132e+00   5.4592801042010941e-01
   6.2421843828365517e+00   1.9628345772594906e+00
   6.2590138901028496e+00   1.9689822856983330e+00
   6.2805263246186165e+00   1.9759191133304947e+00
   2.4999573740835501e-02   1.9827213189023727e+00
   6.0700941160654054e-02   1.9878130342581555e+00
   1.0673197440100779e-01   1.9884934129379517e+00
   1.6551120361994265e-01   1.9801260621902677e+00
   2.3884591039541903e-01   1.9547666216827966e+00
   3.2624586376680753e-01   1.8989332568084065e+00
   4.2171310059140055e-01   1.7905014415026848e+00
   5.0869261051535730e-01   1.5971744631806872e+00
   6.1992703995989551e+00   1.8895435325957370e+00
   6.2081459387406497e+00   1.8991595597781874e+00
   6.2188554362215100e+00   1.9106749991721779e+00


==> cyl_specDL.tex <==
  -9.7983427533653430e+03   0.0000000000000000e+00
  -8.2279319013144832e+03   0.0000000000000000e+00
  -7.2541960677076340e+03   0.0000000000000000e+00
  -7.1006321791471555e+03   0.0000000000000000e+00
  -6.5480398815439139e+03   0.0000000000000000e+00
  -6.4659695983125457e+03   0.0000000000000000e+00
  -6.0221185324432681e+03   0.0000000000000000e+00
  -5.8862823314573989e+03   0.0000000000000000e+00
  -5.8194729622009754e+03   0.0000000000000000e+00
  -5.6262241153133482e+03   0.0000000000000000e+00
  -5.4463515135201360e+03   0.0000000000000000e+00
  -5.3096672839237017e+03   0.0000000000000000e+00
  -5.1167703035445165e+03   0.0000000000000000e+00
  -4.9698248277463799e+03   0.0000000000000000e+00
  -4.7557229728917264e+03   0.0000000000000000e+00
  -4.7684171467033693e+03   0.0000000000000000e+00
  -4.6211916538101787e+03   0.0000000000000000e+00
  -4.3563820714796166e+03   0.0000000000000000e+00
  -4.0114159595040110e+03   0.0000000000000000e+00
  -3.8840519880749280e+03   0.0000000000000000e+00
  -3.8115623650491511e+03   0.0000000000000000e+00
  -3.7516737845317457e+03   0.0000000000000000e+00
  -3.6651333999634276e+03   0.0000000000000000e+00
  -3.6537980598411209e+03   0.0000000000000000e+00
  -3.6286085162150034e+03   0.0000000000000000e+00
  -3.5573814585622172e+03   0.0000000000000000e+00
  -3.5127990296232679e+03   0.0000000000000000e+00
  -3.3422380664419220e+03   0.0000000000000000e+00
  -3.2799975555775181e+03   0.0000000000000000e+00
  -3.2373700125412256e+03   0.0000000000000000e+00
  -3.2049752476941635e+03   0.0000000000000000e+00
  -3.1932384181600646e+03   8.8305361718663598e+00
  -3.1932384181600646e+03  -8.8305361718663598e+00
  -3.1388116848404966e+03   0.0000000000000000e+00
  -3.1143729750382349e+03   0.0000000000000000e+00
  -3.0900306786898013e+03   0.0000000000000000e+00
  -3.0450990509265816e+03   0.0000000000000000e+00
  -3.0443747627397993e+03   0.0000000000000000e+00
  -3.0167649101433399e+03   0.0000000000000000e+00
  -2.9943588170585504e+03   0.0000000000000000e+00
  -2.9580549655954710e+03   0.0000000000000000e+00
  -2.9446700392527046e+03   0.0000000000000000e+00
  -2.9282821639317322e+03   0.0000000000000000e+00
  -2.8868315573701639e+03   0.0000000000000000e+00
  -2.8845660388441979e+03   0.0000000000000000e+00
  -2.8760374993253504e+03   0.0000000000000000e+00
  -2.8706479491638379e+03   1.0428604873079095e+01
  -2.8706479491638379e+03  -1.0428604873079095e+01
  -2.8513871310418763e+03   0.0000000000000000e+00
  -2.8399341029318030e+03   0.0000000000000000e+00
  -2.8194492025266118e+03   0.0000000000000000e+00
  -2.7808999927254358e+03   0.0000000000000000e+00
  -2.7765834294497708e+03   0.0000000000000000e+00
  -2.7552775335732176e+03   0.0000000000000000e+00
  -2.7484333794741869e+03   0.0000000000000000e+00
  -2.7454211542569751e+03   0.0000000000000000e+00
  -2.7196960070436971e+03   0.0000000000000000e+00
  -2.7129332657817072e+03   0.0000000000000000e+00
  -2.6976322874485531e+03   0.0000000000000000e+00
  -2.6721146390625618e+03   0.0000000000000000e+00
  -2.6606538860921341e+03   4.2003127138079819e+00
  -2.6606538860921341e+03  -4.2003127138079819e+00
  -2.6450680586349290e+03   0.0000000000000000e+00
  -2.6228871847574269e+03   0.0000000000000000e+00
  -2.6097341692716373e+03   0.0000000000000000e+00
  -2.6043626787563285e+03   0.0000000000000000e+00
  -2.5962145286100135e+03   0.0000000000000000e+00
  -2.5919118430448357e+03   0.0000000000000000e+00
  -2.5862850338437042e+03   0.0000000000000000e+00
  -2.5733103076120583e+03   0.0000000000000000e+00
  -2.5648834944077958e+03   0.0000000000000000e+00
  -2.5542902754583356e+03   8.5347071442989841e-01
  -2.5542902754583356e+03  -8.5347071442989841e-01
  -2.5431497571761674e+03   0.0000000000000000e+00
  -2.5319218027971579e+03   0.0000000000000000e+00
  -2.5190267128620180e+03   0.0000000000000000e+00
  -2.5114158327128803e+03   2.5673522482761384e+00
  -2.5114158327128803e+03  -2.5673522482761384e+00
  -2.5013166570315771e+03   0.0000000000000000e+00
  -2.4995191659857464e+03   0.0000000000000000e+00
  -2.4944481609321697e+03   0.0000000000000000e+00
  -2.4858833480998064e+03   0.0000000000000000e+00
  -2.4738448550855296e+03   7.3589336059289556e-01
  -2.4738448550855296e+03  -7.3589336059289556e-01
  -2.4688792072866863e+03   0.0000000000000000e+00
  -2.4651852820909653e+03   0.0000000000000000e+00
  -2.4631005110297333e+03   3.9548154183615497e-01
  -2.4631005110297333e+03  -3.9548154183615497e-01
  -2.4540822162718059e+03   0.0000000000000000e+00
  -2.4338946811350925e+03   0.0000000000000000e+00
  -2.4287656979677813e+03   0.0000000000000000e+00
  -2.4215504885015057e+03   0.0000000000000000e+00
  -2.4183814080104903e+03   0.0000000000000000e+00
  -2.4162869805881846e+03   0.0000000000000000e+00
  -2.4045887821215147e+03   0.0000000000000000e+00
  -2.3938611698017676e+03   2.9195467792831571e+00
  -2.3938611698017676e+03  -2.9195467792831571e+00
  -2.3942946020589920e+03   0.0000000000000000e+00
  -2.3853116888871191e+03   0.0000000000000000e+00
  -2.3718020745524764e+03   3.7625668852036132e+00
  -2.3718020745524764e+03  -3.7625668852036132e+00
  -2.3545593930942459e+03   4.6581201607560336e+00
  -2.3545593930942459e+03  -4.6581201607560336e+00
  -2.3346078619020509e+03   0.0000000000000000e+00
  -2.3275254537626779e+03   4.8945128982267994e+00
  -2.3275254537626779e+03  -4.8945128982267994e+00
  -2.3199321711846201e+03   7.9270186386193342e-01
  -2.3199321711846201e+03  -7.9270186386193342e-01
  -2.3161353583043033e+03   0.0000000000000000e+00
  -2.3027877681099931e+03   0.0000000000000000e+00
  -2.2941684674991211e+03   4.9520471973482181e+00
  -2.2941684674991211e+03  -4.9520471973482181e+00
  -2.2886327941430513e+03   0.0000000000000000e+00
  -2.2808341287937319e+03   0.0000000000000000e+00
  -2.2789683209466825e+03   0.0000000000000000e+00
  -2.2745421675515313e+03   0.0000000000000000e+00
  -2.2703450581870252e+03   0.0000000000000000e+00
  -2.2636741840477325e+03   1.3631416799574072e+00
  -2.2636741840477325e+03  -1.3631416799574072e+00
  -2.2540420033513801e+03   0.0000000000000000e+00
  -2.2529926397923064e+03   0.0000000000000000e+00
  -2.2404563098323229e+03   0.0000000000000000e+00
  -2.2385860875787675e+03   0.0000000000000000e+00
  -2.2301836921850822e+03   3.0788156005872427e+00
  -2.2301836921850822e+03  -3.0788156005872427e+00
  -2.2212588679137084e+03   7.3691848886691744e+00
  -2.2212588679137084e+03  -7.3691848886691744e+00
  -2.2195872008283709e+03   0.0000000000000000e+00
  -2.2129036867831942e+03   2.1412866129571113e+00
  -2.2129036867831942e+03  -2.1412866129571113e+00
  -2.2060059343798030e+03   1.1804861965764697e+00
  -2.2060059343798030e+03  -1.1804861965764697e+00
  -2.2098863720091922e+03   0.0000000000000000e+00
  -2.1930133816862985e+03   0.0000000000000000e+00
  -2.1922092638416962e+03   0.0000000000000000e+00
  -2.1868465183391618e+03   0.0000000000000000e+00
  -2.1847809048057447e+03   0.0000000000000000e+00
  -2.1757089311805084e+03   0.0000000000000000e+00
  -2.1712483071789834e+03   0.0000000000000000e+00
  -2.1686259528843689e+03   1.0053837855077321e+00
  -2.1686259528843689e+03  -1.0053837855077321e+00
  -2.1655305111061271e+03   0.0000000000000000e+00
  -2.1552572891526629e+03   0.0000000000000000e+00
  -2.1530880362956955e+03   0.0000000000000000e+00
  -2.1500669868352338e+03   2.5752458003093941e+00
  -2.1500669868352338e+03  -2.5752458003093941e+00
  -2.1408552722297632e+03   0.0000000000000000e+00
  -2.1335283522963364e+03   9.2674901293008709e+00
  -2.1335283522963364e+03  -9.2674901293008709e+00
  -2.1332361366338469e+03   0.0000000000000000e+00
  -2.1287407940483199e+03   2.5022126117113230e+00
  -2.1287407940483199e+03  -2.5022126117113230e+00
  -2.1176607366861258e+03   0.0000000000000000e+00
  -2.1082234655273937e+03   0.0000000000000000e+00
  -2.1015014650113671e+03   5.9760681034019338e+00
  -2.1015014650113671e+03  -5.9760681034019338e+00
  -2.1012398844328991e+03   0.0000000000000000e+00
  -2.0934404244387556e+03   0.0000000000000000e+00
  -2.0951112640432889e+03   0.0000000000000000e+00
  -2.0812737963300387e+03   1.3155036882761020e+00
  -2.0812737963300387e+03  -1.3155036882761020e+00
  -2.0775149033882840e+03   0.0000000000000000e+00
  -2.0763961871794863e+03   0.0000000000000000e+00
  -2.0733256681483972e+03   9.5683541913993100e+00
  -2.0733256681483972e+03  -9.5683541913993100e+00
  -2.0727983785588276e+03   0.0000000000000000e+00
  -2.0676686961174578e+03   0.0000000000000000e+00
  -2.0640602965965454e+03   0.0000000000000000e+00
  -2.0601598101549853e+03   3.5799263587442911e+00
  -2.0601598101549853e+03  -3.5799263587442911e+00
  -2.0546846009932647e+03   1.2198946017317052e+00
  -2.0546846009932647e+03  -1.2198946017317052e+00
  -2.0410113024878092e+03   3.5936859609375706e+00
  -2.0410113024878092e+03  -3.5936859609375706e+00
  -2.0445180910576796e+03   0.0000000000000000e+00
  -2.0425262466889485e+03   8.6181434087088038e-01
  -2.0425262466889485e+03  -8.6181434087088038e-01
  -2.0300802299521956e+03   1.2184054748996407e+00
  -2.0300802299521956e+03  -1.2184054748996407e+00
   2.5073561575939263e-01   0.0000000000000000e+00
  -2.0217947732357336e+03   0.0000000000000000e+00
  -2.0228034515021650e+03   4.0409327084547879e+00
  -2.0228034515021650e+03  -4.0409327084547879e+00
  -2.0076819927334727e+03   5.8780652138568206e+00
  -2.0076819927334727e+03  -5.8780652138568206e+00
  -2.0074703438171032e+03   0.0000000000000000e+00
  -1.9982388354651039e+03   0.0000000000000000e+00
  -1.9958658413137373e+03   2.6141829621355321e+00
  -1.9958658413137373e+03  -2.6141829621355321e+00
  -1.9915615892789251e+03   0.0000000000000000e+00
  -1.9887609808938757e+03   0.0000000000000000e+00
  -1.9856652209866786e+03   0.0000000000000000e+00
  -1.9836507266874019e+03   0.0000000000000000e+00
  -1.9743350934939949e+03   4.4874239797157012e+00
  -1.9743350934939949e+03  -4.4874239797157012e+00
  -1.9747838710520834e+03   0.0000000000000000e+00
  -1.9702793131126368e+03   1.9024606263663519e+00
  -1.9702793131126368e+03  -1.9024606263663519e+00
  -1.9609227957812225e+03   5.1102916115684636e+00
  -1.9609227957812225e+03  -5.1102916115684636e+00
  -1.9554184035888190e+03   5.1004149818101077e+00
  -1.9554184035888190e+03  -5.1004149818101077e+00
  -1.9578198872375333e+03   0.0000000000000000e+00
  -1.9514484151715410e+03   0.0000000000000000e+00
  -1.9479259047670007e+03   4.5672703569818749e+00
  -1.9479259047670007e+03  -4.5672703569818749e+00
  -1.9433795985658403e+03   0.0000000000000000e+00
  -1.9399695451678961e+03   0.0000000000000000e+00
  -1.9322255900783052e+03   5.1362119256193395e-01
  -1.9322255900783052e+03  -5.1362119256193395e-01
  -1.9332790406373333e+03   2.2381670506553850e+00
  -1.9332790406373333e+03  -2.2381670506553850e+00
  -1.9257440448178099e+03   1.8865557473385735e+00
  -1.9257440448178099e+03  -1.8865557473385735e+00
  -1.9222122296617322e+03   0.0000000000000000e+00
  -1.9114874301515533e+03   6.3214055405959444e+00
  -1.9114874301515533e+03  -6.3214055405959444e+00
  -1.9192196199983293e+03   0.0000000000000000e+00
  -1.9166844137515498e+03   0.0000000000000000e+00
  -1.9150100513625050e+03   0.0000000000000000e+00
  -1.9109981018276535e+03   0.0000000000000000e+00
  -1.9066095496225539e+03   0.0000000000000000e+00
  -1.9019326262771820e+03   4.5038443088092111e+00
  -1.9019326262771820e+03  -4.5038443088092111e+00
  -1.8999605184318450e+03   0.0000000000000000e+00
  -1.8859648775968435e+03   2.4559100541872732e+00
  -1.8859648775968435e+03  -2.4559100541872732e+00
  -1.8880616044824874e+03   0.0000000000000000e+00
  -1.8773554010013249e+03   5.4454419089952566e+00
  -1.8773554010013249e+03  -5.4454419089952566e+00
  -1.8920330445634065e+03   0.0000000000000000e+00
  -1.8994502534549949e+03   0.0000000000000000e+00
  -1.8686150958863718e+03   0.0000000000000000e+00
  -1.8575687930671938e+03   0.0000000000000000e+00
  -1.8781376223278830e+03   0.0000000000000000e+00
  -1.8633120826267718e+03   3.0968729470063812e+00
  -1.8633120826267718e+03  -3.0968729470063812e+00
  -1.8656740681446033e+03   0.0000000000000000e+00
  -1.8586328312652888e+03   0.0000000000000000e+00
  -1.8761909228191703e+03   0.0000000000000000e+00
  -1.8540311255614959e+03   0.0000000000000000e+00
  -1.8524653244875135e+03   0.0000000000000000e+00
  -1.8503268975345723e+03   6.5368456621389983e+00
  -1.8503268975345723e+03  -6.5368456621389983e+00
  -1.8441882102744762e+03   4.7050566374099079e+00
  -1.8441882102744762e+03  -4.7050566374099079e+00
  -1.8427576207221794e+03   0.0000000000000000e+00
  -1.8416865802196060e+03   0.0000000000000000e+00
  -1.8390755870042608e+03   0.0000000000000000e+00
  -1.8352506086075264e+03   1.0491552689565877e+00
  -1.8352506086075264e+03  -1.0491552689565877e+00
  -1.8307113109239619e+03   4.1891281218287277e+00
  -1.8307113109239619e+03  -4.1891281218287277e+00
  -1.8296906104134737e+03   0.0000000000000000e+00
  -1.8269060379413088e+03   0.0000000000000000e+00
  -1.8192370787949671e+03   5.2512606602519636e+00
  -1.8192370787949671e+03  -5.2512606602519636e+00
  -1.8234440215310860e+03   0.0000000000000000e+00
  -1.8194961117124719e+03   0.0000000000000000e+00
  -1.8129596809089198e+03   0.0000000000000000e+00
  -1.8073221506814775e+03   0.0000000000000000e+00
  -1.8088759380508659e+03   2.6658226153152262e+00
  -1.8088759380508659e+03  -2.6658226153152262e+00
  -1.8003307451399310e+03   5.1748101551627519e+00
  -1.8003307451399310e+03  -5.1748101551627519e+00
  -1.8006530323850288e+03   1.6926394724072477e-01
  -1.8006530323850288e+03  -1.6926394724072477e-01
  -1.7964479312718472e+03   0.0000000000000000e+00
  -1.7898599559690842e+03   4.1539899468749599e+00
  -1.7898599559690842e+03  -4.1539899468749599e+00
  -1.7921514771325787e+03   0.0000000000000000e+00
  -1.7847811126130248e+03   0.0000000000000000e+00
  -1.7813174603232601e+03   0.0000000000000000e+00
  -1.7698034352682653e+03   7.7087163972494386e+00
  -1.7698034352682653e+03  -7.7087163972494386e+00
  -1.7786166535228890e+03   4.7286279811152082e-01
  -1.7786166535228890e+03  -4.7286279811152082e-01
  -1.7771291254027019e+03   0.0000000000000000e+00
  -1.7729655284258258e+03   1.5245374846712816e+00
  -1.7729655284258258e+03  -1.5245374846712816e+00
  -1.7663156658070925e+03   1.5696549114392528e+00
  -1.7663156658070925e+03  -1.5696549114392528e+00
  -1.7624170242387975e+03   0.0000000000000000e+00
  -1.7672083409718775e+03   0.0000000000000000e+00
  -1.7581892146011992e+03   0.0000000000000000e+00
  -1.7566077082699298e+03   1.3904438444824958e+00
  -1.7566077082699298e+03  -1.3904438444824958e+00
  -1.7509972091392106e+03   6.6112575078068248e-01
  -1.7509972091392106e+03  -6.6112575078068248e-01
  -1.7465127525528753e+03   0.0000000000000000e+00
  -1.7415519712881514e+03   3.4214726877289827e+00
  -1.7415519712881514e+03  -3.4214726877289827e+00
  -1.7321694025779143e+03   7.2761620937385967e+00
  -1.7321694025779143e+03  -7.2761620937385967e+00
  -1.7406577005201113e+03   0.0000000000000000e+00
  -1.7365466185650830e+03   0.0000000000000000e+00
  -1.7162999587975028e+03   5.9495285904759232e-01
  -1.7162999587975028e+03  -5.9495285904759232e-01
  -1.7231346096760840e+03   2.2408245458099700e+00
  -1.7231346096760840e+03  -2.2408245458099700e+00
  -1.7290922401374773e+03   0.0000000000000000e+00
  -1.7215675228802202e+03   1.6429150355600282e+00
  -1.7215675228802202e+03  -1.6429150355600282e+00
  -1.7255500136456617e+03   0.0000000000000000e+00
  -1.7339254690107819e+03   8.7414723234956104e-01
  -1.7339254690107819e+03  -8.7414723234956104e-01
  -1.7139278033478015e+03   0.0000000000000000e+00
  -1.7110992339079371e+03   7.1759837446404828e-01
  -1.7110992339079371e+03  -7.1759837446404828e-01
  -1.7057256035425630e+03   1.3810501501100321e+00
  -1.7057256035425630e+03  -1.3810501501100321e+00
  -1.7015983870856430e+03   3.9537132061029157e-01
  -1.7015983870856430e+03  -3.9537132061029157e-01
  -1.6968286887921322e+03   4.4839036384604007e+00
  -1.6968286887921322e+03  -4.4839036384604007e+00
  -1.6977635381050716e+03   9.6768666534451842e-01
  -1.6977635381050716e+03  -9.6768666534451842e-01
  -1.6950295659050487e+03   0.0000000000000000e+00
  -1.6926721828699099e+03   0.0000000000000000e+00
  -1.6908899821913769e+03   0.0000000000000000e+00
  -1.6873960502317123e+03   1.8502310343925382e-01
  -1.6873960502317123e+03  -1.8502310343925382e-01
  -1.6835690026033458e+03   4.3599850884639029e+00
  -1.6835690026033458e+03  -4.3599850884639029e+00
  -1.6830539045093215e+03   3.8677084443242506e+00
  -1.6830539045093215e+03  -3.8677084443242506e+00
  -1.6818793178519829e+03   0.0000000000000000e+00
  -1.6790374832782995e+03   0.0000000000000000e+00
  -1.6757374064233163e+03   2.0269868884498652e+00
  -1.6757374064233163e+03  -2.0269868884498652e+00
  -1.6735062604598861e+03   0.0000000000000000e+00
  -1.6720316479909773e+03   0.0000000000000000e+00
  -1.6677529958822263e+03   2.1144806742017761e+00
  -1.6677529958822263e+03  -2.1144806742017761e+00
  -1.6680389776867426e+03   0.0000000000000000e+00
  -1.6641966705944203e+03   0.0000000000000000e+00
  -1.6586472043360002e+03   5.6675951420681496e+00
  -1.6586472043360002e+03  -5.6675951420681496e+00
  -1.6624942577194818e+03   0.0000000000000000e+00
  -1.6598384754900692e+03   0.0000000000000000e+00
  -1.6255779938181004e+03   2.7014806680510279e+00
  -1.6255779938181004e+03  -2.7014806680510279e+00
  -1.6246088489306399e+03   1.3157639628978548e+00
  -1.6246088489306399e+03  -1.3157639628978548e+00
  -1.6283587214698118e+03   3.1806110452238889e+00
  -1.6283587214698118e+03  -3.1806110452238889e+00
  -1.6572975926717579e+03   0.0000000000000000e+00
  -1.6511083581642652e+03   4.2905605575610289e-01
  -1.6511083581642652e+03  -4.2905605575610289e-01
  -1.6486383148505929e+03   0.0000000000000000e+00
  -1.6562093458588754e+03   0.0000000000000000e+00
  -1.6318325780459286e+03   0.0000000000000000e+00
  -1.6419465136510821e+03   9.8556597729206974e-01
  -1.6419465136510821e+03  -9.8556597729206974e-01
  -1.6358104821218740e+03   0.0000000000000000e+00
  -1.6385340174399671e+03   1.3017309862981603e+00
  -1.6385340174399671e+03  -1.3017309862981603e+00
  -1.6427028632404169e+03   0.0000000000000000e+00
  -1.6363901683492472e+03   3.1939385061445589e+00
  -1.6363901683492472e+03  -3.1939385061445589e+00
  -1.6282962911619961e+03   0.0000000000000000e+00
  -1.6541259316237868e+03   4.6193768090479409e-01
  -1.6541259316237868e+03  -4.6193768090479409e-01
  -1.6464090236004288e+03   0.0000000000000000e+00
  -1.6191295160170716e+03   0.0000000000000000e+00
  -1.6187594497459177e+03   1.6344690845684791e+00
  -1.6187594497459177e+03  -1.6344690845684791e+00
  -1.6157790465116507e+03   0.0000000000000000e+00
  -1.6117687314782838e+03   2.6665497161673892e+00
  -1.6117687314782838e+03  -2.6665497161673892e+00
  -1.6133428522273459e+03   0.0000000000000000e+00
  -1.6108801940370035e+03   0.0000000000000000e+00
  -1.6090115176728098e+03   3.2426397689232642e+00
  -1.6090115176728098e+03  -3.2426397689232642e+00
  -1.5576291101010795e+03   3.9733263786402588e+00
  -1.5576291101010795e+03  -3.9733263786402588e+00
  -1.6075211467587385e+03   0.0000000000000000e+00
  -1.6073066673891935e+03   0.0000000000000000e+00
  -1.6034381569101765e+03   6.4978071235225121e-01
  -1.6034381569101765e+03  -6.4978071235225121e-01
  -1.5600772211980843e+03   0.0000000000000000e+00
  -1.6015373933077435e+03   0.0000000000000000e+00
  -1.5994516616038186e+03   2.8636576649015142e+00
  -1.5994516616038186e+03  -2.8636576649015142e+00
  -1.5630848467083483e+03   1.0743034346769127e+00
  -1.5630848467083483e+03  -1.0743034346769127e+00
  -1.5674646296158144e+03   4.3723665909885812e+00
  -1.5674646296158144e+03  -4.3723665909885812e+00
  -1.5858013259193713e+03   2.7681232935556750e+00
  -1.5858013259193713e+03  -2.7681232935556750e+00
  -1.5938824943502041e+03   1.4331221225808273e+00
  -1.5938824943502041e+03  -1.4331221225808273e+00
  -1.5860606295438704e+03   0.0000000000000000e+00
  -1.5971697178500740e+03   0.0000000000000000e+00
  -1.5827386245707373e+03   4.7236590665151829e-01
  -1.5827386245707373e+03  -4.7236590665151829e-01
  -1.5740698700840658e+03   2.0012300961482348e+00
  -1.5740698700840658e+03  -2.0012300961482348e+00
  -1.5689543409099188e+03   0.0000000000000000e+00
  -1.5911757046183270e+03   1.3051436826798386e+00
  -1.5911757046183270e+03  -1.3051436826798386e+00
  -1.5925088954264479e+03   0.0000000000000000e+00
  -1.5790062990609713e+03   0.0000000000000000e+00
  -1.5772764121466607e+03   1.4333414455278797e+00
  -1.5772764121466607e+03  -1.4333414455278797e+00
  -1.5734673338916962e+03   0.0000000000000000e+00
  -1.5717496739996604e+03   0.0000000000000000e+00
  -5.8985336269975086e+00   0.0000000000000000e+00
  -1.5560804608867948e+03   0.0000000000000000e+00
  -1.5530061008622320e+03   2.6839256606381565e+00
  -1.5530061008622320e+03  -2.6839256606381565e+00
  -1.5527338453188581e+03   1.0911286117182408e+00
  -1.5527338453188581e+03  -1.0911286117182408e+00
  -1.5491485511587523e+03   0.0000000000000000e+00
  -1.5462661701109605e+03   0.0000000000000000e+00
  -1.5451341641749907e+03   3.2815902992295571e+00
  -1.5451341641749907e+03  -3.2815902992295571e+00
  -1.5433423165365141e+03   0.0000000000000000e+00
  -1.5414148955637802e+03   2.0106896940718597e+00
  -1.5414148955637802e+03  -2.0106896940718597e+00
  -1.5395741882592074e+03   8.8308734636347619e-01
  -1.5395741882592074e+03  -8.8308734636347619e-01
  -1.5365782980097106e+03   2.6094287940276648e+00
  -1.5365782980097106e+03  -2.6094287940276648e+00
  -1.5344161834281836e+03   0.0000000000000000e+00
  -1.5329982353076366e+03   0.0000000000000000e+00
  -1.5028221761308703e+03   2.9540721988742478e+00
  -1.5028221761308703e+03  -2.9540721988742478e+00
  -1.5304806374833440e+03   1.8674273573652735e+00
  -1.5304806374833440e+03  -1.8674273573652735e+00
  -1.5251591526696509e+03   3.7521987538641111e+00
  -1.5251591526696509e+03  -3.7521987538641111e+00
  -1.5067179405142501e+03   2.5992840344433872e+00
  -1.5067179405142501e+03  -2.5992840344433872e+00
  -1.5081689565293011e+03   2.6450598310139766e+00
  -1.5081689565293011e+03  -2.6450598310139766e+00
  -1.5135516544933789e+03   3.3243819181965284e+00
  -1.5135516544933789e+03  -3.3243819181965284e+00
  -1.5272757920369031e+03   9.4764214246599987e-01
  -1.5272757920369031e+03  -9.4764214246599987e-01
  -1.5213267827808518e+03   1.9564283624109196e+00
  -1.5213267827808518e+03  -1.9564283624109196e+00
  -1.5152533684555915e+03   1.4690395027752898e+00
  -1.5152533684555915e+03  -1.4690395027752898e+00
  -1.5261358750523975e+03   0.0000000000000000e+00
  -1.5063297281597047e+03   0.0000000000000000e+00
  -1.5072046268978252e+03   0.0000000000000000e+00
  -1.5172684117018666e+03   0.0000000000000000e+00
  -1.5196865509545617e+03   0.0000000000000000e+00
  -1.5205139371728942e+03   0.0000000000000000e+00
  -8.0450170703788242e+00   0.0000000000000000e+00
  -2.2414510891488803e+01   0.0000000000000000e+00
  -2.2359169343796363e+01   0.0000000000000000e+00
  -2.5752967557499264e+01   0.0000000000000000e+00
  -2.5519555633533979e+01   0.0000000000000000e+00
  -2.5604023772886094e+01   0.0000000000000000e+00
  -3.1025611882959808e+01   0.0000000000000000e+00
  -1.5001110526296020e+03   8.7390784975189095e-01
  -1.5001110526296020e+03  -8.7390784975189095e-01
  -1.4978894582917042e+03   6.6809203173717513e-01
  -1.4978894582917042e+03  -6.6809203173717513e-01
  -1.4946293290165256e+03   0.0000000000000000e+00
  -1.4932442182261339e+03   3.3113639023651187e-01
  -1.4932442182261339e+03  -3.3113639023651187e-01
  -1.4916311050987356e+03   1.3148365599910949e+00
  -1.4916311050987356e+03  -1.3148365599910949e+00
  -1.4881970357302280e+03   0.0000000000000000e+00
  -1.4630830948728897e+03   4.7356252968819801e+00
  -1.4630830948728897e+03  -4.7356252968819801e+00
  -1.4608932275001216e+03   0.0000000000000000e+00
  -1.4855221125223084e+03   1.0468388616913660e+00
  -1.4855221125223084e+03  -1.0468388616913660e+00
  -1.4841493414470242e+03   1.4531286914046218e+00
  -1.4841493414470242e+03  -1.4531286914046218e+00
  -1.4632964215089030e+03   0.0000000000000000e+00
  -1.4775310032054317e+03   2.5768178773162824e+00
  -1.4775310032054317e+03  -2.5768178773162824e+00
  -1.4788245887094320e+03   2.1086357635276447e+00
  -1.4788245887094320e+03  -2.1086357635276447e+00
  -1.4844083801991139e+03   0.0000000000000000e+00
  -1.4666197045906019e+03   1.6948981878550196e+00
  -1.4666197045906019e+03  -1.6948981878550196e+00
  -1.4662547721086107e+03   0.0000000000000000e+00
  -1.4730142964257643e+03   9.4951387375057428e-01
  -1.4730142964257643e+03  -9.4951387375057428e-01
  -1.4745194597671659e+03   0.0000000000000000e+00
  -1.4699114474946352e+03   0.0000000000000000e+00
  -1.4693215736641200e+03   0.0000000000000000e+00
  -1.4807865372495278e+03   0.0000000000000000e+00
  -1.4787505622092376e+03   0.0000000000000000e+00
  -4.7853568509803722e+01   0.0000000000000000e+00
  -5.0095896330363246e+01   0.0000000000000000e+00
  -5.1692187086405241e+01   0.0000000000000000e+00
  -5.1996523560538847e+01   0.0000000000000000e+00
  -5.3234941719640545e+01   0.0000000000000000e+00
  -5.6034684419346668e+01   0.0000000000000000e+00
  -5.8393925680871497e+01   0.0000000000000000e+00
  -6.0745057185867658e+01   0.0000000000000000e+00
  -6.2356539625945999e+01   0.0000000000000000e+00
  -6.3499600801820961e+01   0.0000000000000000e+00
  -1.4587418777916928e+03   1.5834859791909621e+00
  -1.4587418777916928e+03  -1.5834859791909621e+00
  -1.4568261449928284e+03   2.4903260073420079e+00
  -1.4568261449928284e+03  -2.4903260073420079e+00
  -1.4576913367873492e+03   0.0000000000000000e+00
  -1.4547801755152566e+03   0.0000000000000000e+00
  -1.4523161747172028e+03   0.0000000000000000e+00
  -1.4498234405705534e+03   2.1705643781142925e+00
  -1.4498234405705534e+03  -2.1705643781142925e+00
  -1.4478085878151858e+03   5.8722174591024090e-01
  -1.4478085878151858e+03  -5.8722174591024090e-01
  -1.4460251916468833e+03   1.9933887567115007e+00
  -1.4460251916468833e+03  -1.9933887567115007e+00
  -1.4388723505037262e+03   6.5421007823855568e+00
  -1.4388723505037262e+03  -6.5421007823855568e+00
  -1.4443449538891589e+03   0.0000000000000000e+00
  -1.4421964087961205e+03   0.0000000000000000e+00
  -1.4395068657035154e+03   1.5859707360535846e+00
  -1.4395068657035154e+03  -1.5859707360535846e+00
  -1.4366015488424748e+03   3.3210846094964070e+00
  -1.4366015488424748e+03  -3.3210846094964070e+00
  -1.4380267642198173e+03   0.0000000000000000e+00
  -1.4402294301476509e+03   0.0000000000000000e+00
  -1.4271821446330728e+03   3.9933949700664781e+00
  -1.4271821446330728e+03  -3.9933949700664781e+00
  -1.4324578501418707e+03   0.0000000000000000e+00
  -1.4347601793585632e+03   0.0000000000000000e+00
  -1.4223082215228305e+03   3.2033929776530985e+00
  -1.4223082215228305e+03  -3.2033929776530985e+00
  -1.4305982297973146e+03   0.0000000000000000e+00
  -1.4301538221201513e+03   0.0000000000000000e+00
  -1.4282136098307947e+03   0.0000000000000000e+00
  -1.4210245732586673e+03   2.4304708184400967e+00
  -1.4210245732586673e+03  -2.4304708184400967e+00
  -1.4249888544816695e+03   0.0000000000000000e+00
  -1.4262902681496168e+03   0.0000000000000000e+00
  -1.4213550642954717e+03   0.0000000000000000e+00
  -1.4117855431787052e+03   4.3733550884570063e+00
  -1.4117855431787052e+03  -4.3733550884570063e+00
  -1.4142670450078508e+03   2.4257473740830116e+00
  -1.4142670450078508e+03  -2.4257473740830116e+00
  -1.4173023104294293e+03   0.0000000000000000e+00
  -1.4165906251315239e+03   0.0000000000000000e+00
  -1.4075455793622673e+03   2.2070850118362006e+00
  -1.4075455793622673e+03  -2.2070850118362006e+00
  -1.4089728394314493e+03   5.3466940121688367e-01
  -1.4089728394314493e+03  -5.3466940121688367e-01
  -1.4034969023095200e+03   1.6009318408287583e+00
  -1.4034969023095200e+03  -1.6009318408287583e+00
  -1.4017881203558777e+03   0.0000000000000000e+00
  -1.4002887742751607e+03   1.2057749680365952e+00
  -1.4002887742751607e+03  -1.2057749680365952e+00
  -1.3457262594975268e+03   3.6985572081124953e+00
  -1.3457262594975268e+03  -3.6985572081124953e+00
  -1.3972575989323375e+03   0.0000000000000000e+00
  -1.3938193913811920e+03   3.1504213722943528e+00
  -1.3938193913811920e+03  -3.1504213722943528e+00
  -1.3961367575916870e+03   1.6569997040192641e+00
  -1.3961367575916870e+03  -1.6569997040192641e+00
  -1.3470680360014078e+03   0.0000000000000000e+00
  -1.3950179289957068e+03   1.6475108635392630e-01
  -1.3950179289957068e+03  -1.6475108635392630e-01
  -1.3494642265967032e+03   2.8213544428987314e+00
  -1.3494642265967032e+03  -2.8213544428987314e+00
  -1.3916201980948902e+03   0.0000000000000000e+00
  -1.3512526668423266e+03   0.0000000000000000e+00
  -1.3889873387924829e+03   0.0000000000000000e+00
  -1.3881588932646237e+03   1.5537821032046086e+00
  -1.3881588932646237e+03  -1.5537821032046086e+00
  -1.3865709104232762e+03   0.0000000000000000e+00
  -1.3539701505002479e+03   0.0000000000000000e+00
  -1.3555124833212608e+03   2.0560774339368102e+00
  -1.3555124833212608e+03  -2.0560774339368102e+00
  -1.3840331336701061e+03   2.1410281261956041e+00
  -1.3840331336701061e+03  -2.1410281261956041e+00
  -1.3553035810841784e+03   0.0000000000000000e+00
  -1.3845522551876741e+03   0.0000000000000000e+00
  -1.3826489994279511e+03   0.0000000000000000e+00
  -1.3663101119142184e+03   4.2138144283407826e+00
  -1.3663101119142184e+03  -4.2138144283407826e+00
  -1.3790745306107315e+03   2.2166637974370733e+00
  -1.3790745306107315e+03  -2.2166637974370733e+00
  -1.3659132419691600e+03   3.6411863006757832e+00
  -1.3659132419691600e+03  -3.6411863006757832e+00
  -1.3594960818770091e+03   1.9054249974959256e+00
  -1.3594960818770091e+03  -1.9054249974959256e+00
  -1.3703271745133525e+03   2.4438275513411054e+00
  -1.3703271745133525e+03  -2.4438275513411054e+00
  -1.3757403711811312e+03   8.2174051630065392e-01
  -1.3757403711811312e+03  -8.2174051630065392e-01
  -1.3815846673887293e+03   0.0000000000000000e+00
  -1.3593549594935380e+03   0.0000000000000000e+00
  -1.3780575856362163e+03   0.0000000000000000e+00
  -1.3650521470412391e+03   0.0000000000000000e+00
  -1.3622656912689808e+03   8.6841173047191278e-01
  -1.3622656912689808e+03  -8.6841173047191278e-01
  -1.3717719740288105e+03   0.0000000000000000e+00
  -1.3735392588105135e+03   1.0359615813698071e-01
  -1.3735392588105135e+03  -1.0359615813698071e-01
  -1.3700409646350906e+03   0.0000000000000000e+00
  -6.8307538999317643e+01   0.0000000000000000e+00
  -6.9297813278846917e+01   0.0000000000000000e+00
  -6.9794587111197131e+01   0.0000000000000000e+00
  -7.1238725704046686e+01   0.0000000000000000e+00
  -1.3375278947520133e+03   0.0000000000000000e+00
  -1.3399492923931471e+03   9.0092797800403779e-01
  -1.3399492923931471e+03  -9.0092797800403779e-01
  -1.3413842851050911e+03   2.7788984643800672e+00
  -1.3413842851050911e+03  -2.7788984643800672e+00
  -1.3438335219448343e+03   1.1772771090337781e+00
  -1.3438335219448343e+03  -1.1772771090337781e+00
  -1.3456715786498626e+03   0.0000000000000000e+00
  -1.3421021884046661e+03   0.0000000000000000e+00
  -7.3364526475194339e+01   0.0000000000000000e+00
  -7.4633507615361708e+01   0.0000000000000000e+00
  -7.5544425373694352e+01   0.0000000000000000e+00
  -7.6922594006860820e+01   0.0000000000000000e+00
  -1.3287321851016131e+03   5.5366619693954999e-01
  -1.3287321851016131e+03  -5.5366619693954999e-01
  -1.3300392944544221e+03   2.5570911278026633e+00
  -1.3300392944544221e+03  -2.5570911278026633e+00
  -1.3312487396517095e+03   0.0000000000000000e+00
  -1.3322044622951730e+03   0.0000000000000000e+00
  -1.3353879514683817e+03   2.3375521075123058e+00
  -1.3353879514683817e+03  -2.3375521075123058e+00
  -1.3330885667805671e+03   0.0000000000000000e+00
  -1.3339592894416467e+03   0.0000000000000000e+00
  -7.9627112484861968e+01   0.0000000000000000e+00
  -7.9978650343614063e+01   0.0000000000000000e+00
  -8.0514929591335829e+01   0.0000000000000000e+00
  -8.1301294015100339e+01   0.0000000000000000e+00
  -8.2679930785372562e+01   0.0000000000000000e+00
  -8.4748961581898897e+01   0.0000000000000000e+00
  -1.3169774505837090e+03   2.9729636050350967e+00
  -1.3169774505837090e+03  -2.9729636050350967e+00
  -1.3164503595707670e+03   5.9452480444045441e-02
  -1.3164503595707670e+03  -5.9452480444045441e-02
  -1.3205183125676083e+03   1.4756529841640798e-01
  -1.3205183125676083e+03  -1.4756529841640798e-01
  -1.3233431392459049e+03   2.0116953368851713e+00
  -1.3233431392459049e+03  -2.0116953368851713e+00
  -1.3254428269223695e+03   0.0000000000000000e+00
  -8.6535340655098850e+01   0.0000000000000000e+00
  -8.6953517807767085e+01   0.0000000000000000e+00
  -8.7388774693155284e+01   0.0000000000000000e+00
  -8.8655692876381138e+01   0.0000000000000000e+00
  -8.9771572184677069e+01   0.0000000000000000e+00
  -8.9173668164597146e+01   0.0000000000000000e+00
  -8.9311005328451742e+01   0.0000000000000000e+00
  -9.1196148728183772e+01   0.0000000000000000e+00
  -1.3058685679335301e+03   0.0000000000000000e+00
  -1.3074569097108656e+03   9.4798443915362163e-01
  -1.3074569097108656e+03  -9.4798443915362163e-01
  -1.3132395091920116e+03   4.5739701745180854e+00
  -1.3132395091920116e+03  -4.5739701745180854e+00
  -1.3105122495269470e+03   1.4607798684943110e+00
  -1.3105122495269470e+03  -1.4607798684943110e+00
  -1.3130421625579665e+03   2.8611037265757941e+00
  -1.3130421625579665e+03  -2.8611037265757941e+00
  -1.3139093429977074e+03   0.0000000000000000e+00
  -9.4552441837492907e+01   0.0000000000000000e+00
  -9.6510703506796290e+01   0.0000000000000000e+00
  -9.5088795526858618e+01   0.0000000000000000e+00
  -9.5272159857992634e+01   0.0000000000000000e+00
  -9.5809094863384828e+01   0.0000000000000000e+00
  -9.7218163535850209e+01   0.0000000000000000e+00
  -9.8790045268513211e+01   0.0000000000000000e+00
  -1.2942438940977265e+03   0.0000000000000000e+00
  -1.2944910542722646e+03   0.0000000000000000e+00
  -1.2968535151624915e+03   1.0499231300293019e+00
  -1.2968535151624915e+03  -1.0499231300293019e+00
  -1.2968080903526961e+03   0.0000000000000000e+00
  -1.3011746572010377e+03   1.7402545915276251e+00
  -1.3011746572010377e+03  -1.7402545915276251e+00
  -1.2994997511797251e+03   0.0000000000000000e+00
  -1.3047005287541401e+03   7.5408398923983266e-01
  -1.3047005287541401e+03  -7.5408398923983266e-01
  -1.3036781130578454e+03   0.0000000000000000e+00
  -9.9533833368555037e+01   0.0000000000000000e+00
  -1.0062286728706724e+02   0.0000000000000000e+00
  -1.0112314438135347e+02   0.0000000000000000e+00
  -1.0249163318264718e+02   0.0000000000000000e+00
  -1.0356394205282915e+02   1.6408608646060724e-01
  -1.0356394205282915e+02  -1.6408608646060724e-01
  -1.0431580672638350e+02   0.0000000000000000e+00
  -1.0429954040247374e+02   0.0000000000000000e+00
  -1.0722086838608664e+02   0.0000000000000000e+00
  -1.0803738453592220e+02   0.0000000000000000e+00
  -1.2811348845001853e+03   0.0000000000000000e+00
  -1.2838491016663529e+03   2.5154844857436642e+00
  -1.2838491016663529e+03  -2.5154844857436642e+00
  -1.2919491453508442e+03   3.8364369323413747e+00
  -1.2919491453508442e+03  -3.8364369323413747e+00
  -1.2844264449350596e+03   0.0000000000000000e+00
  -1.2819422986296711e+03   0.0000000000000000e+00
  -1.2865330174712367e+03   0.0000000000000000e+00
  -1.2860284775497303e+03   0.0000000000000000e+00
  -1.2931745337082502e+03   0.0000000000000000e+00
  -1.2915678995516839e+03   0.0000000000000000e+00
  -1.2899419845854720e+03   0.0000000000000000e+00
  -1.0873430940256455e+02   0.0000000000000000e+00
  -1.0951328883415854e+02   0.0000000000000000e+00
  -1.1015580148574291e+02   0.0000000000000000e+00
  -1.1104942037201128e+02   0.0000000000000000e+00
  -1.1189536533287459e+02   0.0000000000000000e+00
  -1.1308422184143471e+02   0.0000000000000000e+00
  -1.1498175675304536e+02   0.0000000000000000e+00
  -1.1486659727228074e+02   0.0000000000000000e+00
  -1.1580535994031914e+02   0.0000000000000000e+00
  -1.1715444956350308e+02   0.0000000000000000e+00
  -1.1804699977964923e+02   0.0000000000000000e+00
  -1.1853482611461490e+02   0.0000000000000000e+00
  -1.1933581539422403e+02   0.0000000000000000e+00
  -1.1979924888939777e+02   0.0000000000000000e+00
  -1.2228743433115233e+02   0.0000000000000000e+00
  -1.2094610224312717e+02   0.0000000000000000e+00
  -1.2112036505323819e+02   0.0000000000000000e+00
  -1.2787859173929446e+03   9.0949711207533979e-01
  -1.2787859173929446e+03  -9.0949711207533979e-01
  -1.2746633424649081e+03   4.2509185098312443e+00
  -1.2746633424649081e+03  -4.2509185098312443e+00
  -1.2765359099390666e+03   1.6054068271081279e+00
  -1.2765359099390666e+03  -1.6054068271081279e+00
  -1.2632655671277396e+03   4.8955378520676351e+00
  -1.2632655671277396e+03  -4.8955378520676351e+00
  -1.2729402112386401e+03   2.0148440514995949e+00
  -1.2729402112386401e+03  -2.0148440514995949e+00
  -1.2723377112072251e+03   6.5143675584790617e-01
  -1.2723377112072251e+03  -6.5143675584790617e-01
  -1.2673759275848042e+03   1.7021359455254426e+00
  -1.2673759275848042e+03  -1.7021359455254426e+00
  -1.2661127367698891e+03   3.0452369161425192e+00
  -1.2661127367698891e+03  -3.0452369161425192e+00
  -1.2664102345920717e+03   0.0000000000000000e+00
  -1.2672036859971051e+03   0.0000000000000000e+00
  -1.2286946084848034e+02   0.0000000000000000e+00
  -1.2622124007743025e+03   2.5734373347533079e-01
  -1.2622124007743025e+03  -2.5734373347533079e-01
  -1.2612310066426542e+03   0.0000000000000000e+00
  -1.2597243161163169e+03   0.0000000000000000e+00
  -1.2540665206898470e+03   3.8385906980628555e+00
  -1.2540665206898470e+03  -3.8385906980628555e+00
  -1.2567014159534781e+03   0.0000000000000000e+00
  -1.2565940368385204e+03   2.4079814719622226e+00
  -1.2565940368385204e+03  -2.4079814719622226e+00
  -1.2505952757661194e+03   5.8576609657988881e+00
  -1.2505952757661194e+03  -5.8576609657988881e+00
  -1.2542482087826786e+03   0.0000000000000000e+00
  -1.2519047035203730e+03   0.0000000000000000e+00
  -1.2481175695482520e+03   4.6274700728407531e-01
  -1.2481175695482520e+03  -4.6274700728407531e-01
  -1.2458535245325688e+03   8.9298770109367598e-01
  -1.2458535245325688e+03  -8.9298770109367598e-01
  -1.2063958848375901e+03   8.2234655573856830e-01
  -1.2063958848375901e+03  -8.2234655573856830e-01
  -1.2444392567219963e+03   0.0000000000000000e+00
  -1.2417052014486744e+03   2.1787431418838774e+00
  -1.2417052014486744e+03  -2.1787431418838774e+00
  -1.2430489225904057e+03   6.6391325528485245e-01
  -1.2430489225904057e+03  -6.6391325528485245e-01
  -1.2385569668892488e+03   0.0000000000000000e+00
  -1.2358880991696656e+03   2.2523560250920962e+00
  -1.2358880991696656e+03  -2.2523560250920962e+00
  -1.2417476280474921e+03   0.0000000000000000e+00
  -1.2096785465568069e+03   1.6031222387592687e+00
  -1.2096785465568069e+03  -1.6031222387592687e+00
  -1.2368662468598245e+03   0.0000000000000000e+00
  -1.2360465952201000e+03   0.0000000000000000e+00
  -1.2130043693606444e+03   2.8403392609384568e+00
  -1.2130043693606444e+03  -2.8403392609384568e+00
  -1.2323463766164064e+03   0.0000000000000000e+00
  -1.2293024069243747e+03   3.0278386069227645e+00
  -1.2293024069243747e+03  -3.0278386069227645e+00
  -1.2107605307234289e+03   0.0000000000000000e+00
  -1.2205246794000923e+03   4.2820020975778350e+00
  -1.2205246794000923e+03  -4.2820020975778350e+00
  -1.2149954580984179e+03   0.0000000000000000e+00
  -1.2282876912320125e+03   1.2740419456699155e+00
  -1.2282876912320125e+03  -1.2740419456699155e+00
  -1.2229096831427237e+03   1.9449643663761407e+00
  -1.2229096831427237e+03  -1.9449643663761407e+00
  -1.2286728010846641e+03   0.0000000000000000e+00
  -1.2260276437922721e+03   0.0000000000000000e+00
  -1.2171575910438737e+03   1.2745885296881179e+00
  -1.2171575910438737e+03  -1.2745885296881179e+00
  -1.2273511373121846e+03   0.0000000000000000e+00
  -1.2239581286257069e+03   0.0000000000000000e+00
  -1.2208877971218881e+03   2.1086302544666480e-01
  -1.2208877971218881e+03  -2.1086302544666480e-01
  -1.2177940513989713e+03   0.0000000000000000e+00
  -1.2373859496284751e+02   0.0000000000000000e+00
  -1.2568756608631732e+02   0.0000000000000000e+00
  -1.2705376260986498e+02   0.0000000000000000e+00
  -1.2468402446532124e+02   0.0000000000000000e+00
  -1.2487816096763241e+02   0.0000000000000000e+00
  -1.2028263036270944e+03   0.0000000000000000e+00
  -1.2047319950606211e+03   4.1751023163950158e+00
  -1.2047319950606211e+03  -4.1751023163950158e+00
  -1.2035633260735412e+03   1.2776671954907446e+00
  -1.2035633260735412e+03  -1.2776671954907446e+00
  -1.2079880244469875e+03   0.0000000000000000e+00
  -1.2792603633784260e+02   0.0000000000000000e+00
  -1.2994676016161594e+02   0.0000000000000000e+00
  -1.3067024463809315e+02   0.0000000000000000e+00
  -1.3123325750764556e+02   0.0000000000000000e+00
  -1.3214861322355864e+02   0.0000000000000000e+00
  -1.3329818255656772e+02   0.0000000000000000e+00
  -1.3369381851846006e+02   0.0000000000000000e+00
  -1.3434651027061437e+02   0.0000000000000000e+00
  -1.1935279735216404e+03   3.2276831663084455e+00
  -1.1935279735216404e+03  -3.2276831663084455e+00
  -1.1910626293771288e+03   5.9319843828100038e-01
  -1.1910626293771288e+03  -5.9319843828100038e-01
  -1.1933642751189029e+03   0.0000000000000000e+00
  -1.1960932303824225e+03   0.0000000000000000e+00
  -1.1967008834158758e+03   8.9504983785884418e-01
  -1.1967008834158758e+03  -8.9504983785884418e-01
  -1.2003244259291846e+03   0.0000000000000000e+00
  -1.1985248218784252e+03   3.9006030702930683e-01
  -1.1985248218784252e+03  -3.9006030702930683e-01
  -1.3617921472992185e+02   0.0000000000000000e+00
  -1.3658967922033310e+02   1.0602723040664183e-01
  -1.3658967922033310e+02  -1.0602723040664183e-01
  -1.3773231201547597e+02   0.0000000000000000e+00
  -1.3816105531329305e+02   0.0000000000000000e+00
  -1.3987958906430057e+02   0.0000000000000000e+00
  -1.4004173874562022e+02   0.0000000000000000e+00
  -1.4094875277001663e+02   0.0000000000000000e+00
  -1.4132982016357013e+02   0.0000000000000000e+00
  -1.4164723645202884e+02   0.0000000000000000e+00
  -1.4214236331231874e+02   0.0000000000000000e+00
  -1.4250448640682603e+02   0.0000000000000000e+00
  -1.4289211336730753e+02   0.0000000000000000e+00
  -1.4444090670898495e+02   0.0000000000000000e+00
  -1.4404113508550236e+02   0.0000000000000000e+00
  -1.4378803022576420e+02   0.0000000000000000e+00
  -1.1873556251743303e+03   1.5464209260085431e+00
  -1.1873556251743303e+03  -1.5464209260085431e+00
  -1.1783880278769595e+03   4.0644543620512614e+00
  -1.1783880278769595e+03  -4.0644543620512614e+00
  -1.1818043025461689e+03   3.1735611991363770e+00
  -1.1818043025461689e+03  -3.1735611991363770e+00
  -1.1858969294798399e+03   5.7979001203082536e-01
  -1.1858969294798399e+03  -5.7979001203082536e-01
  -1.1719065231659145e+03   2.5591369665569674e+00
  -1.1719065231659145e+03  -2.5591369665569674e+00
  -1.1836866380675849e+03   0.0000000000000000e+00
  -1.1752692114054157e+03   1.5822572385860827e+00
  -1.1752692114054157e+03  -1.5822572385860827e+00
  -1.1799999998104893e+03   1.3794572702532981e+00
  -1.1799999998104893e+03  -1.3794572702532981e+00
  -1.1775129280538231e+03   0.0000000000000000e+00
  -1.1819617028404293e+03   0.0000000000000000e+00
  -1.5027055311148305e+02   0.0000000000000000e+00
  -1.4486915126531210e+02   0.0000000000000000e+00
  -1.4517125669802746e+02   0.0000000000000000e+00
  -1.4579723324101781e+02   0.0000000000000000e+00
  -1.4958395612538880e+02   0.0000000000000000e+00
  -1.4908901158033984e+02   0.0000000000000000e+00
  -1.4690455071695754e+02   0.0000000000000000e+00
  -1.4868219186317646e+02   0.0000000000000000e+00
  -1.4800028668596241e+02   0.0000000000000000e+00
  -1.4748103183877643e+02   0.0000000000000000e+00
  -1.4647579522776331e+02   0.0000000000000000e+00
  -1.1738374264349538e+03   0.0000000000000000e+00
  -1.1699379182837047e+03   3.5363632683488477e+00
  -1.1699379182837047e+03  -3.5363632683488477e+00
  -1.1675624952801277e+03   1.2024385569301141e+00
  -1.1675624952801277e+03  -1.2024385569301141e+00
  -1.1671168174038025e+03   1.6852468636216520e+00
  -1.1671168174038025e+03  -1.6852468636216520e+00
  -1.1641322785476345e+03   2.2727037738789679e+00
  -1.1641322785476345e+03  -2.2727037738789679e+00
  -1.1600425386565441e+03   0.0000000000000000e+00
  -1.1612706980758744e+03   1.5656871969464026e+00
  -1.1612706980758744e+03  -1.5656871969464026e+00
  -1.1643721758080746e+03   2.1739263322895594e-01
  -1.1643721758080746e+03  -2.1739263322895594e-01
  -1.1292835362708249e+03   4.9434712915707557e+00
  -1.1292835362708249e+03  -4.9434712915707557e+00
  -1.1558882532834018e+03   2.1574083759625520e+00
  -1.1558882532834018e+03  -2.1574083759625520e+00
  -1.1582319275566704e+03   0.0000000000000000e+00
  -1.1570550026049195e+03   0.0000000000000000e+00
  -1.1298599532869946e+03   0.0000000000000000e+00
  -1.1454150168984729e+03   5.3309850760897683e+00
  -1.1454150168984729e+03  -5.3309850760897683e+00
  -1.1536355688539538e+03   0.0000000000000000e+00
  -1.1534104838588642e+03   0.0000000000000000e+00
  -1.1498901346451762e+03   2.7841872504914291e+00
  -1.1498901346451762e+03  -2.7841872504914291e+00
  -1.1322356098911830e+03   1.9721185681256750e-01
  -1.1322356098911830e+03  -1.9721185681256750e-01
  -1.1506128331287248e+03   6.5886951055339416e-01
  -1.1506128331287248e+03  -6.5886951055339416e-01
  -1.1341233110552359e+03   1.9151187690263345e+00
  -1.1341233110552359e+03  -1.9151187690263345e+00
  -1.1410829545112097e+03   3.1008416909284828e+00
  -1.1410829545112097e+03  -3.1008416909284828e+00
  -1.1461423813387678e+03   0.0000000000000000e+00
  -1.1475951307093940e+03   7.4883525764841874e-01
  -1.1475951307093940e+03  -7.4883525764841874e-01
  -1.1367737670922600e+03   0.0000000000000000e+00
  -1.1426136898363645e+03   1.0107696343189045e+00
  -1.1426136898363645e+03  -1.0107696343189045e+00
  -1.1396917062742161e+03   6.0364194505873303e-01
  -1.1396917062742161e+03  -6.0364194505873303e-01
  -1.1386782868886680e+03   0.0000000000000000e+00
  -1.1443095300868529e+03   0.0000000000000000e+00
  -1.5107139987522129e+02   0.0000000000000000e+00
  -1.5122804301390852e+02   0.0000000000000000e+00
  -1.5210172888062075e+02   0.0000000000000000e+00
  -1.5323326423250288e+02   0.0000000000000000e+00
  -1.5301404070018125e+02   0.0000000000000000e+00
  -1.5397997438912009e+02   0.0000000000000000e+00
  -1.1279317532357475e+03   0.0000000000000000e+00
  -1.1231903346598806e+03   8.1205756321705014e-01
  -1.1231903346598806e+03  -8.1205756321705014e-01
  -1.1246883619812857e+03   8.4150628979370268e-01
  -1.1246883619812857e+03  -8.4150628979370268e-01
  -1.1259592194079260e+03   6.5545287703191224e-01
  -1.1259592194079260e+03  -6.5545287703191224e-01
  -1.5568984962976060e+02   0.0000000000000000e+00
  -1.5502901424330270e+02   0.0000000000000000e+00
  -1.5465391165340279e+02   0.0000000000000000e+00
  -1.5383518737808896e+02   0.0000000000000000e+00
  -1.5733072527515640e+02   0.0000000000000000e+00
  -1.5638199296102778e+02   0.0000000000000000e+00
  -1.5933855282611188e+02   0.0000000000000000e+00
  -1.5823530020000217e+02   0.0000000000000000e+00
  -1.5709090995980088e+02   0.0000000000000000e+00
  -1.5780790268213164e+02   0.0000000000000000e+00
  -1.6037787752927508e+02   0.0000000000000000e+00
  -1.6115567207431519e+02   0.0000000000000000e+00
  -1.6256734571587666e+02   0.0000000000000000e+00
  -1.6164782778893294e+02   0.0000000000000000e+00
  -1.6184064567134735e+02   0.0000000000000000e+00
  -1.1215439334967957e+03   0.0000000000000000e+00
  -1.1189604989368286e+03   5.4958159520912035e+00
  -1.1189604989368286e+03  -5.4958159520912035e+00
  -1.1177842602605099e+03   0.0000000000000000e+00
  -1.1117509448552723e+03   2.3300849340302512e+00
  -1.1117509448552723e+03  -2.3300849340302512e+00
  -1.1156011771343551e+03   8.2760673279788907e-02
  -1.1156011771343551e+03  -8.2760673279788907e-02
  -1.1072649849341919e+03   7.1880471093534437e-01
  -1.1072649849341919e+03  -7.1880471093534437e-01
  -1.1132024198692666e+03   0.0000000000000000e+00
  -1.1083218422516929e+03   0.0000000000000000e+00
  -1.1129171203691328e+03   0.0000000000000000e+00
  -1.1113304658960888e+03   6.8306544349422216e-01
  -1.1113304658960888e+03  -6.8306544349422216e-01
  -1.6792045280482702e+02   0.0000000000000000e+00
  -1.6284485121371327e+02   0.0000000000000000e+00
  -1.6348270599766187e+02   0.0000000000000000e+00
  -1.6485450869236601e+02   0.0000000000000000e+00
  -1.6757080497646186e+02   0.0000000000000000e+00
  -1.6675235793445273e+02   1.9385597858245399e-01
  -1.6675235793445273e+02  -1.9385597858245399e-01
  -1.6573117724136637e+02   0.0000000000000000e+00
  -1.6536949172980653e+02   0.0000000000000000e+00
  -1.1032158004935818e+03   3.3262082636205781e+00
  -1.1032158004935818e+03  -3.3262082636205781e+00
  -1.1019349930163651e+03   0.0000000000000000e+00
  -1.1035276633606481e+03   1.0484841935395726e+00
  -1.1035276633606481e+03  -1.0484841935395726e+00
  -1.0991994185569508e+03   3.4742954634272163e+00
  -1.0991994185569508e+03  -3.4742954634272163e+00
  -1.0947524393286913e+03   3.0754726911296686e+00
  -1.0947524393286913e+03  -3.0754726911296686e+00
  -1.0970748921091019e+03   1.2394577478863240e+00
  -1.0970748921091019e+03  -1.2394577478863240e+00
  -1.0958013306174080e+03   1.1239881893732024e+00
  -1.0958013306174080e+03  -1.1239881893732024e+00
  -1.0915312958170580e+03   1.9875589115831540e+00
  -1.0915312958170580e+03  -1.9875589115831540e+00
  -1.0927949254102607e+03   0.0000000000000000e+00
  -1.0884618480948930e+03   4.3335313554607785e-01
  -1.0884618480948930e+03  -4.3335313554607785e-01
  -1.0686293792882987e+03   7.5619690582230348e-01
  -1.0686293792882987e+03  -7.5619690582230348e-01
  -1.0702541611500478e+03   2.5751755093949988e+00
  -1.0702541611500478e+03  -2.5751755093949988e+00
  -1.0825319799040349e+03   2.6594012742936455e+00
  -1.0825319799040349e+03  -2.6594012742936455e+00
  -1.0865987745084965e+03   0.0000000000000000e+00
  -1.0796430090687820e+03   2.1934718979834615e+00
  -1.0796430090687820e+03  -2.1934718979834615e+00
  -1.0856680982699338e+03   0.0000000000000000e+00
  -1.0839971132943033e+03   7.5758245489515819e-01
  -1.0839971132943033e+03  -7.5758245489515819e-01
  -1.0742342754559281e+03   1.5079727479886305e+00
  -1.0742342754559281e+03  -1.5079727479886305e+00
  -1.0762093062688496e+03   0.0000000000000000e+00
  -1.0800298730183345e+03   1.1025002348846659e-01
  -1.0800298730183345e+03  -1.1025002348846659e-01
  -1.0709121545476214e+03   5.0557067890268936e-01
  -1.0709121545476214e+03  -5.0557067890268936e-01
  -1.0703819665880167e+03   0.0000000000000000e+00
  -1.0736405238661589e+03   0.0000000000000000e+00
  -1.0838470148201786e+03   0.0000000000000000e+00
  -1.6944616132594749e+02   0.0000000000000000e+00
  -1.6981060573005195e+02   0.0000000000000000e+00
  -1.7045860131196022e+02   0.0000000000000000e+00
  -1.7061507216377436e+02   0.0000000000000000e+00
  -1.7226719335062120e+02   0.0000000000000000e+00
  -1.0641982578599864e+03   2.9092878918742029e+00
  -1.0641982578599864e+03  -2.9092878918742029e+00
  -1.0629233755634830e+03   0.0000000000000000e+00
  -1.0639354087644454e+03   0.0000000000000000e+00
  -1.0659557797335053e+03   0.0000000000000000e+00
  -1.7333147735885927e+02   4.4064366930472637e-02
  -1.7333147735885927e+02  -4.4064366930472637e-02
  -1.7384380819232791e+02   0.0000000000000000e+00
  -1.7439573278612630e+02   0.0000000000000000e+00
  -1.7474629854742585e+02   0.0000000000000000e+00
  -1.7583021083398822e+02   0.0000000000000000e+00
  -1.7545456964366409e+02   0.0000000000000000e+00
  -1.7753789957532558e+02   0.0000000000000000e+00
  -1.7762988457392692e+02   3.0006624045315133e-01
  -1.7762988457392692e+02  -3.0006624045315133e-01
  -1.7678173986776076e+02   0.0000000000000000e+00
  -1.7824195991038351e+02   0.0000000000000000e+00
  -1.7904280251595540e+02   0.0000000000000000e+00
  -1.8055581567559273e+02   0.0000000000000000e+00
  -1.8148731918523944e+02   0.0000000000000000e+00
  -1.0609674284095768e+03   8.2500552577889474e-01
  -1.0609674284095768e+03  -8.2500552577889474e-01
  -1.0586788724565774e+03   6.7139419561885727e-01
  -1.0586788724565774e+03  -6.7139419561885727e-01
  -1.0520652178561227e+03   3.1372273685559935e+00
  -1.0520652178561227e+03  -3.1372273685559935e+00
  -1.0482631575089681e+03   2.4994207294710655e+00
  -1.0482631575089681e+03  -2.4994207294710655e+00
  -1.0478423923077557e+03   1.0851149666027513e+00
  -1.0478423923077557e+03  -1.0851149666027513e+00
  -1.0563409747629537e+03   0.0000000000000000e+00
  -1.0567613488728703e+03   2.1795546335792735e+00
  -1.0567613488728703e+03  -2.1795546335792735e+00
  -1.0481968468681732e+03   0.0000000000000000e+00
  -1.0555369378441983e+03   9.9279264210983909e-01
  -1.0555369378441983e+03  -9.9279264210983909e-01
  -1.0526808901050485e+03   0.0000000000000000e+00
  -1.0550558014097380e+03   0.0000000000000000e+00
  -1.0507458926153276e+03   0.0000000000000000e+00
  -1.8194470671120874e+02   0.0000000000000000e+00
  -1.8119978383294085e+02   0.0000000000000000e+00
  -1.8489018593359947e+02   2.1955846061356302e-01
  -1.8489018593359947e+02  -2.1955846061356302e-01
  -1.8326392481404176e+02   1.0369404747258643e-01
  -1.8326392481404176e+02  -1.0369404747258643e-01
  -1.8602991746130516e+02   0.0000000000000000e+00
  -1.8625792544212916e+02   0.0000000000000000e+00
  -1.0406548487128018e+03   3.7793115145178047e+00
  -1.0406548487128018e+03  -3.7793115145178047e+00
  -1.0447670755512522e+03   0.0000000000000000e+00
  -1.0448926004630575e+03   0.0000000000000000e+00
  -1.0354093630107418e+03   2.8218625218720690e+00
  -1.0354093630107418e+03  -2.8218625218720690e+00
  -1.0423970078709217e+03   0.0000000000000000e+00
  -1.0388887801597580e+03   0.0000000000000000e+00
  -1.0412582000182858e+03   8.1649367535345230e-01
  -1.0412582000182858e+03  -8.1649367535345230e-01
  -1.0371727230002189e+03   0.0000000000000000e+00
  -1.0328248580928398e+03   1.8753523136139802e+00
  -1.0328248580928398e+03  -1.8753523136139802e+00
  -1.0336557182757326e+03   0.0000000000000000e+00
  -1.0317268764675962e+03   0.0000000000000000e+00
  -1.0282997197193190e+03   3.2066880687570216e+00
  -1.0282997197193190e+03  -3.2066880687570216e+00
  -1.0289652411255004e+03   1.4833051700262345e+00
  -1.0289652411255004e+03  -1.4833051700262345e+00
  -1.0271718727212779e+03   1.9579433276114060e+00
  -1.0271718727212779e+03  -1.9579433276114060e+00
  -1.0192822639815890e+03   3.7310610259312003e+00
  -1.0192822639815890e+03  -3.7310610259312003e+00
  -1.0106016093317876e+03   1.3211700892249978e+00
  -1.0106016093317876e+03  -1.3211700892249978e+00
  -1.0124091037527523e+03   1.8656058717632011e+00
  -1.0124091037527523e+03  -1.8656058717632011e+00
  -1.0228383899259574e+03   1.2854370619154996e+00
  -1.0228383899259574e+03  -1.2854370619154996e+00
  -1.0211370279674736e+03   1.3478987667680078e+00
  -1.0211370279674736e+03  -1.3478987667680078e+00
  -1.0256623588126613e+03   0.0000000000000000e+00
  -1.0095356399607788e+03   0.0000000000000000e+00
  -1.0152255121051066e+03   1.3992478975182066e+00
  -1.0152255121051066e+03  -1.3992478975182066e+00
  -1.0190879795229199e+03   0.0000000000000000e+00
  -1.0120231087250625e+03   0.0000000000000000e+00
  -1.0246720900024743e+03   0.0000000000000000e+00
  -1.0139600144973175e+03   0.0000000000000000e+00
  -1.0170381421452063e+03   0.0000000000000000e+00
  -1.8861094156821423e+02   0.0000000000000000e+00
  -1.8751162885572748e+02   0.0000000000000000e+00
  -1.8785755841320216e+02   0.0000000000000000e+00
  -1.8970416270462238e+02   1.5638239793134892e-01
  -1.8970416270462238e+02  -1.5638239793134892e-01
  -1.0027983835838004e+03   2.7627411509488402e+00
  -1.0027983835838004e+03  -2.7627411509488402e+00
  -1.0067011057849160e+03   7.5469043403088676e-01
  -1.0067011057849160e+03  -7.5469043403088676e-01
  -1.0078984252939894e+03   0.0000000000000000e+00
  -1.0052075665516734e+03   0.0000000000000000e+00
  -1.0059624609275148e+03   0.0000000000000000e+00
  -1.9038783457869005e+02   0.0000000000000000e+00
  -1.9123029916231621e+02   1.5191994060405598e-01
  -1.9123029916231621e+02  -1.5191994060405598e-01
  -1.9212822583788636e+02   0.0000000000000000e+00
  -1.9322155380446705e+02   0.0000000000000000e+00
  -1.9272250790125850e+02   0.0000000000000000e+00
  -1.9356505900049146e+02   0.0000000000000000e+00
  -1.9458267935459722e+02   0.0000000000000000e+00
  -1.9568943031186541e+02   2.6553434870159126e-01
  -1.9568943031186541e+02  -2.6553434870159126e-01
  -1.9696956343013312e+02   3.7676216359850356e-01
  -1.9696956343013312e+02  -3.7676216359850356e-01
  -9.9149130223508064e+02   4.4678188711815698e+00
  -9.9149130223508064e+02  -4.4678188711815698e+00
  -9.9876484027227866e+02   2.8085638727306841e+00
  -9.9876484027227866e+02  -2.8085638727306841e+00
  -1.0004212246062943e+03   1.8062901180682349e+00
  -1.0004212246062943e+03  -1.8062901180682349e+00
  -9.9381568742430363e+02   1.4390822939948666e+00
  -9.9381568742430363e+02  -1.4390822939948666e+00
  -9.9351056707743749e+02   0.0000000000000000e+00
  -9.8964848790747214e+02   0.0000000000000000e+00
  -9.9309849596462698e+02   0.0000000000000000e+00
  -9.9825513489351783e+02   3.3038344775250911e-01
  -9.9825513489351783e+02  -3.3038344775250911e-01
  -9.9581973907026907e+02   0.0000000000000000e+00
  -9.9058194823164888e+02   0.0000000000000000e+00
  -1.0027607369126468e+03   0.0000000000000000e+00
  -1.9875399796912930e+02   0.0000000000000000e+00
  -1.9853340527565672e+02   0.0000000000000000e+00
  -2.0247193761388976e+02   0.0000000000000000e+00
  -1.9921241244233909e+02   0.0000000000000000e+00
  -1.9939343929253531e+02   0.0000000000000000e+00
  -2.0084964085993036e+02   0.0000000000000000e+00
  -2.0302121446945114e+02   1.0591877006088300e-02
  -2.0302121446945114e+02  -1.0591877006088300e-02
  -2.0126283923862155e+02   0.0000000000000000e+00
  -2.0185133797303030e+02   1.9600576093326569e-01
  -2.0185133797303030e+02  -1.9600576093326569e-01
  -2.0198104410404360e+02   0.0000000000000000e+00
  -9.8692545879548584e+02   1.5591511286318691e+00
  -9.8692545879548584e+02  -1.5591511286318691e+00
  -9.8361848859642555e+02   2.6936771044404240e+00
  -9.8361848859642555e+02  -2.6936771044404240e+00
  -9.8677636381945331e+02   0.0000000000000000e+00
  -9.7998043473704570e+02   2.5231864979715803e+00
  -9.7998043473704570e+02  -2.5231864979715803e+00
  -9.8541529455664352e+02   0.0000000000000000e+00
  -9.8408942189244863e+02   4.9706392731128263e-01
  -9.8408942189244863e+02  -4.9706392731128263e-01
  -9.8242760384168866e+02   0.0000000000000000e+00
  -9.8104344094493945e+02   4.8851798251594231e-01
  -9.8104344094493945e+02  -4.8851798251594231e-01
  -9.7330356528664390e+02   2.9224017430318310e+00
  -9.7330356528664390e+02  -2.9224017430318310e+00
  -9.7285733539547550e+02   2.9025009660098453e+00
  -9.7285733539547550e+02  -2.9025009660098453e+00
  -9.7714815530563897e+02   2.2261980620069965e-01
  -9.7714815530563897e+02  -2.2261980620069965e-01
  -9.5683110384911140e+02   9.0878281149841922e-01
  -9.5683110384911140e+02  -9.0878281149841922e-01
  -9.5610624053152924e+02   0.0000000000000000e+00
  -9.6545345887037342e+02   3.2595282292695900e+00
  -9.6545345887037342e+02  -3.2595282292695900e+00
  -9.7412773115047423e+02   0.0000000000000000e+00
  -9.7564137089760209e+02   0.0000000000000000e+00
  -9.5882311560939809e+02   1.1899355214681229e+00
  -9.5882311560939809e+02  -1.1899355214681229e+00
  -9.6904793200293750e+02   0.0000000000000000e+00
  -9.5859261960668925e+02   0.0000000000000000e+00
  -9.6769719937710556e+02   3.7739000854674876e-01
  -9.6769719937710556e+02  -3.7739000854674876e-01
  -9.6217491023584762e+02   0.0000000000000000e+00
  -9.6536330526225674e+02   5.1801703065658111e-01
  -9.6536330526225674e+02  -5.1801703065658111e-01
  -9.6404155445659194e+02   4.4503396819619678e-01
  -9.6404155445659194e+02  -4.4503396819619678e-01
  -9.6975313410270041e+02   0.0000000000000000e+00
  -2.0468029359619180e+02   2.0860008637554348e-01
  -2.0468029359619180e+02  -2.0860008637554348e-01
  -2.0543110722193853e+02   1.4573928737446118e-01
  -2.0543110722193853e+02  -1.4573928737446118e-01
  -9.5391532859789459e+02   1.1297461622796297e+00
  -9.5391532859789459e+02  -1.1297461622796297e+00
  -2.0664195420637671e+02   3.0243288325918033e-01
  -2.0664195420637671e+02  -3.0243288325918033e-01
  -2.0777386233483566e+02   5.3184418607315509e-01
  -2.0777386233483566e+02  -5.3184418607315509e-01
  -2.0872421083939315e+02   6.0588239743334590e-03
  -2.0872421083939315e+02  -6.0588239743334590e-03
  -9.4226526382689224e+02   1.8979823414984540e+00
  -9.4226526382689224e+02  -1.8979823414984540e+00
  -9.4747828320725932e+02   4.1885935680251887e+00
  -9.4747828320725932e+02  -4.1885935680251887e+00
  -9.4552313252725480e+02   1.6245323042603391e-01
  -9.4552313252725480e+02  -1.6245323042603391e-01
  -9.4937195084802124e+02   9.2784537621629581e-01
  -9.4937195084802124e+02  -9.2784537621629581e-01
  -9.5022609033927938e+02   8.8675916282018108e-01
  -9.5022609033927938e+02  -8.8675916282018108e-01
  -9.5152439770886213e+02   5.1414706241750663e-01
  -9.5152439770886213e+02  -5.1414706241750663e-01
  -2.1090257273604854e+02   2.8661966838979192e-01
  -2.1090257273604854e+02  -2.8661966838979192e-01
  -2.1001671574620951e+02   0.0000000000000000e+00
  -2.1104539784510214e+02   0.0000000000000000e+00
  -2.1231212316847368e+02   6.4424911649372174e-01
  -2.1231212316847368e+02  -6.4424911649372174e-01
  -2.1198955224506804e+02   0.0000000000000000e+00
  -2.1507010012289768e+02   1.3189774591376818e-01
  -2.1507010012289768e+02  -1.3189774591376818e-01
  -2.1400563660740164e+02   0.0000000000000000e+00
  -2.1360168278508283e+02   0.0000000000000000e+00
  -2.1362068076732311e+02   0.0000000000000000e+00
  -9.3146470366003859e+02   3.4551998582320427e+00
  -9.3146470366003859e+02  -3.4551998582320427e+00
  -9.2766018884227196e+02   0.0000000000000000e+00
  -9.4067308485232309e+02   2.7073914919773205e+00
  -9.4067308485232309e+02  -2.7073914919773205e+00
  -9.3425544343289403e+02   2.8448161253697939e+00
  -9.3425544343289403e+02  -2.8448161253697939e+00
  -9.3708340631191504e+02   2.2297257940598540e+00
  -9.3708340631191504e+02  -2.2297257940598540e+00
  -9.3813685975563715e+02   0.0000000000000000e+00
  -9.3170066989498764e+02   2.8913407996263485e-01
  -9.3170066989498764e+02  -2.8913407996263485e-01
  -9.4089158507277330e+02   1.8757743703831556e-01
  -9.4089158507277330e+02  -1.8757743703831556e-01
  -9.3620096487082026e+02   0.0000000000000000e+00
  -9.3532978428663853e+02   0.0000000000000000e+00
  -2.1593582035509829e+02   0.0000000000000000e+00
  -2.1650234502752360e+02   0.0000000000000000e+00
  -2.1727016518513511e+02   0.0000000000000000e+00
  -2.1701050265597806e+02   0.0000000000000000e+00
  -2.1837316064957119e+02   0.0000000000000000e+00
  -2.2073769734757124e+02   0.0000000000000000e+00
  -2.2056915540785360e+02   0.0000000000000000e+00
  -2.1907819916478709e+02   1.3510057292613484e-01
  -2.1907819916478709e+02  -1.3510057292613484e-01
  -2.1971326201561959e+02   0.0000000000000000e+00
  -2.2156616363311156e+02   0.0000000000000000e+00
  -9.2723308972859331e+02   0.0000000000000000e+00
  -9.2158506142310944e+02   4.6757496921241692e+00
  -9.2158506142310944e+02  -4.6757496921241692e+00
  -9.2559268664567719e+02   1.0492667774899445e+00
  -9.2559268664567719e+02  -1.0492667774899445e+00
  -9.2451351063751576e+02   0.0000000000000000e+00
  -9.2273819779810958e+02   7.7065004574558826e-01
  -9.2273819779810958e+02  -7.7065004574558826e-01
  -9.2211789469455698e+02   0.0000000000000000e+00
  -9.2072984210279628e+02   0.0000000000000000e+00
  -9.1575460131028808e+02   3.2894337145763992e+00
  -9.1575460131028808e+02  -3.2894337145763992e+00
  -9.1999788372680837e+02   0.0000000000000000e+00
  -9.1114223190156508e+02   3.4538353673397157e+00
  -9.1114223190156508e+02  -3.4538353673397157e+00
  -9.1557719678199987e+02   1.2717659548874716e+00
  -9.1557719678199987e+02  -1.2717659548874716e+00
  -9.1774777096096113e+02   3.8538349673166544e-01
  -9.1774777096096113e+02  -3.8538349673166544e-01
  -9.0053193758088378e+02   3.1797631750794780e-01
  -9.0053193758088378e+02  -3.1797631750794780e-01
  -9.0557376487350780e+02   3.5423961727001760e+00
  -9.0557376487350780e+02  -3.5423961727001760e+00
  -9.1180672636870418e+02   0.0000000000000000e+00
  -9.1046587482243172e+02   0.0000000000000000e+00
  -9.0953352480212925e+02   0.0000000000000000e+00
  -9.0381658808628572e+02   1.3473938559702445e+00
  -9.0381658808628572e+02  -1.3473938559702445e+00
  -9.0584955764809354e+02   0.0000000000000000e+00
  -9.0704443282664488e+02   0.0000000000000000e+00
  -9.0409132055639168e+02   0.0000000000000000e+00
  -9.0211384443249540e+02   0.0000000000000000e+00
  -9.0796212183547937e+02   0.0000000000000000e+00
  -2.2499347641967762e+02   0.0000000000000000e+00
  -2.2319014549065864e+02   5.1576747694924863e-01
  -2.2319014549065864e+02  -5.1576747694924863e-01
  -2.2242700472478094e+02   0.0000000000000000e+00
  -2.2222051341769867e+02   0.0000000000000000e+00
  -8.9581273390587967e+02   2.2102433899396501e+00
  -8.9581273390587967e+02  -2.2102433899396501e+00
  -8.9543306424473781e+02   1.0045686061370389e+00
  -8.9543306424473781e+02  -1.0045686061370389e+00
  -8.9729647942300949e+02   0.0000000000000000e+00
  -8.9861589945975106e+02   3.0766227394352846e-01
  -8.9861589945975106e+02  -3.0766227394352846e-01
  -2.2525452328438485e+02   3.7568629204411180e-01
  -2.2525452328438485e+02  -3.7568629204411180e-01
  -2.2648122597314125e+02   1.0432721713244493e-01
  -2.2648122597314125e+02  -1.0432721713244493e-01
  -2.2704375270731214e+02   0.0000000000000000e+00
  -2.2732282813966611e+02   3.0148166821274591e-01
  -2.2732282813966611e+02  -3.0148166821274591e-01
  -2.2943126346883759e+02   0.0000000000000000e+00
  -2.2777163425428694e+02   0.0000000000000000e+00
  -2.2858142899852871e+02   0.0000000000000000e+00
  -2.2823116258563823e+02   0.0000000000000000e+00
  -2.3048574227167006e+02   6.1491252587300294e-01
  -2.3048574227167006e+02  -6.1491252587300294e-01
  -8.8932880758527676e+02   3.4308497275666578e+00
  -8.8932880758527676e+02  -3.4308497275666578e+00
  -8.8328300255947966e+02   1.9613818012457482e+00
  -8.8328300255947966e+02  -1.9613818012457482e+00
  -8.8551818650392852e+02   2.1820046607072170e+00
  -8.8551818650392852e+02  -2.1820046607072170e+00
  -8.9087823215476533e+02   9.4341337593160934e-01
  -8.9087823215476533e+02  -9.4341337593160934e-01
  -8.8438995138520738e+02   8.8780784295834514e-01
  -8.8438995138520738e+02  -8.8780784295834514e-01
  -8.8204483261389066e+02   0.0000000000000000e+00
  -8.9209677840650431e+02   0.0000000000000000e+00
  -8.9269863091211414e+02   9.4643643386715093e-01
  -8.9269863091211414e+02  -9.4643643386715093e-01
  -8.8883294199531008e+02   0.0000000000000000e+00
  -2.3135824259621552e+02   0.0000000000000000e+00
  -2.3244718024105242e+02   0.0000000000000000e+00
  -2.3212543051958451e+02   0.0000000000000000e+00
  -2.3642109792483603e+02   5.3517195913291271e-01
  -2.3642109792483603e+02  -5.3517195913291271e-01
  -2.3535092144302436e+02   6.2686186713967884e-01
  -2.3535092144302436e+02  -6.2686186713967884e-01
  -2.3452478397586245e+02   0.0000000000000000e+00
  -2.3283487310703879e+02   0.0000000000000000e+00
  -2.3369302887023960e+02   0.0000000000000000e+00
  -2.3340285812240410e+02   0.0000000000000000e+00
  -2.3530868168726261e+02   0.0000000000000000e+00
  -8.8021061816338045e+02   0.0000000000000000e+00
  -8.7917435386003717e+02   0.0000000000000000e+00
  -8.7788761769379812e+02   1.3261266591407472e+00
  -8.7788761769379812e+02  -1.3261266591407472e+00
  -8.7674544060134826e+02   1.7192841648175932e+00
  -8.7674544060134826e+02  -1.7192841648175932e+00
  -8.7625877952365408e+02   0.0000000000000000e+00
  -8.7049745912283095e+02   3.3883414852348288e+00
  -8.7049745912283095e+02  -3.3883414852348288e+00
  -8.7230323476140131e+02   1.9191581333408496e+00
  -8.7230323476140131e+02  -1.9191581333408496e+00
  -8.6873129516201834e+02   2.4214157172617474e+00
  -8.6873129516201834e+02  -2.4214157172617474e+00
  -8.7172988161111800e+02   0.0000000000000000e+00
  -8.5461899472618938e+02   9.2850442591643079e-01
  -8.5461899472618938e+02  -9.2850442591643079e-01
  -8.5680822882054827e+02   2.7210781610739025e+00
  -8.5680822882054827e+02  -2.7210781610739025e+00
  -8.6744714014736405e+02   1.1681713390118926e+00
  -8.6744714014736405e+02  -1.1681713390118926e+00
  -8.5965010109172670e+02   2.4888638965490668e+00
  -8.5965010109172670e+02  -2.4888638965490668e+00
  -8.6481743893435555e+02   0.0000000000000000e+00
  -8.7108808613051212e+02   0.0000000000000000e+00
  -8.5710001780816219e+02   9.8662109583174140e-01
  -8.5710001780816219e+02  -9.8662109583174140e-01
  -8.6998672613264171e+02   0.0000000000000000e+00
  -8.6320664268221901e+02   0.0000000000000000e+00
  -8.6186793712048507e+02   7.0699811931250678e-01
  -8.6186793712048507e+02  -7.0699811931250678e-01
  -8.5517941370648248e+02   0.0000000000000000e+00
  -8.6590669450686801e+02   0.0000000000000000e+00
  -8.6138678080178101e+02   0.0000000000000000e+00
  -2.3779590270283344e+02   0.0000000000000000e+00
  -2.3864321538245775e+02   4.2167434203290449e-01
  -2.3864321538245775e+02  -4.2167434203290449e-01
  -2.3913904711605971e+02   0.0000000000000000e+00
  -2.3832340032498627e+02   0.0000000000000000e+00
  -8.5098527728093154e+02   8.8888657497226065e-01
  -8.5098527728093154e+02  -8.8888657497226065e-01
  -8.5248801158318292e+02   4.1364490260276138e-01
  -8.5248801158318292e+02  -4.1364490260276138e-01
  -2.4008362879823662e+02   0.0000000000000000e+00
  -2.4092176649139370e+02   0.0000000000000000e+00
  -2.4140348857691637e+02   0.0000000000000000e+00
  -2.4239970382189438e+02   2.6806902251397097e-01
  -2.4239970382189438e+02  -2.6806902251397097e-01
  -2.4292004828343460e+02   0.0000000000000000e+00
  -2.4312332055735723e+02   0.0000000000000000e+00
  -2.4397638644989723e+02   1.9780426558117675e-01
  -2.4397638644989723e+02  -1.9780426558117675e-01
  -2.4426542857602712e+02   0.0000000000000000e+00
  -8.4152180565981530e+02   2.7405719594035713e+00
  -8.4152180565981530e+02  -2.7405719594035713e+00
  -8.5000072890505805e+02   0.0000000000000000e+00
  -8.3527878875160593e+02   3.4223111073701173e+00
  -8.3527878875160593e+02  -3.4223111073701173e+00
  -8.4531748937388716e+02   1.5123722185442499e+00
  -8.4531748937388716e+02  -1.5123722185442499e+00
  -8.4849338649639822e+02   1.8914259099669966e+00
  -8.4849338649639822e+02  -1.8914259099669966e+00
  -8.4514611322987025e+02   0.0000000000000000e+00
  -8.4727519036450258e+02   0.0000000000000000e+00
  -8.4054032689407654e+02   0.0000000000000000e+00
  -8.4227750132802498e+02   0.0000000000000000e+00
  -8.4098834219746163e+02   0.0000000000000000e+00
  -2.4504711103347398e+02   0.0000000000000000e+00
  -2.4585691692168990e+02   0.0000000000000000e+00
  -2.4622616773717084e+02   2.1690448524060219e-01
  -2.4622616773717084e+02  -2.1690448524060219e-01
  -2.4632674076940992e+02   0.0000000000000000e+00
  -2.4738591169386456e+02   2.4966296144013225e-01
  -2.4738591169386456e+02  -2.4966296144013225e-01
  -2.5201390435898068e+02   7.0628974066787686e-01
  -2.5201390435898068e+02  -7.0628974066787686e-01
  -2.5034077067423044e+02   6.1182646081291847e-01
  -2.5034077067423044e+02  -6.1182646081291847e-01
  -2.4845703936670208e+02   4.2842988507271901e-01
  -2.4845703936670208e+02  -4.2842988507271901e-01
  -2.5027998446636749e+02   0.0000000000000000e+00
  -2.5260941069018736e+02   0.0000000000000000e+00
  -2.4870394805306069e+02   0.0000000000000000e+00
  -8.3703464155043673e+02   2.0084226418418960e+00
  -8.3703464155043673e+02  -2.0084226418418960e+00
  -8.3761961013748453e+02   0.0000000000000000e+00
  -8.3608273858197504e+02   1.0030849171539999e+00
  -8.3608273858197504e+02  -1.0030849171539999e+00
  -8.3246846217833593e+02   0.0000000000000000e+00
  -8.3197294345361865e+02   2.4706873967060119e+00
  -8.3197294345361865e+02  -2.4706873967060119e+00
  -8.3416376022588247e+02   7.8038946920057761e-01
  -8.3416376022588247e+02  -7.8038946920057761e-01
  -8.2979558361200441e+02   0.0000000000000000e+00
  -8.1294779375969813e+02   2.1346016211799816e+00
  -8.1294779375969813e+02  -2.1346016211799816e+00
  -8.2438180986212785e+02   3.3259121422003814e+00
  -8.2438180986212785e+02  -3.3259121422003814e+00
  -8.2872067096498290e+02   0.0000000000000000e+00
  -8.1459386657884113e+02   2.3983020225938225e+00
  -8.1459386657884113e+02  -2.3983020225938225e+00
  -8.2651220627828775e+02   1.3279833446860791e+00
  -8.2651220627828775e+02  -1.3279833446860791e+00
  -8.1899424342949419e+02   2.4363654938139119e+00
  -8.1899424342949419e+02  -2.4363654938139119e+00
  -8.2713171080429345e+02   4.7556380759370159e-01
  -8.2713171080429345e+02  -4.7556380759370159e-01
  -8.2500204359055749e+02   0.0000000000000000e+00
  -8.2659311752000553e+02   0.0000000000000000e+00
  -8.2215040447146828e+02   0.0000000000000000e+00
  -8.1457420415175625e+02   2.2451075123588513e-01
  -8.1457420415175625e+02  -2.2451075123588513e-01
  -8.1862664700587220e+02   1.0314890702898964e+00
  -8.1862664700587220e+02  -1.0314890702898964e+00
  -8.2359696904202906e+02   0.0000000000000000e+00
  -8.1573897971455676e+02   0.0000000000000000e+00
  -8.1924667491602747e+02   0.0000000000000000e+00
  -2.5362072982351083e+02   0.0000000000000000e+00
  -2.5462213742734167e+02   3.3811668415059265e-01
  -2.5462213742734167e+02  -3.3811668415059265e-01
  -8.1038580365473979e+02   2.8638612918570758e+00
  -8.1038580365473979e+02  -2.8638612918570758e+00
  -8.1142753915426283e+02   0.0000000000000000e+00
  -8.1249189976978653e+02   0.0000000000000000e+00
  -2.5563612447980606e+02   3.6259022660476620e-01
  -2.5563612447980606e+02  -3.6259022660476620e-01
  -2.5494182747475190e+02   0.0000000000000000e+00
  -2.5702295611799298e+02   8.4935273628759667e-01
  -2.5702295611799298e+02  -8.4935273628759667e-01
  -2.5643325471293815e+02   0.0000000000000000e+00
  -2.5806403935602941e+02   1.6955988885902420e-01
  -2.5806403935602941e+02  -1.6955988885902420e-01
  -2.5990501164971403e+02   3.2378921482503609e-01
  -2.5990501164971403e+02  -3.2378921482503609e-01
  -2.5904904328242702e+02   1.2168684256222317e-01
  -2.5904904328242702e+02  -1.2168684256222317e-01
  -8.0147921520500313e+02   4.5373789239998823e+00
  -8.0147921520500313e+02  -4.5373789239998823e+00
  -7.9944199490475842e+02   2.7424806465307285e+00
  -7.9944199490475842e+02  -2.7424806465307285e+00
  -8.0927824965675416e+02   0.0000000000000000e+00
  -8.0560226544523380e+02   0.0000000000000000e+00
  -8.0826657913365887e+02   0.0000000000000000e+00
  -8.0748057744430275e+02   0.0000000000000000e+00
  -7.9942378374109092e+02   9.2787176367735114e-01
  -7.9942378374109092e+02  -9.2787176367735114e-01
  -8.0249927184697492e+02   0.0000000000000000e+00
  -8.0165275190445948e+02   0.0000000000000000e+00
  -8.0419639839870672e+02   0.0000000000000000e+00
  -2.6082312495500167e+02   0.0000000000000000e+00
  -2.6157722596118208e+02   0.0000000000000000e+00
  -2.6223451509988013e+02   0.0000000000000000e+00
  -2.6265667958875662e+02   7.0371170150867224e-01
  -2.6265667958875662e+02  -7.0371170150867224e-01
  -2.6829448999038834e+02   1.4726533462754374e-01
  -2.6829448999038834e+02  -1.4726533462754374e-01
  -2.6317260366878850e+02   0.0000000000000000e+00
  -2.6724569243549405e+02   0.0000000000000000e+00
  -2.6667368556740189e+02   0.0000000000000000e+00
  -2.6364274625633811e+02   0.0000000000000000e+00
  -2.6589198997104813e+02   9.3056854067785799e-02
  -2.6589198997104813e+02  -9.3056854067785799e-02
  -2.6524328480515567e+02   0.0000000000000000e+00
  -2.6473743915651153e+02   0.0000000000000000e+00
  -2.6564204060439243e+02   0.0000000000000000e+00
  -2.6405921403401271e+02   0.0000000000000000e+00
  -2.6436558837116047e+02   2.9467905480658990e-01
  -2.6436558837116047e+02  -2.9467905480658990e-01
  -7.9738676803768749e+02   1.5692240235488883e+00
  -7.9738676803768749e+02  -1.5692240235488883e+00
  -7.9537400596466944e+02   0.0000000000000000e+00
  -7.9585404810351713e+02   7.8367443519947111e-01
  -7.9585404810351713e+02  -7.8367443519947111e-01
  -7.9336989625104479e+02   8.2565043562584950e-01
  -7.9336989625104479e+02  -8.2565043562584950e-01
  -7.9231090885380195e+02   7.8962441454239241e-01
  -7.9231090885380195e+02  -7.8962441454239241e-01
  -7.9044539079464721e+02   7.0782043132315497e-01
  -7.9044539079464721e+02  -7.0782043132315497e-01
  -7.9039812819050508e+02   0.0000000000000000e+00
  -7.7659758881514449e+02   3.3611957149702518e+00
  -7.7659758881514449e+02  -3.3611957149702518e+00
  -7.8803169026695878e+02   3.4702911692911026e-01
  -7.8803169026695878e+02  -3.4702911692911026e-01
  -7.8207066547574107e+02   3.2716988631874440e+00
  -7.8207066547574107e+02  -3.2716988631874440e+00
  -7.8688693925261146e+02   0.0000000000000000e+00
  -7.8500828257484864e+02   1.0967531878758030e+00
  -7.8500828257484864e+02  -1.0967531878758030e+00
  -7.7618818529444025e+02   8.3902744203003909e-01
  -7.7618818529444025e+02  -8.3902744203003909e-01
  -7.7784368239226364e+02   6.4878005515186121e-01
  -7.7784368239226364e+02  -6.4878005515186121e-01
  -7.8090877891400146e+02   1.3883691184412044e+00
  -7.8090877891400146e+02  -1.3883691184412044e+00
  -7.8217963145684666e+02   0.0000000000000000e+00
  -7.8090423431310580e+02   0.0000000000000000e+00
  -7.8195887697950263e+02   0.0000000000000000e+00
  -7.8050983751547210e+02   0.0000000000000000e+00
  -2.7022704114759347e+02   5.2056654684652381e-01
  -2.7022704114759347e+02  -5.2056654684652381e-01
  -2.7037355537956057e+02   0.0000000000000000e+00
  -7.7263018426053577e+02   1.6409141016530717e+00
  -7.7263018426053577e+02  -1.6409141016530717e+00
  -7.7568449627924042e+02   0.0000000000000000e+00
  -7.7459610479861783e+02   0.0000000000000000e+00
  -2.7074175934580899e+02   0.0000000000000000e+00
  -2.7166324660614572e+02   1.2189456374808501e-01
  -2.7166324660614572e+02  -1.2189456374808501e-01
  -2.7237233005009637e+02   0.0000000000000000e+00
  -2.7332021902985599e+02   1.1994776891011977e-01
  -2.7332021902985599e+02  -1.1994776891011977e-01
  -2.7435642447428199e+02   0.0000000000000000e+00
  -2.7509887693835458e+02   0.0000000000000000e+00
  -2.7624364785069827e+02   4.9246899520586235e-01
  -2.7624364785069827e+02  -4.9246899520586235e-01
  -2.7558318629578696e+02   4.5167236907973224e-01
  -2.7558318629578696e+02  -4.5167236907973224e-01
  -7.7037695092703348e+02   2.1310250726541247e+00
  -7.7037695092703348e+02  -2.1310250726541247e+00
  -7.6527557951396352e+02   1.2513508228519479e+00
  -7.6527557951396352e+02  -1.2513508228519479e+00
  -7.6898980626321190e+02   5.0560790028187363e-01
  -7.6898980626321190e+02  -5.0560790028187363e-01
  -7.6973385061348006e+02   0.0000000000000000e+00
  -2.7575221971424492e+02   0.0000000000000000e+00
  -2.7754491948739712e+02   0.0000000000000000e+00
  -2.7649019394275081e+02   0.0000000000000000e+00
  -2.7894992600572499e+02   0.0000000000000000e+00
  -2.7961889802180480e+02   6.3263535211001021e-01
  -2.7961889802180480e+02  -6.3263535211001021e-01
  -2.8383194457813943e+02   0.0000000000000000e+00
  -2.7967465279007882e+02   0.0000000000000000e+00
  -2.8155560988349657e+02   8.7206545732921459e-01
  -2.8155560988349657e+02  -8.7206545732921459e-01
  -2.8262161076087830e+02   9.2814596560372387e-01
  -2.8262161076087830e+02  -9.2814596560372387e-01
  -2.8038306306220102e+02   0.0000000000000000e+00
  -2.8293200574805383e+02   0.0000000000000000e+00
  -2.8137489734035103e+02   0.0000000000000000e+00
  -7.6579025953636392e+02   0.0000000000000000e+00
  -7.6484979877263470e+02   0.0000000000000000e+00
  -7.6085887645852529e+02   2.2644313479883147e+00
  -7.6085887645852529e+02  -2.2644313479883147e+00
  -7.6341769742913459e+02   0.0000000000000000e+00
  -7.6235309526984088e+02   5.3380120114318785e-01
  -7.6235309526984088e+02  -5.3380120114318785e-01
  -7.6119145365947600e+02   0.0000000000000000e+00
  -7.4820470837743653e+02   5.4709739874857872e+00
  -7.4820470837743653e+02  -5.4709739874857872e+00
  -7.5736985401352808e+02   2.5460441671853582e+00
  -7.5736985401352808e+02  -2.5460441671853582e+00
  -7.5906036014199913e+02   1.5011143418132529e+00
  -7.5906036014199913e+02  -1.5011143418132529e+00
  -7.5945541829945273e+02   0.0000000000000000e+00
  -7.5605905856395736e+02   1.0863614546409985e+00
  -7.5605905856395736e+02  -1.0863614546409985e+00
  -7.5407893306333028e+02   0.0000000000000000e+00
  -7.5258477367925047e+02   1.1156714991421717e+00
  -7.5258477367925047e+02  -1.1156714991421717e+00
  -7.5084039656007030e+02   2.1506665336523150e+00
  -7.5084039656007030e+02  -2.1506665336523150e+00
  -7.4518331679522373e+02   1.1192089523172575e+00
  -7.4518331679522373e+02  -1.1192089523172575e+00
  -7.4600037504407896e+02   1.4903053405616238e+00
  -7.4600037504407896e+02  -1.4903053405616238e+00
  -7.5144639525109255e+02   0.0000000000000000e+00
  -7.4969789980158180e+02   1.0706867621960710e+00
  -7.4969789980158180e+02  -1.0706867621960710e+00
  -7.4678767080215425e+02   1.0203326685727032e+00
  -7.4678767080215425e+02  -1.0203326685727032e+00
  -2.8538761216855312e+02   3.1540817628874862e-01
  -2.8538761216855312e+02  -3.1540817628874862e-01
  -2.8659714398024948e+02   0.0000000000000000e+00
  -2.8494510372598228e+02   0.0000000000000000e+00
  -7.4255274962347107e+02   1.1810729211757713e+00
  -7.4255274962347107e+02  -1.1810729211757713e+00
  -7.4346508276020631e+02   0.0000000000000000e+00
  -2.8815243370413521e+02   1.1714805535992809e+00
  -2.8815243370413521e+02  -1.1714805535992809e+00
  -2.8731377701309282e+02   0.0000000000000000e+00
  -2.8809528741805309e+02   0.0000000000000000e+00
  -2.8905694125777819e+02   0.0000000000000000e+00
  -2.8988520288651341e+02   2.8088931682407753e-01
  -2.8988520288651341e+02  -2.8088931682407753e-01
  -7.3002456727632284e+02   1.5770716675611072e+00
  -7.3002456727632284e+02  -1.5770716675611072e+00
  -7.3807274658893095e+02   2.6838557154631655e+00
  -7.3807274658893095e+02  -2.6838557154631655e+00
  -7.3265554802711711e+02   1.9409768770294833e+00
  -7.3265554802711711e+02  -1.9409768770294833e+00
  -7.3638447873745690e+02   1.3369562903160088e+00
  -7.3638447873745690e+02  -1.3369562903160088e+00
  -7.3463157103490573e+02   1.0697277076982485e+00
  -7.3463157103490573e+02  -1.0697277076982485e+00
  -7.4116040394887307e+02   6.2156146035398263e-01
  -7.4116040394887307e+02  -6.2156146035398263e-01
  -7.3315440981887343e+02   5.0070118580362610e-01
  -7.3315440981887343e+02  -5.0070118580362610e-01
  -7.3723054036528822e+02   0.0000000000000000e+00
  -7.3822497819545663e+02   0.0000000000000000e+00
  -2.9181842457009816e+02   0.0000000000000000e+00
  -2.9245599905217091e+02   9.7111505973478562e-02
  -2.9245599905217091e+02  -9.7111505973478562e-02
  -2.9285651080453920e+02   0.0000000000000000e+00
  -2.9375231339505257e+02   1.7945238728626875e-01
  -2.9375231339505257e+02  -1.7945238728626875e-01
  -2.9831628842129339e+02   7.3589245980736695e-01
  -2.9831628842129339e+02  -7.3589245980736695e-01
  -2.9497975576195500e+02   0.0000000000000000e+00
  -2.9528726685554415e+02   0.0000000000000000e+00
  -2.9628560209385728e+02   5.2127452498976901e-01
  -2.9628560209385728e+02  -5.2127452498976901e-01
  -2.9556750854019367e+02   0.0000000000000000e+00
  -2.9740970630543450e+02   0.0000000000000000e+00
  -2.9656098356803568e+02   0.0000000000000000e+00
  -2.9781677029087530e+02   0.0000000000000000e+00
  -7.3185346088991935e+02   0.0000000000000000e+00
  -7.2715978161177532e+02   2.5121058496816522e+00
  -7.2715978161177532e+02  -2.5121058496816522e+00
  -7.2836871313799350e+02   0.0000000000000000e+00
  -7.2711492279368565e+02   0.0000000000000000e+00
  -7.2646244624221015e+02   0.0000000000000000e+00
  -7.2285990505115819e+02   2.3329007548627572e+00
  -7.2285990505115819e+02  -2.3329007548627572e+00
  -7.2471477540346564e+02   4.7459833418683128e-01
  -7.2471477540346564e+02  -4.7459833418683128e-01
  -7.2220908569719245e+02   2.0654924184360564e+00
  -7.2220908569719245e+02  -2.0654924184360564e+00
  -7.2198360222572717e+02   0.0000000000000000e+00
  -7.1467559543774814e+02   2.9619431843065880e+00
  -7.1467559543774814e+02  -2.9619431843065880e+00
  -7.2120789637882785e+02   0.0000000000000000e+00
  -7.1902969241582434e+02   1.3831241261129246e+00
  -7.1902969241582434e+02  -1.3831241261129246e+00
  -7.2005950746249812e+02   0.0000000000000000e+00
  -7.1674695916569522e+02   1.2512458190162095e+00
  -7.1674695916569522e+02  -1.2512458190162095e+00
  -7.1249582838174081e+02   1.9168053185915377e+00
  -7.1249582838174081e+02  -1.9168053185915377e+00
  -7.1741278612237295e+02   0.0000000000000000e+00
  -7.1516972842054429e+02   0.0000000000000000e+00
  -7.1341173757262152e+02   0.0000000000000000e+00
  -7.1246957454277822e+02   4.2234602918883846e-01
  -7.1246957454277822e+02  -4.2234602918883846e-01
  -7.1135179924883130e+02   0.0000000000000000e+00
  -2.9999010681532832e+02   0.0000000000000000e+00
  -3.0054792698319295e+02   4.3369971565055609e-01
  -3.0054792698319295e+02  -4.3369971565055609e-01
  -7.0358319535412215e+02   4.2039014555105290e+00
  -7.0358319535412215e+02  -4.2039014555105290e+00
  -7.0599777414028335e+02   4.2807733777903667e-01
  -7.0599777414028335e+02  -4.2807733777903667e-01
  -7.0837346185472666e+02   7.6443877740298249e-01
  -7.0837346185472666e+02  -7.6443877740298249e-01
  -7.1012836871798606e+02   0.0000000000000000e+00
  -3.0235438708491142e+02   6.3353222871218018e-01
  -3.0235438708491142e+02  -6.3353222871218018e-01
  -3.0189284113278615e+02   0.0000000000000000e+00
  -3.0305194997160010e+02   0.0000000000000000e+00
  -3.0403108642675494e+02   6.9605117583491105e-01
  -3.0403108642675494e+02  -6.9605117583491105e-01
  -3.0407035921667483e+02   0.0000000000000000e+00
  -3.0537312660805253e+02   5.6134326015427360e-01
  -3.0537312660805253e+02  -5.6134326015427360e-01
  -3.0620377134676448e+02   7.7369203030136791e-01
  -3.0620377134676448e+02  -7.7369203030136791e-01
  -3.0578052233486494e+02   0.0000000000000000e+00
  -7.0197772999776942e+02   3.5688036394155684e+00
  -7.0197772999776942e+02  -3.5688036394155684e+00
  -6.9868130942415723e+02   2.3335784512598599e+00
  -6.9868130942415723e+02  -2.3335784512598599e+00
  -7.0382091717593028e+02   0.0000000000000000e+00
  -6.9845096985911312e+02   0.0000000000000000e+00
  -7.0264011433260146e+02   0.0000000000000000e+00
  -6.9982046558154605e+02   1.0232082777956750e+00
  -6.9982046558154605e+02  -1.0232082777956750e+00
  -7.0295248172232834e+02   0.0000000000000000e+00
  -7.0970476497414552e+02   0.0000000000000000e+00
  -7.0033657794531291e+02   0.0000000000000000e+00
  -3.0767414558334264e+02   7.8383490170242054e-01
  -3.0767414558334264e+02  -7.8383490170242054e-01
  -3.1438323877565642e+02   1.3414695717070180e+00
  -3.1438323877565642e+02  -1.3414695717070180e+00
  -3.0832376631124123e+02   0.0000000000000000e+00
  -3.0907112019480076e+02   5.7839948287576826e-01
  -3.0907112019480076e+02  -5.7839948287576826e-01
  -3.0936452138967616e+02   3.2599398247734884e-01
  -3.0936452138967616e+02  -3.2599398247734884e-01
  -3.1044942913227840e+02   4.0753374437153983e-01
  -3.1044942913227840e+02  -4.0753374437153983e-01
  -3.1178931970511212e+02   2.3561434215246890e-01
  -3.1178931970511212e+02  -2.3561434215246890e-01
  -3.1291404579454206e+02   0.0000000000000000e+00
  -3.1254391028949851e+02   0.0000000000000000e+00
  -3.1353065218606815e+02   0.0000000000000000e+00
  -6.9297011520156047e+02   3.6720924223947451e+00
  -6.9297011520156047e+02  -3.6720924223947451e+00
  -6.9513584836358132e+02   2.0392642586600322e+00
  -6.9513584836358132e+02  -2.0392642586600322e+00
  -6.9577612137357426e+02   0.0000000000000000e+00
  -6.9507231030980552e+02   0.0000000000000000e+00
  -6.9114814735959726e+02   2.3070595070084972e+00
  -6.9114814735959726e+02  -2.3070595070084972e+00
  -6.9152653360305624e+02   0.0000000000000000e+00
  -6.7843464020038732e+02   1.6875301906215709e+00
  -6.7843464020038732e+02  -1.6875301906215709e+00
  -6.9135936627049546e+02   4.3462568757489461e-01
  -6.9135936627049546e+02  -4.3462568757489461e-01
  -6.7782671529828929e+02   0.0000000000000000e+00
  -6.8665882723468690e+02   2.3050683487895229e+00
  -6.8665882723468690e+02  -2.3050683487895229e+00
  -6.8996084142565337e+02   0.0000000000000000e+00
  -6.8514190610726723e+02   2.2312892323920317e+00
  -6.8514190610726723e+02  -2.2312892323920317e+00
  -6.8864846882100176e+02   6.1229515366499720e-01
  -6.8864846882100176e+02  -6.1229515366499720e-01
  -6.7966748002575810e+02   0.0000000000000000e+00
  -6.8667825111639934e+02   0.0000000000000000e+00
  -6.8528325806971327e+02   0.0000000000000000e+00
  -6.8139184548207174e+02   0.0000000000000000e+00
  -6.8618503477365925e+02   0.0000000000000000e+00
  -6.8363771520233649e+02   4.5874213444254042e-01
  -6.8363771520233649e+02  -4.5874213444254042e-01
  -6.8235300381763113e+02   0.0000000000000000e+00
  -3.1592528933708013e+02   1.0664231978684287e+00
  -3.1592528933708013e+02  -1.0664231978684287e+00
  -6.7566191164000793e+02   2.8655194848744081e+00
  -6.7566191164000793e+02  -2.8655194848744081e+00
  -6.7619313153704570e+02   0.0000000000000000e+00
  -6.7558024789989815e+02   0.0000000000000000e+00
  -3.1595582815036619e+02   0.0000000000000000e+00
  -3.1738587744732422e+02   3.5114754582987040e-01
  -3.1738587744732422e+02  -3.5114754582987040e-01
  -3.1683098605462988e+02   1.1143699622639369e-01
  -3.1683098605462988e+02  -1.1143699622639369e-01
  -3.1887154299339386e+02   6.1649696850292790e-01
  -3.1887154299339386e+02  -6.1649696850292790e-01
  -3.1965056216871767e+02   0.0000000000000000e+00
  -3.2075320084616152e+02   0.0000000000000000e+00
  -6.7022216580384861e+02   4.9448595607368064e+00
  -6.7022216580384861e+02  -4.9448595607368064e+00
  -6.7385473088843332e+02   1.1228445731149104e+00
  -6.7385473088843332e+02  -1.1228445731149104e+00
  -6.6795613180804730e+02   3.6433536609721873e-01
  -6.6795613180804730e+02  -3.6433536609721873e-01
  -6.6546419122699672e+02   1.0921550412711243e+00
  -6.6546419122699672e+02  -1.0921550412711243e+00
  -6.6730759344032947e+02   0.0000000000000000e+00
  -6.7468274595207674e+02   5.5807969296574611e-01
  -6.7468274595207674e+02  -5.5807969296574611e-01
  -6.7010730188607772e+02   0.0000000000000000e+00
  -6.7009698178634881e+02   4.1146275389643910e-01
  -6.7009698178634881e+02  -4.1146275389643910e-01
  -3.2036690075187653e+02   0.0000000000000000e+00
  -3.2196937114678940e+02   5.1970953946035114e-01
  -3.2196937114678940e+02  -5.1970953946035114e-01
  -3.2179510842417966e+02   0.0000000000000000e+00
  -3.2277810397260970e+02   2.7432760860772792e-01
  -3.2277810397260970e+02  -2.7432760860772792e-01
  -3.2881619664135997e+02   7.0483517194079637e-01
  -3.2881619664135997e+02  -7.0483517194079637e-01
  -3.2665507690238667e+02   1.0931875009462719e+00
  -3.2665507690238667e+02  -1.0931875009462719e+00
  -3.2810475910964072e+02   5.1412773400847189e-01
  -3.2810475910964072e+02  -5.1412773400847189e-01
  -3.2811117822295711e+02   0.0000000000000000e+00
  -3.2370690979482833e+02   3.7295494938965251e-01
  -3.2370690979482833e+02  -3.7295494938965251e-01
  -3.2610255769682419e+02   0.0000000000000000e+00
  -3.2644268494139465e+02   0.0000000000000000e+00
  -3.2439987327623646e+02   0.0000000000000000e+00
  -3.2396871918701260e+02   0.0000000000000000e+00
  -3.2544292159533279e+02   0.0000000000000000e+00
  -6.6557162292261307e+02   0.0000000000000000e+00
  -6.5609353665297954e+02   4.6606507294167452e+00
  -6.5609353665297954e+02  -4.6606507294167452e+00
  -6.6342685047728651e+02   1.0852008641526758e+00
  -6.6342685047728651e+02  -1.0852008641526758e+00
  -6.6368573372060803e+02   0.0000000000000000e+00
  -6.5879745383603120e+02   2.5439277657218793e+00
  -6.5879745383603120e+02  -2.5439277657218793e+00
  -6.4913402712043660e+02   1.7288423982010410e+00
  -6.4913402712043660e+02  -1.7288423982010410e+00
  -6.5945870482313194e+02   1.6598162870202122e+00
  -6.5945870482313194e+02  -1.6598162870202122e+00
  -6.6039399713528871e+02   0.0000000000000000e+00
  -6.5862033858124823e+02   0.0000000000000000e+00
  -6.5787602431018536e+02   0.0000000000000000e+00
  -6.5527764497768567e+02   1.0506897130038682e+00
  -6.5527764497768567e+02  -1.0506897130038682e+00
  -6.5265837518200942e+02   4.5103682729144301e-01
  -6.5265837518200942e+02  -4.5103682729144301e-01
  -6.5628487195027935e+02   0.0000000000000000e+00
  -6.5193590575316898e+02   4.8259861494142664e-01
  -6.5193590575316898e+02  -4.8259861494142664e-01
  -6.5435848294234302e+02   0.0000000000000000e+00
  -6.4587667447139779e+02   3.2918524065486188e+00
  -6.4587667447139779e+02  -3.2918524065486188e+00
  -6.4654985678075604e+02   1.9574721101192605e+00
  -6.4654985678075604e+02  -1.9574721101192605e+00
  -6.5065650990544486e+02   0.0000000000000000e+00
  -3.3145162956133481e+02   7.3316432618958893e-01
  -3.3145162956133481e+02  -7.3316432618958893e-01
  -3.3299865479918378e+02   5.3517105462501313e-01
  -3.3299865479918378e+02  -5.3517105462501313e-01
  -3.3084697583672028e+02   6.4217707983325745e-01
  -3.3084697583672028e+02  -6.4217707983325745e-01
  -3.3042677604462108e+02   3.0612954130524211e-01
  -3.3042677604462108e+02  -3.0612954130524211e-01
  -3.3224655635145348e+02   3.4372659711301257e-01
  -3.3224655635145348e+02  -3.4372659711301257e-01
  -6.4293887303690167e+02   2.4183047746341608e+00
  -6.4293887303690167e+02  -2.4183047746341608e+00
  -6.4704652692844002e+02   0.0000000000000000e+00
  -6.4839411711929233e+02   0.0000000000000000e+00
  -3.3449765138977114e+02   1.9211889943373212e-01
  -3.3449765138977114e+02  -1.9211889943373212e-01
  -3.3812769551442312e+02   9.0976330856669785e-01
  -3.3812769551442312e+02  -9.0976330856669785e-01
  -3.3631734177317367e+02   7.3450164266999562e-01
  -3.3631734177317367e+02  -7.3450164266999562e-01
  -3.3529344644335788e+02   0.0000000000000000e+00
  -3.3632182737604148e+02   0.0000000000000000e+00
  -6.3850977178585288e+02   3.6735732549595181e+00
  -6.3850977178585288e+02  -3.6735732549595181e+00
  -6.4227484907052371e+02   1.6495562910819903e+00
  -6.4227484907052371e+02  -1.6495562910819903e+00
  -6.4355877653860341e+02   0.0000000000000000e+00
  -6.3846712410131568e+02   3.6429557027876042e-01
  -6.3846712410131568e+02  -3.6429557027876042e-01
  -6.3918515844699721e+02   0.0000000000000000e+00
  -6.4096933550201857e+02   9.8154874536556791e-01
  -6.4096933550201857e+02  -9.8154874536556791e-01
  -6.4192617131987367e+02   0.0000000000000000e+00
  -3.3894139370993071e+02   1.4076105756651760e+00
  -3.3894139370993071e+02  -1.4076105756651760e+00
  -3.4000198387558055e+02   1.2976847518360850e+00
  -3.4000198387558055e+02  -1.2976847518360850e+00
  -3.3905107106371969e+02   0.0000000000000000e+00
  -3.4261152943608340e+02   1.7372829732173631e-01
  -3.4261152943608340e+02  -1.7372829732173631e-01
  -3.3971031866015767e+02   0.0000000000000000e+00
  -6.3290657659406406e+02   3.0035870428648974e+00
  -6.3290657659406406e+02  -3.0035870428648974e+00
  -6.3508282660837517e+02   9.9159641547107624e-01
  -6.3508282660837517e+02  -9.9159641547107624e-01
  -6.3641243875640578e+02   0.0000000000000000e+00
  -6.3279322048968254e+02   1.5054082437720853e+00
  -6.3279322048968254e+02  -1.5054082437720853e+00
  -6.3419099364953524e+02   0.0000000000000000e+00
  -6.2176244270876350e+02   4.4461838690675890e+00
  -6.2176244270876350e+02  -4.4461838690675890e+00
  -6.3199270222868449e+02   0.0000000000000000e+00
  -6.3025316495574907e+02   7.0935970996409037e-01
  -6.3025316495574907e+02  -7.0935970996409037e-01
  -6.2676315187133298e+02   2.0845810623450740e+00
  -6.2676315187133298e+02  -2.0845810623450740e+00
  -6.2867609010121305e+02   1.4397422347967601e+00
  -6.2867609010121305e+02  -1.4397422347967601e+00
  -6.2907358800559575e+02   0.0000000000000000e+00
  -6.2196059715166984e+02   4.8815865461505425e-01
  -6.2196059715166984e+02  -4.8815865461505425e-01
  -6.2668053213105861e+02   0.0000000000000000e+00
  -6.2746482634621725e+02   0.0000000000000000e+00
  -6.2551622673790757e+02   2.9332329488253950e-01
  -6.2551622673790757e+02  -2.9332329488253950e-01
  -6.2377697425706071e+02   0.0000000000000000e+00
  -6.2350220452477583e+02   0.0000000000000000e+00
  -3.4465975411531770e+02   7.7402013153125526e-01
  -3.4465975411531770e+02  -7.7402013153125526e-01
  -3.4368040167453671e+02   0.0000000000000000e+00
  -3.4333539200037660e+02   0.0000000000000000e+00
  -6.1868386879419768e+02   2.1907527276947665e+00
  -6.1868386879419768e+02  -2.1907527276947665e+00
  -6.2057137887995214e+02   0.0000000000000000e+00
  -3.4427487300891096e+02   0.0000000000000000e+00
  -3.4586325271451574e+02   0.0000000000000000e+00
  -3.4621307578909551e+02   0.0000000000000000e+00
  -3.4665000317982407e+02   0.0000000000000000e+00
  -3.5002319439540184e+02   0.0000000000000000e+00
  -3.4834676725986822e+02   5.7535570212288678e-01
  -3.4834676725986822e+02  -5.7535570212288678e-01
  -3.4878408967153314e+02   0.0000000000000000e+00
  -3.4768490108802899e+02   0.0000000000000000e+00
  -6.1130000241836387e+02   2.5544799116946222e+00
  -6.1130000241836387e+02  -2.5544799116946222e+00
  -6.1798326156958842e+02   6.2859569606184662e-01
  -6.1798326156958842e+02  -6.2859569606184662e-01
  -6.1671931335914962e+02   6.2321581232914591e-01
  -6.1671931335914962e+02  -6.2321581232914591e-01
  -6.1340241179043926e+02   1.3225548272415246e+00
  -6.1340241179043926e+02  -1.3225548272415246e+00
  -6.1394498722236267e+02   8.5766905423834661e-01
  -6.1394498722236267e+02  -8.5766905423834661e-01
  -6.1359232677890202e+02   0.0000000000000000e+00
  -3.4710394397100379e+02   0.0000000000000000e+00
  -3.5554661903548327e+02   3.6686225082294097e+00
  -3.5554661903548327e+02  -3.6686225082294097e+00
  -3.5071187804116920e+02   2.3659068485301510e-01
  -3.5071187804116920e+02  -2.3659068485301510e-01
  -3.4752879896047301e+02   0.0000000000000000e+00
  -3.5203676887846404e+02   4.2207615609588434e-01
  -3.5203676887846404e+02  -4.2207615609588434e-01
  -3.5286213304631241e+02   7.2608802686554508e-01
  -3.5286213304631241e+02  -7.2608802686554508e-01
  -3.5232567669961378e+02   0.0000000000000000e+00
  -3.5324164586748185e+02   0.0000000000000000e+00
  -3.5495699004373660e+02   0.0000000000000000e+00
  -3.5826515623728346e+02   3.7055086069271931e-01
  -3.5826515623728346e+02  -3.7055086069271931e-01
  -3.5553425921147419e+02   7.9524720053158426e-01
  -3.5553425921147419e+02  -7.9524720053158426e-01
  -3.5629207787809327e+02   0.0000000000000000e+00
  -3.5787051786564541e+02   1.3892286164205511e-01
  -3.5787051786564541e+02  -1.3892286164205511e-01
  -3.5578279238845579e+02   0.0000000000000000e+00
  -6.0728252476359989e+02   4.0802647440919868e+00
  -6.0728252476359989e+02  -4.0802647440919868e+00
  -5.9895159134189316e+02   5.6729223689454811e+00
  -5.9895159134189316e+02  -5.6729223689454811e+00
  -6.1189087202971393e+02   0.0000000000000000e+00
  -6.1069319155493963e+02   0.0000000000000000e+00
  -6.0912843741368897e+02   9.9595838639356460e-01
  -6.0912843741368897e+02  -9.9595838639356460e-01
  -6.0846968838398311e+02   0.0000000000000000e+00
  -5.9587090724715972e+02   2.7795791752213810e+00
  -5.9587090724715972e+02  -2.7795791752213810e+00
  -6.0823847161377216e+02   9.8031481907275553e-01
  -6.0823847161377216e+02  -9.8031481907275553e-01
  -6.0663310823904669e+02   3.1836839385262533e-01
  -6.0663310823904669e+02  -3.1836839385262533e-01
  -5.9610516150822752e+02   0.0000000000000000e+00
  -6.0569025738068353e+02   0.0000000000000000e+00
  -5.9963708693058425e+02   2.3435739774707902e+00
  -5.9963708693058425e+02  -2.3435739774707902e+00
  -6.0271532938412724e+02   1.5741903602425416e+00
  -6.0271532938412724e+02  -1.5741903602425416e+00
  -5.9885784247186268e+02   8.8484961940420048e-01
  -5.9885784247186268e+02  -8.8484961940420048e-01
  -6.0281553376274428e+02   9.4538254749503364e-02
  -6.0281553376274428e+02  -9.4538254749503364e-02
  -6.0129734482639628e+02   9.3575533998213653e-02
  -6.0129734482639628e+02  -9.3575533998213653e-02
  -3.5959037430581378e+02   0.0000000000000000e+00
  -5.9652348763486043e+02   7.0091076773607675e-01
  -5.9652348763486043e+02  -7.0091076773607675e-01
  -3.6142377400868719e+02   8.1044399802117773e-01
  -3.6142377400868719e+02  -8.1044399802117773e-01
  -3.6046131984265372e+02   0.0000000000000000e+00
  -3.6071285523300566e+02   0.0000000000000000e+00
  -3.6458320146300343e+02   1.2585082375462704e+00
  -3.6458320146300343e+02  -1.2585082375462704e+00
  -3.6157240803541089e+02   0.0000000000000000e+00
  -3.6298091965281003e+02   3.4494501473538058e-01
  -3.6298091965281003e+02  -3.4494501473538058e-01
  -3.6217776929781388e+02   0.0000000000000000e+00
  -5.9299090792722041e+02   2.0293227303036421e+00
  -5.9299090792722041e+02  -2.0293227303036421e+00
  -5.9366691305486052e+02   0.0000000000000000e+00
  -5.9212260663279983e+02   0.0000000000000000e+00
  -5.9077413357807222e+02   0.0000000000000000e+00
  -5.8963015110014885e+02   0.0000000000000000e+00
  -5.8949885525113791e+02   0.0000000000000000e+00
  -5.9501941629428427e+02   0.0000000000000000e+00
  -5.8863415687381314e+02   0.0000000000000000e+00
  -5.8720083993331832e+02   1.5827177371828624e-01
  -5.8720083993331832e+02  -1.5827177371828624e-01
  -5.8559343849456627e+02   1.8350807454749207e+00
  -5.8559343849456627e+02  -1.8350807454749207e+00
  -5.8192411464678912e+02   3.5384057530517654e+00
  -5.8192411464678912e+02  -3.5384057530517654e+00
  -5.8611255794565022e+02   0.0000000000000000e+00
  -3.6411490353826412e+02   0.0000000000000000e+00
  -3.6583732590236065e+02   9.8562811276259188e-01
  -3.6583732590236065e+02  -9.8562811276259188e-01
  -3.6484485846880580e+02   0.0000000000000000e+00
  -5.7617064171490574e+02   2.1790652080576467e+00
  -5.7617064171490574e+02  -2.1790652080576467e+00
  -3.6544923026596069e+02   0.0000000000000000e+00
  -5.8456059093622025e+02   0.0000000000000000e+00
  -3.6640218051067683e+02   0.0000000000000000e+00
  -5.7922767175202137e+02   2.8754490109419537e+00
  -5.7922767175202137e+02  -2.8754490109419537e+00
  -3.6844980227844081e+02   1.2170684901534690e+00
  -3.6844980227844081e+02  -1.2170684901534690e+00
  -3.6725576482095551e+02   2.8738269431789693e-01
  -3.6725576482095551e+02  -2.8738269431789693e-01
  -3.6910578660394128e+02   5.9381141523500236e-01
  -3.6910578660394128e+02  -5.9381141523500236e-01
  -5.8332822098369775e+02   2.4003944875115510e-01
  -5.8332822098369775e+02  -2.4003944875115510e-01
  -3.7404452322911845e+02   1.5953404767728971e+00
  -3.7404452322911845e+02  -1.5953404767728971e+00
  -5.8089625797780559e+02   9.2899238956898511e-01
  -5.8089625797780559e+02  -9.2899238956898511e-01
  -3.7148237758268965e+02   4.5624317376459067e-01
  -3.7148237758268965e+02  -4.5624317376459067e-01
  -3.7457480574428189e+02   5.5945075744572137e-01
  -3.7457480574428189e+02  -5.5945075744572137e-01
  -3.7310956404460876e+02   9.1275732816008326e-01
  -3.7310956404460876e+02  -9.1275732816008326e-01
  -3.7026618651781331e+02   0.0000000000000000e+00
  -3.7312882463293579e+02   0.0000000000000000e+00
  -5.7657048177356137e+02   0.0000000000000000e+00
  -3.7047329411247000e+02   0.0000000000000000e+00
  -5.8174896082147484e+02   0.0000000000000000e+00
  -3.7433187888423811e+02   0.0000000000000000e+00
  -5.7949743886054262e+02   0.0000000000000000e+00
  -5.8053359321003234e+02   0.0000000000000000e+00
  -3.7625526338579760e+02   4.0494372718512489e-01
  -3.7625526338579760e+02  -4.0494372718512489e-01
  -5.7552806319495176e+02   0.0000000000000000e+00
  -3.7904942233439687e+02   0.0000000000000000e+00
  -3.7748951524856216e+02   5.9093558284871361e-01
  -3.7748951524856216e+02  -5.9093558284871361e-01
  -3.7831796781015902e+02   3.8778643403667301e-01
  -3.7831796781015902e+02  -3.8778643403667301e-01
  -5.7136586134653044e+02   3.5380189825891919e+00
  -5.7136586134653044e+02  -3.5380189825891919e+00
  -5.7292970493830796e+02   2.7828210774386748e+00
  -5.7292970493830796e+02  -2.7828210774386748e+00
  -3.7733769570113031e+02   0.0000000000000000e+00
  -3.8029805865374385e+02   0.0000000000000000e+00
  -3.8129710618399139e+02   0.0000000000000000e+00
  -5.7315531051745779e+02   4.7733174801826100e-01
  -5.7315531051745779e+02  -4.7733174801826100e-01
  -5.7060689079393921e+02   0.0000000000000000e+00
  -5.7363608490882734e+02   0.0000000000000000e+00
  -3.8245379692122691e+02   7.3237266289572112e-01
  -3.8245379692122691e+02  -7.3237266289572112e-01
  -3.8226998821835144e+02   3.5193705789856233e-01
  -3.8226998821835144e+02  -3.5193705789856233e-01
  -3.8186650237419951e+02   0.0000000000000000e+00
  -3.8648914475552374e+02   6.9631241039313363e-01
  -3.8648914475552374e+02  -6.9631241039313363e-01
  -3.8400945284171769e+02   2.5953002511166534e-01
  -3.8400945284171769e+02  -2.5953002511166534e-01
  -3.8611209520690909e+02   0.0000000000000000e+00
  -3.8465612333699579e+02   0.0000000000000000e+00
  -5.6842265529167184e+02   1.5723115779959147e+00
  -5.6842265529167184e+02  -1.5723115779959147e+00
  -5.6911564423124855e+02   0.0000000000000000e+00
  -5.6677026808096787e+02   2.1826795817779390e+00
  -5.6677026808096787e+02  -2.1826795817779390e+00
  -5.6782349812421057e+02   6.3040731469232203e-01
  -5.6782349812421057e+02  -6.3040731469232203e-01
  -5.6503307105191016e+02   5.8145249013981659e-01
  -5.6503307105191016e+02  -5.8145249013981659e-01
  -5.6664112551678340e+02   0.0000000000000000e+00
  -5.5755727798224962e+02   3.4498136064499132e+00
  -5.5755727798224962e+02  -3.4498136064499132e+00
  -5.6187860198040175e+02   8.5860864548613258e-01
  -5.6187860198040175e+02  -8.5860864548613258e-01
  -5.6390328590167633e+02   7.7543759284465119e-01
  -5.6390328590167633e+02  -7.7543759284465119e-01
  -5.5445435723013975e+02   3.0589442374163935e+00
  -5.5445435723013975e+02  -3.0589442374163935e+00
  -5.5929899473910768e+02   1.3637398897401172e+00
  -5.5929899473910768e+02  -1.3637398897401172e+00
  -5.4801544871737337e+02   1.8439315073663862e+00
  -5.4801544871737337e+02  -1.8439315073663862e+00
  -5.5970527240510194e+02   0.0000000000000000e+00
  -5.4895354316750922e+02   6.0424534243711348e-01
  -5.4895354316750922e+02  -6.0424534243711348e-01
  -5.5645361537516101e+02   1.1481747871822603e+00
  -5.5645361537516101e+02  -1.1481747871822603e+00
  -5.5024354696717478e+02   1.0164632910747398e+00
  -5.5024354696717478e+02  -1.0164632910747398e+00
  -5.5865512951859364e+02   0.0000000000000000e+00
  -5.5641250130940068e+02   0.0000000000000000e+00
  -5.6352482849570379e+02   0.0000000000000000e+00
  -5.5301639167042742e+02   0.0000000000000000e+00
  -5.5375589750800066e+02   0.0000000000000000e+00
  -5.5559922161220209e+02   0.0000000000000000e+00
  -5.5166219778871164e+02   0.0000000000000000e+00
  -5.5245517612624951e+02   0.0000000000000000e+00
  -3.8989324041666748e+02   7.3613202437462721e-01
  -3.8989324041666748e+02  -7.3613202437462721e-01
  -3.8791344490372990e+02   2.8224864320890147e-01
  -3.8791344490372990e+02  -2.8224864320890147e-01
  -3.8831051218441701e+02   4.2320914646790475e-01
  -3.8831051218441701e+02  -4.2320914646790475e-01
  -5.4686502393543287e+02   2.6520255649105486e+00
  -5.4686502393543287e+02  -2.6520255649105486e+00
  -5.4793504145272345e+02   0.0000000000000000e+00
  -3.8983863813921937e+02   0.0000000000000000e+00
  -5.4297452236050503e+02   3.1859548595748572e+00
  -5.4297452236050503e+02  -3.1859548595748572e+00
  -3.9091016107031140e+02   8.9485396124437222e-01
  -3.9091016107031140e+02  -8.9485396124437222e-01
  -3.9227265279462313e+02   1.5301176977444446e+00
  -3.9227265279462313e+02  -1.5301176977444446e+00
  -3.9083315568075238e+02   0.0000000000000000e+00
  -3.9213100844058584e+02   0.0000000000000000e+00
  -5.4352663006755893e+02   0.0000000000000000e+00
  -5.4119464115096775e+02   1.6232491698464491e+00
  -5.4119464115096775e+02  -1.6232491698464491e+00
  -3.9827503456308102e+02   1.8262303419807033e+00
  -3.9827503456308102e+02  -1.8262303419807033e+00
  -3.9301851036521992e+02   0.0000000000000000e+00
  -3.9321900539620111e+02   0.0000000000000000e+00
  -5.4291628077613075e+02   0.0000000000000000e+00
  -3.9530189488765154e+02   7.3276897924310669e-01
  -3.9530189488765154e+02  -7.3276897924310669e-01
  -3.9598261505732535e+02   0.0000000000000000e+00
  -5.4039134059503078e+02   1.1216246918106576e+00
  -5.4039134059503078e+02  -1.1216246918106576e+00
  -3.9705529264145264e+02   6.8588992400015858e-01
  -3.9705529264145264e+02  -6.8588992400015858e-01
  -3.9425871518756639e+02   2.0104565920715081e-01
  -3.9425871518756639e+02  -2.0104565920715081e-01
  -5.4655300531178898e+02   0.0000000000000000e+00
  -5.4570835241165310e+02   0.0000000000000000e+00
  -3.9861066461387850e+02   9.9115616750364968e-02
  -3.9861066461387850e+02  -9.9115616750364968e-02
  -3.9976022178237469e+02   0.0000000000000000e+00
  -4.0355031615930818e+02   1.2033417179279413e+00
  -4.0355031615930818e+02  -1.2033417179279413e+00
  -4.0071939281633780e+02   6.8086232364294341e-01
  -4.0071939281633780e+02  -6.8086232364294341e-01
  -4.0107415439706102e+02   0.0000000000000000e+00
  -4.0210192229667734e+02   0.0000000000000000e+00
  -4.0247238308599179e+02   0.0000000000000000e+00
  -5.3994863222369656e+02   0.0000000000000000e+00
  -5.3931310857036226e+02   0.0000000000000000e+00
  -5.3770850666687829e+02   0.0000000000000000e+00
  -5.3703746545882450e+02   0.0000000000000000e+00
  -5.3729789236538932e+02   0.0000000000000000e+00
  -5.3322486592218502e+02   2.7725101981158091e+00
  -5.3322486592218502e+02  -2.7725101981158091e+00
  -5.3591253768237675e+02   0.0000000000000000e+00
  -5.3263767955614162e+02   2.5919047183698511e+00
  -5.3263767955614162e+02  -2.5919047183698511e+00
  -5.3520210547327611e+02   0.0000000000000000e+00
  -5.3393208385500498e+02   0.0000000000000000e+00
  -5.2829170211708924e+02   2.0160251586964848e+00
  -5.2829170211708924e+02  -2.0160251586964848e+00
  -5.2451272451250748e+02   1.8299729358571537e+00
  -5.2451272451250748e+02  -1.8299729358571537e+00
  -5.3181920658904301e+02   1.3834102476404813e+00
  -5.3181920658904301e+02  -1.3834102476404813e+00
  -5.2657307650020084e+02   1.7043092118049412e+00
  -5.2657307650020084e+02  -1.7043092118049412e+00
  -5.3309454233188376e+02   0.0000000000000000e+00
  -5.2348440731315907e+02   0.0000000000000000e+00
  -5.2396183094067555e+02   4.4614326234905843e-01
  -5.2396183094067555e+02  -4.4614326234905843e-01
  -5.3043818414249722e+02   7.0192531921717194e-01
  -5.3043818414249722e+02  -7.0192531921717194e-01
  -5.2550847330232045e+02   0.0000000000000000e+00
  -5.3194493429298416e+02   0.0000000000000000e+00
  -5.2626736865566966e+02   0.0000000000000000e+00
  -5.2866495299960491e+02   0.0000000000000000e+00
  -5.2913349229633081e+02   0.0000000000000000e+00
  -4.0401663666186198e+02   0.0000000000000000e+00
  -5.2038840233465214e+02   1.2273348434964158e+00
  -5.2038840233465214e+02  -1.2273348434964158e+00
  -4.0658269199436518e+02   1.4045571026942780e+00
  -4.0658269199436518e+02  -1.4045571026942780e+00
  -4.0482929058287959e+02   1.4901885431643996e-01
  -4.0482929058287959e+02  -1.4901885431643996e-01
  -4.0871737684506695e+02   5.0033589452973970e-01
  -4.0871737684506695e+02  -5.0033589452973970e-01
  -4.0768773775354668e+02   4.4927549637295749e-01
  -4.0768773775354668e+02  -4.4927549637295749e-01
  -4.0569229197950392e+02   0.0000000000000000e+00
  -5.1388074384890376e+02   1.6597794621125959e+00
  -5.1388074384890376e+02  -1.6597794621125959e+00
  -5.1755636297688068e+02   9.1849076463876733e-01
  -5.1755636297688068e+02  -9.1849076463876733e-01
  -5.1693039456734755e+02   4.8826068712654086e-01
  -5.1693039456734755e+02  -4.8826068712654086e-01
  -5.1888854064227371e+02   5.3017298176695637e-01
  -5.1888854064227371e+02  -5.3017298176695637e-01
  -5.2059773259576366e+02   0.0000000000000000e+00
  -4.0697201233972771e+02   0.0000000000000000e+00
  -4.2254022567427410e+02   1.5771867989496011e+00
  -4.2254022567427410e+02  -1.5771867989496011e+00
  -4.2329666545812245e+02   0.0000000000000000e+00
  -4.0952255780642571e+02   0.0000000000000000e+00
  -4.2140086501350368e+02   9.8204825778717542e-01
  -4.2140086501350368e+02  -9.8204825778717542e-01
  -4.1074233785564115e+02   5.8750835123991507e-01
  -4.1074233785564115e+02  -5.8750835123991507e-01
  -4.1343021392652849e+02   1.5292521948840596e+00
  -4.1343021392652849e+02  -1.5292521948840596e+00
  -4.1623180045255987e+02   7.7219743087516957e-01
  -4.1623180045255987e+02  -7.7219743087516957e-01
  -4.1575393937022380e+02   5.8686417433138993e-01
  -4.1575393937022380e+02  -5.8686417433138993e-01
  -4.1458723830189314e+02   0.0000000000000000e+00
  -4.1411281518694392e+02   0.0000000000000000e+00
  -5.0717692233884719e+02   2.7622581410838389e+00
  -5.0717692233884719e+02  -2.7622581410838389e+00
  -5.1054211807469312e+02   2.0124069790414998e+00
  -5.1054211807469312e+02  -2.0124069790414998e+00
  -5.2031953931490000e+02   0.0000000000000000e+00
  -5.0849510983967042e+02   0.0000000000000000e+00
  -5.0726356022993104e+02   4.5519129774913125e-01
  -5.0726356022993104e+02  -4.5519129774913125e-01
  -5.1156737952810016e+02   1.2227945560912863e+00
  -5.1156737952810016e+02  -1.2227945560912863e+00
  -5.1428766063722924e+02   0.0000000000000000e+00
  -5.1136844498391940e+02   0.0000000000000000e+00
  -5.1283089407322359e+02   0.0000000000000000e+00
  -5.1538142406820714e+02   0.0000000000000000e+00
  -5.1570757419781785e+02   0.0000000000000000e+00
  -5.0561516223204359e+02   4.1427300808728740e-01
  -5.0561516223204359e+02  -4.1427300808728740e-01
  -5.0975166123909742e+02   0.0000000000000000e+00
  -5.1234015553082816e+02   0.0000000000000000e+00
  -4.3280935198746778e+02   0.0000000000000000e+00
  -4.3225671051102427e+02   0.0000000000000000e+00
  -4.3135997001584298e+02   0.0000000000000000e+00
  -4.1888426421038480e+02   1.2267436335760427e+00
  -4.1888426421038480e+02  -1.2267436335760427e+00
  -4.3017272454371465e+02   8.6189999713628807e-01
  -4.3017272454371465e+02  -8.6189999713628807e-01
  -4.3062141157267462e+02   0.0000000000000000e+00
  -4.2553016179411628e+02   1.4102213233166503e+00
  -4.2553016179411628e+02  -1.4102213233166503e+00
  -4.2997387145835285e+02   0.0000000000000000e+00
  -4.2466404024838630e+02   1.8354719861920937e-01
  -4.2466404024838630e+02  -1.8354719861920937e-01
  -4.2507639307066415e+02   0.0000000000000000e+00
  -4.1198987546877146e+02   0.0000000000000000e+00
  -4.1967795019116033e+02   5.6747296478131060e-01
  -4.1967795019116033e+02  -5.6747296478131060e-01
  -4.2876159984565601e+02   0.0000000000000000e+00
  -4.2820532431511560e+02   0.0000000000000000e+00
  -4.2612021401972743e+02   0.0000000000000000e+00
  -4.1758636681460740e+02   0.0000000000000000e+00
  -4.9773353320053207e+02   2.6217345523410769e+00
  -4.9773353320053207e+02  -2.6217345523410769e+00
  -5.0381500760615967e+02   9.6120250451471645e-01
  -5.0381500760615967e+02  -9.6120250451471645e-01
  -5.0142943296312785e+02   1.3663895975814040e+00
  -5.0142943296312785e+02  -1.3663895975814040e+00
  -5.0402281349928808e+02   0.0000000000000000e+00
  -4.0654789030256518e+02   0.0000000000000000e+00
  -4.3453349124121564e+02   1.0882140067348778e+00
  -4.3453349124121564e+02  -1.0882140067348778e+00
  -4.3341153377494362e+02   0.0000000000000000e+00
  -5.0142936999535357e+02   2.3240623893862450e-01
  -5.0142936999535357e+02  -2.3240623893862450e-01
  -4.1234386731655775e+02   2.6147094917069796e-01
  -4.1234386731655775e+02  -2.6147094917069796e-01
  -4.2655478490809418e+02   7.6113397678352146e-01
  -4.2655478490809418e+02  -7.6113397678352146e-01
  -4.1320463274001645e+02   0.0000000000000000e+00
  -4.3788417222129783e+02   2.0558969525112323e+00
  -4.3788417222129783e+02  -2.0558969525112323e+00
  -4.9970761098151661e+02   1.1477506453952400e+00
  -4.9970761098151661e+02  -1.1477506453952400e+00
  -4.3692094133424723e+02   1.0443459187069311e+00
  -4.3692094133424723e+02  -1.0443459187069311e+00
  -4.6965194715544953e+02   2.4850209649974002e+00
  -4.6965194715544953e+02  -2.4850209649974002e+00
  -4.9886909852778575e+02   0.0000000000000000e+00
  -4.9418557255596676e+02   1.8490045554240697e+00
  -4.9418557255596676e+02  -1.8490045554240697e+00
  -4.4143785444604339e+02   1.4736905554135673e+00
  -4.4143785444604339e+02  -1.4736905554135673e+00
  -4.4707212795535895e+02   1.3630324438717065e+00
  -4.4707212795535895e+02  -1.3630324438717065e+00
  -4.9119083010996337e+02   1.1258368399206868e+00
  -4.9119083010996337e+02  -1.1258368399206868e+00
  -4.9324457677482883e+02   1.1852941254761122e+00
  -4.9324457677482883e+02  -1.1852941254761122e+00
  -4.4658905570982131e+02   0.0000000000000000e+00
  -4.4490391142938370e+02   0.0000000000000000e+00
  -4.9440954907885879e+02   8.0707784413304628e-01
  -4.9440954907885879e+02  -8.0707784413304628e-01
  -4.4417697808216616e+02   0.0000000000000000e+00
  -4.4522865960084630e+02   0.0000000000000000e+00
  -4.7591581523371849e+02   2.4324926308411756e+00
  -4.7591581523371849e+02  -2.4324926308411756e+00
  -4.5014888393476235e+02   1.2637908789597059e+00
  -4.5014888393476235e+02  -1.2637908789597059e+00
  -4.7540172759998950e+02   2.2538299217028528e+00
  -4.7540172759998950e+02  -2.2538299217028528e+00
  -4.4288545039228552e+02   2.8876259908686780e-01
  -4.4288545039228552e+02  -2.8876259908686780e-01
  -4.9822343755942546e+02   0.0000000000000000e+00
  -4.9042946502353760e+02   0.0000000000000000e+00
  -4.9543366893071709e+02   6.3484419190049116e-02
  -4.9543366893071709e+02  -6.3484419190049116e-02
  -4.1915315088050238e+02   0.0000000000000000e+00
  -4.3620515246985434e+02   0.0000000000000000e+00
  -4.8931778623190496e+02   8.6598417263505478e-01
  -4.8931778623190496e+02  -8.6598417263505478e-01
  -4.4032323615133572e+02   6.7290186748344005e-01
  -4.4032323615133572e+02  -6.7290186748344005e-01
  -4.8934550228090899e+02   0.0000000000000000e+00
  -4.8418203164187355e+02   2.2687011820214629e+00
  -4.8418203164187355e+02  -2.2687011820214629e+00
  -4.8598877392788631e+02   8.2869791680622340e-01
  -4.8598877392788631e+02  -8.2869791680622340e-01
  -4.3936678899703520e+02   0.0000000000000000e+00
  -4.7277545898214021e+02   1.6254878899982874e+00
  -4.7277545898214021e+02  -1.6254878899982874e+00
  -4.4180400850655303e+02   4.7221020347748632e-01
  -4.4180400850655303e+02  -4.7221020347748632e-01
  -4.7404313619529671e+02   1.5358837935543275e+00
  -4.7404313619529671e+02  -1.5358837935543275e+00
  -4.4842026897931885e+02   0.0000000000000000e+00
  -4.7045817583118594e+02   0.0000000000000000e+00
  -4.7926446216798530e+02   1.6064536440937658e+00
  -4.7926446216798530e+02  -1.6064536440937658e+00
  -4.6924070215396506e+02   0.0000000000000000e+00
  -4.6794487092400539e+02   4.2553276992131439e-01
  -4.6794487092400539e+02  -4.2553276992131439e-01
  -4.5012505857038173e+02   0.0000000000000000e+00
  -4.6743688683892117e+02   0.0000000000000000e+00
  -4.6664201464733884e+02   0.0000000000000000e+00
  -4.6471040930604693e+02   1.7842793622953625e+00
  -4.6471040930604693e+02  -1.7842793622953625e+00
  -4.5132029247800989e+02   0.0000000000000000e+00
  -4.7777752527399741e+02   1.0372271543614304e+00
  -4.7777752527399741e+02  -1.0372271543614304e+00
  -4.8107501003594331e+02   0.0000000000000000e+00
  -4.5975051731664490e+02   2.2397240079489360e+00
  -4.5975051731664490e+02  -2.2397240079489360e+00
  -4.5332654093848998e+02   1.3001690873239176e+00
  -4.5332654093848998e+02  -1.3001690873239176e+00
  -4.7990832327460066e+02   0.0000000000000000e+00
  -4.4915911141441109e+02   0.0000000000000000e+00
  -4.6090153706377566e+02   1.6883420913427376e+00
  -4.6090153706377566e+02  -1.6883420913427376e+00
  -4.5478932452860300e+02   0.0000000000000000e+00
  -4.5583947580394397e+02   6.1679389159919906e-01
  -4.5583947580394397e+02  -6.1679389159919906e-01
  -4.6285414729936667e+02   8.9908138252870118e-01
  -4.6285414729936667e+02  -8.9908138252870118e-01
  -4.5429704503021418e+02   0.0000000000000000e+00
  -4.5327882571296868e+02   1.9994570907498410e-01
  -4.5327882571296868e+02  -1.9994570907498410e-01
  -4.5687901940965946e+02   5.8211907311912603e-01
  -4.5687901940965946e+02  -5.8211907311912603e-01
  -4.1038993462996444e+02   0.0000000000000000e+00
  -4.1852025066870215e+02   0.0000000000000000e+00
  -4.7933252389891612e+02   0.0000000000000000e+00
  -4.6506881882369782e+02   0.0000000000000000e+00
  -4.3573764682454652e+02   0.0000000000000000e+00
  -4.3823289492407355e+02   0.0000000000000000e+00
  -4.3784992306087560e+02   0.0000000000000000e+00
  -4.4902731991022699e+02   0.0000000000000000e+00
  -4.8816447989652573e+02   0.0000000000000000e+00
  -4.8578752402565914e+02   0.0000000000000000e+00
  -4.8357045987842145e+02   8.0323915140087243e-01
  -4.8357045987842145e+02  -8.0323915140087243e-01
  -4.7244414811224834e+02   0.0000000000000000e+00
  -4.5878732587003537e+02   0.0000000000000000e+00
  -4.7797590970607587e+02   0.0000000000000000e+00
  -4.6208938647348538e+02   0.0000000000000000e+00
  -4.5976375626130829e+02   0.0000000000000000e+00
  -4.7240586454597553e+02   0.0000000000000000e+00
  -4.7538223674781068e+02   0.0000000000000000e+00
  -4.5849641014843235e+02   0.0000000000000000e+00
  -4.6378088133070867e+02   0.0000000000000000e+00
  -4.8395635710446771e+02   0.0000000000000000e+00
  -4.8324324522713562e+02   0.0000000000000000e+00
  -4.6093787190321933e+02   1.1698556482637558e-01
  -4.6093787190321933e+02  -1.1698556482637558e-01
  -4.2127035104583138e+02   0.0000000000000000e+00
  -5.0249316674735428e+02   0.0000000000000000e+00
  -4.9751238939449064e+02   0.0000000000000000e+00
  -4.8732141257722714e+02   0.0000000000000000e+00
  -4.8287542419873864e+02   0.0000000000000000e+00


==> cyl_specDL_close.tex <==
1    0.2507 
2   -5.8985 
3   -8.0450 
4  -22.4145 
5  -22.3592  
6  -25.7530  
7  -25.5196  
8  -25.6040  
9  -31.0256  
10  -47.8536 


==> std_map_cheeger.tex <==
  -7.9547547458862522e-01   7.4024981989052261e+00
  -7.9368999911403659e-01   6.6608505916816370e+00
  -7.9190452363944797e-01   6.6271474783398752e+00
  -7.9011904816485934e-01   6.4890426575656086e+00
  -7.8833357269027071e-01   6.1051923037848903e+00
  -7.8654809721568208e-01   5.9797338444770887e+00
  -7.8476262174109346e-01   5.7981944232688818e+00
  -7.8297714626650483e-01   5.5196083281699746e+00
  -7.8119167079191620e-01   5.4933927946685257e+00
  -7.7940619531732758e-01   5.2422659081916638e+00
  -7.7762071984273895e-01   5.1089061181446791e+00
  -7.7583524436815032e-01   5.0301660408118565e+00
  -7.7404976889356170e-01   4.6178309229647061e+00
  -7.7226429341897307e-01   4.5418356821622892e+00
  -7.7047881794438444e-01   4.5288602186371278e+00
  -7.6869334246979582e-01   4.4077134418158881e+00
  -7.6690786699520719e-01   4.1509848373954217e+00
  -7.6512239152061856e-01   4.1294560580102431e+00
  -7.6333691604602993e-01   4.0443269393821826e+00
  -7.6155144057144131e-01   3.9631878849399556e+00
  -7.5976596509685268e-01   3.8674539530892149e+00
  -7.5798048962226405e-01   3.8282966307192132e+00
  -7.5619501414767543e-01   3.7400323094368022e+00
  -7.5440953867308680e-01   3.7028790434011492e+00
  -7.5262406319849817e-01   3.6352437809947871e+00
  -7.5083858772390955e-01   3.5844940224928652e+00
  -7.4905311224932092e-01   3.5633854978994273e+00
  -7.4726763677473229e-01   3.5155377020558962e+00
  -7.4548216130014366e-01   3.4570671125467292e+00
  -7.4369668582555504e-01   3.4134578539868565e+00
  -7.4191121035096641e-01   3.3947980045398558e+00
  -7.4012573487637789e-01   3.3413986692112227e+00
  -7.3834025940178916e-01   3.2791177170105787e+00
  -7.3655478392720064e-01   3.2304254020028749e+00
  -7.3476930845261190e-01   3.2559284012948440e+00
  -7.3298383297802339e-01   3.2189486513480787e+00
  -7.3119835750343465e-01   3.1351010945696292e+00
  -7.2941288202884613e-01   3.1494487023022733e+00
  -7.2762740655425751e-01   3.1074833363170922e+00
  -7.2584193107966888e-01   3.0762232961022535e+00
  -7.2405645560508025e-01   3.0547575006704109e+00
  -7.2227098013049162e-01   3.0088142695388962e+00
  -7.2048550465590300e-01   2.9976352732238367e+00
  -7.1870002918131437e-01   2.9708874029753241e+00
  -7.1691455370672574e-01   2.9375665043845705e+00
  -7.1512907823213712e-01   2.9284307241901590e+00
  -7.1334360275754849e-01   2.9049681290240237e+00
  -7.1155812728295986e-01   2.8757388507925605e+00
  -7.0977265180837124e-01   2.8690442797246565e+00
  -7.0798717633378261e-01   2.8558829515879633e+00
  -7.0620170085919398e-01   2.7967122304109169e+00
  -7.0441622538460535e-01   2.7799107007330424e+00
  -7.0263074991001673e-01   2.7580101224863687e+00
  -7.0084527443542810e-01   2.7495264063933442e+00
  -6.9905979896083947e-01   2.7296783102814186e+00
  -6.9727432348625085e-01   2.7348610180207893e+00
  -6.9548884801166222e-01   2.6996284093769378e+00
  -6.9370337253707359e-01   2.6943671360282089e+00
  -6.9191789706248497e-01   2.6949786325992031e+00
  -6.9013242158789634e-01   2.6361938187432372e+00
  -6.8834694611330771e-01   2.6069283756042418e+00
  -6.8656147063871908e-01   2.5789992971488092e+00
  -6.8477599516413046e-01   2.5763025972793989e+00
  -6.8299051968954183e-01   2.5832869481096647e+00
  -6.8120504421495320e-01   2.5709053059106894e+00
  -6.7941956874036458e-01   2.5494815628631691e+00
  -6.7763409326577595e-01   2.5239798214668330e+00
  -6.7584861779118732e-01   2.5125074113291985e+00
  -6.7406314231659870e-01   2.4968457250463478e+00
  -6.7227766684201007e-01   2.4688563997573287e+00
  -6.7049219136742144e-01   2.4417562819911267e+00
  -6.6870671589283281e-01   2.4276324677385204e+00
  -6.6692124041824419e-01   2.4256921597862071e+00
  -6.6513576494365556e-01   2.4082229063411402e+00
  -6.6335028946906693e-01   2.3910709628472970e+00
  -6.6156481399447831e-01   2.3817495556039163e+00
  -6.5977933851988968e-01   2.3691528745397439e+00
  -6.5799386304530105e-01   2.3426440419757433e+00
  -6.5620838757071243e-01   2.3274230914351817e+00
  -6.5442291209612380e-01   2.3091007101595764e+00
  -6.5263743662153517e-01   2.3012576277510268e+00
  -6.5085196114694654e-01   2.2837283881562715e+00
  -6.4906648567235792e-01   2.2825430781877278e+00
  -6.4728101019776929e-01   2.2528128230496329e+00
  -6.4549553472318066e-01   2.2424208108076265e+00
  -6.4371005924859204e-01   2.2321278593432345e+00
  -6.4192458377400341e-01   2.2159299721355996e+00
  -6.4013910829941478e-01   2.2116669635879740e+00
  -6.3835363282482627e-01   2.1957510498563604e+00
  -6.3656815735023753e-01   2.1802545487773828e+00
  -6.3478268187564901e-01   2.1624000853891356e+00
  -6.3299720640106028e-01   2.1637017321581440e+00
  -6.3121173092647176e-01   2.1488704825344516e+00
  -6.2942625545188302e-01   2.1446899352339441e+00
  -6.2764077997729451e-01   2.1353638171208615e+00
  -6.2585530450270577e-01   2.1263011266732601e+00
  -6.2406982902811725e-01   2.0975858853613443e+00
  -6.2228435355352851e-01   2.0940897729355141e+00
  -6.2049887807894000e-01   2.0882865672302673e+00
  -6.1871340260435126e-01   2.0778157014872645e+00
  -6.1692792712976274e-01   2.0722700488312960e+00
  -6.1514245165517401e-01   2.0578594276286695e+00
  -6.1335697618058549e-01   2.0463497988020061e+00
  -6.1157150070599675e-01   2.0396858738434944e+00
  -6.0978602523140824e-01   2.0419944161694827e+00
  -6.0800054975681961e-01   2.0356070303489404e+00
  -6.0621507428223098e-01   2.0275694740476045e+00
  -6.0442959880764235e-01   2.0222020946732773e+00
  -6.0264412333305373e-01   2.0109239322047663e+00
  -6.0085864785846510e-01   2.0063442191583265e+00
  -5.9907317238387647e-01   1.9881159436737104e+00
  -5.9728769690928785e-01   1.9868286573596610e+00
  -5.9550222143469922e-01   1.9799908966605388e+00
  -5.9371674596011059e-01   1.9717199565687169e+00
  -5.9193127048552197e-01   1.9698766774703913e+00
  -5.9014579501093334e-01   1.9684803319346544e+00
  -5.8836031953634471e-01   1.9767652292941365e+00
  -5.8657484406175608e-01   1.9646887356318992e+00
  -5.8478936858716746e-01   1.9624220001773558e+00
  -5.8300389311257883e-01   1.9530032189336428e+00
  -5.8121841763799020e-01   1.9529752161727181e+00
  -5.7943294216340158e-01   1.9441248235395465e+00
  -5.7764746668881295e-01   1.9426378599193077e+00
  -5.7586199121422432e-01   1.9428851997960093e+00
  -5.7407651573963570e-01   1.9244896952662245e+00
  -5.7229104026504707e-01   1.9186320150051561e+00
  -5.7050556479045844e-01   1.9195084030400280e+00
  -5.6872008931586981e-01   1.9123790344077185e+00
  -5.6693461384128119e-01   1.9170159066749242e+00
  -5.6514913836669256e-01   1.9106444167754117e+00
  -5.6336366289210393e-01   1.9045942226004986e+00
  -5.6157818741751531e-01   1.9050112358523199e+00
  -5.5979271194292668e-01   1.8979604722998811e+00
  -5.5800723646833805e-01   1.8956051297778269e+00
  -5.5622176099374943e-01   1.8948561906468959e+00
  -5.5443628551916080e-01   1.8897376112487423e+00
  -5.5265081004457217e-01   1.8816222393562947e+00
  -5.5086533456998354e-01   1.8823604499248732e+00
  -5.4907985909539492e-01   1.8717826057888771e+00
  -5.4729438362080629e-01   1.8627700727530658e+00
  -5.4550890814621766e-01   1.8569211618649677e+00
  -5.4372343267162904e-01   1.8527420711629010e+00
  -5.4193795719704041e-01   1.8487637121214200e+00
  -5.4015248172245178e-01   1.8399103036394335e+00
  -5.3836700624786316e-01   1.8472323242471427e+00
  -5.3658153077327464e-01   1.8428639313835780e+00
  -5.3479605529868590e-01   1.8439269414061048e+00
  -5.3301057982409739e-01   1.8403300660130246e+00
  -5.3122510434950865e-01   1.8382769373333936e+00
  -5.2943962887492013e-01   1.8318911703155831e+00
  -5.2765415340033139e-01   1.8303828237609219e+00
  -5.2586867792574288e-01   1.8348168130439795e+00
  -5.2408320245115414e-01   1.8408125277444276e+00
  -5.2229772697656562e-01   1.8369034929520405e+00
  -5.2051225150197689e-01   1.8529810533068078e+00
  -5.1872677602738837e-01   1.8500285207678535e+00
  -5.1694130055279963e-01   1.8486115781007320e+00
  -5.1515582507821112e-01   1.8456974093750433e+00
  -5.1337034960362238e-01   1.8418739400994724e+00
  -5.1158487412903386e-01   1.8474510566535682e+00
  -5.0979939865444512e-01   1.8573073705578942e+00
  -5.0801392317985661e-01   1.9062068855537593e+00
  -5.0622844770526787e-01   1.9592558205949295e+00
  -5.0444297223067935e-01   1.9460601422430279e+00
  -5.0265749675609062e-01   1.9291078655837226e+00
  -5.0087202128150210e-01   1.9079275116273289e+00
  -4.9908654580691342e-01   1.8748418421707038e+00
  -4.9730107033232479e-01   1.8446170423612116e+00
  -4.9551559485773616e-01   1.8222465538194683e+00
  -4.9373011938314754e-01   1.7969389190342457e+00
  -4.9194464390855891e-01   1.7807880424815556e+00
  -4.9015916843397028e-01   1.7577776417440725e+00
  -4.8837369295938166e-01   1.7441993927247221e+00
  -4.8658821748479303e-01   1.7257424209033425e+00
  -4.8480274201020440e-01   1.7094455982046661e+00
  -4.8301726653561577e-01   1.6927127033213376e+00
  -4.8123179106102720e-01   1.6755273687851633e+00
  -4.7944631558643858e-01   1.6587294873278717e+00
  -4.7766084011184995e-01   1.6517498024440005e+00
  -4.7587536463726132e-01   1.6370730441102312e+00
  -4.7408988916267270e-01   1.6242228014392543e+00
  -4.7230441368808407e-01   1.6108405080020591e+00
  -4.7051893821349544e-01   1.5954676744237231e+00
  -4.6873346273890681e-01   1.5833140868063247e+00
  -4.6694798726431819e-01   1.5706447541852360e+00
  -4.6516251178972956e-01   1.5603136538631777e+00
  -4.6337703631514093e-01   1.5487375768270724e+00
  -4.6159156084055231e-01   1.5352928273093798e+00
  -4.5980608536596368e-01   1.5234450328241533e+00
  -4.5802060989137505e-01   1.5131115255561272e+00
  -4.5623513441678643e-01   1.5042377311521862e+00
  -4.5444965894219780e-01   1.4935166151401233e+00
  -4.5266418346760917e-01   1.4823150308159432e+00
  -4.5087870799302054e-01   1.4757052944660716e+00
  -4.4909323251843192e-01   1.4666518689305093e+00
  -4.4730775704384329e-01   1.4601922385901618e+00
  -4.4552228156925466e-01   1.4513361051638203e+00
  -4.4373680609466604e-01   1.4413817931626061e+00
  -4.4195133062007741e-01   1.4327614175451848e+00
  -4.4016585514548878e-01   1.4224777503257831e+00
  -4.3838037967090016e-01   1.4140937073268247e+00
  -4.3659490419631153e-01   1.4035120803752694e+00
  -4.3480942872172290e-01   1.3970626595118811e+00
  -4.3302395324713427e-01   1.3878597959429266e+00
  -4.3123847777254565e-01   1.3837871532636721e+00
  -4.2945300229795702e-01   1.3753135873693390e+00
  -4.2766752682336839e-01   1.3664006697267472e+00
  -4.2588205134877977e-01   1.3592177286134639e+00
  -4.2409657587419114e-01   1.3515808246727734e+00
  -4.2231110039960257e-01   1.3429814521108046e+00
  -4.2052562492501394e-01   1.3376142533989888e+00
  -4.1874014945042531e-01   1.3302216407827374e+00
  -4.1695467397583669e-01   1.3249604950101770e+00
  -4.1516919850124806e-01   1.3177143379587746e+00
  -4.1338372302665943e-01   1.3085480003694729e+00
  -4.1159824755207081e-01   1.3009923217438726e+00
  -4.0981277207748218e-01   1.2964629954288105e+00
  -4.0802729660289355e-01   1.2900229319489023e+00
  -4.0624182112830493e-01   1.2850956351609124e+00
  -4.0445634565371630e-01   1.2811649596296626e+00
  -4.0267087017912767e-01   1.2729869895063377e+00
  -4.0088539470453904e-01   1.2696037104439628e+00
  -3.9909991922995042e-01   1.2620410168042413e+00
  -3.9731444375536179e-01   1.2550280337446673e+00
  -3.9552896828077316e-01   1.2508312479214947e+00
  -3.9374349280618454e-01   1.2425920574204261e+00
  -3.9195801733159591e-01   1.2366932156456165e+00
  -3.9017254185700728e-01   1.2299699301227915e+00
  -3.8838706638241866e-01   1.2241946067051950e+00
  -3.8660159090783003e-01   1.2202116360233934e+00
  -3.8481611543324140e-01   1.2149622066552748e+00
  -3.8303063995865277e-01   1.2119012901345163e+00
  -3.8124516448406415e-01   1.2050270050569829e+00
  -3.7945968900947552e-01   1.1990726555766231e+00
  -3.7767421353488689e-01   1.1965147285937874e+00
  -3.7588873806029827e-01   1.1894060224165630e+00
  -3.7410326258570964e-01   1.1868945579991501e+00
  -3.7231778711112101e-01   1.1831683948382350e+00
  -3.7053231163653239e-01   1.1778460137296329e+00
  -3.6874683616194376e-01   1.1725727099326768e+00
  -3.6696136068735519e-01   1.1669508298880769e+00
  -3.6517588521276656e-01   1.1590266207648559e+00
  -3.6339040973817793e-01   1.1543166155728581e+00
  -3.6160493426358931e-01   1.1511921210980363e+00
  -3.5981945878900068e-01   1.1477013504699334e+00
  -3.5803398331441205e-01   1.1419421356443691e+00
  -3.5624850783982343e-01   1.1377524505001091e+00
  -3.5446303236523480e-01   1.1343450541866800e+00
  -3.5267755689064617e-01   1.1302117406880459e+00
  -3.5089208141605754e-01   1.1261112785072152e+00
  -3.4910660594146892e-01   1.1227795087655288e+00
  -3.4732113046688029e-01   1.1191014615194883e+00
  -3.4553565499229166e-01   1.1139976772359164e+00
  -3.4375017951770304e-01   1.1096620372592143e+00
  -3.4196470404311441e-01   1.1067924627200179e+00
  -3.4017922856852578e-01   1.1021627728606198e+00
  -3.3839375309393716e-01   1.0975744583759504e+00
  -3.3660827761934853e-01   1.0930268553732239e+00
  -3.3482280214475990e-01   1.0892107945910863e+00
  -3.3303732667017127e-01   1.0850779341184011e+00
  -3.3125185119558265e-01   1.0813192677991279e+00
  -3.2946637572099402e-01   1.0772493061971542e+00
  -3.2768090024640539e-01   1.0732106346159032e+00
  -3.2589542477181677e-01   1.0702053726621092e+00
  -3.2410994929722814e-01   1.0675509990962890e+00
  -3.2232447382263951e-01   1.0645798502839616e+00
  -3.2053899834805089e-01   1.0606394200995684e+00
  -3.1875352287346226e-01   1.0570560675558924e+00
  -3.1696804739887363e-01   1.0538229755488659e+00
  -3.1518257192428500e-01   1.0502889696179787e+00
  -3.1339709644969638e-01   1.0464609985451157e+00
  -3.1161162097510775e-01   1.0423449485255549e+00
  -3.0982614550051912e-01   1.0388923125983967e+00
  -3.0804067002593055e-01   1.0345254185449022e+00
  -3.0625519455134192e-01   1.0311274875902479e+00
  -3.0446971907675330e-01   1.0296081088949627e+00
  -3.0268424360216467e-01   1.0256305965505317e+00
  -3.0089876812757604e-01   1.0213809559898008e+00
  -2.9911329265298742e-01   1.0180752135323150e+00
  -2.9732781717839879e-01   1.0153934308517198e+00
  -2.9554234170381016e-01   1.0124278763959949e+00
  -2.9375686622922148e-01   1.0079948045983060e+00
  -2.9197139075463285e-01   1.0068475237674561e+00
  -2.9018591528004423e-01   1.0042301801235245e+00
  -2.8840043980545560e-01   1.0007497464480648e+00
  -2.8661496433086697e-01   9.9874905154840277e-01
  -2.8482948885627835e-01   9.9502035085151797e-01
  -2.8304401338168972e-01   9.9160807684985852e-01
  -2.8125853790710109e-01   9.8822139162352163e-01
  -2.7947306243251258e-01   9.8400985318530632e-01
  -2.7768758695792395e-01   9.8095798176432192e-01
  -2.7590211148333532e-01   9.7848517450001526e-01
  -2.7411663600874669e-01   9.7713979410410956e-01
  -2.7233116053415807e-01   9.7496686193483062e-01
  -2.7054568505956944e-01   9.6950128202132835e-01
  -2.6876020958498081e-01   9.6709164350789611e-01
  -2.6697473411039219e-01   9.6361048158478813e-01
  -2.6518925863580356e-01   9.6123324894766904e-01
  -2.6340378316121493e-01   9.5886889968983458e-01
  -2.6161830768662631e-01   9.5705201139980856e-01
  -2.5983283221203768e-01   9.5417948176491818e-01
  -2.5804735673744905e-01   9.5264769030400864e-01
  -2.5626188126286042e-01   9.5059413784617930e-01
  -2.5447640578827180e-01   9.4776356975016995e-01
  -2.5269093031368317e-01   9.4495196983463214e-01
  -2.5090545483909454e-01   9.4086659286665997e-01
  -2.4911997936450592e-01   9.3681890168015847e-01
  -2.4733450388991729e-01   9.3458791133500008e-01
  -2.4554902841532866e-01   9.3160901934375728e-01
  -2.4376355294074004e-01   9.2990966298520350e-01
  -2.4197807746615141e-01   9.2771561800807600e-01
  -2.4019260199156278e-01   9.2603351104943732e-01
  -2.3840712651697415e-01   9.2237107771636540e-01
  -2.3662165104238553e-01   9.1972432003431015e-01
  -2.3483617556779690e-01   9.1660493579079061e-01
  -2.3305070009320827e-01   9.1472560310500239e-01
  -2.3126522461861965e-01   9.1309793600025757e-01
  -2.2947974914403102e-01   9.1026828763288226e-01
  -2.2769427366944239e-01   9.0865880491412243e-01
  -2.2590879819485377e-01   9.0681677091790613e-01
  -2.2412332272026514e-01   9.0426898805442912e-01
  -2.2233784724567651e-01   9.0292256340751686e-01
  -2.2055237177108789e-01   9.0016370284279679e-01
  -2.1876689629649926e-01   8.9718920684933712e-01
  -2.1698142082191063e-01   8.9586863011760176e-01
  -2.1519594534732200e-01   8.9222970262570866e-01
  -2.1341046987273338e-01   8.8908310189082218e-01
  -2.1162499439814475e-01   8.8687569856049397e-01
  -2.0983951892355612e-01   8.8399818167842648e-01
  -2.0805404344896750e-01   8.8181945859287580e-01
  -2.0626856797437887e-01   8.7852847552897750e-01
  -2.0448309249979024e-01   8.7660368763391694e-01
  -2.0269761702520162e-01   8.7535703804145315e-01
  -2.0091214155061299e-01   8.7367101620842524e-01
  -1.9912666607602436e-01   8.7199343463035717e-01
  -1.9734119060143573e-01   8.6988387853155469e-01
  -1.9555571512684711e-01   8.6910173677233482e-01
  -1.9377023965225848e-01   8.6700862353917985e-01
  -1.9198476417766985e-01   8.6427461868974753e-01
  -1.9019928870308123e-01   8.6177605504378774e-01
  -1.8841381322849260e-01   8.5993854804844150e-01
  -1.8662833775390397e-01   8.5746834134467753e-01
  -1.8484286227931535e-01   8.5629054955700268e-01
  -1.8305738680472672e-01   8.5342068447189656e-01
  -1.8127191133013809e-01   8.5078188238670416e-01
  -1.7948643585554946e-01   8.4941692915006051e-01
  -1.7770096038096084e-01   8.4659791632073400e-01
  -1.7591548490637221e-01   8.4400620530081816e-01
  -1.7413000943178358e-01   8.4246175624551567e-01
  -1.7234453395719496e-01   8.4030948857005949e-01
  -1.7055905848260633e-01   8.3837432544561308e-01
  -1.6877358300801770e-01   8.3604323915796275e-01
  -1.6698810753342919e-01   8.3473621301691547e-01
  -1.6520263205884056e-01   8.3383797650906832e-01
  -1.6341715658425193e-01   8.3193807003207287e-01
  -1.6163168110966331e-01   8.2944909302614467e-01
  -1.5984620563507468e-01   8.2836775454885203e-01
  -1.5806073016048605e-01   8.2649617837040845e-01
  -1.5627525468589742e-01   8.2424040574073210e-01
  -1.5448977921130880e-01   8.2180266971693205e-01
  -1.5270430373672017e-01   8.2074592089423726e-01
  -1.5091882826213154e-01   8.1852589529200104e-01
  -1.4913335278754292e-01   8.1631938636509416e-01
  -1.4734787731295429e-01   8.1470332814682000e-01
  -1.4556240183836566e-01   8.1271234513538382e-01
  -1.4377692636377704e-01   8.1054189642076369e-01
  -1.4199145088918841e-01   8.0914291693987705e-01
  -1.4020597541459978e-01   8.0775013964889530e-01
  -1.3842049994001115e-01   8.0617529301572699e-01
  -1.3663502446542253e-01   8.0423298773616847e-01
  -1.3484954899083390e-01   8.0267452953098772e-01
  -1.3306407351624527e-01   8.0019541772224712e-01
  -1.3127859804165665e-01   7.9754915075034505e-01
  -1.2949312256706802e-01   7.9602067623571504e-01
  -1.2770764709247939e-01   7.9486443625194958e-01
  -1.2592217161789077e-01   7.9262105254960169e-01
  -1.2413669614330214e-01   7.9147796423391426e-01
  -1.2235122066871351e-01   7.8961697900277239e-01
  -1.2056574519412488e-01   7.8848421811277136e-01
  -1.1878026971953626e-01   7.8663956233946208e-01
  -1.1699479424494763e-01   7.8551796621647130e-01
  -1.1520931877035900e-01   7.8386792091271207e-01
  -1.1342384329577038e-01   7.8240369904213725e-01
  -1.1163836782118175e-01   7.8059422308220761e-01
  -1.0985289234659312e-01   7.7914464554441931e-01
  -1.0806741687200450e-01   7.7682932908841285e-01
  -1.0628194139741587e-01   7.7574463235737456e-01
  -1.0449646592282724e-01   7.7414454522255105e-01
  -1.0271099044823861e-01   7.7306919549172493e-01
  -1.0092551497364999e-01   7.7011084695509302e-01
  -9.9140039499061361e-02   7.6870857504781986e-01
  -9.7354564024472734e-02   7.6782274716840471e-01
  -9.5569088549884107e-02   7.6457245984990452e-01
  -9.3783613075295480e-02   7.6336371107676448e-01
  -9.1998137600706853e-02   7.6266244890359880e-01
  -9.0212662126118226e-02   7.6179603270134877e-01
  -8.8427186651529599e-02   7.5910136166771935e-01
  -8.6641711176940972e-02   7.5741911567874565e-01
  -8.4856235702352345e-02   7.5640516630024857e-01
  -8.3070760227763718e-02   7.5506646917734543e-01
  -8.1285284753175091e-02   7.5373358357431053e-01
  -7.9499809278586464e-02   7.5208116138250070e-01
  -7.7714333803997837e-02   7.5043817647328170e-01
  -7.5928858329409210e-02   7.4944987626687243e-01
  -7.4143382854820583e-02   7.4749922680286451e-01
  -7.2357907380231956e-02   7.4652144180716484e-01
  -7.0572431905643329e-02   7.4538827982955602e-01
  -6.8786956431054702e-02   7.4410114994248755e-01
  -6.7001480956466075e-02   7.4202738124390288e-01
  -6.5216005481877448e-02   7.4028206466929536e-01
  -6.3430530007288821e-02   7.3870401008255360e-01
  -6.1645054532700194e-02   7.3729066489433392e-01
  -5.9859579058111567e-02   7.3604020020700323e-01
  -5.8074103583522940e-02   7.3402115945137769e-01
  -5.6288628108934313e-02   7.3324896169166487e-01
  -5.4503152634345686e-02   7.3155647019136627e-01
  -5.2717677159757059e-02   7.2956762430422284e-01
  -5.0932201685168543e-02   7.2850478893805204e-01
  -4.9146726210579916e-02   7.2714316470828255e-01
  -4.7361250735991289e-02   7.2624209510975146e-01
  -4.5575775261402662e-02   7.2474242558707469e-01
  -4.3790299786814035e-02   7.2355145921860431e-01
  -4.2004824312225408e-02   7.2266598197072052e-01
  -4.0219348837636781e-02   7.2163473057113747e-01
  -3.8433873363048154e-02   7.2001348275416355e-01
  -3.6648397888459527e-02   7.1854972107550430e-01
  -3.4862922413870900e-02   7.1724134472017276e-01
  -3.3077446939282273e-02   7.1564625954414707e-01
  -3.1291971464693646e-02   7.1391457169500483e-01
  -2.9506495990105019e-02   7.1292037624749016e-01
  -2.7721020515516392e-02   7.1207597256281197e-01
  -2.5935545040927765e-02   7.1007987634431469e-01
  -2.4150069566339138e-02   7.0824169216217892e-01
  -2.2364594091750511e-02   7.0741600634578883e-01
  -2.0579118617161885e-02   7.0573878830724934e-01
  -1.8793643142573258e-02   7.0492319407415105e-01
  -1.7008167667984631e-02   7.0326236442794665e-01
  -1.5222692193396004e-02   7.0217538122948264e-01
  -1.3437216718807377e-02   7.0081327769242896e-01
  -1.1651741244218750e-02   7.0099912004183973e-01
  -9.8662657696301226e-03   7.0259288093797001e-01
  -8.0807902950414956e-03   7.0433603705787085e-01
  -6.2953148204528686e-03   7.0566269080699984e-01
  -4.5098393458642416e-03   7.0699551050038856e-01
  -2.7243638712756146e-03   7.0919465429675987e-01
  -9.3888839668698765e-04   7.1155272461987873e-01
   8.4658707790163934e-04   7.1349206381483676e-01
   2.6320625524902663e-03   7.1456926315756308e-01
   4.4175380270788933e-03   7.1638147335006197e-01
   6.2030135016675203e-03   7.1732343156791445e-01
   7.9884889762561473e-03   7.1900473804105336e-01
   9.7739644508447743e-03   7.2084330980359623e-01
   1.1559439925433401e-02   7.2269206774288353e-01
   1.3344915400022028e-02   7.2410298122603223e-01
   1.5130390874610655e-02   7.2582088331181960e-01
   1.6915866349199282e-02   7.2739797717573240e-01
   1.8701341823787909e-02   7.3049706620522770e-01
   2.0486817298376536e-02   7.3255583184185724e-01
   2.2272292772965163e-02   7.3478040996214344e-01
   2.4057768247553790e-02   7.3732822094045780e-01
   2.5843243722142417e-02   7.3943039305707259e-01
   2.7628719196731044e-02   7.4061076158292116e-01
   2.9414194671319671e-02   7.4226479527230904e-01
   3.1199670145908298e-02   7.4361428814530073e-01
   3.2985145620496925e-02   7.4560015940971769e-01
   3.4770621095085552e-02   7.4775611112272145e-01
   3.6556096569674179e-02   7.4897265432873805e-01
   3.8341572044262806e-02   7.5067340149457407e-01
   4.0127047518851433e-02   7.5254344966065001e-01
   4.1912522993440060e-02   7.5426423891162675e-01
   4.3697998468028687e-02   7.5696549414297698e-01
   4.5483473942617314e-02   7.5936171913178530e-01
   4.7268949417205941e-02   7.6177558691662306e-01
   4.9054424891794568e-02   7.6371221013848234e-01
   5.0839900366383195e-02   7.6582559032378161e-01
   5.2625375840971822e-02   7.6862072661399861e-01
   5.4410851315560449e-02   7.6976232135544354e-01
   5.6196326790149076e-02   7.7191748498874624e-01
   5.7981802264737703e-02   7.7442533351043585e-01
   5.9767277739326330e-02   7.7559165875561042e-01
   6.1552753213914846e-02   7.7880927821981194e-01
   6.3338228688503473e-02   7.8050945897198998e-01
   6.5123704163092100e-02   7.8325499176329505e-01
   6.6909179637680727e-02   7.8532780507720046e-01
   6.8694655112269354e-02   7.8881080845102514e-01
   7.0480130586857981e-02   7.9056596774307042e-01
   7.2265606061446608e-02   7.9427682751274153e-01
   7.4051081536035235e-02   7.9641819594798235e-01
   7.5836557010623862e-02   7.9803694402008318e-01
   7.7622032485212489e-02   8.0002451980335565e-01
   7.9407507959801116e-02   8.0311200998604415e-01
   8.1192983434389743e-02   8.0459123285683531e-01
   8.2978458908978370e-02   8.0571417672710532e-01
   8.4763934383566997e-02   8.0830493145239235e-01
   8.6549409858155624e-02   8.1091561837582127e-01
   8.8334885332744251e-02   8.1336100471424588e-01
   9.0120360807332878e-02   8.1656777398506597e-01
   9.1905836281921505e-02   8.1999303513109412e-01
   9.3691311756510132e-02   8.2345187394089359e-01
   9.5476787231098759e-02   8.2579919580687489e-01
   9.7262262705687386e-02   8.2873874631914057e-01
   9.9047738180276013e-02   8.3112525159451955e-01
   1.0083321365486464e-01   8.3236667070324233e-01
   1.0261868912945327e-01   8.3672458007502371e-01
   1.0440416460404189e-01   8.3936653105325754e-01
   1.0618964007863052e-01   8.4301889642164296e-01
   1.0797511555321915e-01   8.4551827405412694e-01
   1.0976059102780777e-01   8.4903796185603642e-01
   1.1154606650239640e-01   8.5178349862975167e-01
   1.1333154197698503e-01   8.5455171925045148e-01
   1.1511701745157366e-01   8.5632323805605171e-01
   1.1690249292616228e-01   8.5994834316734003e-01
   1.1868796840075091e-01   8.6381526735362568e-01
   1.2047344387533954e-01   8.6689276740215304e-01
   1.2225891934992816e-01   8.7042388324241826e-01
   1.2404439482451679e-01   8.7335967599486197e-01
   1.2582987029910542e-01   8.7632525414279250e-01
   1.2761534577369404e-01   8.8060114729498373e-01
   1.2940082124828267e-01   8.8363054224201298e-01
   1.3118629672287130e-01   8.8647272296140878e-01
   1.3297177219745993e-01   8.8977414010706546e-01
   1.3475724767204844e-01   8.9223525473797161e-01
   1.3654272314663707e-01   8.9605373140463795e-01
   1.3832819862122570e-01   8.9991719865205255e-01
   1.4011367409581432e-01   9.0315446604493033e-01
   1.4189914957040295e-01   9.0778121574636972e-01
   1.4368462504499158e-01   9.1383506411864590e-01
   1.4547010051958020e-01   9.1720496231435289e-01
   1.4725557599416883e-01   9.2294796931679246e-01
   1.4904105146875746e-01   9.2644049239180748e-01
   1.5082652694334608e-01   9.2998493918044556e-01
   1.5261200241793471e-01   9.3405350380129071e-01
   1.5439747789252334e-01   9.3793590282643269e-01
   1.5618295336711197e-01   9.4235718073837671e-01
   1.5796842884170059e-01   9.4661471174395873e-01
   1.5975390431628922e-01   9.5119476072726838e-01
   1.6153937979087785e-01   9.5687074587474663e-01
   1.6332485526546647e-01   9.6215319651634024e-01
   1.6511033074005510e-01   9.6678423990619033e-01
   1.6689580621464373e-01   9.7178788430103413e-01
   1.6868128168923235e-01   9.7847505965627712e-01
   1.7046675716382098e-01   9.8537755805103611e-01
   1.7225223263840961e-01   9.9012724911890693e-01
   1.7403770811299824e-01   9.9457534419116289e-01
   1.7582318358758686e-01   1.0030627936046088e+00
   1.7760865906217549e-01   1.0116077774857128e+00
   1.7939413453676412e-01   1.0198324844543070e+00
   1.8117961001135274e-01   1.0315983162518694e+00
   1.8296508548594137e-01   1.0363484177860365e+00
   1.8475056096053000e-01   1.0301938276045584e+00
   1.8653603643511862e-01   1.0256867031470784e+00
   1.8832151190970725e-01   1.0262003738677239e+00
   1.9010698738429588e-01   1.0255161234267154e+00
   1.9189246285888450e-01   1.0253354456257855e+00
   1.9367793833347313e-01   1.0258725321704660e+00
   1.9546341380806176e-01   1.0272611015616584e+00
   1.9724888928265039e-01   1.0262978932752185e+00
   1.9903436475723901e-01   1.0291050502189538e+00
   2.0081984023182764e-01   1.0279205476087065e+00
   2.0260531570641627e-01   1.0266409416185238e+00
   2.0439079118100489e-01   1.0273706265130116e+00
   2.0617626665559352e-01   1.0282410716127814e+00
   2.0796174213018215e-01   1.0298770382120739e+00
   2.0974721760477077e-01   1.0298610333588929e+00
   2.1153269307935940e-01   1.0294064121389517e+00
   2.1331816855394803e-01   1.0312207529065147e+00
   2.1510364402853666e-01   1.0331602370901931e+00
   2.1688911950312528e-01   1.0327470405979717e+00
   2.1867459497771391e-01   1.0336727050658945e+00
   2.2046007045230254e-01   1.0362824919957763e+00
   2.2224554592689116e-01   1.0380500010655545e+00
   2.2403102140147979e-01   1.0379981154641358e+00
   2.2581649687606842e-01   1.0389675256799245e+00
   2.2760197235065704e-01   1.0390416310307358e+00
   2.2938744782524567e-01   1.0414234859262099e+00
   2.3117292329983430e-01   1.0422657323535764e+00
   2.3295839877442293e-01   1.0425060179858212e+00
   2.3474387424901155e-01   1.0440929348908627e+00
   2.3652934972360018e-01   1.0473782555226716e+00
   2.3831482519818881e-01   1.0470859352392670e+00
   2.4010030067277743e-01   1.0514756095257389e+00
   2.4188577614736606e-01   1.0519394582806219e+00
   2.4367125162195469e-01   1.0524284009646663e+00
   2.4545672709654331e-01   1.0539589551670328e+00
   2.4724220257113183e-01   1.0565472761883696e+00
   2.4902767804572046e-01   1.0574680289162841e+00
   2.5081315352030908e-01   1.0608205101138557e+00
   2.5259862899489771e-01   1.0604369499857715e+00
   2.5438410446948634e-01   1.0604189119110128e+00
   2.5616957994407497e-01   1.0618067078763580e+00
   2.5795505541866359e-01   1.0618302332856790e+00
   2.5974053089325222e-01   1.0622208894020411e+00
   2.6152600636784085e-01   1.0629762929243938e+00
   2.6331148184242947e-01   1.0655106519758755e+00
   2.6509695731701810e-01   1.0680882189564807e+00
   2.6688243279160673e-01   1.0703500403975941e+00
   2.6866790826619535e-01   1.0722856893668766e+00
   2.7045338374078398e-01   1.0738893202967357e+00
   2.7223885921537261e-01   1.0755192561842208e+00
   2.7402433468996124e-01   1.0779055340110630e+00
   2.7580981016454986e-01   1.0777536416621929e+00
   2.7759528563913849e-01   1.0794497033991255e+00
   2.7938076111372712e-01   1.0841425239558342e+00
   2.8116623658831574e-01   1.0851566918708264e+00
   2.8295171206290437e-01   1.0861907281947187e+00
   2.8473718753749300e-01   1.0868638154844930e+00
   2.8652266301208162e-01   1.0867969582235095e+00
   2.8830813848667025e-01   1.0893918649278385e+00
   2.9009361396125888e-01   1.0908736517396922e+00
   2.9187908943584751e-01   1.0931453725595413e+00
   2.9366456491043613e-01   1.0946701465645028e+00
   2.9545004038502476e-01   1.0954384821976069e+00
   2.9723551585961339e-01   1.0997335300734308e+00
   2.9902099133420201e-01   1.1025135073852883e+00
   3.0080646680879064e-01   1.1045384031454153e+00
   3.0259194228337927e-01   1.1034058662996036e+00
   3.0437741775796789e-01   1.1026745814062549e+00
   3.0616289323255652e-01   1.1063369078699623e+00
   3.0794836870714515e-01   1.1064232741366586e+00
   3.0973384418173378e-01   1.1101500009364091e+00
   3.1151931965632240e-01   1.1098586621728936e+00
   3.1330479513091103e-01   1.1136545230668116e+00
   3.1509027060549966e-01   1.1146202923943063e+00
   3.1687574608008828e-01   1.1164235589667189e+00
   3.1866122155467691e-01   1.1199134405953048e+00
   3.2044669702926554e-01   1.1196865434257384e+00
   3.2223217250385416e-01   1.1240792871752903e+00
   3.2401764797844279e-01   1.1281081542530802e+00
   3.2580312345303142e-01   1.1296284931880369e+00
   3.2758859892762004e-01   1.1298879196612612e+00
   3.2937407440220867e-01   1.1331730591360440e+00
   3.3115954987679730e-01   1.1351956429485481e+00
   3.3294502535138593e-01   1.1368067178256001e+00
   3.3473050082597455e-01   1.1371257114946787e+00
   3.3651597630056318e-01   1.1374568904553140e+00
   3.3830145177515181e-01   1.1386782457667775e+00
   3.4008692724974043e-01   1.1434643512279379e+00
   3.4187240272432906e-01   1.1451872623145600e+00
   3.4365787819891769e-01   1.1455852562697153e+00
   3.4544335367350631e-01   1.1491534810867863e+00
   3.4722882914809494e-01   1.1509517840907493e+00
   3.4901430462268357e-01   1.1545997336493805e+00
   3.5079978009727220e-01   1.1582945518263617e+00
   3.5258525557186082e-01   1.1583222256451753e+00
   3.5437073104644945e-01   1.1592847863140818e+00
   3.5615620652103808e-01   1.1593305850914506e+00
   3.5794168199562670e-01   1.1603175593673245e+00
   3.5972715747021533e-01   1.1622541744919925e+00
   3.6151263294480396e-01   1.1642101678731120e+00
   3.6329810841939247e-01   1.1680908736257161e+00
   3.6508358389398110e-01   1.1696254102656201e+00
   3.6686905936856973e-01   1.1764870490530048e+00
   3.6865453484315835e-01   1.1785678716956591e+00
   3.7044001031774698e-01   1.1811579809480626e+00
   3.7222548579233561e-01   1.1857538114263597e+00
   3.7401096126692424e-01   1.1864238539203076e+00
   3.7579643674151286e-01   1.1856081565430328e+00
   3.7758191221610149e-01   1.1872839870308480e+00
   3.7936738769069012e-01   1.1884724916908516e+00
   3.8115286316527874e-01   1.1916901304965057e+00
   3.8293833863986737e-01   1.1929116257727421e+00
   3.8472381411445600e-01   1.1926186818233573e+00
   3.8650928958904462e-01   1.1923291016529343e+00
   3.8829476506363325e-01   1.1976740066536826e+00
   3.9008024053822188e-01   1.2010175724675431e+00
   3.9186571601281051e-01   1.2038714366802152e+00
   3.9365119148739913e-01   1.2067542011115822e+00
   3.9543666696198776e-01   1.2091368607792585e+00
   3.9722214243657639e-01   1.2110095337530371e+00
   3.9900761791116501e-01   1.2155701511906356e+00
   4.0079309338575364e-01   1.2169459117383448e+00
   4.0257856886034227e-01   1.2183352417765951e+00
   4.0436404433493089e-01   1.2181091713676964e+00
   4.0614951980951952e-01   1.2206014257450910e+00
   4.0793499528410815e-01   1.2236640755594859e+00
   4.0972047075869678e-01   1.2267555097197349e+00
   4.1150594623328540e-01   1.2282100951175334e+00
   4.1329142170787403e-01   1.2302319483399518e+00
   4.1507689718246266e-01   1.2356430151930415e+00
   4.1686237265705128e-01   1.2388494594884629e+00
   4.1864784813163991e-01   1.2409422978727531e+00
   4.2043332360622854e-01   1.2413318211699296e+00
   4.2221879908081716e-01   1.2422984259214191e+00
   4.2400427455540579e-01   1.2455822125874554e+00
   4.2578975002999442e-01   1.2471520729431287e+00
   4.2757522550458305e-01   1.2487330812708524e+00
   4.2936070097917167e-01   1.2503266849981309e+00
   4.3114617645376030e-01   1.2531130143253975e+00
   4.3293165192834893e-01   1.2529609953886425e+00
   4.3471712740293755e-01   1.2557766216938240e+00
   4.3650260287752618e-01   1.2598156797473388e+00
   4.3828807835211481e-01   1.2632937636739423e+00
   4.4007355382670343e-01   1.2661979150721798e+00
   4.4185902930129206e-01   1.2697394310918184e+00
   4.4364450477588069e-01   1.2708472766155701e+00
   4.4542998025046932e-01   1.2719617607610789e+00
   4.4721545572505794e-01   1.2774406277600092e+00
   4.4900093119964657e-01   1.2792122030787711e+00
   4.5078640667423520e-01   1.2809969745354635e+00
   4.5257188214882382e-01   1.2834284123178286e+00
   4.5435735762341245e-01   1.2852442205915851e+00
   4.5614283309800108e-01   1.2889992327991517e+00
   4.5792830857258970e-01   1.2908516612734777e+00
   4.5971378404717833e-01   1.2914197812182293e+00
   4.6149925952176696e-01   1.2932926050228042e+00
   4.6328473499635558e-01   1.3010928921724032e+00
   4.6507021047094421e-01   1.3056828957906910e+00
   4.6685568594553284e-01   1.3056353967666765e+00
   4.6864116142012147e-01   1.3055885128164471e+00
   4.7042663689471009e-01   1.3075553526767827e+00
   4.7221211236929872e-01   1.3088619484391577e+00
   4.7399758784388735e-01   1.3095006616051963e+00
   4.7578306331847586e-01   1.3135497496068611e+00
   4.7756853879306449e-01   1.3121567439434587e+00
   4.7935401426765312e-01   1.3176249771974649e+00
   4.8113948974224174e-01   1.3210760323116635e+00
   4.8292496521683037e-01   1.3224646816956871e+00
   4.8471044069141900e-01   1.3302002609446208e+00
   4.8649591616600762e-01   1.3351975314372861e+00
   4.8828139164059625e-01   1.3380919679411545e+00
   4.9006686711518493e-01   1.3388438345838432e+00
   4.9185234258977356e-01   1.3410496776394589e+00
   4.9363781806436219e-01   1.3447313985440059e+00
   4.9542329353895082e-01   1.3477135065362231e+00
   4.9720876901353944e-01   1.3485038377139784e+00
   4.9899424448812807e-01   1.3522688861286025e+00
   5.0077971996271664e-01   1.3538277021059384e+00
   5.0256519543730538e-01   1.3546502735885508e+00
   5.0435067091189389e-01   1.3577393946586984e+00
   5.0613614638648252e-01   1.3608540062154604e+00
   5.0792162186107115e-01   1.3632339993147313e+00
   5.0970709733565978e-01   1.3687131231646030e+00
   5.1149257281024840e-01   1.3688200038584390e+00
   5.1327804828483703e-01   1.3712578859342759e+00
   5.1506352375942566e-01   1.3760670979189327e+00
   5.1684899923401428e-01   1.3801398999628778e+00
   5.1863447470860291e-01   1.3794821128102339e+00
   5.2041995018319154e-01   1.3804115956551626e+00
   5.2220542565778016e-01   1.3853487090484775e+00
   5.2399090113236879e-01   1.3895313344782600e+00
   5.2577637660695742e-01   1.3962122393728806e+00
   5.2756185208154605e-01   1.4013317340152867e+00
   5.2934732755613467e-01   1.4048417834373552e+00
   5.3113280303072330e-01   1.4092229455796870e+00
   5.3291827850531193e-01   1.4102702566921623e+00
   5.3470375397990055e-01   1.4113239613918638e+00
   5.3648922945448918e-01   1.4140838031977507e+00
   5.3827470492907781e-01   1.4142959384856113e+00
   5.4006018040366643e-01   1.4136500273544548e+00
   5.4184565587825506e-01   1.4190207924752942e+00
   5.4363113135284369e-01   1.4201111735419030e+00
   5.4541660682743232e-01   1.4220775998399797e+00
   5.4720208230202094e-01   1.4266881273675351e+00
   5.4898755777660957e-01   1.4322342967967123e+00
   5.5077303325119820e-01   1.4360578764636076e+00
   5.5255850872578682e-01   1.4399177445719007e+00
   5.5434398420037545e-01   1.4456318257245662e+00
   5.5612945967496408e-01   1.4486597522994453e+00
   5.5791493514955270e-01   1.4517152716040664e+00
   5.5970041062414133e-01   1.4557265378703741e+00
   5.6148588609872996e-01   1.4569690887474533e+00
   5.6327136157331847e-01   1.4638650849453241e+00
   5.6505683704790721e-01   1.4698973959826367e+00
   5.6684231252249573e-01   1.4702312097804060e+00
   5.6862778799708447e-01   1.4676913193586356e+00
   5.7041326347167298e-01   1.4709046426917967e+00
   5.7219873894626172e-01   1.4741431512450018e+00
   5.7398421442085024e-01   1.4803421011274016e+00
   5.7576968989543897e-01   1.4836551401083988e+00
   5.7755516537002749e-01   1.4899847455273203e+00
   5.7934064084461623e-01   1.4913705571494413e+00
   5.8112611631920474e-01   1.4988278502684489e+00
   5.8291159179379348e-01   1.5012756382118517e+00
   5.8469706726838200e-01   1.5027158716665048e+00
   5.8648254274297074e-01   1.5082912969528186e+00
   5.8826801821755925e-01   1.5076873387271712e+00
   5.9005349369214799e-01   1.5112407818605225e+00
   5.9183896916673651e-01   1.5201007916501681e+00
   5.9362444464132524e-01   1.5216186697602401e+00
   5.9540992011591376e-01   1.5210085978084869e+00
   5.9719539559050250e-01   1.5279046440185766e+00
   5.9898087106509101e-01   1.5327158503544194e+00
   6.0076634653967975e-01   1.5386737292152237e+00
   6.0255182201426827e-01   1.5369707357884668e+00
   6.0433729748885701e-01   1.5463392672866432e+00
   6.0612277296344552e-01   1.5502247747829778e+00
   6.0790824843803426e-01   1.5541449135271568e+00
   6.0969372391262278e-01   1.5615337824203466e+00
   6.1147919938721151e-01   1.5644002065326614e+00
   6.1326467486180003e-01   1.5638133985085050e+00
   6.1505015033638877e-01   1.5655395189489270e+00
   6.1683562581097728e-01   1.5719561346299959e+00
   6.1862110128556591e-01   1.5772728721936302e+00
   6.2040657676015454e-01   1.5790674599768495e+00
   6.2219205223474316e-01   1.5796766467381764e+00
   6.2397752770933179e-01   1.5850964798345570e+00
   6.2576300318392042e-01   1.5857203807021432e+00
   6.2754847865850905e-01   1.5948908401333324e+00
   6.2933395413309767e-01   1.6004820322881703e+00
   6.3111942960768630e-01   1.6073845637639443e+00
   6.3290490508227493e-01   1.6105831359370151e+00
   6.3469038055686355e-01   1.6176262987587500e+00
   6.3647585603145218e-01   1.6208955505331324e+00
   6.3826133150604081e-01   1.6267841835798098e+00
   6.4004680698062943e-01   1.6327442735036888e+00
   6.4183228245521806e-01   1.6334952506666951e+00
   6.4361775792980669e-01   1.6408780820435449e+00
   6.4540323340439532e-01   1.6456727498761901e+00
   6.4718870887898394e-01   1.6491655936709044e+00
   6.4897418435357257e-01   1.6540472799668944e+00
   6.5075965982816120e-01   1.6534901443742465e+00
   6.5254513530274982e-01   1.6570448498556891e+00
   6.5433061077733845e-01   1.6578563619787530e+00
   6.5611608625192708e-01   1.6656366221760415e+00
   6.5790156172651570e-01   1.6664751541563023e+00
   6.5968703720110433e-01   1.6786676488532208e+00
   6.6147251267569296e-01   1.6795369164567246e+00
   6.6325798815028159e-01   1.6861901844586318e+00
   6.6504346362487021e-01   1.6973358217125503e+00
   6.6682893909945884e-01   1.7012217297402494e+00
   6.6861441457404747e-01   1.7171948274743267e+00
   6.7039989004863609e-01   1.7151282346541401e+00
   6.7218536552322472e-01   1.7191483822439246e+00
   6.7397084099781335e-01   1.7185892056681353e+00
   6.7575631647240197e-01   1.7195634555739605e+00
   6.7754179194699060e-01   1.7298734411251120e+00
   6.7932726742157912e-01   1.7340287630802256e+00
   6.8111274289616786e-01   1.7413987925546535e+00
   6.8289821837075637e-01   1.7408397737973054e+00
   6.8468369384534511e-01   1.7418750389166939e+00
   6.8646916931993363e-01   1.7575311267784852e+00
   6.8825464479452236e-01   1.7602589413245555e+00
   6.9004012026911088e-01   1.7646591370990070e+00
   6.9182559574369962e-01   1.7674210064241331e+00
   6.9361107121828813e-01   1.7718873257401082e+00
   6.9539654669287687e-01   1.7814987136930065e+00
   6.9718202216746539e-01   1.7895313290835473e+00
   6.9896749764205413e-01   1.8011819626510848e+00
   7.0075297311664264e-01   1.8023705931498566e+00
   7.0253844859123138e-01   1.8124881317576906e+00
   7.0432392406581990e-01   1.8155190943954027e+00
   7.0610939954040863e-01   1.8222139106650093e+00
   7.0789487501499715e-01   1.8216375062384860e+00
   7.0968035048958589e-01   1.8265657812702583e+00
   7.1146582596417440e-01   1.8296828857523739e+00
   7.1325130143876314e-01   1.8328184628289963e+00
   7.1503677691335166e-01   1.8416387140757877e+00
   7.1682225238794040e-01   1.8525090503761286e+00
   7.1860772786252891e-01   1.8577120359961403e+00
   7.2039320333711765e-01   1.8668941182533079e+00
   7.2217867881170617e-01   1.8782032922970762e+00
   7.2396415428629490e-01   1.8756058874581716e+00
   7.2574962976088342e-01   1.8830577899878318e+00
   7.2753510523547216e-01   1.8906003217596901e+00
   7.2932058071006067e-01   1.9023821958139935e+00
   7.3110605618464941e-01   1.9101654767098402e+00
   7.3289153165923793e-01   1.9201782264903582e+00
   7.3467700713382655e-01   1.9217244713290513e+00
   7.3646248260841518e-01   1.9254295951215481e+00
   7.3824795808300381e-01   1.9401151382954029e+00
   7.4003343355759243e-01   1.9439498608390380e+00
   7.4181890903218106e-01   1.9411218238766714e+00
   7.4360438450676969e-01   1.9427220194441146e+00
   7.4538985998135832e-01   1.9556300131203144e+00
   7.4717533545594694e-01   1.9664742836092011e+00
   7.4896081093053557e-01   1.9728365852604144e+00
   7.5074628640512420e-01   1.9839883777782614e+00
   7.5253176187971282e-01   1.9905257967224763e+00
   7.5431723735430145e-01   1.9923115069067074e+00
   7.5610271282889008e-01   2.0062694742582416e+00
   7.5788818830347870e-01   2.0230067534744789e+00
   7.5967366377806733e-01   2.0299743444324561e+00
   7.6145913925265596e-01   2.0344688336772969e+00
   7.6324461472724459e-01   2.0415799809990482e+00
   7.6503009020183321e-01   2.0409914006490051e+00
   7.6681556567642184e-01   2.0560795082534891e+00
   7.6860104115101047e-01   2.0688063528870653e+00
   7.7038651662559909e-01   2.0682359245544859e+00
   7.7217199210018772e-01   2.0676441523992870e+00
   7.7395746757477635e-01   2.0752009674664431e+00
   7.7574294304936497e-01   2.0939696978358775e+00
   7.7752841852395360e-01   2.0990414877691106e+00
   7.7931389399854223e-01   2.1070112776666683e+00
   7.8109936947313086e-01   2.1208536829780416e+00
   7.8288484494771948e-01   2.1408834599401985e+00
   7.8467032042230811e-01   2.1583999656048203e+00
   7.8645579589689674e-01   2.1609681612994973e+00
   7.8824127137148536e-01   2.1635476378823379e+00
   7.9002674684607399e-01   2.1692306558196850e+00
   7.9181222232066262e-01   2.1781058651517022e+00
   7.9359769779525124e-01   2.1934941870013622e+00
   7.9538317326983987e-01   2.1898245478066203e+00
   7.9716864874442850e-01   2.2055517974989121e+00
   7.9895412421901713e-01   2.2051093154657440e+00
   8.0073959969360575e-01   2.2279484541971009e+00
   8.0252507516819438e-01   2.2275416966873185e+00
   8.0431055064278301e-01   2.2373316244201726e+00
   8.0609602611737152e-01   2.2542413213102828e+00
   8.0788150159196026e-01   2.2750751996560550e+00
   8.0966697706654878e-01   2.2891519791450028e+00
   8.1145245254113751e-01   2.2961262965853004e+00
   8.1323792801572603e-01   2.3143864721631382e+00
   8.1502340349031477e-01   2.3140848487397241e+00
   8.1680887896490328e-01   2.3099623351990761e+00
   8.1859435443949202e-01   2.3325698594382844e+00
   8.2037982991408054e-01   2.3518667736967314e+00
   8.2216530538866928e-01   2.3555717909936620e+00
   8.2395078086325779e-01   2.3593006329759403e+00
   8.2573625633784653e-01   2.3711815926206810e+00
   8.2752173181243505e-01   2.3832757968966130e+00
   8.2930720728702378e-01   2.3955858943973594e+00
   8.3109268276161230e-01   2.4253431887366137e+00
   8.3287815823620104e-01   2.4471531049899529e+00
   8.3466363371078955e-01   2.4559131044557168e+00
   8.3644910918537818e-01   2.4602306593301915e+00
   8.3823458465996681e-01   2.4737849421421449e+00
   8.4002006013455544e-01   2.4875972552486973e+00
   8.4180553560914406e-01   2.4921123498899136e+00
   8.4359101108373269e-01   2.4966448639411336e+00
   8.4537648655832132e-01   2.5109246826735045e+00
   8.4716196203290994e-01   2.5404019225193695e+00
   8.4894743750749857e-01   2.5452867010187203e+00
   8.5073291298208720e-01   2.5604351917717345e+00
   8.5251838845667582e-01   2.5758486471044910e+00
   8.5430386393126445e-01   2.6131213204732613e+00
   8.5608933940585308e-01   2.6405724009039275e+00
   8.5787481488044171e-01   2.6517209464575768e+00
   8.5966029035503033e-01   2.6515655078020974e+00
   8.6144576582961896e-01   2.6571010983928263e+00
   8.6323124130420759e-01   2.6981057241699533e+00
   8.6501671677879621e-01   2.6919190420402908e+00
   8.6680219225338484e-01   2.7037375112921587e+00
   8.6858766772797347e-01   2.7157068978818466e+00
   8.7037314320256209e-01   2.7532444163310155e+00
   8.7215861867715072e-01   2.7724311607735928e+00
   8.7394409415173935e-01   2.8122061537160850e+00
   8.7572956962632797e-01   2.8256132977356461e+00
   8.7751504510091660e-01   2.8675282493900736e+00
   8.7930052057550523e-01   2.8672482874577763e+00
   8.8108599605009386e-01   2.8888470292748187e+00
   8.8287147152468248e-01   2.9033795010238852e+00
   8.8465694699927111e-01   2.8953708411459300e+00
   8.8644242247385974e-01   2.9409763685150376e+00
   8.8822789794844836e-01   2.9482272450061622e+00
   8.9001337342303699e-01   2.9635496832176877e+00
   8.9179884889762562e-01   3.0124139197069710e+00
   8.9358432437221424e-01   3.0811456250655276e+00
   8.9536979984680287e-01   3.1077410412356814e+00
   8.9715527532139150e-01   3.1071048208283738e+00
   8.9894075079598013e-01   3.1344404105339745e+00
   9.0072622627056875e-01   3.1527958589115390e+00
   9.0251170174515738e-01   3.1814348191398234e+00
   9.0429717721974601e-01   3.1805015045208460e+00
   9.0608265269433463e-01   3.2099664209326924e+00
   9.0786812816892326e-01   3.2507101018334223e+00
   9.0965360364351189e-01   3.2820113781691607e+00
   9.1143907911810051e-01   3.3719762753693874e+00
   9.1322455459268914e-01   3.4069509895272283e+00
   9.1501003006727777e-01   3.4429801844809664e+00
   9.1679550554186640e-01   3.4674637790402842e+00
   9.1858098101645502e-01   3.4796441635756690e+00
   9.2036645649104365e-01   3.5049939564765489e+00
   9.2215193196563228e-01   3.5587509733153602e+00
   9.2393740744022090e-01   3.5716767755875902e+00
   9.2572288291480942e-01   3.6739832725244987e+00
   9.2750835838939816e-01   3.7200026212828519e+00
   9.2929383386398667e-01   3.8180832989403095e+00
   9.3107930933857541e-01   3.7835347879882462e+00
   9.3286478481316393e-01   3.8517073274261309e+00
   9.3465026028775267e-01   3.8507574536302567e+00
   9.3643573576234118e-01   3.9049065701368533e+00
   9.3822121123692981e-01   4.0008711248228046e+00
   9.4000668671151844e-01   3.9795716306099966e+00
   9.4179216218610706e-01   4.1473186528733557e+00
   9.4357763766069569e-01   4.2149347641952453e+00
   9.4536311313528432e-01   4.2621650195542760e+00
   9.4714858860987294e-01   4.2862151534347799e+00
   9.4893406408446157e-01   4.4152720011046434e+00
   9.5071953955905020e-01   4.4426124052464067e+00
   9.5250501503363882e-01   4.4988847737858615e+00
   9.5429049050822745e-01   4.6183399737355080e+00
   9.5607596598281608e-01   4.7142906101209956e+00
   9.5786144145740471e-01   4.9253993062325696e+00
   9.5964691693199333e-01   4.8893028769222244e+00
   9.6143239240658196e-01   5.0867836051755297e+00
   9.6321786788117059e-01   5.0873854355891934e+00
   9.6500334335575921e-01   5.2640695613294781e+00
   9.6678881883034784e-01   5.3604209486488408e+00
   9.6857429430493647e-01   5.5141777086415980e+00
   9.7035976977952509e-01   5.7433373529151552e+00
   9.7214524525411372e-01   6.0024352508874310e+00
   9.7393072072870235e-01   6.0747215902438167e+00
   9.7571619620329098e-01   6.3023953362242606e+00
   9.7750167167787960e-01   6.5579656121083874e+00
   9.7928714715246823e-01   6.8512465146395449e+00
   9.8107262262705686e-01   7.0686040711552245e+00
   9.8285809810164548e-01   7.4330097732898164e+00
   9.8464357357623411e-01   8.2040982297804206e+00
   9.8642904905082274e-01   8.3936370100364428e+00
   9.8821452452541136e-01   8.8162530738288414e+00
   9.8999999999999999e-01   9.8767174584970352e+00


==> stdmap3_specDL.tex <==
  -1.5653089921958133e+02   0.0000000000000000e+00
  -1.4465245908813702e+02   0.0000000000000000e+00
  -1.4400232060928514e+02   0.0000000000000000e+00
  -1.4276856692589490e+02   0.0000000000000000e+00
  -1.3600080039275284e+02   0.0000000000000000e+00
  -1.3536216003304639e+02   0.0000000000000000e+00
  -1.3351371197074681e+02   0.0000000000000000e+00
  -1.3212755033887137e+02   0.0000000000000000e+00
  -1.3081700831114688e+02   0.0000000000000000e+00
  -1.2954576470027220e+02   0.0000000000000000e+00
  -1.2898916442768370e+02   0.0000000000000000e+00
  -1.2874400754264866e+02   0.0000000000000000e+00
  -1.2817630229833296e+02   0.0000000000000000e+00
  -1.2747656870858243e+02   0.0000000000000000e+00
  -1.2611583935322308e+02   0.0000000000000000e+00
  -1.2551537154310161e+02   0.0000000000000000e+00
  -1.2515283602275592e+02   0.0000000000000000e+00
  -1.2406613918142264e+02   0.0000000000000000e+00
  -1.2358676321031949e+02   0.0000000000000000e+00
  -1.2307915148113716e+02   0.0000000000000000e+00
  -1.2268390847051242e+02   0.0000000000000000e+00
  -1.2251161011080613e+02   0.0000000000000000e+00
  -1.2175365633958269e+02   0.0000000000000000e+00
  -1.2106373091162999e+02   0.0000000000000000e+00
  -1.2042733870083951e+02   0.0000000000000000e+00
  -1.1990156496511734e+02   0.0000000000000000e+00
  -1.1917932628453333e+02   0.0000000000000000e+00
  -1.1884775942130467e+02   0.0000000000000000e+00
  -1.1793831323395514e+02   0.0000000000000000e+00
  -5.9715069801514375e-05   0.0000000000000000e+00
  -1.1538162098667049e+00   0.0000000000000000e+00
  -1.1690601947669406e+00   0.0000000000000000e+00
  -2.2239809942108191e+00   0.0000000000000000e+00
  -2.1042845888461663e+00   0.0000000000000000e+00
  -3.2240758605414839e+00   0.0000000000000000e+00
  -3.3248435716689730e+00   0.0000000000000000e+00
  -3.3953010552629674e+00   0.0000000000000000e+00
  -3.4153833630591302e+00   0.0000000000000000e+00
  -3.9954402546263923e+00   0.0000000000000000e+00
  -4.0139083320838225e+00   0.0000000000000000e+00
  -6.4530828363036195e+00   0.0000000000000000e+00
  -6.4799311081857152e+00   0.0000000000000000e+00
  -6.6679143014253466e+00   0.0000000000000000e+00
  -6.6723404282619851e+00   0.0000000000000000e+00
  -9.6847750596363333e+00   0.0000000000000000e+00
  -8.9165804234717090e+00   0.0000000000000000e+00
  -8.0952689802689584e+00   0.0000000000000000e+00
  -8.1940389436068788e+00   0.0000000000000000e+00
  -8.5305037803439454e+00   0.0000000000000000e+00
  -1.1783558184688737e+02   0.0000000000000000e+00
  -1.1724152605021159e+02   0.0000000000000000e+00
  -1.1650229478163627e+02   0.0000000000000000e+00
  -1.1624123052628556e+02   0.0000000000000000e+00
  -1.1597048846277310e+02   0.0000000000000000e+00
  -1.1552987396080405e+02   0.0000000000000000e+00
  -1.1460729303333265e+02   0.0000000000000000e+00
  -1.1384623616955587e+02   0.0000000000000000e+00
  -1.1395926854310741e+02   0.0000000000000000e+00
  -9.9223396995682425e+00   0.0000000000000000e+00
  -1.0383947518759770e+01   0.0000000000000000e+00
  -1.0420219843317350e+01   0.0000000000000000e+00
  -1.0820260099383592e+01   0.0000000000000000e+00
  -1.0822128881686016e+01   0.0000000000000000e+00
  -1.1906433978024973e+01   0.0000000000000000e+00
  -1.1898820788374412e+01   0.0000000000000000e+00
  -1.3364658001849437e+01   0.0000000000000000e+00
  -1.3391412695874443e+01   0.0000000000000000e+00
  -1.3572321661831429e+01   0.0000000000000000e+00
  -1.3548187468684640e+01   0.0000000000000000e+00
  -1.5449106573285494e+01   0.0000000000000000e+00
  -1.5420339655931768e+01   0.0000000000000000e+00
  -1.5984631051081085e+01   0.0000000000000000e+00
  -1.5956908593058705e+01   0.0000000000000000e+00
  -1.1246080818969729e+02   0.0000000000000000e+00
  -1.1221782357897655e+02   0.0000000000000000e+00
  -1.1223512394966895e+02   0.0000000000000000e+00
  -1.1160854004145489e+02   0.0000000000000000e+00
  -1.1112601395842306e+02   0.0000000000000000e+00
  -1.1063465197983012e+02   0.0000000000000000e+00
  -1.1048331798535290e+02   0.0000000000000000e+00
  -1.1025941611986300e+02   0.0000000000000000e+00
  -1.0936366826604038e+02   0.0000000000000000e+00
  -1.0962127878782378e+02   0.0000000000000000e+00
  -1.0987674926164514e+02   0.0000000000000000e+00
  -1.6786147266125692e+01   0.0000000000000000e+00
  -1.6762751446422556e+01   0.0000000000000000e+00
  -1.8400364589738530e+01   0.0000000000000000e+00
  -1.8328084991740063e+01   0.0000000000000000e+00
  -1.9531713455159714e+01   0.0000000000000000e+00
  -1.9410258728801463e+01   0.0000000000000000e+00
  -1.0904901880179195e+02   0.0000000000000000e+00
  -1.0882882213558518e+02   0.0000000000000000e+00
  -1.0809271021832051e+02   0.0000000000000000e+00
  -1.0701709938253224e+02   0.0000000000000000e+00
  -1.0754701166687988e+02   0.0000000000000000e+00
  -1.0746190277840441e+02   0.0000000000000000e+00
  -1.0723775619180458e+02   0.0000000000000000e+00
  -2.0241647334832837e+01   0.0000000000000000e+00
  -2.0526435669706217e+01   0.0000000000000000e+00
  -2.1248095587053452e+01   0.0000000000000000e+00
  -2.0940434611239496e+01   0.0000000000000000e+00
  -2.0762664498680799e+01   7.6745297623313068e-03
  -2.0762664498680799e+01  -7.6745297623313068e-03
  -1.0602066532602319e+02   0.0000000000000000e+00
  -1.0586535766124267e+02   0.0000000000000000e+00
  -1.0561333163969812e+02   0.0000000000000000e+00
  -1.0415015739178432e+02   0.0000000000000000e+00
  -1.0440812330688648e+02   0.0000000000000000e+00
  -1.0477495026494562e+02   0.0000000000000000e+00
  -1.0471124481684508e+02   0.0000000000000000e+00
  -1.0468120186539458e+02   0.0000000000000000e+00
  -2.1643524158874126e+01   0.0000000000000000e+00
  -2.1662833128263912e+01   0.0000000000000000e+00
  -2.2303468712607557e+01   0.0000000000000000e+00
  -2.2205427360247565e+01   0.0000000000000000e+00
  -2.3073714883964861e+01   0.0000000000000000e+00
  -2.3332896475523516e+01   0.0000000000000000e+00
  -2.3693716465038925e+01   0.0000000000000000e+00
  -2.3816247082707939e+01   0.0000000000000000e+00
  -1.0368669993297804e+02   0.0000000000000000e+00
  -1.0317347605398416e+02   0.0000000000000000e+00
  -1.0252192035396607e+02   0.0000000000000000e+00
  -1.0174375048733015e+02   0.0000000000000000e+00
  -1.0212050714263809e+02   0.0000000000000000e+00
  -2.4336718246527898e+01   0.0000000000000000e+00
  -2.4428223391682685e+01   0.0000000000000000e+00
  -2.4689970507468939e+01   0.0000000000000000e+00
  -2.5218721706907907e+01   0.0000000000000000e+00
  -2.5350444731388297e+01   4.8135602108521297e-03
  -2.5350444731388297e+01  -4.8135602108521297e-03
  -2.6108565945175307e+01   0.0000000000000000e+00
  -2.6190115079037874e+01   0.0000000000000000e+00
  -2.6687889273434017e+01   0.0000000000000000e+00
  -1.0149640050205755e+02   0.0000000000000000e+00
  -1.0086126072399441e+02   0.0000000000000000e+00
  -1.0112084617745427e+02   0.0000000000000000e+00
  -1.0033742236169330e+02   0.0000000000000000e+00
  -9.9707292107332449e+01   0.0000000000000000e+00
  -9.9307259753569340e+01   0.0000000000000000e+00
  -9.9162381127977326e+01   0.0000000000000000e+00
  -9.8721804989461276e+01   0.0000000000000000e+00
  -9.7987939421623039e+01   0.0000000000000000e+00
  -9.8215885368464711e+01   0.0000000000000000e+00
  -9.7278210295744373e+01   0.0000000000000000e+00
  -9.7208255881222868e+01   0.0000000000000000e+00
  -9.6651555368960899e+01   0.0000000000000000e+00
  -9.6122408043718309e+01   0.0000000000000000e+00
  -9.6012104352733232e+01   0.0000000000000000e+00
  -9.4671022005020902e+01   0.0000000000000000e+00
  -9.5037023071563638e+01   0.0000000000000000e+00
  -9.5307831127556796e+01   0.0000000000000000e+00
  -9.5409252094138282e+01   0.0000000000000000e+00
  -2.6507121205197382e+01   0.0000000000000000e+00
  -2.7124805427759082e+01   0.0000000000000000e+00
  -3.1809939934807396e+01   0.0000000000000000e+00
  -3.1524624598542136e+01   0.0000000000000000e+00
  -3.1042548283971342e+01   0.0000000000000000e+00
  -2.7261856201931810e+01   0.0000000000000000e+00
  -3.0449158460641442e+01   0.0000000000000000e+00
  -3.0174053919084930e+01   0.0000000000000000e+00
  -2.9825815639823023e+01   0.0000000000000000e+00
  -2.7845662819546110e+01   0.0000000000000000e+00
  -2.9604035248690987e+01   0.0000000000000000e+00
  -2.9424524973775938e+01   0.0000000000000000e+00
  -2.7936685361831326e+01   0.0000000000000000e+00
  -2.8166963087367368e+01   0.0000000000000000e+00
  -2.8270072980763658e+01   0.0000000000000000e+00
  -2.8333982212264630e+01   0.0000000000000000e+00
  -2.8719385228519183e+01   0.0000000000000000e+00
  -2.8633289445003260e+01   0.0000000000000000e+00
  -2.8661674834819081e+01   0.0000000000000000e+00
  -9.4164115657962796e+01   0.0000000000000000e+00
  -9.4309284282413230e+01   0.0000000000000000e+00
  -3.2393836414748193e+01   0.0000000000000000e+00
  -3.2095053265121656e+01   0.0000000000000000e+00
  -9.3540638720294126e+01   0.0000000000000000e+00
  -9.2772300212297040e+01   0.0000000000000000e+00
  -3.3975880294970899e+01   0.0000000000000000e+00
  -3.2550610111089064e+01   0.0000000000000000e+00
  -3.2885019583945528e+01   0.0000000000000000e+00
  -3.3078746931468793e+01   0.0000000000000000e+00
  -3.3558078481762266e+01   0.0000000000000000e+00
  -3.3397696260308216e+01   0.0000000000000000e+00
  -9.2660224853471149e+01   0.0000000000000000e+00
  -9.2503121804920738e+01   0.0000000000000000e+00
  -9.2066271378623711e+01   0.0000000000000000e+00
  -9.1239134497529875e+01   0.0000000000000000e+00
  -9.1420907346353872e+01   0.0000000000000000e+00
  -9.0802460933485236e+01   0.0000000000000000e+00
  -9.0745253531634617e+01   0.0000000000000000e+00
  -3.4853549244550017e+01   0.0000000000000000e+00
  -3.5158290985238118e+01   0.0000000000000000e+00
  -3.5276224000637008e+01   0.0000000000000000e+00
  -3.5789066627814456e+01   0.0000000000000000e+00
  -3.6085894367436637e+01   0.0000000000000000e+00
  -9.0336235816851612e+01   0.0000000000000000e+00
  -8.9898267247984322e+01   0.0000000000000000e+00
  -8.9682771277515343e+01   0.0000000000000000e+00
  -8.9196601974123553e+01   0.0000000000000000e+00
  -8.8983316644513096e+01   0.0000000000000000e+00
  -8.7764490643561231e+01   0.0000000000000000e+00
  -8.7984099453898864e+01   0.0000000000000000e+00
  -8.8142230718798615e+01   0.0000000000000000e+00
  -8.8630223219607586e+01   0.0000000000000000e+00
  -8.8524988813180642e+01   0.0000000000000000e+00
  -3.6264461870123398e+01   4.3568876894645881e-03
  -3.6264461870123398e+01  -4.3568876894645881e-03
  -3.7791699786775496e+01   0.0000000000000000e+00
  -3.7868527957302156e+01   0.0000000000000000e+00
  -3.8191033002294795e+01   0.0000000000000000e+00
  -3.8303446418749992e+01   0.0000000000000000e+00
  -4.0000576119534301e+01   0.0000000000000000e+00
  -3.9772889920988533e+01   0.0000000000000000e+00
  -3.9641823509890692e+01   0.0000000000000000e+00
  -3.8832619197277793e+01   0.0000000000000000e+00
  -3.9173474220476479e+01   0.0000000000000000e+00
  -3.9035139384781679e+01   0.0000000000000000e+00
  -8.6835306616555670e+01   0.0000000000000000e+00
  -8.7579582906287882e+01   0.0000000000000000e+00
  -8.7389052590568525e+01   0.0000000000000000e+00
  -4.0308388989521255e+01   0.0000000000000000e+00
  -8.6182878701788766e+01   0.0000000000000000e+00
  -8.6017370912163656e+01   0.0000000000000000e+00
  -8.5966469730211756e+01   0.0000000000000000e+00
  -4.2345405142308117e+01   0.0000000000000000e+00
  -4.1522590752785142e+01   0.0000000000000000e+00
  -4.1574372160287510e+01   0.0000000000000000e+00
  -4.0595817154961551e+01   0.0000000000000000e+00
  -4.1040700241840597e+01   0.0000000000000000e+00
  -4.0820812667596151e+01   0.0000000000000000e+00
  -4.2858678451640387e+01   0.0000000000000000e+00
  -4.3737947268984747e+01   0.0000000000000000e+00
  -4.3595501305073839e+01   0.0000000000000000e+00
  -4.4121194171078329e+01   0.0000000000000000e+00
  -4.4441275768901953e+01   0.0000000000000000e+00
  -8.5631622861016623e+01   0.0000000000000000e+00
  -8.5399794435875521e+01   0.0000000000000000e+00
  -8.4909286630142446e+01   0.0000000000000000e+00
  -8.4522658602749999e+01   0.0000000000000000e+00
  -8.4421734878398155e+01   0.0000000000000000e+00
  -8.4040616631375883e+01   0.0000000000000000e+00
  -8.3172681965127126e+01   0.0000000000000000e+00
  -8.3305153948780529e+01   0.0000000000000000e+00
  -4.4806969144140311e+01   0.0000000000000000e+00
  -4.5122986157587079e+01   0.0000000000000000e+00
  -4.5574300138597472e+01   0.0000000000000000e+00
  -4.7076891589255240e+01   0.0000000000000000e+00
  -4.6275146460104160e+01   0.0000000000000000e+00
  -4.6211581315528697e+01   0.0000000000000000e+00
  -4.6633647064527146e+01   0.0000000000000000e+00
  -8.3431302462189777e+01   0.0000000000000000e+00
  -8.2844182923155017e+01   0.0000000000000000e+00
  -8.2529233276566828e+01   0.0000000000000000e+00
  -8.1835700189905964e+01   0.0000000000000000e+00
  -8.1745570979624773e+01   0.0000000000000000e+00
  -7.9594877981771660e+01   0.0000000000000000e+00
  -8.1398876920942357e+01   0.0000000000000000e+00
  -7.9816668600619522e+01   0.0000000000000000e+00
  -8.0116584207226182e+01   0.0000000000000000e+00
  -8.0273551744863198e+01   0.0000000000000000e+00
  -8.0605033182572797e+01   0.0000000000000000e+00
  -8.0983556465226897e+01   0.0000000000000000e+00
  -8.0874863998514883e+01   0.0000000000000000e+00
  -8.1188732629865058e+01   0.0000000000000000e+00
  -4.7398517961691354e+01   0.0000000000000000e+00
  -4.7462738127720932e+01   0.0000000000000000e+00
  -7.8736458526572889e+01   0.0000000000000000e+00
  -7.9198057125603469e+01   0.0000000000000000e+00
  -7.8983527441796809e+01   0.0000000000000000e+00
  -7.8999889357112266e+01   0.0000000000000000e+00
  -4.8740335909862843e+01   0.0000000000000000e+00
  -4.8704533569621937e+01   0.0000000000000000e+00
  -4.7677513532551849e+01   0.0000000000000000e+00
  -4.7862142281819807e+01   0.0000000000000000e+00
  -4.8006155232001966e+01   0.0000000000000000e+00
  -4.8315164122947522e+01   0.0000000000000000e+00
  -4.8178245661462839e+01   0.0000000000000000e+00
  -7.7951923677890164e+01   0.0000000000000000e+00
  -7.8567671225141297e+01   0.0000000000000000e+00
  -7.8352073966660001e+01   0.0000000000000000e+00
  -7.7696918903383079e+01   0.0000000000000000e+00
  -7.7389162328514828e+01   0.0000000000000000e+00
  -7.7215852991150072e+01   0.0000000000000000e+00
  -7.6900202378379518e+01   0.0000000000000000e+00
  -7.7022432879936559e+01   0.0000000000000000e+00
  -4.7743208944395541e+01   0.0000000000000000e+00
  -4.9099482466885163e+01   0.0000000000000000e+00
  -4.9578876075558085e+01   0.0000000000000000e+00
  -4.9726869308868856e+01   0.0000000000000000e+00
  -4.9989982118785001e+01   0.0000000000000000e+00
  -5.0381916428745640e+01   0.0000000000000000e+00
  -5.0245581515370063e+01   0.0000000000000000e+00
  -7.6425537734132405e+01   0.0000000000000000e+00
  -7.6233360651087537e+01   0.0000000000000000e+00
  -7.5976946685877763e+01   0.0000000000000000e+00
  -7.5803790277167778e+01   0.0000000000000000e+00
  -7.5683326257321738e+01   0.0000000000000000e+00
  -7.5273106562102498e+01   0.0000000000000000e+00
  -5.0714818959457695e+01   0.0000000000000000e+00
  -5.0598101135797016e+01   0.0000000000000000e+00
  -5.0935278169635595e+01   0.0000000000000000e+00
  -5.1243739871709906e+01   0.0000000000000000e+00
  -5.2148067704600805e+01   0.0000000000000000e+00
  -5.2015407922135545e+01   0.0000000000000000e+00
  -5.1786112531533639e+01   0.0000000000000000e+00
  -5.1640725781499079e+01   0.0000000000000000e+00
  -7.5129739320938981e+01   0.0000000000000000e+00
  -7.4731086892934087e+01   0.0000000000000000e+00
  -7.4531313334144514e+01   0.0000000000000000e+00
  -7.4214690056791852e+01   0.0000000000000000e+00
  -7.4128358611932384e+01   0.0000000000000000e+00
  -7.3692484978810711e+01   0.0000000000000000e+00
  -5.1044325648412361e+01   0.0000000000000000e+00
  -5.2630576082201685e+01   0.0000000000000000e+00
  -5.2826975542832621e+01   0.0000000000000000e+00
  -5.3461302965514356e+01   0.0000000000000000e+00
  -5.3642016074998267e+01   0.0000000000000000e+00
  -5.3978082837180523e+01   0.0000000000000000e+00
  -5.2960993248689547e+01   0.0000000000000000e+00
  -5.4313784398213706e+01   0.0000000000000000e+00
  -5.4582360447132771e+01   0.0000000000000000e+00
  -5.5020101184202986e+01   0.0000000000000000e+00
  -5.5841229797116220e+01   0.0000000000000000e+00
  -5.5480678874220573e+01   0.0000000000000000e+00
  -5.5159952456324483e+01   0.0000000000000000e+00
  -5.6182747008133475e+01   0.0000000000000000e+00
  -5.7131140391026847e+01   0.0000000000000000e+00
  -5.6468230907110943e+01   0.0000000000000000e+00
  -7.3594988038642867e+01   0.0000000000000000e+00
  -7.3187402119549020e+01   0.0000000000000000e+00
  -7.3241107242637213e+01   0.0000000000000000e+00
  -7.2921497768308427e+01   0.0000000000000000e+00
  -6.8098444132543079e+01   0.0000000000000000e+00
  -6.8517709037169226e+01   0.0000000000000000e+00
  -6.7790167248027700e+01   0.0000000000000000e+00
  -6.7483986028981633e+01   0.0000000000000000e+00
  -6.7032294464660410e+01   0.0000000000000000e+00
  -6.6791477543988563e+01   0.0000000000000000e+00
  -6.6451902419346297e+01   0.0000000000000000e+00
  -6.6336972328457705e+01   0.0000000000000000e+00
  -6.5993405732795523e+01   0.0000000000000000e+00
  -6.5457653044729184e+01   0.0000000000000000e+00
  -6.4723568610600722e+01   0.0000000000000000e+00
  -6.4239297391620624e+01   0.0000000000000000e+00
  -6.4355412040580376e+01   0.0000000000000000e+00
  -6.3826188842018254e+01   0.0000000000000000e+00
  -7.2881840210492683e+01   0.0000000000000000e+00
  -7.2361796142795768e+01   0.0000000000000000e+00
  -7.1943697474316764e+01   0.0000000000000000e+00
  -6.9076879167979129e+01   0.0000000000000000e+00
  -6.9301119450301115e+01   0.0000000000000000e+00
  -6.3661992527308861e+01   0.0000000000000000e+00
  -5.4460844377160498e+01   0.0000000000000000e+00
  -5.9307216883695993e+01   0.0000000000000000e+00
  -5.9106159125215640e+01   0.0000000000000000e+00
  -5.8764648647710018e+01   0.0000000000000000e+00
  -5.8494185451017472e+01   0.0000000000000000e+00
  -5.6363138054574591e+01   0.0000000000000000e+00
  -5.7906379663042365e+01   0.0000000000000000e+00
  -5.7432763746087225e+01   0.0000000000000000e+00
  -5.7700898460764279e+01   0.0000000000000000e+00
  -7.1654830513779885e+01   0.0000000000000000e+00
  -7.0513744557914293e+01   0.0000000000000000e+00
  -7.2569719004724391e+01   0.0000000000000000e+00
  -7.2608027005409610e+01   0.0000000000000000e+00
  -7.0665037149791715e+01   0.0000000000000000e+00
  -6.7411411594685802e+01   0.0000000000000000e+00
  -7.0352969781708524e+01   0.0000000000000000e+00
  -7.0089548968128071e+01   0.0000000000000000e+00
  -7.0049854401166002e+01   0.0000000000000000e+00
  -6.5790461270628583e+01   0.0000000000000000e+00
  -5.7801474838444378e+01   0.0000000000000000e+00
  -5.8600145825066889e+01   0.0000000000000000e+00
  -6.2187065502232691e+01   0.0000000000000000e+00
  -6.2982452848655278e+01   0.0000000000000000e+00
  -6.3064252189464952e+01   0.0000000000000000e+00
  -6.2628893221579105e+01   0.0000000000000000e+00
  -6.1986135430366126e+01   0.0000000000000000e+00
  -6.0027851592212869e+01   0.0000000000000000e+00
  -5.9705045263304619e+01   0.0000000000000000e+00
  -6.0686756342343770e+01   0.0000000000000000e+00
  -6.0227828972030935e+01   0.0000000000000000e+00
  -6.1611152413903966e+01   0.0000000000000000e+00
  -6.0879970083009169e+01   0.0000000000000000e+00
  -6.1083947191259334e+01   0.0000000000000000e+00
  -6.1183905830062493e+01   0.0000000000000000e+00
  -6.1852430599750036e+01   0.0000000000000000e+00
  -6.1485564201845818e+01   0.0000000000000000e+00
  -5.5288824762062880e+01   0.0000000000000000e+00
  -5.6803357198968406e+01   0.0000000000000000e+00
  -6.5320831059994021e+01   0.0000000000000000e+00
  -6.8592229743116590e+01   0.0000000000000000e+00
  -6.9653549642314104e+01   0.0000000000000000e+00
  -6.9677057719210936e+01   0.0000000000000000e+00
  -7.1038048714238414e+01   0.0000000000000000e+00
  -7.1350219136219380e+01   0.0000000000000000e+00
  -7.1392947810029725e+01   0.0000000000000000e+00
  -5.9951101613145497e+01   0.0000000000000000e+00
  -6.3123273014606958e+01   0.0000000000000000e+00
  -7.1157525770050668e+01   0.0000000000000000e+00


==> stdmap3_specDL_close.tex <==
1  -5.9715069801514375e-05 
2  -1.1538162098667049e+00  
3  -1.1690601947669406e+00  
4  -2.1042845888461663e+00  
5  -2.2239809942108191e+00  
6  -3.2240758605414839e+00  
7  -3.3248435716689730e+00  
8  -3.3953010552629674e+00  
9  -3.4153833630591302e+00  
10  -3.9954402546263923e+00 


==> stdmap_ev_err_vs_eps_N20_phi31.tex <==
   1.1111111111111112e+00   5.9421016610108746e-01
   1.1516559219159610e+00   4.0627290811612909e-01
   1.1936802262356920e+00   1.5181129342141969e-01
   1.2372380112764869e+00   2.2162645482594656e-01
   1.2823852342554833e+00   3.4808968211609936e-01
   1.3291798942871231e+00   4.4771983726616199e-01
   1.3776821068926566e+00   5.5909470379797654e-01
   1.4279541812285272e+00   4.8987729047048778e-01
   1.4800607001328419e+00   4.3244427345864422e-01
   1.5340686030927637e+00   3.5818554394767527e-01
   1.5900472722394146e+00   3.0959055605777347e-01
   1.6480686214807578e+00   2.6573644226249765e-01
   1.7082071888869705e+00   2.2384452288230483e-01
   1.7705402324469866e+00   1.8640085465713466e-01
   1.8351478293192307e+00   1.5663730597528017e-01
   1.9021129787040418e+00   1.3323482998302733e-01
   1.9715217084699463e+00   1.1373098797977346e-01
   2.0434631856707579e+00   9.6783874531652547e-02
   2.1180298310954853e+00   8.1735663760927557e-02
   2.1953174379982006e+00   6.9377347121785504e-02
   2.2754252951604030e+00   5.9437330724706985e-02
   2.3584563144439663e+00   5.7660811099484836e-02
   2.4445171629985372e+00   5.0897960785283879e-02
   2.5337184002932229e+00   4.3222366212857431e-02
   2.6261746201486131e+00   3.6451205070843852e-02
   2.7220045979515950e+00   3.2624946972783279e-02
   2.8213314432420855e+00   2.8619875661541533e-02
   2.9242827578677080e+00   2.4124061508341742e-02
   3.0309907999095760e+00   2.1827515491286992e-02
   3.1415926535897927e+00   1.9485379124263923e-02


==> stdmap_ev_err_vs_eps_N20_phi42.tex <==
   1.1111111111111112e+00   9.8098606589966442e-02
   1.1516559219159610e+00   2.8383625038634119e-01
   1.1936802262356920e+00   4.4073434644030351e-01
   1.2372380112764869e+00   5.7437047861624013e-01
   1.2823852342554833e+00   4.6711910343180874e-01
   1.3291798942871231e+00   4.0285010555295925e-01
   1.3776821068926566e+00   3.3119576226661579e-01
   1.4279541812285272e+00   2.7449413968169717e-01
   1.4800607001328419e+00   2.2824330659651854e-01
   1.5340686030927637e+00   1.8892757617339376e-01
   1.5900472722394146e+00   1.5540339829743283e-01
   1.6480686214807578e+00   1.2811639929127647e-01
   1.7082071888869705e+00   1.0636106215452697e-01
   1.7705402324469866e+00   8.8692498175497902e-02
   1.8351478293192307e+00   7.3934430369424972e-02
   1.9021129787040418e+00   6.1537011163433193e-02
   1.9715217084699463e+00   5.2614409505048268e-02
   2.0434631856707579e+00   4.3516900743379321e-02
   2.1180298310954853e+00   3.5976563696889889e-02
   2.1953174379982006e+00   3.0210301399645995e-02
   2.2754252951604030e+00   2.5398282151186266e-02
   2.3584563144439663e+00   2.1409475580052847e-02
   2.4445171629985372e+00   1.8111026766984579e-02
   2.5337184002932229e+00   1.5370714383756756e-02
   2.6261746201486131e+00   1.3079059081052381e-02
   2.7220045979515950e+00   1.1169438694294521e-02
   2.8213314432420855e+00   9.5791365948083365e-03
   2.9242827578677080e+00   8.2598894979247217e-03
   3.0309907999095760e+00   7.1482910447983059e-03
   3.1415926535897927e+00   6.2226280055073958e-03


==> stdmap_ev_err_vs_eps_N20_phi53.tex <==
   1.1111111111111112e+00   3.2708805501239591e-01
   1.1516559219159610e+00   2.3621955429685812e-01
   1.1936802262356920e+00   1.7288705515995595e-01
   1.2372380112764869e+00   1.2827795544646522e-01
   1.2823852342554833e+00   9.5742513502443422e-02
   1.3291798942871231e+00   7.0933558608008304e-02
   1.3776821068926566e+00   5.1696015851635378e-02
   1.4279541812285272e+00   3.7181125236623210e-02
   1.4800607001328419e+00   2.6779282946525519e-02
   1.5340686030927637e+00   1.9623123288095182e-02
   1.5900472722394146e+00   1.4617565653856525e-02
   1.6480686214807578e+00   1.0864381513110312e-02
   1.7082071888869705e+00   7.9604189779571340e-03
   1.7705402324469866e+00   5.7915342151733081e-03
   1.8351478293192307e+00   4.2525520366256120e-03
   1.9021129787040418e+00   3.1726023361331006e-03
   1.9715217084699463e+00   2.3863982251141887e-03
   2.0434631856707579e+00   2.5407640612072260e-03
   2.1180298310954853e+00   3.0096338337010950e-03
   2.1953174379982006e+00   3.3769031118471913e-03
   2.2754252951604030e+00   3.6436413577213165e-03
   2.3584563144439663e+00   3.8247814934444535e-03
   2.4445171629985372e+00   3.9615734216977604e-03
   2.5337184002932229e+00   4.0726097151274855e-03
   2.6261746201486131e+00   4.1493042608879245e-03
   2.7220045979515950e+00   4.1995527735222606e-03
   2.8213314432420855e+00   4.2412969079705185e-03
   2.9242827578677080e+00   4.2737055430534538e-03
   3.0309907999095760e+00   4.2959775808665002e-03
   3.1415926535897927e+00   4.3150907726311879e-03


==> stdmap_ev_err_vs_eps_N20_phi64.tex <==
   1.1111111111111112e+00   3.8972474687657394e-01
   1.1516559219159610e+00   2.6932244223290569e-01
   1.1936802262356920e+00   1.8387325492082346e-01
   1.2372380112764869e+00   1.2460808852569019e-01
   1.2823852342554833e+00   8.4523042570920665e-02
   1.3291798942871231e+00   5.8295860688454423e-02
   1.3776821068926566e+00   4.0009309104728254e-02
   1.4279541812285272e+00   2.7785002036042651e-02
   1.4800607001328419e+00   1.9177598417522659e-02
   1.5340686030927637e+00   1.3090074856232932e-02
   1.5900472722394146e+00   8.8879842487598754e-03
   1.6480686214807578e+00   6.1094895031246774e-03
   1.7082071888869705e+00   4.2169243475109102e-03
   1.7705402324469866e+00   2.9508229259811551e-03
   1.8351478293192307e+00   2.2714177549861374e-03
   1.9021129787040418e+00   2.9381706100275033e-03
   1.9715217084699463e+00   3.4069771178242589e-03
   2.0434631856707579e+00   3.7301169511541146e-03
   2.1180298310954853e+00   3.9454155044910564e-03
   2.1953174379982006e+00   4.0890851521261260e-03
   2.2754252951604030e+00   4.1895424594213075e-03
   2.3584563144439663e+00   4.2607113184227165e-03
   2.4445171629985372e+00   4.3087407634270249e-03
   2.5337184002932229e+00   4.3411010191028955e-03
   2.6261746201486131e+00   4.3647531545483835e-03
   2.7220045979515950e+00   4.3818504705444745e-03
   2.8213314432420855e+00   4.3930491369066444e-03
   2.9242827578677080e+00   4.4004100993455227e-03
   3.0309907999095760e+00   4.4051610454916967e-03
   3.1415926535897927e+00   4.4081317539489918e-03


==> stdmap_ev_err_vs_h_eps08_phi31.tex <==
   2.2214414690791831e-01   2.6382846354926770e-01
   2.1156585419801746e-01   3.3551346424923184e-01
   2.0194922446174393e-01   4.2704868118706540e-01
   1.9316882339818983e-01   5.3237731495623741e-01
   1.8512012242326525e-01   5.1125032228151912e-01
   1.7771531752633468e-01   4.6109295666601868e-01
   1.7088011300609102e-01   4.6084835948480846e-01
   1.6455121993179134e-01   4.1193625795384414e-01
   1.5867439064851308e-01   3.6178709215147975e-01
   1.5320285993649541e-01   3.1914742247447558e-01
   1.4809609793861220e-01   2.9019979036789517e-01
   1.4331880445672149e-01   2.6799190312844762e-01
   1.3884009181744894e-01   2.4696078381941139e-01
   1.3463281630782928e-01   2.2350204439492286e-01
   1.3067302759289312e-01   1.9953331942206057e-01
   1.2693951251881047e-01   1.8054430041067457e-01
   1.2341341494884350e-01   1.7170789053524896e-01
   1.2007791724752341e-01   1.6142587693791152e-01
   1.1691797205679912e-01   1.4519929810000870e-01
   1.1392007533739401e-01   1.3166756626707754e-01
   1.1107207345395916e-01   1.2224674656994249e-01
   1.0836299849166749e-01   1.1676499036481736e-01
   1.0578292709900873e-01   1.0883238020414500e-01
   1.0332285902693876e-01   1.0076612805236637e-01
   1.0097461223087197e-01   9.2740384969085543e-02


==> stdmap_ev_err_vs_h_eps08_phi42.tex <==
   2.2214414690791831e-01   5.4499160856824014e-01
   2.1156585419801746e-01   4.6616776418081579e-01
   2.0194922446174393e-01   3.9973994261774470e-01
   1.9316882339818983e-01   3.4471121817479139e-01
   1.8512012242326525e-01   2.9990469893435967e-01
   1.7771531752633468e-01   2.5937012150173316e-01
   1.7088011300609102e-01   2.2448330704705385e-01
   1.6455121993179134e-01   1.9694243280018192e-01
   1.5867439064851308e-01   1.7527055756870130e-01
   1.5320285993649541e-01   1.5630839779436445e-01
   1.4809609793861220e-01   1.3926170829209669e-01
   1.4331880445672149e-01   1.2425357848196465e-01
   1.3884009181744894e-01   1.1157621081084652e-01
   1.3463281630782928e-01   1.0111834471929101e-01
   1.3067302759289312e-01   9.2047623647354262e-02
   1.2693951251881047e-01   8.3715810664369367e-02
   1.2341341494884350e-01   7.6049590636829451e-02
   1.2007791724752341e-01   6.9414229013413153e-02
   1.1691797205679912e-01   6.3905617533626322e-02
   1.1392007533739401e-01   5.9217575765850891e-02
   1.1107207345395916e-01   5.5362005951046941e-02
   1.0836299849166749e-01   5.1038187766259145e-02
   1.0578292709900873e-01   4.7201010289070297e-02
   1.0332285902693876e-01   4.3786912357771983e-02
   1.0097461223087197e-01   4.0721970497921624e-02


==> stdmap_ev_err_vs_h_eps08_phi53.tex <==
   2.2214414690791831e-01   1.1796376792073821e-01
   2.1156585419801746e-01   8.6337706466742312e-02
   2.0194922446174393e-01   6.2600628393670463e-02
   1.9316882339818983e-01   4.5016192249903018e-02
   1.8512012242326525e-01   3.2943997440730462e-02
   1.7771531752633468e-01   2.5328416927820958e-02
   1.7088011300609102e-01   1.9828943986682290e-02
   1.6455121993179134e-01   1.5201676295092224e-02
   1.5867439064851308e-01   1.1680701214339489e-02
   1.5320285993649541e-01   9.0114906935884007e-03
   1.4809609793861220e-01   7.2003469132405828e-03
   1.4331880445672149e-01   5.8508563546003185e-03
   1.3884009181744894e-01   4.7301873779421267e-03
   1.3463281630782928e-01   3.7889703162900389e-03
   1.3067302759289312e-01   3.0325291464350502e-03
   1.2693951251881047e-01   2.5018902977652826e-03
   1.2341341494884350e-01   2.1287231500731326e-03
   1.2007791724752341e-01   1.7787910346870614e-03
   1.1691797205679912e-01   1.4676293376642841e-03
   1.1392007533739401e-01   1.2129289330160633e-03
   1.1107207345395916e-01   1.0349691569194451e-03
   1.0836299849166749e-01   9.1382919708367448e-04
   1.0578292709900873e-01   7.7296728740605702e-04
   1.0332285902693876e-01   6.6686609472373082e-04
   1.0097461223087197e-01   5.8159115064371431e-04


==> stdmap_ev_err_vs_h_eps08_phi64.tex <==
   2.2214414690791831e-01   1.1144562185890895e-01
   2.1156585419801746e-01   7.1830858845026324e-02
   2.0194922446174393e-01   4.8253819309058352e-02
   1.9316882339818983e-01   3.3376530066287970e-02
   1.8512012242326525e-01   2.2987517221929123e-02
   1.7771531752633468e-01   1.5922901038177204e-02
   1.7088011300609102e-01   1.1155216320492522e-02
   1.6455121993179134e-01   7.9637304270633105e-03
   1.5867439064851308e-01   5.9726565493486827e-03
   1.5320285993649541e-01   4.3907073479745951e-03
   1.4809609793861220e-01   3.2215308352439970e-03
   1.4331880445672149e-01   2.3887207928059446e-03
   1.3884009181744894e-01   1.8097863484477961e-03
   1.3463281630782928e-01   1.4284804933059653e-03
   1.3067302759289312e-01   1.0942641340502693e-03
   1.2693951251881047e-01   8.4905818964501115e-04
   1.2341341494884350e-01   6.8941363715364413e-04
   1.2007791724752341e-01   6.9882226587327510e-04
   1.1691797205679912e-01   7.4585560967377568e-04
   1.1392007533739401e-01   7.6101892289580104e-04
   1.1107207345395916e-01   7.6608426637156271e-04
   1.0836299849166749e-01   7.5677301249657428e-04
   1.0578292709900873e-01   7.4989936642380444e-04
   1.0332285902693876e-01   7.3162249254048965e-04
   1.0097461223087197e-01   7.1849134117662160e-04

